LSTM-based Selective Dense Text Retrieval Guided by Sparse Lexical Retrieval

This paper studies fast fusion of dense retrieval and sparse lexical retrieval, and proposes a cluster-based selective dense retrieval method called CluSD guided by sparse lexical retrieval. CluSD takes a lightweight cluster-based approach and exploits the overlap of sparse retrieval results and embedding clusters in a two-stage selection process with an LSTM model to quickly identify relevant clusters while incurring limited extra memory space overhead. CluSD triggers partial dense retrieval and performs cluster-based block disk I/O if needed. This paper evaluates CluSD and compares it with several baselines for searching in-memory and on-disk MS MARCO and BEIR datasets.

==> abstract.tex <==

\comments{
{\bf Abstract for Oct 5 abstract submission:}
Recent studies show that sparse retrieval with a learned representation
can be greatly accelerated by BM25-guided index traversal with a tradeoff  in its relevance effectiveness.
This paper proposes the relevance argumentation of fast sparse  retrieval with selective dense retrieval 
while only adds   a modest amount of extra computing cost on  a CPU-only platform.
This scheme takes an advantage of an advanced  dense retrieval model and 
boosts sparse retrieval with limited  embedding  computation.  
This paper provides a detailed evaluatin with MS MARCO and BEIR  datasets  
on the usefulness of the proposed scheme  in improving the recall and relevance metric of sparse retrieval.
The emprial findings suggest that it  can outperform other baselines for a balanced effectiveness and efficiency. 

{\bf Abstract Version 1  (weakness too much like LADR):}
Recent studies show that sparse retrieval with a learned representation
can be greatly accelerated by BM25-guided index traversal with a tradeoff  in its relevance effectiveness.
This paper proposes the relevance argumentation of fast sparse  retrieval with cluster-based selective dense retrieval called CSDR 
while only imposes   a modest amount of extra computing cost on  a CPU-only platform.
CSDR takes an advantage of clustering under an advanced  dense retrieval model and
detects clusters of documents that can boost sparse retrieval with  limited  embedding  computation.
This paper provides a detailed evaluatin with MS MARCO and BEIR  datasets  
on the usefulness of CSDR in improving the recall and relevance metric of sparse retrieval.
The emprial findings suggest that CSRF  can outperform other baselines for a balanced effectiveness and efficiency. 

%make a determination if  a query can  benefit from additional dense retrieval results,  

{\bf Version 2  (weakness too much on fusion)}
Dense and sparse retrievers are two main categories of the
first-stage search techniques for text  documents, and both of them have benefited 
from pretrained language models to provide effective semantic text matching between a query and a document.
Previous work has shown that  ranking of documents from dense and sparse retrievers could be combined for higher relevance effectiveness. 
The downside is that dense retrieval is time consuming on a CPU-only server platform.
This paper considers the optimization of dense and sparse retrieval fusion and 
 proposes a cluster-based selective dense retrieval scheme called CSDR which only requires triggering of dense retrieval 
computation for a relatively small subset of documents after  fast sparse retrieval. 
CSDR takes an advantage of clustering under an advanced  dense retrieval model and
detects clusters of documents that can boost sparse retrieval with  embedding  computation.
This paper provides a detailed evaluation with MS MARCO and BEIR  datasets  
on the usefulness of CSDR in improving the effectiveness of sparse retrieval with limited dense  retrieval
traversal.  Our empirical findings suggest that CSDR can outperform other baselines on a single CPU server 
without GPUs, and achieve a strong tradeoff of effectiveness and efficiency compared to an exhaustive dense retrieval search.
}
%{\bf Version 3  (combine 2 and 3)}
%Dense and sparse retrievers are two main categories of the
%first-stage search techniques for text  documents, and both of them have benefited 
%from pretrained language models to provide effective semantic text matching between a query and a document.
%Previous work has shown that  ranking of documents from dense and sparse retrievers could be combined for higher relevance effectiveness. 
%The downside is that dense retrieval is time consuming on a CPU-only server platform.

%Sparse retrieval and dense retrieval with a learned representation space
%can be greatly accelerated with tradeoffs  in its relevance effectiveness.
%suggest  that both categories  of retrievers tend to capture  different relevant signals.

%Sparse and dense  sparse retrievers are two main categories of the
%first-stage search techniques for text  documents, and both of them can be accelerated with various relevance tradeoffs. 
%This paper studies how to fuse them but avoid  excessive redundant computation.

Recent studies show that sparse retrieval with a learned representation
can be greatly accelerated but there are  tradeoffs  in its relevance effectiveness.
This paper proposes a relevance augmentation scheme of fast sparse  retrieval with cluster-based selective dense retrieval called CluSD
on  a CPU-only platform.
CluSD takes an advantage of clustering under an advanced  dense retrieval model and
detects clusters of documents that can boost sparse retrieval with  limited  extra memory space overhead and embedding selection and computing time. 
This paper provides a detailed evaluation of CluSD with MS MARCO and BEIR  datasets, 
and demonstrates its effectiveness in improving the relevance metric of sparse retrieval by scoring  selected clusters 
at a low time and space cost.

%  This paper proposes the relevance argumentation of fast sparse  retrieval with cluster-based selective dense retrieval called CluSD 
%  This paper proposes the relevance augmentation of fast sparse  retrieval with cluster-based selective dense retrieval called CluSD,
%  while only imposing   a modest amount of extra cost on  a CPU-only platform.
%  CluSD takes an advantage of clustering under an advanced  dense retrieval model and
%  detects clusters of documents that can boost sparse retrieval with  limited  extra memory space overhead and embedding  computation. 
%  This paper provides a detailed evaluatin of CluSD when searching  in-domain MS MARCO passages and out-of-domain BEIR  datasets 
%  This paper provides a detailed evaluation of CluSD when searching  in-domain MS MARCO passages and out-of-domain BEIR  datasets 
%  and demonstrates its effectivness in improving the relevance metric of sparse retrieval by scoring  selected clusters with dense embeddings
%  at a low time and space cost.
 



%The emprial findings suggest that CSRF  can outperform other baselines for a balanced effectiveness and efficiency. 


==> background.tex <==
%\section{Related Work}
%\label{sect:background}

{\bf Sparse and dense retrieval}. 
%A traditional method for first-stage retrieval uses 
%BM25 based additive ranking with a bag-of-words sparse document representation~\cite{Robertson2009BM25}
%and fast retrieval can be designed  using the inverted index data structure to exploit this
%sparse representation.
To improve traditional BM25 lexical sparse retrieval, 
%Meanwhile, an advancement in sparse retrieval with inverted indices is to 
%adopt learned sparse representations with neural term weights, which has
%yielded in  a significant relevance gain. 
%severl studies  have developed  
learned sparse representations with neural term weights have been studied in 
DeepCT~\cite{Dai2020deepct},
DeepImpact~\cite{Mallia2021deepimpact}, uniCOIL~\cite{Lin2021unicoil,2021NAACL-Gao-COIL},
SPLADE~\cite{Formal2021SPLADE, Formal2021SPLADEV2}. 
Pre-training optimization of a language model for SPLADE-like retrieval 
is studied in LexMAE~\cite{shen2023lexmae}. 
%following the pretraining optimization in SimLM~\cite{Wang2022SimLM}
and RetroMAE~\cite{Liu2022RetroMAE}.
\comments{
The  evaluation of our work for the first-stage retrieval
centers on the SPLADE family of sparse retrieval~\cite{Formal2021SPLADE, Formal2021SPLADEV2} 
because it can deliver a strong relevance with maintaining low space and time costs during inference.
For instance, SPLADE++~\cite{Formal2022SPLADE++} 
delivers 0.38 MRR@10 for the MS MARCO passage Dev set and it is possible to improve this score 
to 0.394 as shown in Section~\ref{sect:evaluation}.  
}
We use SPLADE in our evaluation because it has been well studied by  
a number of papers  with various efficiency optimization options as discussed below
and LexMAE has not made its checkpoints available for evaluation. 
Besides, using a sparse model like LexMAE with better language model pretraining is orthogonal and complementary to our study.
% not sure if the last sentence is needed

Initially there was a concern
that online traversal  of  a learned  inverted index is significantly slower than a BM25 based index,
the recent efficiency studies such as guided traversal and index pruning with sparsification 
show that the  latency of learned sparse retrieval  can be 
reduced dramatically~\cite{Lassance2022SPLADE-efficient,mallia2022faster,qiao2023optimizing,2023SIGIR-SPLADE-pruning}.
%In~\cite{Qiao20222GT}, the model retrieves top 1000 documents in 43ms with 0.394 MRR@10, 25ms with 0.388 MRR@10, or 
%15ms with 0.379 MRR@10, under different index sizes respectively.

% should be approximate search or approximate nearest neighbor search
\comments{
This performance score is very close to 0.395 produced by
AR2 dense retrieval with approximate search which requires 8 NVIDIA Tesla A100 GPUs.
AR2 dense retrieval with approximate search using faiss 
IndexFlatIP~\footnote{https://faiss.ai/cpp_api/struct/structfaiss_1_1IndexFlatIP.html} 
which uses a flat index with exhaustive search.  
%Qiao20222GT.
%takes about a few hundred milliseconds without GPA support and can be further reduced to  up-to 80ms with a small relevance 
%tradeoff~\cite{Lassance2022SPLADE-efficient,AskYifan}.
Meanwhile, avoiding exhaustive exact search in  dense retrieval with approximate search comes with a 
tradeoff of  a relevance drop~\cite{2021Facebook-DrBoost-Lewis, johnson2019billion, Xiao2022Distill-VQ}.
For instance, %AR2 dense retrieval with exact search yields an MRR@10 of 0.395 while 
with Distill-VQ~\cite{Xiao2022Distill-VQ} , a recent 
joint IVF and PQ based ANN search framework, AR2 has an MRR@10 of 0.361 as opposed to 0.395.
%, which still needs GPU support
%because a dense retriever has a significant relerence loss when using faster but 

Notice that for a large-scale search system containing billions of documents, 
the first-stage fast retrieval is typically executed in parallel across many index partitions hosted on
a large number of  machines. In such cases, efficient retrieval with inexpensive hardware could be preferred. 

}

Dense retrieval is an alternative approach for the first-stage search with a dual encoder architecture
%For example, TCT-ColBERT~\cite{Lin2021tctcolbert} and  JPQ~\cite{2021CIKM-JPQ-Zhan}
(e.g. ~\cite{xiong2021-ANCE,gao-2021-condenser}).
Since the representation  for a document and a query is a dense vector,
%Efficiency studies for dense retrieval have been conducted on
fast dense retrieval for a large dataset requires
approximate nearest neighbor (ANN) search~\cite{johnson2019billion} 
%exhaustive exact search~\cite{2021Facebook-DrBoost-Lewis}  
%and ~\cite{Xiao2022Distill-VQ}, 
or  a more expensive GPU server.
%and quantization~\citep{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ},
%applying dense retrieval on  a large dataset requires requires an approximate nereast neighbor search a more expensive GPU 
%, which is more suitable for a GPU-based platform for fast processing.
There are numerous studies recently to enhance  dense retrieval with knowledge distillation
and  improved  language model pretraining~\cite{Lin2021tctcolbert, Santhanam2021ColBERTv2,  Ren2021RocketQAv2,
Wang2022SimLM,  Liu2022RetroMAE}.

\comments{
Retrieval that uses a dense representation of documents and a dual-encoder (or also called bi-encoder) architecture 
outperforms BM25 significantly in relevance at the cost of relatively more expensive similarity computation
%For example, TCT-ColBERT~\cite{Lin2021tctcolbert} and  JPQ~\cite{2021CIKM-JPQ-Zhan}
(e.g. ~\cite{Lin2021tctcolbert, 2021CIKM-JPQ-Zhan, xiong2021-ANCE,gao-2021-condenser,2021SIGIR-Zhan-ADORE-dense,Ren2021RocketQAv2}). 
Efficiency studies for dense retrieval have been conducted on
approximate nearest neighbor (ANN) search~\cite{johnson2019billion} to avoid
exhaustive exact search~\cite{2021Facebook-DrBoost-Lewis}  and  quantization~\citep{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ}, 
%Meanwhile, avoiding exhaustive exact search in  dense retrieval with approximate search 
and these optimizations come with a tradeoff of  a relevance drop.
}

{\bf Combining  dense and sparse retrieval.}
%The earlier IR studies use the term fusion to combine rankers, e.g.  the reciprocal rank fusion (RRF)~\cite{Cormack2009RRF}.
The neural IR studies  have  considered combining the traditional lexical ranking signals and neural semantic matching signals~\cite{Mitra2017LearningTM,Shao2019PrivacyawareDR,Gao2020ComplementingLR,Luan2020SparseDA,Yang2021WSDM-BECR}. 
It is found that combining  sparse and dense retrieval scores  
can further boost recall and/or other relevance metrics~\cite{Lin2021unicoil,2022LinearInterpolationJimLin, kuzi2020leveraging}, which
suggest  that both categories  of retrievers tend to capture  different relevant signals. However, these studies do not address slow  latency  of
dense retrieval on a CPU-only server.
% and do not consider impact of data compression  in dense retrieval. 
%The focus of this paper follows ~\cite{Lin2021unicoil,2022LinearInterpolationJimLin,kuzi2020leveraging} to 
%to combine the ranking results of two retrievers with a linear interpolation,
%
\comments{
We adopt 
a simple fusion wit linear combination ~\cite{Lin2021unicoil,2022LinearInterpolationJimLin,kuzi2020leveraging}, 
which allows the proposed techniques to  easily adopt the latest dense or sparse retriever models.
Our query filtering work is motivated by
the dense and sparse retriever selection study~\cite{2021CIKM-PredictDenseSparse}
when to use BM25 retriever or a  dense retriever.
The difference is our work always assumes sparse retrieval is conducted first, and our selection focuses on how to choose part of dense clusters.
Another difference is that we exploit the characteristics of a learned lexical representation in query encoding and expansion in making a query-level decision.
% filtering exploits the SPLADE encoding as SPLADE is our primary targeted sparse retrieval, even 
%our work is applicable to other sparse retrivers such as BM25. 
}

{\bf Re-ranking.} 
There  are many studies that exploit advanced re-ranking in a multi-stage search pipeline with modern
neural IR techniques(e.g. ~\cite{MacAvaney2019SIGIR-cedr, MacAvaney2020SIGIR-prettr, 2023SIGIR-ZhuangRankT5,Yang2022CQ,Zhuang2021TILDEv2,2022WWWforwardIndex}),
possibly leveraging more expense GPU platforms to conduct complex scoring.
These  re-ranking pipelines perform very well but are inherently limited by the recall of the first-stage retrieval
as pointed out in  ~\cite{2022CIKM-MacAvaneyGraphReRank, 2023SIGIR-LADR}. 
A  focus of this work is to enhance the relevance of retrieval with CPU-friendly low-cost optimization by expanding the candidate pool of  
fast sparse retrieval using selective  dense retrieval at a modest amount of extra CPU cost and without incurring significant  space cost.  

{\bf Cluster based retrieval and proximity graph navigation based on inter-document similarity.}
%with lexical matching
There has been a large body of studies on cluster-based document retrieval  in traditional IR
throughout the last few decades (e.g.  ~\cite{liu2004cluster,2022SIGIR-KurlandClusterRank,kurland2008opposite}).
In most of cases, it has been applied to re-rank an initial retrieved list by creating clusters of similar  documents in this list. Then the clusters are ranked and the cluster ranking may be further transformed to document ranking.  
%{\bf Proximity graph navagation based on inter-document similarity.}
Search with  inter-document similarity is  also studied~\cite{2006NAACL-docExpan}.
The above studies follow traditional IR   with  lexical signals. 
Advance in neural representations introduces new opportunities and challenges, as studied in  
GAR~\cite{2022CIKM-MacAvaneyGraphReRank} and LADR~\cite{2023SIGIR-LADR} following
HNSW~\cite{2020TPAMI-HNSW} for proximity graph based search with inter-document similarity.
%~\cite{2020TPAMI-HNSW,2022CIKM-MacAvaneyGraphReRank, 2023SIGIR-LADR}.
% is viewed as  a modern instantiation 
%of the clustering hypothesis to revisit these ideas in a new context.  

Motivated by such studies, our work emphasizes on fast selective dense retrieval to augment sparse retrieval effectively
without introducing substantial memory space overhead  by exploiting  inter-cluster and query-cluster similarity at a coarse grain level. 
%Result overlapping degree of sparse retrieval with the dense clusters also plays a key role in the low-cost selection  of dense clusters.

{\bf  Dense retrieval with approximate nearest neighbor search and IVF clustering.}
Faster dense retrieval can be accomplished by approximate nearest neighbor search~\cite{2021Facebook-DrBoost-Lewis, johnson2019billion} with 
a small number of top clusters  (e.g. IVF-based), which can run efficiently on a CPU-only  server.
Memory space cost of dense retrieval can be reduced significantly by 
embedding  quantization (e.g.  ~\cite{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ}).
Using these techniques has a tradeoff with a significant relevance drop as shown in these previous studies. 
Our evaluation confirms  that sparse retrieval aided with top IVF-based dense clusters does not yield a competitive relevance 
under a tight time budget.  


There is also a line of work on cluster-based earlier termination studies for nearest neighbor search over a large   high dimensional 
feature vector collection~\cite{2020SIGMOD-ANNadaptive,2023USENIX-ANNcluster}.
The above techniques are targeted for generic data applications and  are not investigated in the context of text document  retrieval where
semantic  relevance presents   its unique ranking challenge and  
requires new design considerations and model structuring.  Another difference is that in our context,
dense cluster selection is conducted after sparse retrieval, which demands optimization that  exploits the interaction  between
these two stages.




==> cikmabs.tex <==



\comment{
{\bf Old abstract:}
Recent studies show that neural sparse retrieval for searching  text documents with a learned neural representation
can be greatly accelerated but there are  tradeoffs  in its relevance effectiveness.
This paper proposes a relevance augmentation scheme of fast sparse  document retrieval with cluster-based selective dense retrieval called CluSD
on  a CPU-only platform.
CluSD takes an advantage of clustering under an advanced  dense retrieval model and
detects clusters of neural embeddings  that can boost sparse retrieval with  limited  extra memory space overhead and embedding selection and computing time. 
This paper provides a detailed evaluation of CluSD for searching  MS MARCO and BEIR  datasets, 
and demonstrates its effectiveness in improving the relevance metric of sparse retrieval by scoring  selected dense embedding clusters 
at a low time and space cost.


{\bf New abstract:}
 both of which have benefited from pretrained language models.
}
%Dense retrieval and sparse lexical retrieval are two main categories of the first-stage search techniques for 
%text  documents.  
Dense retrieval is attractive  in semantic  matching between queries and
text  documents, though it can be time-consuming on a CPU-only platform.
The cost of dense retrieval can be mitigated through approximate nearest neighbor search techniques, including IVF clustering, quantization, and/or 
proximity graph navigation. However, the reduction in latency by using these techniques comes with a tradeoff  in relevance effectiveness. 
This paper proposes a cluster-based selective dense retrieval method called CluSD with an augmentation from sparse lexical retrieval 
at a low space and CPU time cost. 
CluSD takes a lightweight cluster-based approach and exploits the overlap of sparse retrieval results and embedding clusters
in a two-stage selection process with an LSTM model to quickly identify relevant clusters  while incurring limited  extra memory space overhead. 
CluSD  triggers partial dense retrieval, performs cluster-based block disk I/O if needed, and combines dense scores  with  sparse results to enhance relevance. 
%advantage of clustering of embeddings from an advanced dense retrieval model, 
This paper provides a comprehensive evaluation of CluSD on in-memory and on-disk search of the MS MARCO and BEIR  datasets.
%(the MS MARCO dataset) and out-of-domain (BEIR  datasets) search tasks
%and demonstrates its effectiveness in relevance and efficiency.




==> cikmbackground.tex <==
%\section{Related Work}
%\label{sect:background}

\textbf{Sparse and dense retrieval.}
%A traditional method for first-stage retrieval uses 
%BM25 based additive ranking with a bag-of-words sparse document representation~\cite{Robertson2009BM25}
%and fast retrieval can be designed  using the inverted index data structure to exploit this
%sparse representation.
To improve traditional BM25 lexical sparse retrieval, 
%Meanwhile, an advancement in sparse retrieval with inverted indices is to 
%adopt learned sparse representations with neural term weights, which has
%yielded in  a significant relevance gain. 
%severl studies  have developed  
learned sparse representations with neural term weights have been studied in 
DeepCT~\cite{Dai2020deepct},
DeepImpact~\cite{Mallia2021deepimpact}, uniCOIL~\cite{Lin2021unicoil,2021NAACL-Gao-COIL},
and SPLADE~\cite{Formal2021SPLADE, Formal2021SPLADEV2}. 
Pre-training optimization of a language model for SPLADE-like retrieval is studied in LexMAE~\cite{shen2023lexmae}. 
Retriever efficiency optimization techniques have been developed for learned
sparse representations~\cite{Lassance2022SPLADE-efficient,mallia2022faster,qiao2023optimizing,2023SIGIR-Qiao, 2023SIGIR-SPLADE-pruning,2022ACMTransAnytime, 2022EMNLP-mackenzie-clipping} at various  efficiency and relevance tradeoffs.
%following the pretraining optimization in SimLM~\cite{Wang2022SimLM} and RetroMAE~\cite{Liu2022RetroMAE}.
% should be approximate search or approximate nearest neighbor search
\comments{
This performance score is very close to 0.395 produced by
AR2 dense retrieval with approximate search which requires 8 NVIDIA Tesla A100 GPUs.
AR2 dense retrieval with approximate search using faiss 
IndexFlatIP~\footnote{https://faiss.ai/cpp_api/struct/structfaiss_1_1IndexFlatIP.html} 
which uses a flat index with exhaustive search.  
%Qiao20222GT.
%takes about a few hundred milliseconds without GPA support and can be further reduced to  up-to 80ms with a small relevance 
%tradeoff~\cite{Lassance2022SPLADE-efficient,AskYifan}.
Meanwhile, avoiding exhaustive exact search in  dense retrieval with approximate search comes with a 
tradeoff of  a relevance drop~\cite{2021Facebook-DrBoost-Lewis, johnson2019billion, Xiao2022Distill-VQ}.
For instance, %AR2 dense retrieval with exact search yields an MRR@10 of 0.395 while 
with Distill-VQ~\cite{Xiao2022Distill-VQ} , a recent 
joint IVF and PQ based ANN search framework, AR2 has an MRR@10 of 0.361 as opposed to 0.395.
%, which still needs GPU support
%because a dense retriever has a significant relerence loss when using faster but 

Notice that for a large-scale search system containing billions of documents, 
the first-stage fast retrieval is typically executed in parallel across many index partitions hosted on
a large number of  machines. In such cases, efficient retrieval with inexpensive hardware could be preferred. 

}
Dense retrieval is an alternative approach for the first-stage search with a dual encoder architecture
%For example, TCT-ColBERT~\cite{Lin2021tctcolbert} and  JPQ~\cite{2021CIKM-JPQ-Zhan}
(e.g. ~\cite{xiong2021-ANCE,gao-2021-condenser}).
Since the representation  for a document and a query is a dense vector,
%Efficiency studies for dense retrieval have been conducted on
fast dense retrieval for a large dataset requires
approximate nearest neighbor (ANN) search~\cite{johnson2019billion},
%exhaustive exact search~\cite{2021Facebook-DrBoost-Lewis}  
%and ~\cite{Xiao2022Distill-VQ}, 
or  a more expensive GPU server.
%and quantization~\citep{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ},
%applying dense retrieval on  a large dataset requires requires an approximate nereast neighbor search a more expensive GPU 
%, which is more suitable for a GPU-based platform for fast processing.
There are numerous recent studies to enhance  dense retrieval with knowledge distillation
and  improved  language model pretraining~\cite{Lin2021tctcolbert, Santhanam2021ColBERTv2,  Ren2021RocketQAv2,
Wang2022SimLM,  Liu2022RetroMAE}.

\comments{
Retrieval that uses a dense representation of documents and a dual-encoder (or also called bi-encoder) architecture 
outperforms BM25 significantly in relevance at the cost of relatively more expensive similarity computation
%For example, TCT-ColBERT~\cite{Lin2021tctcolbert} and  JPQ~\cite{2021CIKM-JPQ-Zhan}
(e.g. ~\cite{Lin2021tctcolbert, 2021CIKM-JPQ-Zhan, xiong2021-ANCE,gao-2021-condenser,2021SIGIR-Zhan-ADORE-dense,Ren2021RocketQAv2}). 
Efficiency studies for dense retrieval have been conducted on
approximate nearest neighbor (ANN) search~\cite{johnson2019billion} to avoid
exhaustive exact search~\cite{2021Facebook-DrBoost-Lewis}  and  quantization~\citep{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ}, 
%Meanwhile, avoiding exhaustive exact search in  dense retrieval with approximate search 
and these optimizations come with a tradeoff of  a relevance drop.
}

\textbf{Combining  dense and sparse retrieval.}
%The earlier IR studies use the term fusion to combine rankers, e.g.  the reciprocal rank fusion (RRF)~\cite{Cormack2009RRF}.
Previous neural IR studies  have  considered combining the traditional lexical ranking signals and neural semantic matching signals~\cite{Mitra2017LearningTM,Shao2019PrivacyawareDR,Gao2020ComplementingLR,Luan2020SparseDA,Yang2021WSDM-BECR}. 
Recent work has found that combining  sparse and dense retrieval scores  
can further boost recall and/or other relevance metrics~\cite{Lin2021unicoil,2022LinearInterpolationJimLin, kuzi2020leveraging}, which
suggests  that both categories  of retrievers tend to capture  different relevant signals. However, these studies do not address the high  latency  of
dense retrieval on a CPU-only server.
% and do not consider impact of data compression  in dense retrieval. 
%The focus of this paper follows ~\cite{Lin2021unicoil,2022LinearInterpolationJimLin,kuzi2020leveraging} to 
%to combine the ranking results of two retrievers with a linear interpolation,
%
\comments{
We adopt 
a simple fusion wit linear combination ~\cite{Lin2021unicoil,2022LinearInterpolationJimLin,kuzi2020leveraging}, 
which allows the proposed techniques to  easily adopt the latest dense or sparse retriever models.
Our query filtering work is motivated by
the dense and sparse retriever selection study~\cite{2021CIKM-PredictDenseSparse}
when to use BM25 retriever or a  dense retriever.
The difference is our work always assumes sparse retrieval is conducted first, and our selection focuses on how to choose part of dense clusters.
Another difference is that we exploit the characteristics of a learned lexical representation in query encoding and expansion in making a query-level decision.
% filtering exploits the SPLADE encoding as SPLADE is our primary targeted sparse retrieval, even 
%our work is applicable to other sparse retrivers such as BM25. 
}

\textbf{Reranking.}
There  are many studies that exploit advanced re-ranking in a multi-stage search pipeline with modern
neural IR techniques (e.g. ~\cite{MacAvaney2019SIGIR-cedr, MacAvaney2020SIGIR-prettr, 2023SIGIR-ZhuangRankT5,Yang2022CQ,Zhuang2021TILDEv2,2022WWWforwardIndex}),
possibly leveraging more expensive GPU platforms to conduct complex scoring.
These  re-ranking pipelines perform very well but are inherently limited by the recall of the first-stage retrieval,
as noted in  ~\cite{2022CIKM-MacAvaneyGraphReRank, 2023SIGIR-LADR}. 
A focus of this work is improving the relevance of fast sparse retrievers by expanding the candidate pool of first-stage retrieval using 
selective dense retrieval, and by a CPU-friendly optimization that incurs small or modest additional CPU and space cost.
% Parker: I reworked below into above. Still might need work, but let me come back to it
%A  focus of this work is to enhance the relevance of retrieval with CPU-friendly low-cost optimization by expanding the candidate pool of  
%fast sparse retrieval using selective  dense retrieval at a modest amount of extra CPU cost and without incurring significant  space cost.  

\comments{
{\bf Cluster based retrieval and proximity graph navigation based on inter-document similarity.}
%with lexical matching
There is a large body of work on cluster-based document retrieval  in traditional IR
throughout the past few decades (e.g.  ~\cite{liu2004cluster,2022SIGIR-KurlandClusterRank,kurland2008opposite}).
In most cases, it has been applied to re-rank an initial retrieved list by creating clusters of similar  documents in this list. 
Then, the clusters are ranked, which may be further transformed to document rankings.  
%{\bf Proximity graph navagation based on inter-document similarity.}
Search with  inter-document similarity has also been studied~\cite{2006NAACL-docExpan}.
The above studies follow traditional IR   with  lexical signals. 
Advances in neural representations introduce new opportunities and challenges, as studied in  
GAR~\cite{2022CIKM-MacAvaneyGraphReRank} and LADR~\cite{2023SIGIR-LADR}, following
HNSW~\cite{2020TPAMI-HNSW} and NAPG~\cite{2021KDDgraphANN}
for proximity graph based search with inter-document similarity.
%~\cite{2020TPAMI-HNSW,2022CIKM-MacAvaneyGraphReRank, 2023SIGIR-LADR}.
% is viewed as  a modern instantiation 
%of the clustering hypothesis to revisit these ideas in a new context.  

Motivated by such studies, our work emphasizes fast selective dense retrieval to augment sparse retrieval effectively
without introducing substantial memory overhead by exploiting inter-cluster similarity and query-cluster similarity at a coarse-grain level. 
%Result overlapping degree of sparse retrieval with the dense clusters also plays a key role in the low-cost selection  of dense clusters.
}

\textbf{Approximate nearest neighbor search.}
In addition to the IVF cluster 
search~\cite{johnson2019billion}, and proximity graph navigation such as HNSW~\cite{2020TPAMI-HNSW}, NAPG~\cite{2021KDDgraphANN},
GAR~\cite{2022CIKM-MacAvaneyGraphReRank},  and LADR~\cite{2023SIGIR-LADR}, discussed in Section~\ref{sect:intro}, 
\comments{
Faster dense retrieval can be accomplished by approximate nearest neighbor search~\cite{2021Facebook-DrBoost-Lewis, johnson2019billion} with 
a small number of top clusters  (e.g. IVF-based), which can run efficiently on a CPU-only  server.
The memory space cost of dense retrieval can be reduced significantly by 
embedding  quantization (e.g.  ~\cite{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ}).
However, these techniques have a tradeoff: a significant drop in relevance, as shown in these previous studies.
%Using these techniques has a tradeoff with a significant relevance drop as shown in these previous studies. 
Our evaluation confirms  that sparse retrieval aided with top IVF-based dense clusters does not yield a competitive relevance 
under a tight time budget.  
}
there  are studies on  cluster-based earlier termination studies for nearest neighbor search over a large   
feature vector collection~\cite{2020SIGMOD-ANNadaptive,2023USENIX-ANNcluster, 2023VLDB-FARGO}.
The use of locality sensitive hashing  for high-dimensional ANN search 
is studied in~\cite{2020VLDB-ANN-LSH,2023VLDB-FARGO,2015KDD-LSH-ANN} to approximate in
a projected space, and the improvement of a proximity graph is studied in~\cite{2021KDDgraphANN}.
DiskANN, SPANN,  and other follow-up studies~\cite{NEURIPS2019_DiskANN,2023Web-Filtered-DiskANN,2020NIPS-HM-ANN, chen2021spann}
address ANN search when data cannot fit in memory. 
The above techniques are targeted at general data applications and have not been studied in the context of text document retrieval.
%where the importance of semantic matching presents a unique challenge and requires new design considerations.
Another key difference is that the above studies assume a standalone search task with dense retrieval,
whereas we exploit overlapping of sparse and dense retrieval to guide  optimization.
Running sparse retrieval initially narrows the search scope quickly at a low cost, as 
sparse retrieval leverages the inverted index. Sparse and dense models capture different relevant signals with 
varying weights, but they share substantial overlap in content semantics. By exploiting this overlap, we can quickly identify top results for dense retrieval. The fusion of scores from these two representations reinforces top-ranked documents.

%The above techniques are targeted for general data applications and  have not investigated in the context of text document  retrieval where
%semantic  matching relevance presents   its unique ranking challenge and  
%requires new design considerations and model structuring.  Another key difference is that the above studies assume a standalone search task.
%in our context the interaction of sparse retreival and dense retrieval  is exploited, which demands new optimization. 



==> cikmconcl.tex <==
%\section{Limitations and Future Work}
%\vspace*{-2mm}
\section{Concluding Remarks}

We have demonstrated that CluSD, a lightweight cluster-based partial dense retrieval method,
can deliver fast response time and competitive relevance on affordable computing platforms,
without the need of an expensive document-wise proximity graph.
%The main contribution of this work is  to  show  how 
%a lightweight cluster-based partial dense retrieval 
%with competitive  relevance can be made possible
%to deliver fast response time on affordable computing platforms, without the need of an expensive  document-wise  proximity graph.
%CluSD carries with minimal space overhead compared to the orginal dense retrieval
%and incurrs a small amount of CPU latency time due to the limited dense computation.
\comments{
CluSD uses  an LSTM-based  model and  leverages sparse retrieval results to effectively identify  a small number of 
clusters that can supplement and boost the relevance of partial dense  retrieval.  
With this lightweight low-cost design,  
CluSD is suitable for a CPU-only low-cost server while delivering  a fairly strong  in-domain and out-of-domain relevance.  
For example, CluSD delivers 0.423 MRR@10  for searching 8.8M MS MARCO passages 
with 11.4ms  latency and  1.13GB space mainly for compressed dense embeddings, to augment sparse retrieval under
a fraction of its  cost. The same  CluSD version  reaches  0.514 average NDCG@10 for BEIR with compression.
That represents state-of-the-art relevance performance for a retriever that  runs on a CPU-only server. 
}
Guided by sparse retrieval, CluSD significantly outperforms previous cluster-based partial dense retrieval with IVF 
search in relevance under the same time budget.
For example, CluSD delivers 0.431 MRR@10  for searching 8.8M MS MARCO passages with SimLM and LexMAE 
on its Dev test set, while taking only tens of milliseconds on a low-end CPU server,
%and reaches  0.516 average NDCG@10 for BEIR.  
and reaches an average NDCG@10 of 0.541 for BEIR with RepLLaMA and SPLADE.  
The MRR@10 achieved is close to that of RankT5 (0.434)~\cite{2023SIGIR-ZhuangRankT5},
which is an expensive cross-encoder.
Thus, CluSD can deliver a state-of-the-art relevance performance for a retriever that runs efficiently on 
a CPU-only server. 
%The othe recent efficient retrievers reported 0.426  for MS MARCO Dev, and 0.48 for BEIR by LexMAE.
%Its MRR@10 number is close to one reported recently using an expensive cross-encoder RankT5 which reaches 0.434~\cite{2023SIGIR-ZhuangRankT5}. 
%ClusD's BEIR performance is close to  that  of  Promptagator++~\cite{dai2023promptagator}.  Both  RankT5 and Promptagtor++h employ an expensive cross-encoder.
%Noted that user search experience is highly impacted by the ranking order and its relevance thus a relatively small percentage point increase  
%in metrics for the standard public test benchmarks used in this paper is viewed to be hard and valuable in the IR research literature.

%For example,
%Table ~\ref{tab:mainspace} shows CluSD is as fast as IVFOPQ top 2\% search at m=64 and 2x fast at m=128 while its MRR@10  is 11.5\% and 9.5\% higher 
%that only use query-centroid distances to select clusters. 

Under the same time budget, CluSD delivers similar or higher relevance than methods that rely upon
a document-level proximity graph, such as LADR and HNSW, with negligible extra space overhead.
Further, CluSD is up-to 12.1x faster by avoiding fine-grained document-level disk I/O when embeddings do not fit in memory.
When compared to general on-disk ANN search methods DiskANN and SPANN~\cite{NEURIPS2019_DiskANN,2023Web-Filtered-DiskANN},
CluSD is 2.2x and 4.97x faster respectively, while achieving better relevance
% for text document search 
by leveraging sparse retrieval.
Thus, compared to graph navigation approaches, CluSD is lightweight, with both low space overhead and low I/O cost.
%Compared to LADR and HNSW, our evaluation demonstrates that without a document-level proximity graph, CluSD can 
%deliver a similar or higher 
%relevance under the same time budget
%with negligible extra space overhead when embeddings are available in memory  and  up-to 6.9x   faster by avoiding fine-grained document-level disk I/O
%when embeddings do not fit in  memory.  
%Thus the lightweight with low-space overhead  and low-I/O cost is the main advantage of CluSD compared to a graph navigation approach.
\comments{
For example, Table ~\ref{tab:maintime} shows
CluSD has 2\% higher MRR@10  than LADR and 1.2\% higher than HNSW under a time budget of 25ms.
%It is attractive to run such an algorithm on a first-stage retrieval low-cost machine
%that can significantly reduce the overall infrastructure cost when scaling  data size and search traffic. 
}
%Compared to several on-disk nearest-search efforts  with DiskANN and SPANN~\cite{NEURIPS2019_DiskANN,2023Web-Filtered-DiskANN},
%like HNSW, they are targeted for a general ANN problem while our
%work takes advantage of sparse retrieval with 15.6x and 7x faster  latency and better relevance in the context of text document search.


CluSD is also stronger and more versatile than reranking. 
Simple reranking does surprisingly well if sparse results are strong. But as stated in~\cite{2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR},
when the sparse retriever doesn’t achieve high relevance, reranking is too 
restrictive and recall@1K does not increase as shown in Table 5. 
\comments{
For example, after 
sparse retrieval with SPLADE-effi-HT3 with 0.944 recall@1K, reranking does not increase it while CluSD increases it to 0.984.
While reranking restricts candidate documents to the top sparse results, CluSD adds more diversified results from selected dense clusters. 
}
CluSD’s advantage becomes more significant in zero-shot retrieval as shown in Table 6 with 13 BEIR datasets. CluSD’s average NDCG number is 
7.2\% higher than reranking with RetroMAE. With SimLM, CluSD is 4\% higher than reranking.
In addition, when embeddings are not available in memory, reranking is 2.85x slower in mean latency.

%becomes very slow with a large number of document-level random I/O operations. 

CluSD works well  with LLaMA-2 based RepLLaMA dense  model for the tested datasets.
With more dense models  developed in the future using large language models of high dimensionality for better relevance,
our study  sheds a light on how to take advantages of such models on low-cost CPU servers, 
especially when their embeddings cannot fit into memory and are hosted on disk.

Our evaluation has not used ColBERT with a multi-vector representation because 
ColBERTv2's MRR@10~\cite{Santhanam2021ColBERTv2}  for MS MARCO is 0.397, which is lower than that the single-vector dense models studied in this paper. 
CluSD techniques are  orthogonal to ColBERTv2 and could be used with ColBERTv2 after small modifications.

\comments{
Our evaluation uses OPQ in FAISS. 
Switching to a different quantization affects the compression ratio and  the relevance outcome. 
However, we expect that our findings remain similar and  the recent  quantization 
methods~\cite{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ}
also have  a significant relevance drop pattern when the compression ratio increases.
%A limitation of the current  CluSD work is that the training of the LSTM model has a dependence on the sparse retrieval model used. 
%While  CluSD can  boost the relevance of a weaker sparse retriever model such as BM25, the augmented relevance still has not reached a level
%comparable  to the one where CluSD is coupled with a stronger sparse retriever. There is room for improvement in future work.

}

%the dependency on a training dataset. Unlike rule-based or unsupervised pipelines, our pipeline requires labeled data on at least one search task. However, the number of queries with labels is not large and a trained model is robust on never-seen corpus and tasks. 
%
%Another limitation is the dependency on the sparse retrieval model performance. CluSD benefit from a good sparse retrieval top results. When using a BM25 based retrieval, the quality of the clusters selected degrades slightly. 


==> cikmdesign.tex <==

\comments{
Sparse retrieval with a learned representation  is much slower than BM25
        Guided sparse retrieval can speedup, but there is a trade in  effectiveness
        Augmenting sparse retrieval with dense retrieval through fusion can make up the loss
        Selective dense  retrieval can make up the loss argument sparse retiieval more effective with limited extra computing cost.

Points to market: Option 2

                New dense retrieval algorithms have been developed every year that beat new performance records.
                New fast  sparse retrieval algorithms are developed.
                Fusion of  sparse retrieval and dense retrieval is helpful, but slow on a CPU server, dominating by dense computation.
                There is a clear redudance of computation as both retrievers scan the same dataset with different representation
                        for push for the same top documents.
                How to avoid redudant computation?
                        1) Select dense retrieval. We donot need to scan all dense documents. We can take advanrage of
                clusters of dense documents
                        and only  need to visit top clusters which are similar to a query.
                        2) The use of dense retrieval reduces the relevance reqirement of sparse retrieval. We can use a fast sparse
retrieval BM25-guided sparse retrieval or effient SPLADE version, which quickly retrieves top results. Selective dense retrieval
                can augment  a weaker but faster sparse retriever by only adding limited  extra computing cost
to  improve the recall and relevance metric.

                Challenges:
                        1) How to accomplish  selective clusetrs.
                        Which clusters  can make most contributions
                        2) What queries definitely need dense retrieval boosting?

}
%\section{Design Considerations}
%label{sect:design}
\section{Selective Dense Cluster Retrieval}
\label{sec:clusd}


\comments{
The availability of a dense retriever model, possibly  trained separately by a different language model,
offers opportunities to re-confirm and adjust the ranking of top quality documents in  the initial
candidate pool and improve the  recall by introducing more diversified
candidates.  On the other hand, there is a clear redundancy of computation as both retrievers visit the same dataset 
with different representation, possibly  pursing the  same subset of top documents.
}
 
%{\bf Yingrui, please add a table or figure which shows the distribution of training
%queries if possible, otherise the Dev set of MS MARCOS,  that has the various level of MRR increase.
%I remeber you show us some data you collected during summer or spring.} 
%Table~\ref{tab:fusionanalysis} shows 



%We found that among 33\% of queries in the MSMARCO training set, there is no increase in terms of the MRR@10 when dense retrieval results are added to sparse retrieval results. Namely there are many queries that do not actually benefit from the use of dense retrieval after sparse retrieval.
% two retrievers, and explicitly skipping some of fusion can avoid the unnecessary computing cost.
%Motivated by the above data, 

%Our design considerations are:

%of selective dense retrieval  
%has  the following considerations.
%\begin{itemize} [leftmargin=*]
\comments{
\item  {\bf Partial dense retrieval after  full sparse retrieval.}

%and also there are several techniques developed recently to accelerate learned sparse retrieval,
}

%\item {Inter-cluster vs. inter-document similarity.}
\comments{
{\bf Cluster-based  dense retrieval.}
After the  fusion option is determined for a  query,
there is an option to follow LADR~\cite{2023SIGIR-LADR} and select documents that are similar to
the top sparse retrieval results  using a similarity graph.
These similar documents form candidates  for partial dense retrieval and  rest of un-selected
documents in a dataset can be skipped.  
Maintaining a large inter-document similarity graph online is quite expensive from
offline  data collection, online storage space, and   inference time.


The experience with the learned sparse models such as SPLADE~\cite{Formal2021SPLADE, Formal2021SPLADEV2} showed that
learned sparse representations from  BERT can be very effective.
For example, without optimization in language model pretraining, SPLADE's MRR performance is on par to
the dense retriever by RocketQA~\ref{Ren2021RocketQAv2}. 
Thus there is an opportunity to skip some of scoring computation in dense or sparse retrieval.
Since it is not easy to recognize and separate part of an inverted index  that contains high scoring documents,
we follow the approach of LADR~\cite{2023SIGIR-LADR} and GAR~\cite{2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}
run a sparse retriever completely first and steer partial dense  retrieval. 
}

%Previous studies  with the learned sparse models~\cite{Mallia2021deepimpact, 
%Lin2021unicoil,2021NAACL-Gao-COIL, Formal2021SPLADE, Formal_etal_SIGIR2022_splade++, shen2023lexmae
%Formal2021SPLADE, Formal2021SPLADEV2} showed that
%the relevance resutls from learned sparse representations from  BERT can be  fairly strong.
We aim to identify the opportunity to skip a substantial portion of dense retrieval 
%by exploiting the potential overlap of sparse and  dense retrieval results.
by taking the IVF clustering approach~\cite{johnson2019billion} that  groups similar documents. 
This  helps CluSD to recognize similar relevant documents during inference while avoiding the 
need of a document-level proximity graph. The number of clusters needs to be as large as possible (meaning a small size per cluster) to avoid unnecessary I/O and computing cost. That imposes a significant challenge for accurate and fast selection of dense clusters.

Thus unlike IVF cluster search, our selection goes beyond using the similarity between the query and cluster centroids to 
choose top clusters.  Instead, our work proposes a two-stage selection algorithm that explicitly exploits the overlap of sparse retrieval results with the potential dense clusters for better efficiency and relevance.   

\comments{
As discussed in Section~\ref{sect:intro}, we do not take a document-to-document similarity graph approach~\cite{2020TPAMI-HNSW, 
2022CIKM-MacAvaneyGraphReRank,  2023SIGIR-LADR} to avoid both the large space requirement of hosting such a graph and the high cost of random fine-grained
disk I/O to 
either the dense embedding set or the graph when one of them is hosted on the disk.
}

%and also there are several techniques developed recently to accelerate learned sparse retrieval,
\comments{
There are two ways  to select documents for dense retrieval.
One way is to take a graph navigation approach such as HNSW~\cite{2020TPAMI-HNSW}, GAR~\cite{2022CIKM-MacAvaneyGraphReRank} and LADR~\cite{2023SIGIR-LADR}, 
exploiting  document-to-document similarity links during inference time.
Another way is to follow a clustering  approach to group  documents based on their embedding similarity at offline 
time~\cite{johnson2019billion} and select a small set of  clusters.
%~\cite{2020TPAMI-HNSW,2022CIKM-MacAvaneyGraphReRank, 2023SIGIR-LADR}.
% is viewed as  a modern instantiation
%of the clustering hypothesis to revisit these ideas in a new context.  
We opt to take  the clustering based approach with two reasons.
1) Maintaing a large document-to-document similarity graph with a qudradical complexity is not scalable for  a large  data collection size. 
%As illustrated in  Table~\ref{tab:costbudget}, compression with embedding  quantization is necessary to meet the space constraint.
%due to the memory usage of stroing  embedding vectors. 
%For 8.8M MS MACRO passages, that takes  about 27GB space.
%Fortunately the quantization techniques can significantly compress this space into 1-2GB or even 0.5GB depending on the configuration. 
%Our feature design does not opt for  inter-document similarity since it is space-consuming, but  plans to exploit cluster-based summary information, 
%which  only adds  insignificant  space overhead.  
%\end{itemize}
%, and set a limit on the number of dense clusters used.
2) Embedding vectors of a large dataset with a high dimension per vector may not fit into the memory.
Cluster-based on selection exploits the block-level disk I/O for lower access overhead and higher bandwidth. 
In comparison, random access of selected documents in a graph based approach can suffer higher I/O overhead. 

}
\comments{
We intend to exploit coarse grain cluster-level similarity to reduce the complexity in selective dense retrieval with two reasons.
%The challenge is to how to select clusters  which can make most contributions.
%We opt to take a cluster-level skipping approach with two reasons.
1) Documents can be clustered in advance during offline processing 
%Documents within a cluster similar to a query can provide a large variety of strong candidates to supplement sparse retrieval results.  
2) Cluster-level computation allows  aggregation of  similarity computation for query-document dot products as a fast matrix operation 
to fully  utilize on-chip CPU caches. 
%In comparsion, there is a less chance for online inference to fully benefit from  CPU cache based on an irregular  graph structure.
%During offline processing, it is computationally expensive to drive document-level similarity for all pairs for documents in a large datset.
A research problem  is how to adaptively identify a subset of clusters  which yield sufficient relevance benefits.
% benefitial fusion if  sparse retrieval scoring may be sufficient. In addition to the influence of sparse retrieval results,
% a dynamically-visited dense cluster may provide sufficient high quality documents, reducing the necessarity of visiting
%the remaining dense clusters.   
%Thus we will develop a dynamic feature-driven decision scheme based the results of sparse retrieval.
%and incremtentally navigated  dense document clusters  as input. 
}
\comments{
Another consideration is that there are various relevance and efficiency tradeoff in selecting  a sparse retrieval 
model~\cite{Lassance2022SPLADE-efficient,mallia2022faster,Qiao20222GT,2023SIGIR-Qiao,2023SIGIR-SPLADE-pruning}.
For example, BM25 guided-sparse retrieval can greatly speedup, but lose some recall or precision
 when this guidance is weighted aggressively.
The use of dense retrieval provides a flexibility and reduces  the relevance requirement of sparse retrieval.
Namely potentially we can choose a relatively fast sparse retrieval with the slightly lower accuracy/recall,
and  let dense retrieval make up the loss. Our design
needs to  adapt to  sparse retrieval quality and plans
We plan to exploit features that reveal  the overlapping degree of top sparse retrieval results with  dense clusters
to guide the selection in addition to query-cluster distances. 
}

\comments{
\item  {\bf Query filtering for skipping dense retrieval}
We want an online system to make an earlier  determination if a query needs an argumentation from dense retrieval with supervised learning.
%A challenge is to identify features and infer based on such features with supervised learning.
Given that sparse retrieval is conducted first,
our idea is to predict the quality of sparse retrieval and its relative strength  compared to unexecuted
dense retrieval based on quality of query token expansion by the sparse model,
the statistical behavior of  sparse retrieval results, and
the relationship between dense document embedding summary and sparse retrieval scoring structure.




{\bf Latency budget.}
%Our heuristic-based fusion selection may suffer from an effectiveness tradeoff
%as full dense retrieval execution likely offers the maximum relevance benefits.
For search latency, our goal is to minimize the relevance effectiveness loss to a small degree while still accomplishing  a fast response time
acceptable to the interactive search system requirement.
In a search system running as an interactive  web service,  a query with multi-stage processing
needs to be completed within a few hundred milliseconds.
%Considering the multi-stage search nature  and other service overhead involved, 
A first-stage retriever operation  for a data partition needs to be completed within several tens of milliseconds without query caching (e.g. 200ms). 
Our targeted time budget to augment sparse retrieval cannot be too high     compared to  sparse retrieval cost.
We will evaluate the latency budget in two settings: around 50ms  and 25ms, including the  sparse retrieval time.
%For the example of Table~\ref{tab:costbudget},
%The studies from~\cite{Lassance2022SPLADE-efficientmallia2022GTI,Qiao20222GT,2023SIGIR-Qiao},
If sparse retrieval can complete  in 30 ms on an  average CPU and the total latency
target is around 50ms,  the cost of dense retrieval is targeted under around  20ms.
% At most the total sparse and dense retrieval cannot be more than 100ms.
%Accuracy of above query-specific cluster skipping while retaining a competiitve relevance is the key to accomplish this latency goal. 
%Notice that the latency target in the  LADR paper~\cite{2023SIGIR-LADR} is in a 4ms-8ms range
%and 
%This latency budget choice is reasonable because for 
%Also our evaluation is conducted in a low-end CPU server and a faster CPU can further accelerate. 
%CPU latency reported in~\cite{2022WWWforwardIndex} is at 11

}
\comments{
For the memory space cost,  our target budget for  dense retrieval augmentation is controlled in  the same level or some fraction of  sparse retrieval cost.
As illustrated in  Table~\ref{tab:costbudget}, compression with embedding  quantization is necessary to meet the space constraint.
%due to the memory usage of stroing  embedding vectors. 
%For 8.8M MS MACRO passages, that takes  about 27GB space.
%Fortunately the quantization techniques can significantly compress this space into 1-2GB or even 0.5GB depending on the configuration. 
Our feature design does not opt for  
inter-document similarity since it is space-consuming,
but  plans to exploit cluster-based summary information, 
which  only adds  insignificant  space overhead.  
%, and set a limit on the number of dense clusters used.
}



==> cikmexp.tex <==
\section{Evaluations}

Our evaluation answers  the following research questions:
% and the corresponding subsections are marked:
\textbf{RQ1} (Sect.~\ref{sect:eval0space}): 
How does CluSD perform when searching in-memory datasets?
The baselines to compare include  IVF-based selective dense retrieval, 
graph navigation based selective retrieval, and reranking.
We also provide details on searching  out-of-domain text content.
%extra space overhead is minimized by augmentation under different compression configurations? 
%\textbf{RQ2} (Section~\ref{sect:evaltimebudget}): 
%  under a retrieval latency time budget when there is no space restriction?
%\textbf{RQ3} (Section~\ref{sect:evalbeir}): 
%Zero-shot retrieval performance is important since a large dataset can contain documents from many domains. 
\textbf{RQ2} (Sect.~\ref{sect:evaldisk}): 
How does  CluSD perform on-disk search when there is not enough memory to host  the dataset?
\textbf{RQ3} (Sect.~\ref{sect:evalsparse}): 
Does CluSD work well with  different sparse retrievers?
\textbf{RQ4} (Sect.~\ref{sect:evalcompress}): 
Does CluSD work  well using different quantization methods?
\textbf{RQ5} (Sect.~\ref{sect:evalLSTM}): 
Is  LSTM 
%with cluster pruning 
preferred compared to other design options?
Are  features designed for LSTM useful?
%\textbf{RQ6} (Section~\ref{sect:clusterno}): 
\textbf{RQ6} (Sect.~\ref{sect:clusterno}): 
How does the number of clusters used affect the relevance and latency of CluSD? 
%\textbf{RQ7} (Sect.~\ref{sect:threshold}):
How does the choice of selection threshold in LSTM affect the average number of clusters selected?
%Does the cluster selection model dynamically select different number of clusters for different queries? How the selection differs for different datasets?



\comments{
To answer \textbf{RQ1},  we compare our proposed approach on the in domain test set, MSMARCO passage dev, DL 19, 20 with other commonly used techniques under storage (Table~\ref{tab:mainspace}) and latency constraints (Tabel~\ref{tab:maintime}).  
For \textbf{RQ2}, as our cluster selection technique requires training, we would like to understand how the approach would work on our domain dataset. In Table~\ref{tab:beir}, we use our cluster selection model trained on MS MARCO datasets on the 13 datasets from BEIR on a zero-shot manner and observe promising performance on all 13 out-domain datasets. 
For \textbf{RQ3} and \textbf{RQ4}, We compare the different cluster selection techniques, including heuristic approaches, a point-wise prediction model xgboost and a vanilla RNN prediction model against the proposed LSTM model (Table~\ref{tab:cluster_feat}).
To answer \textbf{RQ5}, we take two scenarios where the number of clusters is 4096, and 8192. Then we present the relevance in MRR@10, recall@1000, and the latency in terms of mean and 99 percentile time under three settings: when the flat index is used without compression, when we use OPQ to compress with m=128 or 64. Results are shown in Figure~\ref{fig:ncluster}.
For \textbf{RQ6}, we first plot the distribution of the number of clusters selected for each query under different model prediction thresholds. We also plot the average number of clusters for MSMARCO dev set and BEIR in Figure~\ref{fig:thresholds}.
For \textbf{RQ7}, we report the performance using three weaker sparse retrievers in Table~\ref{tab:sparse}. 
}

%\subsection{Settings }
{\bf Datasets and measures}.
Our evaluation uses the MS MARCO dataset with 8.8 million passages for full passage ranking~\cite{Campos2016MSMARCO,Craswell2020OverviewOT}.
The test query sets are the Dev set with 6980 queries and TREC deep learning (DL)  2019/2020 tracks with 43 and 54 queries.
Following the common practice, we report mean reciprocal rank at 10 (MRR@10) and recall at 1000 (recall@1K)
which is the percentage of relevant-labeled results appeared in the final top-1000 results.
For DL19 and DL20 sets, we report NDCG@10.
%We report average NDCG@10 for the 13 publically available BEIR datasets~\cite{thakur2021beir}
%to evaluate  zero-shot retrieval performance.  
We also report average NDCG@10 for 
the  BEIR  collection containing the 13 publicly available datasets~\cite{thakur2021beir} 
for evaluating zero-shot retrieval performance. 
%BEIR is a heterogeneous benchmark containing a variety of IR tasks, 
%including search tasks (e.g.  question-answering, bio-medical IR, and entity retrieval)  
%and semantic relatedness tasks (e.g.  duplicate question retrieval). 
The size of these data sets ranges from 3,633 to 5.4M.
%Their average query length ranges from 5.39 to 192.98, 
%and  their average document length ranges from 11.44 to 634.79. 
%Each dataset has binary or three-level relevance labels.
%The above metrics follow the common practice in the information retrieval literature.

To report the mean latency and 99 percentile latency, 
we  run test queries multiple times using a single thread on  a 2.25GHz AMD EPYC 7742  CPU server with PCIe SSD.
The reason to use a single thread is that each CPU server in a busy search site handles many queries in parallel, and thus we only take
one core resource with one thread from this server and leave other cores  for other queries.
%That is the standard practice in many of the previous efficiency studies in the IR literature.

{\bf Models and parameters}.
For sparse retrieval, we adopt two variations of 
SPLADE~\cite{Formal2021SPLADE, Formal_etal_SIGIR2022_splade++,Lassance2022SPLADE-efficient} 
based on hybrid thresholding~\cite{2023SIGIR-Qiao} and  BM25-guided traversal~\cite{mallia2022faster,qiao2023optimizing}:
% and one BM25 based model with different relevance and efficiency  tradeoffs:
1) SPLADE-HT1 with index space 3.9GB and 31.2 ms retrieval latency; 
%2) SPLADE-HT1-fast is a variation of SPLADE-HT1 with a different parameter setting, which has 3.9GB index space and 22.4 ms latency. 
2) SPLADE-effi-HT3 with  3GB space and  12.4ms latency. 
We also test on three other sparse models:
% uniCOIL~\cite{Lin2021unicoil,2021NAACL-Gao-COIL}, and LexMAE~\cite{shen2023lexmae}.
%2) DeepImpact~\cite{Mallia2021deepimpact};
3) uniCOIL~\cite{ Lin2021unicoil,2021NAACL-Gao-COIL} with 1.2GB index and 35.5ms latency;
4) LexMAE~\cite{shen2023lexmae} with 3.7GB index and 180ms latency;
5) BM25-T5 that applies  BM25 with  DocT5Query document expansion~\cite{Cheriton2019doct5query}.  
BM25-T5 has 1.2GB index and  9.2ms latency. 
%Their index space varies from 1.2GB to  3.7GB.
% with 1.2GB index space.
% with latency 9.2ms.
%5) BM25 after T5-based document expansion~\cite{Cheriton2019doct5query}. 
%They represent the state-of-the-art sparse retrievers.
% with the best relevance performance evaluated on MS MARCO.
For dense retrieval, we adopt the recent dense models
SimLM~\cite{Wang2022SimLM}, RetroMAE~\cite{Liu2022RetroMAE}, and
RepLLaMA~\cite{ma2023finetuning}. 
We use their checkpoints from the Huggingface library to generate document and query embeddings 
and  use  K-means in the FAISS library~\cite{johnson2019billion} to derive dense embedding clusters.
RetroMAE-2~\cite{liu-etal-2023-retromae} is not used because its checkpoint is not released.


Our evaluation implementation uses C++ and Python and the
related code will be released to the public after publication of this paper. 
\comments{
%Note that SimLM model's embeddings are normalized while RetroMAE's embeddings are not. 
For sparse retrieval, we use two fast versions of SPLADE and a SPLADE-efficient model, as well as BM25-T5. 
The implementation of SPLADE models follows 2GTI optimization~\cite{qiao2023optimizing}. %its official release~\cite{spladeRepo}. 
SPLADE-HT1 is the SPLADE model trained with hybrid thresholding scheme~\cite{2023SIGIR-Qiao} using $\lambda_{t}=1$, 
SPLADE-effi-HT3
is the SPLADE-efficient model~\cite{Lassance2022SPLADE-efficient} trained with hybrid thresholding scheme using $\lambda_{t}=3$. Both of these two models use the "accurate" configuration in 2GTI during retrieval, while SPLADE-HT1-fast uses the "fast" configuration.
The sparse retrieval code for Splade and BM25-T5 uses the code from PISA~\cite{mallia2019pisa}
with some optimization~\cite{Lassance2022SPLADE-efficient,2023SIGIR-Qiao}.
}
To train the CluSD model, we sample 5000 queries from the MS MARCO training set 
%and use the LSTM unit in Pyytorch. 
and the hidden dimension for LSTM is 32. The models are trained for 150 epochs. 
For sparse and dense model interpolation, we use min-max normalization to rescale the top results per query. 
%Then we use linear combination with equal weights to combine two ranked lists. 
For  BM25-T5, the interpolation  weights are  0.05 and 0.95 for sparse  and  dense scores, respectively. 
For other learned sparse retrieval models, they are  0.5 and  0.5, respectively. 
%In terms of missing document in either ranked list, as the smallest value from each normalized list is 0, there is no missing imputation needed as we 
%can view the missing  documents taking the value of the worst document in the ranked list automatically. 

%For CluSD, the default setting of number of clusters is $N=8192$, and the input sequence length to the Stage II LSTM model is $n=32$.  

{\bf Time budget.}
%For search latency, our goal is to minimize the relevance effectiveness loss to a small degree while still accomplishing  a fast response time
%acceptable to the interactive search system requirement.
We use  two time budget settings: around 50ms  and 25ms, including the  sparse retrieval time.
We explain the reason as follows.
In a search system running as an interactive  web service,  a query with multi-stage processing
needs to be completed within a few hundred milliseconds.
%Considering the multi-stage search nature  and other service overhead involved,
A first-stage retriever operation  for a data partition needs to be completed within several tens of milliseconds without query caching.
Our targeted time budget to conduct dense retrieval cannot be too high     compared to  sparse retrieval cost.
%For the example of Table~\ref{tab:costbudget},
%The studies from~\cite{Lassance2022SPLADE-efficientmallia2022GTI,Qiao20222GT,2023SIGIR-Qiao},
For example, if sparse retrieval can complete  in 30 ms on an  average CPU and the total latency
target is around 50ms,  the cost of dense retrieval is targeted under around  20ms.
% At most the total sparse and dense retrieval cannot be more than 100ms.
%Accuracy of above query-specific cluster skipping while retaining a competiitve relevance is the key to accomplish this latency goal.
%Notice that the latency target in the  LADR paper~\cite{2023SIGIR-LADR} is in a 4ms-8ms range
%and
%This latency budget choice is reasonable because for
%Also our evaluation is conducted in a low-end CPU server and a faster CPU can further accelerate.
%CPU latency reported in~\cite{2022WWWforwardIndex} is at 11

\comments{
{\bf Baselines.}
We compare CluSD with two groups of baselines under space and time constraints respectively.
The first group compared in Section~\ref{sect:eval0space} 
is to fuse  sparse retrieval with cluster-based selective dense retrieval.
That includes  dense retrieval with quantization option OPQ and  IVFOPQ with IVF clustering available in FAISS.
The second group compared in Section~\ref{sect:evaltimebudget} 
is to fuse  sparse retrieval with reranking and graph-based selective dense retrieval such as HNSW~\cite{2020TPAMI-HNSW} and  LADR~\cite{2023SIGIR-LADR}. 
This group involves random access of embeddings and/or graph nodes, which  can incur high I/O cost when data is not on disk.
}


{\bf Statistical significance.}
For MS MARCO Dev set, the result of a method is marked with  tag $^\dag$ when 
statistically significant drop is observed compared to  a baseline at 95\% confidence level.  In Table~\ref{tab:mainspace}, \ref{tab:maintime} and \ref{tab:sparse}, this baseline 
is sparse retrieval fused with full dense retrieval marked as ``S+D'', which typically delivers the highest relevance  
using all uncompressed or quantized dense embeddings. In Table~\ref{tab:disktime}, \ref{tab:RepLLaMA} and \ref{tab:compress}, the baseline is our proposed method ``S+CluSD''. 


\comments{
{\bf Baselines and notations}
%We select two groups of baselines under space and time constraints respectively.
Table~\ref{tab:mainspace} compares  baselines  with memory space constraint. 
We include dense retrieval with quantization option OPQ and  IVFOPQ with IVF clustering available in FAISS.
OPQ quantization  is configured with  the number of codebooks as $m=$ 128 or 64.  
When IVF clustering is used,  we report its performance  using top 10\%, 5\%, 2\% clusters respectively
as a standard approach which performs   limited top cluster retrieval. 
CluSD execution is also based on the the same OPQ or  IVFOPQ index from  FAISS but clusters are  selected  by our LSTM model. 
%Switching a quantization different  from OPQ  is might result in an improvement in relevance, but it is orthogonal to our proposal. 
We use notation ``S+D'' to report the interpolated performance of a sparse model and a dense model in Table~\ref{tab:mainspace} and Table~\ref{tab:sparse}.

Table~\ref{tab:maintime} compares  baselines  without  memory space constraint. 
For proximity graph-based dense retrieval which incurs additional graph space overhead,
we include  HNSW~\cite{2020TPAMI-HNSW} and  LADR~\cite{2023SIGIR-LADR} as shown in Table~\ref{tab:maintime}. 
%For HNSW, we fix the number of neighbors to be 128 and vary the expansion factor(ef) to meet the latency constraint. 
%For LADR, we use its default setting with seed = 200, number of neighbor = 128 and use the exploration depth as 50 to meet the latency requirements in 
%Table~\ref{tab:maintime}.
%Uncompressed dense embeddings (marked as "flat") are used
%to exclude the impact due to quantization.
We also compare  a simple reranking method,  denoted as ``D-rerank'' or ``rrk'', 
that fetches the dense scores of top 1000 of sparse retrieval to rerank with interpolation. 
%We use the same clustering setting for IVF and CluSD. 

%The reported CluSD performance on the flat index uses the exact same IVF index. 
The configuration we selected to meet the latency requirement for CluSD uses on average 20-25 (0.25 - 0.3\%) clusters per query. 
%For re-ranking, we report the results of re-ranking top 1000 results from the sparse model using the dense model.  

}



==> cikmexp_ablation.tex <==
%\vspace*{-5mm}
%\subsection{Fast search with minimized space overhead}
\begin{table*}[htbp]
	\centering
		\resizebox{1.98\columnwidth}{!}{
		\begin{tabular}{ r r l |l l ll l |llll l|r}
			\hline\hline
			 & & & \multicolumn{2}{c}{ 
{\bf MSMARCO Dev} }& {\bf DL19}& {\bf DL20} & {\bf BEIR} 
& \multicolumn{2}{c} { {\bf MSMARCO Dev} }& {\bf DL19}& {\bf DL20} & {\bf BEIR} 
& {\bf  Latency}    \\
			& &\% D& {MRR@10}& R@1K& {NDCG@10}&  {NDCG@10}& {NDCG@10}& {MRR@10}& {R@1K}& {NDCG@10}&{NDCG@10}& {NDCG@10}& ms \\
    \hline
 1. & S={\bf SPLADE-HT1} & --& 0.396& 0.980 & 0.732   & 0.721    & 0.500 & -- & --& --& --& --&31.2  \\
 & & & \multicolumn{5}{c|}{D=\textbf{SimLM}}& \multicolumn{5}{c|}{D=\textbf{RetroMAE}}&\\
   \hline
   &&& \multicolumn{10}{c}{\bf{Uncompressed flat setting. Embedding space  27.2GB}}\\
     \hline
          2. &   D  & 100 & 0.411$^\dag$ & 0.985$^\dag$& 0.714 &  0.697  & 0.429 & 0.416$^\dag$& 0.988& 0.720&0.703& 0.482 & 1674.1 \\
            3. &   $\blacktriangle$ S $+$ D   &100 & 0.424 & 0.989 & 0.740 & 0.726  & 0.518 & 0.425& 0.988& 0.740&0731& 0.520~&  1705.3 \\
           4. &    \bf S $+$ CluSD &0.3& 0.425 & 0.987 & 0.744 & 0.724  & 0.516 & 0.426& 0.987& 0.744&0.734 & 0.518 & 44.4 \\
              \hline
            &&& \multicolumn{10}{c}{\bf{OPQ $m=128$. Embedding space  1.1GB}}\\
              \hline
            5. &   $\blacktriangle$  S $+$ D-OPQ &100 & 0.420 & 0.988 & 0.735 &  0.719  & 0.508 & 0.416 & 0.988 & 0.737 & 0.732 & 0.515& 600.1 \\
            6. &  S $+$ D-IVFOPQ &10& 0.414$^\dag$& 0.987 & 0.726 & 0.734  & 0.505 & 0.404$^\dag$& 0.987& 0.713&0.722& 0.513 &  126.4 \\
           7. &   &5& 0.407$^\dag$& 0.987 & 0.717 & 0.733  & 0.499  & 0.394$^\dag$& 0.987& 0.687&0.817&0.507&  80.0 \\
           8. &   &2& 0.392$^\dag$& 0.986$^\dag$& 0.691 & 0.738  & 0.467 & 0.374$^\dag$& 0.986$^\dag$& 0.656&0.815& 0.499 & 52.5 \\
           9. &   \textbf{S $+$ CluSD}  &0.3& 0.423 & 0.987 & 0.739& 0.725 &0.514 & 0.417& 0.986& 0.742&0.735& 0.514  & 42.6  \\
             \hline
           & & & \multicolumn{10}{c}{\bf{OPQ $m=64$. Embedding space 0.6GB}}\\
            \hline
           10. & $\blacktriangle$  S $+$ D-OPQ  &100 & 0.409 & 0.986 & 0.718 &  0.721  &0.501 & 0.402 & 0.986 & 0.717 &  0.719 & 0.508 & 321.6 \\
           11. &   S $+$ D-IVFOPQ &10& 0.405 & 0.986 & 0.716 & 0.734 & 0.502 & 0.393$^\dag$& 0.986& 0.676&0.730& 0.505& 75.6 \\
           12. &   &5& 0.397$^\dag$& 0.986 & 0.704 & 0.733  & 0.497 & 0.384$^\dag$& 0.985& 0.659&0.717& 0.500& 55.0 \\ 
            13. &  &2& 0.383$^\dag$& 0.985 & 0.680 & 0.738 & 0.487 & 0.368$^\dag$& 0.985 & 0.643&0.707& 0.493 & 42.4 \\
            14. &  \textbf{S $+$ CluSD}  &0.3& 0.414 & 0.986 & 0.743& 0.726 & 0.511 & 0.403 & 0.987& 0.729&0.724 & 0.506 & 40.8 \\
              \hline\hline
		\end{tabular}
		}
	\caption{
CluSD vs. IVF cluster search with and without quantization.
%Sparse retrieval argumentation with minimum extra space overhead.
%no  with compressed or uncompressed dense emebddings S=SPLADE-HT1, D=SimLM or RetroMAE. 
%Model relevance and latency under compressed or uncompressed dense emebddings S=SPLADE-HT1, D=SimLM or RetroMAE. 
%Row  ``S $+$ D'' marked with $\blacktriangle$ indicates the oracle setting of sparse model interpolated with full dense retrieval. 
For MSMARCO Dev set, $^\dag$ is tagged when statistically significant drop is observed from the oracle $\blacktriangle$ at 95\% confidence level. 
}
\vspace*{-5mm}
	\label{tab:mainspace}
\end{table*}

\subsection{Search with in-memory data}
%\subsection{CluSD vs. IVF  cluster search}
\textbf{CluSD vs. IVF  cluster search}.
\label{sect:eval0space}
Table~\ref{tab:mainspace} compares CluSD with other cluster-based selective retrievals when fusing with sparse retrieval results
in searching the MS MARCO and BEIR datasets with and without compression.  
The result of a method is marked with  tag $^\dag$ when
statistically significant drop is observed compared to  a baseline at 95\% confidence level. 
SPLADE-HT1 is  the sparse model, and two dense models used are SimLM and RetroMAE.
%We compare our models on uncompressed embeddings, as well as two quantization configurations.
%There are the uncompressed setting and  two quantization  configurations. 
%The sparse model used is SPLADE-HT1 while the dense models are SimLM and RetroMAE.
%IVFOPQ is compared against CluSD as it selects only top clusters and does not incur extra space overhead. 
%The top portion of this table reports the performance when compression is not used, which captures a peak possible performance.
We also include dense retrieval with OPQ quantization  and  IVFOPQ from FAISS.
IVFOPQ uses a proportion of top dense clusters sorted by the query-centroid distance.
%IVFOPQ is compared, which use some percentage of top dense clusters sorted by query to centroid clusters.
%against CluSD as it selects only top clusters and does not incur extra space overhead.
OPQ quantization is configured with  the number of codebooks as $m=$ 128 or 64.
We report performance of IVF clustering using the top 10\%, 5\%, or 2\% clusters respectively
as a standard approach which performs   limited top cluster retrieval.
CluSD execution is also based on the the same OPQ or  IVFOPQ index from  FAISS, but clusters are  selected  by our two step algorithm.

Notation ``S+D'' in Table~\ref{tab:mainspace} (and later in other tables)
reports the fused performance of a sparse model and a full search of uncompressed dense model with linear interpolation.
Marker  ``\%D'' means the percentage of document embeddings  evaluated.
The last column,  ``Latency'' is the mean single-query time using SPLADE plus SimLM for MS MARCO Dev set.
We only report SimLM latency because the latency of RetroMAE is similar.
%When    prefix `+' is marked for a latency entry, it indicates  the extra milliseconds is spent for full or selective dense retrieval without counting   sparse retrieval time.
CluSD uses setting  $N=8192$ and 
$n=32$ 
% Tables~\ref{tab:mainspace} and~\ref{tab:maintime} use
which results in  selection of 22.3 clusters on average per query
and allows CluSD to meet  the latency requirement.
%The main space cost for CluSD is to maintain the inter-cluster similar graph, which 
%takes about 32MB with quantization for $N=8192$. 
%Switching a quantization different  from OPQ  is might result in an improvement in relevance, but it is orthogonal to our proposal.
%The reported CluSD performance on the flat index uses the exact same IVF index.
% for CluSD uses on average 20-25 (0.25 - 0.3\%) clusters per query.
%For re-ranking, we report the results of re-ranking top 1000 results from the sparse model using the dense model.
%The mean latency and 99 percentile latency of CluSD are 13.2 ms and 18.1 ms for searching uncompressed flat index, respectively;
%11.4 ms and 14.6ms for searching OPQ m=128 index;  9.6 ms and 11.1ms for searching OPQ m=128 index.





\comments{
For MS MARCO Dev set, the result of a method is marked with  tag $^\dag$ when
statistically significant drop is observed compared to  an oracle baseline
tagged with $\blacktriangle$ at 5\% confidence level.  This oracle
is sparse retrieval fused with full dense retrieval marked as ``S+D'', which typically delivers the highest relevance
using all uncompressed or quantized dense embeddings ($m=128$ or $m=64$).


%In realistic settings, a flat dense index is usually not affordable when corpus size is not small. Certain compression technique need to be used. 
The top portion of this table reports the performance of  SimLM dense model marked as ``D'' in Row 2.
In Row 1, ``S'' denotes sparse retrieval using  a variation of SPLADE with hard thresholding called HT1~\cite{2023SIGIR-Qiao}.
Sparse results merged with full  dense retrieval  results  are marked in Row 3, ``S $+$ D''.  
Our pipeline is reported in Row 4,``S $+$ CluSD''. 
The second and third portions of this table reports
the search performance   with  two compression configurations using OPQ implemented in FAISS:
1) ``m128'' that compresses dense embeddings from about 27GB into 1.1GB with 128 quantization codebooks.
2) ``m64'' that  yields 0.6GB compressed embeddings with 64 codebooks. 
%Setting where the storage for dense index is 1.1GB and 0.6GB. 
Under these two configurations, we report the Sparse model interpolated with dense retrieval under
IVFOPQ or OPQ using the default FAISS setting.


%In the first section of the table, we include the full dense retrieval SimLM (denoted as D in the table), 
%and full sparse retrieval SPLADE-HT1 (denoted as S in the table), 
%and 
%We then report dense retrieval with two compression configurations, using OPQ 
%with m=128 and m=64 respectively, resulting in an index 
%with 1.1GB and 0.6GB. These compressed configuration result in a 96\% and 97.8\% reduction in storage compared to flat index.
% and compare them against our pipeline.
}

Rows 6 and 11 of Table ~\ref{tab:mainspace} 
 show that selective IVF cluster search using  query-centroid distances 
can be under 130ms  when the percentage of clusters searched  drops from 100\% to 10\%. But the relevance drop is significant.  
Moreover, CluSD is as  fast as IVFOPQ  top 2\% search at m=64 (Row 14 vs. Row 13) and 2x fast at m=128 while
its relevance is much higher (Row 9 vs. Row 8).
%CluSD  performs  closely as the oracle at each compression setting, which
There is no statistically significant difference between CluSD and the oracle at each compression setting, which 
indicates CluSD effectively minimizes visitation of unnecessary  dense clusters. 

 



\comments{
 with full dense retrieval can reach a high relevance in all datasets and thus are marked as an oracle sign with or without compression.   
1. Almost no performance degradation when do S+CluSD.  Sometimes S+CluSD achieves slightly higher performance than S+D. It could be due to the fact that when we limit the search scope a lot of noisy documents are not considered by the dense model.

2. Under m=128 setting the performance degradation is acceptable especially on DL19 and 20. 

3. SimLM performs better under compression. This could be due to the fact that SimLM trained embedding is normalized while RetroMAE is not.

4. If we compare S+D-IVFOPQ with S+CluSD, given the same IVFPQ index, S+D-IVFOPQ represents the case where we use default order, even if we use 50x more clusters, the performance is not as good as CluSD. 
}


\begin{table}[htbp]
	\centering
 \resizebox{0.95\columnwidth}{!}{
		\begin{tabular}{r |llll|rr}
			\hline\hline
			& \multicolumn{2}{|c}{\bf{MSMARCO Dev}}& \bf{DL19}& 
\bf{DL20}& \bf{Latency}& \bf{Space}\\
			 & {MRR@10}& {R@1K}& \smaller{NDCG} &   \smaller{NDCG} & Total(ms)& GB\\
			\hline
        \multicolumn{7}{c}{\bf{Time Budget = 50 ms, S=SPLADE-HT1}}\\
        \hline
            D=SimLM & 0.411 & 0.985$^\dag$& 0.714 &  0.697 & 1674.1 & 27.2 \\
          S& 0.396$^\dag$& 0.980$^\dag$& 0.732   & 0.721    &   31.2 & 3.9 \\
           S $+$ D-rerank &  0.421 & 0.980$^\dag$& 0.745 & 0.728 & 34.6 & 31.1 \\
             $\blacktriangle$  S $+$ D  & 0.424 & 0.989 & 0.740 & 0.726 & 1705.0 & 31.1 \\
              \hline
              % D-IVF & 0.398$^\dag$& 0.935$^\dag$& 0.690 & 0.693 & 81.4 & $+$0.0\\
%            D-IVF & 0.389$^\dag$& 0.907$^\dag$& 0.671 & 0.676 & 49.5 & $+\sim$0\\
%            S $+$ D-IVF & 0.393$^\dag$& 0.987  & 0.678 & 0.715 & 56.5 & $+\sim$0\\
            %D-OPQ& 0.314$^\dag$& 0.957$^\dag$& 0.619 & 0.608 & 109.1 & 0.3 \\
           % D-IVFOPQ & 0.386$^\dag$& 0.929$^\dag$& 0.680 & 0.697 & 48.8 & 1.2\\
             HNSW & 0.409$^\dag$& 0.978$^\dag$& 0.669 & 0.695 & 54.4 & 40.3 \\
           S $+$ HNSW & 0.420 & 0.987 & 0.718 & 0.723 & 59.6 & 40.3 \\
            %S $+$ rerank-D &  0.412 & 0.980    &0.715  & 0.811 & 0.698 & 0.815 & $+$2.3 \\
            S $+$ LADR & 0.422 & 0.984$^\dag$& 0.743&0.728& 43.6& 35.4\\
%           7.1 &  S $+$ D-LADR & 0.423 & 0.987$^\dag$& 0.745 &0.728& 53.0 & $+$4.3\\
           % S $+$ D-IVF & 0.398$^\dag$& 0.987  & 0.674 & 0.720 & 64.7 & $+$0.0\\
           %S $+$ D-IVFOPQ & 0.392$^\dag$& 0.987 & 0.656 & 0.700 &  52.5 & 4.0\\
            \bf S $+$ CluSD & 0.426 & 0.987 & 0.744 & 0.724 &46.3& 31.1\\
       \hline       
            \multicolumn{7}{c}{\bf{Time Budget = 25 ms, S=SPLADE-effi-HT3}}\\
            \hline
            S& 0.380$^\dag$& 0.944$^\dag$& 0.721 &  0.726 & 12.4 & 3.0 \\
             S + D-rerank & 0.406 & 0.944$^\dag$& 0.728 & 0.738 & 15.1 & 30.2 \\
            $\blacktriangle$  S + D & 0.413 & 0.984 & 0.721 &0.729 & 1654.2& 30.2  \\
            \hline
            HNSW & 0.406 & 0.971$^\dag$& 0.672 & 0.694 & 28.4 & 39.4\\
             S $+$ HNSW & 0.407 & 0.984 & 0.706 & 0.724 & 28.7 & 39.4\\
            S $+$ LADR & 0.404$^\dag$& 0.984 & 0.728 &  0.736 & 24.2 & 34.5\\
%           16.1 & S $+$ D-LADR & 0.409 & 0.987 & 0.744 &  0.728  & 41.1 & $+$4.3\\
            \bf S $+$ CluSD & 0.412 & 0.984 & 0.733 & 0.728 & 25.4 & 30.2\\
			\hline\hline
		\end{tabular}  }
	\caption{CluSD vs. graph navigation and reranking 
% under time budget but  no memory constraints 
}
 \vspace*{-8mm}
	\label{tab:maintime}
\end{table}
%For pipelines with a time budget, we report the additional overhead in the Storage (GB) column. 


%\subsection{CluSD vs. graph navigation and re-ranking} 
\textbf{CluSD vs. graph navigation and reranking}. 
\label{sect:evaltimebudget}
Table~\ref{tab:maintime} compares  CluSD with  reranking and selective dense retrieval based on proximity graph navigation, which includes HNSW and LADR.
Since LADR has a variety of configurations, we use configurations under two time budgets.
We do not consider memory space restrictions in this evaluation as proximity graph takes a substantial amount of extra space.
We also compare  a simple reranking method,  denoted as ``D-rerank'' or ``rrk'',
that fetches the dense scores of the top-1000 sparse retrieval results to rerank with interpolation.
Uncompressed dense embeddings  are used to exclude the relevance impact by quantization.
The last two columns report the total latency time in milliseconds including sparse retrieval when needed,
and data space cost. %Extra memory space on the top of sparse retrieval is marked with prefix `+'. 
``NDCG'' means  NDCG@10.
%The extra space for quantized inter-cluster distances for CluSD takes about 32MB. 

%As discussed in Section~\ref{sect:design}, the overall latency budget is set as 50ms and 25ms respectively. 
We allow some time for budget relaxation since it is difficult to tune parameters of all baselines to meet the constraints exactly. 
%For IVF, we use 1.5$\%$ and 3$\%$ top clusters for ``S+IVF'' and ``IVF''.
%  but we allow some variation for some baselines because it is difficult to find parameters that exactly control the latency under this budget. 
%In this case, we choose the dense configuration such that the overall latency is within 70 or 30 milliseconds. 
For HNSW under 50ms time budget, we set its expansion factor parameter (ef) as 1024, 
2048 for S$+$HNSW and HNSW. 
Under 25ms time constraint, the expansion factor (ef) is  512 and  1024 respectively. 
%We include option ``S+Re-rank" which uses the top 1,000 sparse retrieval results and only compute dense scores of these top results, and merge the score with an interpolation.
%For HNSW, we fix the number of neighbors to be 128 and vary the expansion factor(ef) to meet the latency constraint.
For LADR, we use its default setting with seed = 200, number of neighbor = 128 and use the exploration depth as 50 to meet the latency budget.
%Table~\ref{tab:maintime}.
\comments{
Under time budget 50ms, 
model  SPLADE-HT1 is used and it has a latency of 31.2 ms in sparse retrieval.  
Under  time budget 25ms, model SPLADE-effi-HT3 is used and it is more aggressive in  efficiency 
with a 12.4ms latency at the cost of a relevance degradation. 

%using the dense model only, We also include sparse retriever 
%IVFOPQ, IVF, OPQ and HNSW using the dense model only, We also include sparse retriever 
%with reranking top 1000 results using the dense model. We also include the results of document evaluation using LADR algorithm. 
Note that when ``S$+$'' is in the row, it means we use the sparse model and the reported results are interpolated. 

}
%[DISCUSS TABLE 4 RESULTS.]
The takeaways from this table are:

\textbullet\ 
%While IVF does not add extra space cost, the relevance  of IVF top cluster search under the time budget performs  worse than others.
Simple reranking ``D-rerank'' achieves good MRR@10 but under-performs on recall.
When the recall of a sparse retriever is relatively low, it cannot boost further as seen in the case of using BM25T5 in Table~\ref{tab:sparse} with recall@1000 being 0.935.

\textbullet\ 
HNSW has a lower relevance number than LADR.
After fusion with sparse results, HNSW becomes  more comparably with LADR.
They  both incur the cost   of extra online memory overhead  and extra complexity to compute offline in advance.
HNSW requires extra 9.2GB and LADR requires extra 4.3GB to store graph data in memory. 
When we  try to reduce their graph size by decreasing  the number of neighbors for HNSW and LADR, their  MRR@10 and/or  recall@1000 numbers drop visibly. For example, 
using the default 32 neighbors for HNSW results in 2.4GB graph space, however  MRR@10 drops from 0.407 to 0.400 under the 25ms time budget. 

\textbullet\ 
CluSD has a higher MRR@10 while its DL19 and DL20 numbers are comparable to HNSW and LADR,
for both time budget=50ms and 25ms.  
Even when we relax the latency requirements for the HNSW or LADR, CluSD still maintains its advantages in different datasets. 
For instance, if we double the time budget to around  110ms
for 	``S+HNSW'' after  SPLADE-HT1 retrieval, its MRR@10 for MS MARCO Dev is 0.422, which is still below S$+$CluSD with 0.426 in 46.3ms.
CluSD incurs negligible extra space cost other than hosting embeddings, compared to HNSW and LADR.




 







==> cikmexp_beir.tex <==


\begin{table*}[h]
	\centering
		\resizebox{1.9\columnwidth}{!}{
		%\begin{small}
		\begin{tabular}{r r r lr  |lllll|lllll}
			\hline\hline
                 &  & &  & &  \multicolumn{5}{c|}{SPLADE-HT1+SimLM} & \multicolumn{5}{c}{SPLADE-HT1+RetroMAE}\\
                  &  & &  & {SPLADE}  &  & &  \textbf{CluSD} & \textbf{CluSD} & \textbf{CluSD} & & & \textbf{CluSD} & \textbf{CluSD} & \textbf{CluSD}\\
		    Dataset & \smaller{BM25} &{SimLM}  &  {RetroMAE} &{-HT1} & \smaller{$\blacktriangle$ 
 flat} &rrk&\textbf{flat}& \textbf{m=128}& \textbf{m=64}& \smaller{$\blacktriangle$ flat} &rrk &\textbf{flat}& \textbf{m=128}& \textbf{m=64}\\
              \hline
              \multicolumn{15}{c}{\bf{Search Tasks}}\\
               \hline
                {DBPedia}	& 0.313	& 0.351 &  0.390&0.447	& 0.426 &0.442& 0.429 & 0.425 & 0.422 & 0.446 & 0.411 & 0.446 & 0.445&0.436 \\
                                {FiQA} &	0.236	& 0.298 &  0.316&0.355 & 0.355 &0.355 &0.365 & 0.361 &0.359 & 0.365 & 0.333 & 0.366 & 0.359& 0.353\\
                {NQ}	& 0.329   & 0.502  &	 0.518&0.550 & 0.568 &0.549&0.568 & 0.566 & 0.560 & 0.563 & 0.520 & 0.564 & 0.553& 0.538\\
                {HotpotQA} & 0.603 & 0.568 &  0.635& {0.681} & 0.672 &0.668&  0.672 & 0.669 & 0.661 & 0.702 & 0.642 & 0.702 & 0.693&0.672 \\
                {NFCorpus}  & 0.325 & 0.318  &  0.308&0.351 & 0.353 &0.347&  0.360 & 0.358 & 0.359 & 0.345 &0.331 & 0.351 & 0.349& 0.346 \\
                {T-COVID}	& 0.656 & 0.515  &  0.772&0.705 & 0.726 &0.692&  0.745 & 0.741 & 0.725 & 0.780 & 0.699 &0.747 &0.740& 0.726\\
                {Touche}	& {0.367}  & 0.292  &  0.237&0.291 & 0.336 &0.292 &0.333 & 0.336 & 0.332 & 0.292 &0.316 & 0.295 &0.288& 0.283\\
                \hline
                \multicolumn{15}{c}{\bf{Semantic Relatedness Tasks}}\\
                 \hline
                {ArguAna} & 0.315 & 0.376  &  0.433&0.446 & 0.481 &0.427&  0.492 & 0.489 & 0.486 & 0.459 & 0.434 & 0.455 &0.455 & 0.451\\
                {C-Fever}	& 0.213 & 0.171  &  0.232&0.234 & {0.239} &0.236&  0.241 & 0.250 & 0.242 & 0.260 &0.198 &0.260 &0.267& 0.262\\
                {Fever} & 0.753  &0.689  &	 0.774& {0.781} & 0.793 &0.784&  0.794 & 0.783 & 0.789 & 0.820 &0.774 &0.820 &0.814& 0.800\\
                {Quora} & 0.789 & 0.797  &	 0.847&0.817 &	0.847 &0.816&  0.847 & 0.849 &0.848 & 0.856 &0.814 &0.855 &0.854& 0.849\\
                {Scidocs}	& 0.158 &0.137  &	 0.15&0.155 &	{0.165} &0.152&  0.166 & 0.166 & 0.165 & 0.167 &0.142 &0.169&0.166& 0.164\\
                {SciFact}	& 0.665 & 0.559  &  0.653& {0.682} & 0.674 &0.682&  0.694 & 0.689 & 0.693 & 0.706  &0.661 &0.703 &0.699& 0.694\\
                            \hline
                \textbf{Avg.} & 0.440 & 0.429  &  0.482&0.500 & 0.518 &0.496&  0.516 & 0.514 & 0.511 & 0.520 &0.483 &0.518 &0.514& 0.506\\
                %\textbf{BM25 Diff} & -- & -2.6\%  &	13.6\% &17.7\% &  6.1\%&12.7\%&14.8\% &  \textbf{15.7\%} \\
                \textbf{{Splade Diff}} & -12.0 \% &  -14.2\%  &	 -3.6\% &-- & 3.6\% & -0.8\% &3.2\% & 2.8\% & 2.2\% &4.0\%& -3.5\%& 3.5\%&2.8\%&1.2\%\\
            \hline\hline
		\end{tabular}
		%\end{small}
		}
%\vspace*{-5mm}
	\caption{Zero-shot performance in average NDCG@10 on BEIR datasets. 
%Row ``SPLADE Diff.'' is the mean relative performance compared to the SPLADE-HT1 performance.
}
 \vspace*{-5mm}
%For quantization approaches, we adopt M=16, K=256, i.e. compression rate 32$\times$ compared to ColBERT.
	\label{tab:beir}

\end{table*}



\comments{
\begin{table}[h]
	\centering
		\resizebox{1\columnwidth}{!}{
		%\begin{small}
		\begin{tabular}{r r r r  |lllll}
              \hline
              \hline
	\multicolumn{4}{c|}{\bf Average NDCG@10}
                     &  \multicolumn{5}{c}{SPLADE-HT1+SimLM}\\
                  &  & & {SPLADE}  & Full  & &  \textbf{CluSD} & \textbf{CluSD} & \textbf{CluSD} \\
		    Dataset & \smaller{BM25} &{SimLM}  &{-HT1} & \smaller{$\blacktriangle$ 
 flat} &rrk&\textbf{flat}& \textbf{m=128}& \textbf{m=64}\\
              \hline
              \multicolumn{9}{c}{\bf{Search Tasks}}\\
               \hline
                {DBPedia}	& 0.313	& 0.351 &0.447	& 0.426 &0.442& 0.429 & 0.425 & 0.422 \\
                                {FiQA} &	0.236	& 0.298 &0.355 & 0.355 &0.355 &0.365 & 0.361 &0.359 \\
                {NQ}	& 0.329   & 0.502  &0.550 & 0.568 &0.549&0.568 & 0.566 & 0.560 \\
                {HotpotQA} & 0.603 & 0.568 & {0.681} & 0.672 &0.668&  0.672 & 0.669 & 0.661 \\
                {NFCorpus}  & 0.325 & 0.318  &0.351 & 0.353 &0.347&  0.360 & 0.358 & 0.359 \\
                {T-COVID}	& 0.656 & 0.515  &0.705 & 0.726 &0.692&  0.745 & 0.741 & 0.725 \\
                {Touche}	& {0.367}  & 0.292  &0.291 & 0.336 &0.292 &0.333 & 0.336 & 0.332 \\
                \hline
                \multicolumn{9}{c}{\bf{Semantic Relatedness Tasks}}\\
                 \hline
                {ArguAna} & 0.315 & 0.376  &0.446 & 0.481 &0.427&  0.492 & 0.489 & 0.486 \\
                {C-Fever}	& 0.213 & 0.171  &0.234 & {0.239} &0.236&  0.241 & 0.250 & 0.242 \\
                {Fever} & 0.753  &0.689  & {0.781} & 0.793 &0.784&  0.794 & 0.783 & 0.789 \\
                {Quora} & 0.789 & 0.797  &0.817 &	0.847 &0.816&  0.847 & 0.849 &0.848 \\
                {Scidocs}	& 0.158 &0.137  &0.155 &	{0.165} &0.152&  0.166 & 0.166 & 0.165 \\
                {SciFact}	& 0.665 & 0.559  & {0.682} & 0.674 &0.682&  0.694 & 0.689 & 0.693 \\
                            \hline
                \textbf{Avg.} & 0.440 & 0.429  &0.500 & 0.518 &0.496&  0.516 & 0.514 & 0.511 \\
                %\textbf{BM25 Diff} & -- & -2.6\%  &	13.6\% &17.7\% &  6.1\%&12.7\%&14.8\% &  \textbf{15.7\%} \\
                \textbf{{Splade Diff}} & -12.0 \% &  -14.2\%  &-- & 3.6\% & -0.8\% &3.2\% & 2.8\% & 2.2\% \\
            \hline\hline
		\end{tabular}
		%\end{small}
		}
%\vspace*{-5mm}
	\caption{Zero-shot retrieval performance 
%in average NDCG@10 
on 13 BEIR datasets 
%Row ``SPLADE Diff.'' is the mean relative performance compared to the SPLADE-HT1 performance.
}
  \vspace*{-5mm}
%For quantization approaches, we adopt M=16, K=256, i.e. compression rate 32$\times$ compared to ColBERT.
	\label{tab:beir}

\end{table}

}


%\subsection{Zero-shot retrieval performance with BEIR}
\textbf{ Detailed zero-shot performance with BEIR}.
\label{sect:evalbeir}
Table~\ref{tab:beir} lists  the performance of  CluSD  
with  SimLM and  RetroMAE after SPLADE-HT1 retrieval in searching each of 13 BEIR datasets.
% that contain out-of-domain documents.
The LSTM model of CluSD  is trained with the  MS MARCO training set,
and it is directly applied to each BEIR  dataset to select clusters without further tuning. 
%Zero-shot out-of-domain performance is important since a large dataset can contain document content from many domains.
% to unseen models and datasets, we evaluate the pipeline on out-domain data. For this experiment, we use the BEIR benchmarks which consists 13 released document 
%sets on various semantic relatedness tasks. 
%We directly apply the CluSD model trained on MSMARCO training set to predict the clusters on the BEIR queries and BEIR specific clusters. 
As a baseline, column ``$\blacktriangle$ flat'' is to fuse  the uncompressed full dense retrieval  with SPLADE-HT1 sparse  retrieval.
Column marked ``rrk'' is to rerank   top 1,000  sparse retrieval results interpolated with their dense scores. 
%The final score are the interpolation of the sparse ranked list and dense re-ranked list. 
Columns with ``CluSD-flat'', ``CluSD-m=128'' and ``CluSD-m=64''  are  CluSD results  using uncompressed or compressed embeddings with
m=128 or m=64. 

%\begin{itemize} [leftmargin=*]
%\item 
%Even SimLM underperforms SPLADE retriever for BEIR,  
Table~\ref{tab:beir} shows
that the relevance of CluSD with selective fusion of sparse and dense results is higher than each individual retriever,
and CluSD with limited dense retrieval   performs  closely to   oracle ``$\blacktriangle$ flat'',
and delivers good NDCG@10under two compression settings.
%While embedding compression affects relevance,  CluSD still performs fairly well for the BEID datasets.  
%This indicates good zero-shot performance of our proposed LSTM based strategy.
%\end{itemize}
  


==> cikmexp_compress.tex <==
\subsection{CluSD with other quantization models}
\label{sect:evalcompress}

% parker's rewrite
%CluSD is efficient and effective when combined with a variety of quantization methods.
Tables~\ref{tab:mainspace}, \ref{tab:beir},
and \ref{tab:RepLLaMA}  use the OPQ quantization method~\cite{Ge_2013_CVPR}  implemented in FAISS.
%We  the performance of CluSD with three quantization methods on the MS MARCO Passage Dev set, 
%OPQ~\cite{Ge_2013_CVPR}, JPQ~\cite{2021CIKM-JPQ-Zhan}, and DistillVQ~\cite{Xiao2022Distill-VQ}.
Table~\ref{tab:compress} shows the use of two other recent quantization methods 
called DistillVQ~\cite{Xiao2022Distill-VQ} and JPQ~\cite{2021CIKM-JPQ-Zhan} 
with in-memory CluSD for MS MARCO Passage Dev set. Latency column includes sparse retrieval time for last two rows where fusion is conducted. 
%We use the OPQ implementation from FAISS with results in Table \ref{tab:sparse}.
For JPQ, we use its released model and compression checkpoints and follow its default setting with $m=96$. 
For DistillVQ, we use its released code to train compression on the RetroMAE model using its default  value $m=128$.
This DistillVQ setting  yields 1.38GB storage space for RetroMAE embeddings while JPQ yields  0.95GB for its dense model. 
%The sparse SPLADE-HT1 model used  has a 3.9GB index.  [alreadly mentioned before]
We set IVF to selectively search 2\% of clusters. 

%This is consistent with our findings with OPQ; thus we conclude that CluSD is effective under many different quantization methods.
% below: old
%The above  evaluation uses the OPQ quantization method~\cite{Ge_2013_CVPR}  implemented in FAISS.



%DistillVQ~\cite{Xiao2022Distill-VQ} and JPQ~\cite{2021CIKM-JPQ-Zhan} using  their released code. 
%and  the recent  quantization
%methods~\cite{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ}
%also have  a significant relevance drop pattern when the compression ratio increases.
%A limitation of the current  CluSD work is that the training of the LSTM model has a dependence on the sparse retrieval model used.
%While  CluSD can  boost the relevance of a weaker sparse retriever model such as BM25, the augmented relevance still has not reached a level
%comparable  to the one where CluSD is coupled with a stronger sparse retriever. There is room for improvement in future work.
%%We will revise the paper to discuss and compare [52, 57, 59] in more details and will include extra evaluation results. 

%This evaluation uses  the  code and checkpoints released from DistillVQ and JPQ authors,
%and follows their default setting  with $m=128$ for DistillVQ and $m=96$ for  JPQ.
%DistillVQ for RetroMAE has  1.38GB embeddings while  JPQ dense model has  0.95GB embeddings. 
%The sparse SPLADE model has 3.9GB index.  IVF setting selectively searches   2\% clusters. 

%Table ~\ref{tab:compress} shows that 
%under the same quantization (DistillVQ or JPQ), CluSD outperforms FAISS IVF in relevance and latency significantly 
%before and after fusion.
%This is   consistent with our findings with OPQ and thus CluSD can work effectively with different  quantization methods. 
%The comparison in ~\cite{Xiao2022Distill-VQ}
%shows the quantization with another quantization method called RepCONC~\cite{2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ}
%has   relevance similar to JPQ  and DistillVQ outperforms them.  Thus we did not directly evaluate RepCONC. 

\comments{
\begin{verbatim}
DistillVQ	MRR@10	Recall@1K	Latency (ms)
IVF	0.365	0.899	20.8
CluSD	0.393	0.977	9.7
SPLADE+ IVF	0.392	0.987	52.0
SPLADE+CluSD	0.417	0.987	40.9

JPQ	MRR@10	Recall@1K	Latency (ms)
IVF	0.326	0.917	21.3
CluSD	0.341	0.969	11.2
SPLADE+IVF	0.379	0.985	52.5
SPLADE+CluSD	0.392	0.985	42.4
\end{verbatim}
}
\begin{table}[htbp]
        \centering
                \resizebox{\columnwidth}{!} {%
                \begin{tabular}{ r |l l l |ll l}
                        \hline\hline
                Quantization & \multicolumn{3}{c|}{\bf{DistillVQ}} & \multicolumn{3}{c}{\bf{JPQ}}   \\
%\cline{1-6}
                        \hline
S=SPLADE-HT1                        & {MRR@10} & {R@1K}  & {Latency } & {MRR@10} & {R@1K}    & {Latency}\\
                        \hline
                        IVF (2\%)  & 0.365$^\dag$ &	0.899$^\dag$ &	20.8 ms
& 0.326$^\dag$	&0.917$^\dag$ &	21.3 ms\\
%CluSD &0.393&	0.977&	9.7ms &0.341&	0.969&	11.2ms\\
S+ IVF (2\%)	&0.392$^\dag$ &	0.987&	52.0 ms
& 0.379$^\dag$ & 	0.985& 	52.5 ms\\
S+CluSD&	 0.417 &	0.987 &	40.9 ms
 &0.392 &	0.985 &	42.4 ms\\
\hline           
\hline           
                \end{tabular}
                }
        \caption{ Use of CluSD with   DistillVQ and JPQ quantization}
\vspace*{-5mm}  
        \label{tab:compress}
\end{table}     

Table ~\ref{tab:compress} shows that 
%use of approximated embedding with the recent quantization methods still reduces relevance visibly 
%compared to uncompressed embeddings shown in Table~\ref{tab:mainspace}, and CluSD can boost relevance substantially.
under the same quantization (DistillVQ or JPQ), CluSD significantly outperforms FAISS IVF in relevance and latency 
before and after fusion.  This is consistent with our findings with OPQ.
Although DistillVQ outperforms OPQ for standalone dense retrieval,
% (0.365 vs. 0.347 MRR@10),
relevance of S+CluSD with OPQ for RetroMAE shown in  Table~\ref{tab:mainspace} is about the same  as S+CluSD with DistillVQ
(same 0.417 MRR@10;  0.986 vs. 0.987 R@1K).  
While switching to a different quantization affects compression and  relevance, 
the result shows that CluSD can work effectively and  outperform other baselines under the same quantization. 
We do not directly evaluate with RepCONC~\cite{2022WSDM-Zhan-RepCONC}
because ~\cite{Xiao2022Distill-VQ} shows that it has similar relevance to JPQ
and is outperformed by DistillVQ.



==> cikmexp_feature.tex <==
\subsection{Design options for CluSD}
%\subsection{Design options and parameters for CluSD}
\label{sect:evalLSTM}

% In this section, we discuss \textbf{RQ3} and \textbf{RQ4}.
Table~\ref{tab:cluster_feat} investigates the impact of the following design options 
for cluster selection in CluSD with  the MS MARCO Dev set. 
For Stage I selection, we explore two options:
\begin{enumerate}
[leftmargin=*]
    \item SortByDist: Choose top clusters sorted by the distance of their  centroids to  the  query embedding.
% as implemented in the faiss IVF index.
    \item SortByOverlap:  Choose top  clusters sorted  by $P(C_i, B_j)$ features discussed in Section~\ref{sec:clusd}.
Namely use the overlap degree of clusters with top result bins of sparse retrieval. 
\end{enumerate}

For Stage II selection, we explore three options:
% select  the centroids based on the number of top10/25/100 sparse retrieval results in the clusters. This is the purning technique we propose in the method section.
 \begin{enumerate}[leftmargin=*]
    \item XGBoost: Use the boosting tree XGBoost model to detect if a cluster should be visited.
The features used are the same ones discussed in Section~\ref{sec:clusd}. This is a pointwise approach as we view query-cluster pairs as independent samples and the decision on one cluster doesn't affect other clusters for the same query.
% excluding inter-cluster distances.
%for each query-centroid pair to predict whether the centroid should be evaluted. This is a pointwise approach.
    \item RNN: Use a vanilla RNN model to predict. The feature and sequence setup is the same as our LSTM model. 
    \item LSTM: the model we used in CluSD.
\end{enumerate}
    We assess  the impact  of removing a  feature group used in CluSD:
%  used CluSD:
\begin{enumerate}[leftmargin=*]
\item w/o inter-cluster dist: removing  the inter-cluster distance feature group;
\item w/o S-C overlap: removing  the overlap-degree feature of top sparse results with each cluster.
\end{enumerate}


The last row marked ``Default'' is the final version used by CluSD with SortByOverlap and LSTM.
To have a fair comparison, this table assumes on average either 3 or 5 clusters are targeted by CluSD.
%We compare the performance of different strategies to select dense clusters.  
For XGBoost, RNN or LSTM, we set their prediction threshold so that 
the average number of clusters is close to the targeted number.
The last column of this table is the time spent to select clusters. 
%chosen depends  on the model prediction thresholds. 
%where top 3 or 5 clusters are selected. 
%In order to compare under same budget, we set the thresholds where on average around 3 or 5 clusters are used averaged over all queries. 
Table~\ref{tab:cluster_feat} shows that  the RNN or LSTM based prediction achieves  higher MRR@10 and recall compared to 
XGBoost. 
%point-wise tree based model. 
%It is reasonable as the tree model doesn't take  into account of incremental the inter-cluster relationships.
%Row  marked ``LSTM+prune'' of Table~\ref{tab:cluster_feat}, we 
%SortbyOverlap in Stage I in CluSD can significantly  decrease  the decision time by reducing the length of input cluster sequence, and can  actually lead a visible relevance increase.
Feature exploration indicates that the overlap degree is important for  cluster selection
while the inter-cluster distance feature group is also useful. 


 

\comments{
%\textbf{Effect of Model Options}
For k-means and topk heuristics, we report the performance where top 3 or 5 clusters are selected. For XGBoost, RNN or LSTM, the number of clusters chosen is dependent on the model prediction thresholds. In order to compare under the same budget, we set the thresholds where on average around 3 or 5 clusters are used averaged over all queries. 
As we can see in Table~\ref{tab:cluster_feat}, RNN or LSTM based prediction achieves much higher MRR and Recall compared to point-wise tree based model. It is reasonable as the tree based model doesn't take into account the relationships between centroids when making predictions. 
}


%\textbf{Impact of feature groups}.  

%  vs. Dense'' has a visible drop in relevance, indicating that the features we use are useful. Especially the sparse vs. dense feature, model performance has a significant drop without the feature group.

\begin{table}
\resizebox{1.0\columnwidth}{!}{
  \begin{tabular}{ r |r r| r r| r }
			\hline\hline
			 Avg \#clusters targeted  & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{5} & Time \\
			& MRR@10 & R@1K& MRR@10 & R@1K & ms\\
                   \hline
                 %RNN+prune & 0.401 & 0.919 & 0.411 & 0.961 & 2.8 \\
                 \multicolumn{6}{l}{\it{Stage II is removed. Stages I only options}}\\
                 SortByDist & 0.297 & 0.655 & 0.331 & 0.740  & 0 \\
                $\blacktriangle$ SortByOverlap & 0.384 & 0.867 & 0.401 & 0.917 & 0.2 \\
                   \hline
                \multicolumn{6}{l}{\it{Stage I=SortByDist;  Stage II model options}}\\
                 XGBoost& 0.398 & 0.888 & 0.404 & 0.929 & 192 \\
                 RNN & 0.404 & 0.908 & 0.406 & 0.938 & 2.8 \\
                 LSTM & 0.406 & 0.923 & 0.406 &0.943 & 2.8\\
                   \hline
             \multicolumn{5}{l}{\it{ Stage II=SortByOverlap;  Stage II LSTM feature group options}}\\
             w/o inter-cluster  dist& 0.402 & 0.915 & 0.406 & 0.941 & --\\
             %w/o Centroid Distance& 0.389 & 0.898 & 0.410 & 0.959 & --\\
             %w/o Sparse vs. Dense& 0.378 & 0.866 & 0.404 & 0.943 & --\\
             w/o  S-C overlap& 0.289 & 0.638 & 0.325 & 0.730 & --\\
             \hline 
             $\blacktriangle$  Default   &  0.408 & 0.943 & 0.410 & 0.953 & 2.8 \\
             %$-$ Query vs. Centroid & 0.405 & 0.925 & 0.406 & 0.941 & --\\
              \hline\hline
		\end{tabular}
}
	\caption{Design options for  CluSD. $\blacktriangle$ is the default choice.}
	 \vspace*{-5mm}
        \label{tab:cluster_feat}
\end{table}

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.42]{ncluster2.pdf}
    \caption{CluSD performance and latency with respect to a different average  number of selected clusters}
 \vspace*{-5mm}
    \label{fig:ncluster}
\end{figure}


\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.48]{threshold.pdf}
    \caption{Left: Distribution  of \#visited clusters under different selection threshold $\Theta$.
Right: Mean \#visited clusters on MS MARCO Dev set and BEIR datasets.}
     \vspace*{-5mm}
    \label{fig:thresholds}
\end{figure}

\subsection{Impact of \#cluster and selection threshold} 
%\subsection{Impact of  selection threshold $\Theta$}
\label{sect:clusterno}

\textbf{Impact of  cluster partitioning size}.
%The cluster selection technique is built on top of a group of defined clusters. It is important to understand how the cluster selection works and a good rule of thumb to 
%determine the model prediction threshold given different number of clusters. 
CluSD assumes the embeddings are pre-partitioned into $N$ clusters.  Figure~\ref{fig:ncluster} shows the impact of CluSD when
$N$ is  4096 and  8192 for MS MARCO Dev set.
% we plot three scenarios where the total number of clusters is 1024, 4096 and 8192 respectively. 
For stage I, we use $n=128$ in this figure to depict the impact of selecting different numbers of clusters on average in a wider range.
A  solid line refers to the use of uncompressed dense embeddings while  a dash-dot line refers to the quantization with OPQ m=128, 
and a dotted line refers to the quantization  with OPQ m=64. X-axis is the average number of clusters selected by CluSD.
We vary the selection threshold parameter $\Theta$ in CluSD to achieve the different average number of clusters selected. 

Figure~\ref{fig:ncluster} shows that with both $N$,
%MRR@10 reaches above 0.420 when above    $<$ 10 clusters 
MRR@10 reaches above 0.420 when above 10 clusters 
are selected.
As more clusters are selected,  the recall ratio does  increase. 
%Note that when total number of clusters increases, the percentage of documents search will be different given a fixed number of clusters are selected. 
%Given a fixed number of selected clusters,  the latency impact is different with different $n$ values.
%This result in difference in average latency. 
For  a fixed average number of selected clusters, 
different $N$ values imply different latency numbers.
For example, when 10 clusters are selected on average, 
CluSD  scans through 0.1\% and  0.2\% of embeddings corresponding to N=4096 and 8192, respectively. 
%As we can see in the bottom two sub-figures, 
When $N= 8192$, its latency 
%in milliseconds 
is smaller  with a  smaller size per cluster
as CluSD time complexity is proportional  to  the size per cluster and the number of clusters selected.
%With $N$ becomes much bigger,  the overhead of clusters in stage II optimization starts to offset or outweigh latency benefits of small clusters. 
% while the overall CluSD time is still  
\comments{
In this case, given a 20 
%(35 ms for 99\%) 
millisecond mean latency constraint, 
CluSD  with flat index can achieve 0.425 and 0.988 in MRR@10 and recall@10 by visiting  about 50 clusters (0.6\% of documents), 
which is the same performance compared to the full index search. 
This observation is logical, as for each cluster, there are possibly only tens or a few hundred relatively important documents to be evaluated for 
a given query. Majority of the documents in the clusters are not worth exploring. As the size of each clusters decreases, we are able to see more top important documents. 
}

Lastly, as CluSD makes a query-specific decision to dynamically select  clusters, each query has  a  different number of clusters visited
given a fixed threshold value and query latency can vary. 
The bottom right subfigure shows that the 99\textsuperscript{th}
percentile latency is around 2x longer than the mean latency, which is reasonable by
looking at the previous retrieval latency studies (e.g. ~\cite{mallia2019pisa, 2022ACMTransAnytime}).
%mackenzie2021anytime




%\subsection{Impact of  selection threshold $\Theta$}
\label{sect:threshold}
\comments{
\textbf{RQ6}: does the cluster selection model dynamically select different numbers of clusters for different queries? How the selection differs for different datasets?
For the first question, we plot out the distribution of number of clusters selected for each query as a boxplot in 
}
\textbf{Impact of  selection threshold $\Theta$}.
%\label{sect:threshold}
The left portion of Figure~\ref{fig:thresholds} shows
the average number of SimLM dense clusters selected by CluSD for MS MARCO Dev set under different threshold $\Theta$ values  when
the input sequence length $n$ for Stage II LSTM is 32.
%Model prediction threshold refers to the threshold which we use to determine the selection of a cluster. 
A threshold can be chosen for CluSD to follow a  time budget. 
%As we can see, there is a variety in the number of clusters selected. 
%While the median number of clusters selected is  10 clusters, the 75th percentile is around 18 clusters. 
In our experiments,  the default setting of
CluSD is to use threshold 0.02  for MS MARCO passages and the average number of clusters selected by CluSD using this threshold is 22.3.

The right portion of Figure~\ref{fig:thresholds} 
shows  the mean number of clusters selected for MS MARCO Dev set and averaged over 
the zero-shot BEIR datasets.
This subfigure shows that for a fixed $\Theta$ value, CluSD  adaptively chooses a fewer number of clusters for a
BEIR dataset compared to the MS MARCO Dev set.  
%This aligns with our expectation that  
This is intuitive as
SimLM underperforms SPLADE on the BEIR datasets in general. Thus, it is unnecessary to evaluate a lot of clusters. 
%CluSD adaptively selects fewer clusters for BEIR% to conduct selective dense retrieval. 



==> cikmexp_io.tex <==
\subsection{ Search with on-disk data}
\label{sect:evaldisk}
%{\bf CDFS vs. re-ranking and nearest-neighbor search baselines with in-memory or on-disk data.}

Table~\ref{tab:disktime} examines the performance  of CluSD fused with SPLADE when MS MARCO passage 
embeddings cannot fit in memory and are stored on an SSD disk.
We use  $N=65,000$ for CluSD to reduce the cluster size, and the extra space for quantized inter-cluster distances takes about 40MB. 
We also compare other selective dense retrieval baselines using  reranking or proximity graph navigation.
%The mean response time (MRT) and 99 percentile time (P99) include the I/O cost while their cost breakdown for I/O and CPU time is also listed. 
The mean response time (MRT) and 99\textsuperscript{th} percentile time (P99) include
the total sparse and dense retrieval time for methods noted ``S+*'', otherwise only the dense retrieval time.
The MRT cost breakdown for I/O and CPU time is also listed. 
All times reported are in milliseconds. 
Column ``\#Doc'' is the number of embeddings fetched for performing full or partial dense retrieval.
MRR stands for MRR@10.
R@1K stands for Recall@1K.
%A small table on the top specifies the data location of configured retrieval algorithms.

The reranking method simply fetches top-$k$ embeddings  from the disk for fusion. 
LADR is designed for in-memory search~\cite{2023SIGIR-LADR} and we run it by  assuming  memory can sufficiently host the proximity  graph while letting LADR access  embeddings from the disk. 
Excluding the I/O cost portion of LADR in this table, the in-memory search cost of LADR is marked in the ``CPU'' column.
We test two configurations of LADR, its default with 128 neighbors, 200 seed documents, and a search depth of 50,
as well as a faster configuration, selected such that its CPU time is similar to CluSD. 
LADR\textsubscript{fast} uses 128 neighbors, 50 seed documents, and a depth of 50.
DiskANN~\cite{NEURIPS2019_DiskANN} assumes the graph and original embeddings are on disk  while the memory  hosts
compressed embeddings for quick guidance.  SPANN~\cite{chen2021spann} searches disk data in a cluster-based manner based on query-centroid distances.
Both DiskANN and SPANN  are designed for on-disk search from scratch without fusing with others, and thus we simply fuse their outcome with SPLADE results.
HNSW~\cite{2020TPAMI-HNSW} is not included because its in-memory relevance  is similar as DiskANN while it is not designed to be on disk. 

\comments{
As the size of dense embeddings or the number of documents in a dataset increases, it is likely that dense embeddings are too large to be fully stored in memory. For instance, RepLLaMA requires 135.6GB for the 8.8M documents in MS MARCO; BERT-based dense embeddings for a 1B document dataset would require 2.8 TB. This problem is exacerbated when a large navigation graph is also required to be loaded in memory. We compare CluSD with several baselines when the embeddings are stored on disk and must be loaded to memory before ranking. We memory-map the dense embeddings and load them on-demand during our algorithm. We measure both the disk access time (I/O) and the associated computation required by each method (Overhead). Our results are shown in Table \ref{tab:disktime}. 
% TODO (above): Latency figures given in the table only represent the dense portion of retrieval. 
% TODO (above): We compare each method with RepLLaMA and SimLM embeddings for WHY DO WE DO THIS?
}


\comments{
We find that the disk access time required by CluSD is significantly less than the time required by LADR or a simple rerank. We suggest that SSD random seeks have significant overhead compared to consecutively reading. Thus, reading many documents consecutively from a cluster is quick, and the number of random seeks is limited to the number of clusters accessed. During other methods, it is likely that the number of random seeks is equal to the number of documents accessed. A simple least-squares model for our RepLLaMA results suggests that each random seek takes 167 us, whereas the time to read one document is only 11.8 us.
}


\comments{
We find that the disk access time required by CluSD is significantly less than the time required by LADR or a simple rerank. We suggest that SSD random seeks have significant overhead compared to consecutively reading. Thus, reading many documents consecutively from a cluster is quick, and the number of random seeks are limited to the number of clusters accessed. During other methods, it is likely that the number of random seeks is equal to the number of documents accessed. A simple least-squares model for our RepLLaMA results suggests that each random seek takes 167 us, whereas the time to read one document is only 11.8 us.
}

% CluSD is with XXXX configuration and XXXX average clusters per query. Reranking reranks the top-1000 documents from bm25 + docT5query. LADR_S are results from a "small" version of adaptive LADR, with k=128, n=8, c=200. LADR_L are results from a "large" version of proactive LADR, with k=128, n=200 that retrieves approximately ten times more documents than LADR_S






%Added for KDD 2024

\comments{
\begin{table}[htbp]
        \centering
 \resizebox{1.0\columnwidth}{!}{
                \begin{tabular}{r |lll|ll|rr}
                        \hline\hline
                        & \multicolumn{2}{c}{\bf{Relevance}}& \bf{\#Docs} &  \multicolumn{4}{c}{\bf{Dense Latency \& Breakdown (ms)}}\\
            & MRR@10 & R@1K & fetched&  MRT & P99 & I/O & CPU  \\
        \hline
        Rerank& 0.421 & 0.980 & 1000.0 & 127.5 & 186.1 & 125.2 & 2.3\\
        LADR\textsubscript{fast} & 0.419 & 0.980 & 2431.0 & 314.9 & 1013 & 1003 & 10.3\\ % ladr n=50, c=50, k=128
        LADR\textsubscript{default} & 0.422 & 0.984 & 8521.6 & -- & -- & -- & --\\ % ladr seed=200, depth=50, k=128
        % ABOVE: NEW NUMBERS WITH REAL UNCACHED DATA
        % BELOW: OLD NUMBERS WITH NoClust DATA
        %Rerank& 0.421 & 0.980 & 1000.0 &  18.8& 95.70 & 454.9  &16.9& 1.9\\
        %LADR\textsubscript{fast} & 0.419 & 0.980 & 2431.0 & 42.3 & 191.5 & 1106 &31.3 & 11.0\\ % ladr n=50, c=50, k=128
        %LADR\textsubscript{default} & 0.422 & 0.984 & 8521.6 &  119.3 & 349.8 & 3877 & 91.4 & 27.9\\ % ladr seed=200, depth=50, k=128
        % Above: LADR with time budget of CPU time ~= CluSD CPU time ~= 6-7ms
        % ========================
      %  D-ANN-Wentai & 0.398 & 0.970 & 271.4 & 5.24 & -- & 276.6 & 321.2\\
   %     SPANN-Wentai & 0.405 & 0.965 & -- & -- & -- & 123.6 & 159.6 \\
         %S+ DiskANN& 0.417 & 0.984 & -- &  276.5 & 321 & -- &272.3& 5.2\\ 
         S+ DiskANN& 0.417 & 0.984 & -- &  276.5 & 321 &272& 5.2\\ 
        DiskANN & 0.398 & 0.970 & --    & 276.5 & 321 & 272 & 5.2\\
        S+SPANN& 0.420 & 0.989 & -- &  123.6 & 159.6  &-- & -- \\
        SPANN& 0.396 & 0.965 & --    & 123.6 & 159.6  & -- & --\\
%Did Yingrui adds fusion and adds this on Wentai's result?  Yes  S+DiskANN & 0.417 & 0.984 & -- & -- & -- & 276.5 & 312.2\\ov
       % S+SPANN* & 0.424 & 0.985 & 6.54 & 6.20 & 3484.9 & +12.74 & 84.73\\
% Above: Parker selected clusters from top-16 SPLADE results -> thus relevance is too strong
        %CluSD& 0.425 & 0.986  & 6.19 & 6.48 & 4423.51 & 12.67 & 42.77\\
    %CluSD& 0.425 & 0.986  & 4423.5&  17.7& 47.8 & 178.1 &6.2& 11.0\\
    % ========================
    S+CluSD& 0.425 & 0.986  & 4423.5& 24.4 & 63.2 & 17.5 & 6.9\\
    % ABOVE: NEW NUMBERS WITH REAL UNCACHED DATA
    % BELOW: OLD NUMBERS WITH NoClust DATA
    %S+CluSD& 0.425 & 0.986  & 4423.5&  17.7& 47.8 & -- &6.2& 11.0\\
                \hline\hline
                \end{tabular}  }
        \caption{Search when uncompressed embeddings and/or the proximity graph are on disk for SPLADE + SimLM}
% Embedding space = 25.9 GB. Here we only report the latency of the dense retrieval part.
\vspace*{-5mm}
        \label{tab:disktime}
\end{table}

From Parker
LADR default without SPLADE
MRT = 643.7 ms
P99 = 2818 ms
CPU = 30.1 ms
IO = 2788 ms
}

% BELOW: new table that improves formatting
\begin{table}[htbp]
        \centering
 \resizebox{1.0\columnwidth}{!}{
                \begin{tabular}{r |ll|ll|rrr}
                        \hline\hline
                        & \multicolumn{2}{c}{\bf{Relevance}} &  \multicolumn{2}{c}{\bf{Latency (ms)}} & \multicolumn{3}{c}{\bf{Breakdown (ms)}}\\
S=SPLADE-HT1            & MRR & R@1K &  MRT & P99 & I/O  & CPU  & \# Docs  \\
        \hline
        %Rerank& 0.421 & 0.980 & 127.5 & 186.1 & 125.2 & 2.3 & 1000.0\\
        S+Rerank& 0.421 & 0.980$^\dag$ & 158.7 & 217.3 & 125.2 & 33.5 & 1000.0\\
       % LADR\textsubscript{fast} & 0.419 & 0.980 & 314.9 & 1013 & 1003 & 10.3 & 2431.0\\ % ladr n=50, c=50, k=128
        S+LADR\textsubscript{fast} & 0.419 & 0.980$^\dag$ & 346.1 & 1013 & 1003 & 41.5 & 2431.0\\ % ladr n=50, c=50, k=128
        %LADR\textsubscript{default} & 0.422 & 0.984 & 643.7 & 2818 & 2788 & 30.1 & 8521.6 \\ % ladr seed=200, depth=50, k=128
        S+LADR\textsubscript{default} & 0.422 & 0.984 & 674.9 & 2849 & 2788 & 61.3 & 8521.6 \\ % ladr seed=200, depth=50, k=128
        DiskANN & 0.398$^\dag$ & 0.970$^\dag$ & 276.5 & 321 & 272 & 5.2 & --    \\
        S+ DiskANN& 0.417$^\dag$ & 0.984 &  307.7 & 352.2 &272& 36.4 & -- \\ 
        SPANN& 0.396$^\dag$ & 0.965$^\dag$ & 123.6 & 159.6  & -- & -- & --    \\
        S+SPANN& 0.420 & 0.989 &  154.8 & 190.8  &-- & -- & -- \\
        %old without sparse time S+CluSD& 0.425 & 0.986 & 24.4 & 63.2 & 17.5 & 6.9 & 4423.5\\
        S+CluSD& 0.425 & 0.986 & 55.6 & 94.4 & 17.5 & 38.1 & 4423.5\\
                \hline\hline
                \end{tabular}  }
        \caption{Search when uncompressed embeddings and/or the proximity graph are on disk for SPLADE + SimLM}
% Embedding space = 25.9 GB. Here we report dense retrieval
\vspace*{-5mm}
        \label{tab:disktime}
\end{table}

CluSD significantly outperforms all other methods by leveraging block I/O.
CluSD is 2.2x faster than the next fastest system (SPANN), while having a noticeably higher relevance.
DiskANN performs similarly to SPANN, but is 4.97x slower than CluSD.
Reranking has a lower MRR@10 and recall@1k while being 2.85x slower.
Both variants of LADR have a lower MRR@10 than CluSD, but are 6.2x and 12.1x slower on average for LADR\textsubscript{fast} and LADR\textsubscript{default} respectively.
We find that  each  I/O operation has about a 0.15ms queueing and other software overhead on our tested PCIe SSD.
%We find that  each  I/O operation has about a 0.3ms queueing and other software overhead on our tested PCIe SSD.
Thus, more fine-grained operations in reranking yields more overhead.
Proximity graph methods such as LADR rely on large amounts of fine-grained I/O operations and significantly suffer in terms of latency when embeddings are stored on disk.
In comparison, CluSD takes advantage of block I/O and issues much fewer I/O operations to fetch 4,423 embeddings per query on average,
searching more documents in less time.

%Reranking is similar to CluSD in terms of  mean latency while having a 2x slower 99\textsuperscript{th} percentile latency, lower MRR@10 and  
%recall@1K. % in this case.
%The CPU-time of reranking is 
%short but its total time is 
%dominated by 1,000 random I/O operations for fetching top embeddings. 
%and reaches about  715MB/second I/O speed. 

%Our setting stores embeddings in clusters grouped by their similarity on disk, thus
%random I/O operations in reranking  benefits from spatial locality in clustered data, because top results tend to be similar. 

%and reranking is 25.7x slower in the mean latency. 
%We find that  each  I/O operation has about a 0.3ms queueing and other software overhead on our tested PCIe SSD.
%Thus, more fine-grained operations in reranking yields more overhead.
%In comparison, CluSD issues  much fewer  I/O operations to fetch 4,423 embeddings per query on average in a block I/O manner.
%Its 99\textsuperscript{th} percentile latency is 2x faster than re-ranking.


                                     
%CluSD outperforms LADR with higher MRR@10 and up-to 6.9x faster  for the two tested configurations.
% taking much less and  99\textsuperscript{th} percentile latency.   
%The above I/O spatial locality  explanation for reranking is also applicable to LADR.  
%CluSD outperforms  DiskANN and SPANN in relevance and is about 15.6x and 7x faster in mean latency, respectively. 
% which is designed for more general nearest neighbor search. 
%CluSD is comparable to SPANN in relevance  but is 6.98x faster in the mean latency.

% while CDFS, which fetches clusters of consecutive embeddings, utilizes block I/O that incurs less access overhead. 



==> cikmexp_llama.tex <==
%\subsection{CluSD with LLaMA-2 based dense retrieval}
{\bf CluSD with LLaMA-2 based dense retrieval}.
%\label{sect:llama}
Table~\ref{tab:RepLLaMA}
demonstrates that CluSD can effectively support selective RepLLaMA dense retrieval~\cite{ma2023finetuning} 
 when taking advantage of  a larger language model  on a low-cost platform for MS MARCO Dev. 
The ``Latency'' column includes sparse retrieval CPU time when ``S+'' is marked in the method name. 
S=SPLADE-HT1.
%This LLaMA-2~\cite{touvron2023llama} based model  
This LLaMA-2 based model uses 145GB embedding space with 4K dimensionality.
% for MS MARCO passages. 
All rows except the last row  conduct in-memory search assuming data fits into memory.
Row 1 shows  it takes 7.9 second CPU time to conduct in-memory full RepLLaMA  retrieval. 
Row 2  shows the performance of RepLLaMA using OPQ quantization but without IVF selective search.
Row 3  shows the performance of RepLLaMA using OPQ and  IVF selective search.
Use  of these optimization techniques leads to  a significant relevance degradation. 
As a reference, Row 4 lists the fusion of sparse results and  full dense retrieval. 
%Rows 5 and 6 are CluSD with SPLADE-HT1 retrieval without or with disk data.
%The latency includes sparse retrieval. 





\comments{
\begin{verbatim}
MRR@10	R@1K	CPU Latency	Space
(1) RepLLaMA	0.412	0.990	7.9s	145GB
(2) RepLLaMA-ivfopq	0.365	0.915	97ms	6.1GB
(3) S + CluSD	0.424	0.986	60ms	149GB
(4) S + RepLLaMA	0.426	0.994	7.9s	149GB
(5) RepLLaMA-OPQ	0.384	0.990	666ms	2.4GB

\end{verbatim}
}

\begin{table}[htbp]
\vspace*{-1em}
\small
        \centering
                \begin{tabular}{r r |l l|l l}
                        \hline\hline 
     &Method    & MRR@10 & R@1K & Latency & Space \\
                        \hline
1.  & RepLLaMA     & 0.412$^\dag$& 	0.990& 	7.9 s& 	145 GB\\
2.   &RepLLaMA-OPQ& 	0.384$^\dag$& 	0.990& 	666 ms& 	2.4 GB \\
3.  & RepLLaMA-IVFOPQ & 	0.365$^\dag$ & 	0.915$^\dag$ & 	97 ms & 	6.1 GB\\
4.   & S + RepLLaMA  & 	0.426& 	0.994& 	7.9 s& 	149 GB\\
5.   & S+CluSD & 0.424	& 0.986& 	39 ms& 	149 GB\\
6.   & S+CluSD (on-disk)& 	0.424	& 0.986& 	60 ms& 	149 GB\\
                \hline\hline
                \end{tabular}  
        \caption{CluSD with  dense RepLLaMA and  sparse SPLADE} 
\vspace*{-2em}
        \label{tab:RepLLaMA}
\end{table}


CluSD applies SPLADE sparse retrieval and then visits  a small number of clusters from 60,000 dense RepLLaMA clusters. 
CluSD  with SPLADE-HT1 takes about 39ms with in-memory search shown in  
Row 5, and  60ms with on-disk search shown in Row 6.  
%The latency time includes both sparse and dense retrieval on a CPU server. 
To use GPU, RepLLaMA inference would require five Nvidia V100 GPUs (each with 32GB) to host data and take 37ms GPU time. 
Thus CluSD  can deliver 1 or 2 order of magnitudes of improvement in total latency or infrastructure cost.

RepLLaMA does very well for zero-shot retrieval on BEIR datasets with average NDCG 
0.561 and CluSD can deliver fast with average NDCG 0.541.
Our LSTM model for RepLLaMA was a zero-short version trained using  BERT-based SimLM on MS MARCO passage 
data and then applied to search MS MARCO Dev and BEIR datasets and we expect that further improvement is possible in the future.
%(a 3.6\% NDCG degradation) 



==> cikmexp_sparse.tex <==
\subsection{CluSD with other sparse models}
\label{sect:evalsparse}

%We explore the model performance when we interpolate different sparse model with SimLM with cluster selection in 
Table~\ref{tab:sparse} examines CluSD's fusion of SimLM
with  other three sparse models.
Last column lists in-memory dense retrieval portion of latency.
% under  different efficiency/relevance tradeoffs.
For each sparse  model, CluSD boosts overall relevance.
%These sparse models accomplish  different relevance  scores: 
%CluSD fused with  the   fastest BM25T5 model delivers the lowest MRR number while its fusion  with the slowest LexMAE delivers
%the highest MRR@10 number.
%The final relevance outcome of using two SPLADE models is better  than that for BM25 retriever.
%That is partially caused by dependence of LSTM training where  the positive clusters are identified by the overlap of top 10 SPLADE results with these  clusters.
As  CluSD's cluster selection  relies on  the overlap feature  of top sparse results with dense clusters,
the guidance from the fastest BM25 results is less accurate than other  sparse models. On the other hand, with a guidance from 
the slowest but stronger LexMAE retrieval, CluSD yields the highest MRR@10, comparable to full search. 
%the quality of top sparse results still has an impact on the final outcome.  
%consists of the distribution of sparse top results into clusters. 
%When the sparse model doesn't identify good top candidates, the input features to the LSTM model becomes more noisy which affect performance. 
\comments{
From left to right, the model performance degrades. 
We can observe that when sparse model performance degrades, 
the performance of S + CluSD degrades as well on the flat index. 
For example, on Splade-HT1-fast, the relevance is around the same as S $+$ D on MRR@10, and 0.6\% degradation on recall@1K. 
When we use BM25-T5 model, the degradation is 1.7\% and 1.5\% respectively on MRR@10 and recall@1K. 
This indicates that when the Splade model model does not perform well, CluSD becomes less effective. 
It is expected because the input to the LSTM model consists of the distribution of sparse top results into clusters. 
When the sparse model does not identify good top candidates, the input features to the LSTM model become more noisy which affects performance.
}

\comments{
\begin{table}[htbp]
	\centering
		\resizebox{\columnwidth}{!}{%
		\begin{tabular}{ r l l  |ll |ll |r }
			\hline\hline
                Sparse model& \multicolumn{2}{c|}{\bf{Splade-HT1-fast}} & \multicolumn{2}{c|}{\bf{Splade\_effi-HT3}}   & \multicolumn{2}{c|}{\bf{BM25-T5}} & Extra\\ 
%\cline{1-7}
%                Latency & \multicolumn{2}{c|}{22.4ms} & \multicolumn{2}{c|}{12.4 ms}   & \multicolumn{2}{c|}{9.2 ms} & Latency\\ 
\cline{1-7}
			& {MRR} & {R@1K}  & {MRR@10} & {R@1K}   & {MRR} & R@1K  & latency \\
   \hline
   \multicolumn{8}{c}{\bf{Uncompressed SimLM embeddings with  27.2 GB space}}\\
			\hline
			S & 0.385$^\dag$& 0.949$^\dag$& 0.380$^\dag$& 0.944$^\dag$& 0.259$^\dag$& 0.935$^\dag$& -\\
                $\blacktriangle$  S $+$ D & 0.416 & 0.986 & 0.413 & 0.984 & 0.415 & 0.985  & +1674.1\\
                {\textbf{S $+$ CluSD}} & 0.415 & 0.981$^\dag$& 0.411 & 0.979$^\dag$& 0.408& 0.970$^\dag$& +12.1 \\
                \hline
                \multicolumn{8}{c}{\bf{OPQ m=128. SimLM embedding space  1.1 GB}}\\
%, Report S+*
\hline
                S $+$ D-IVFOPQ & 0.384$^\dag$& 0.981$^\dag$& 0.381$^\dag$& 0.978$^\dag$& 0.369$^\dag$& 0.975$^\dag$& +21.9 \\
                %S $+$ D=HNSWOPQ & & & & & & &  \\
                \bf{S $+$ CluSD} & 0.413& 0.984& 0.412& 0.984& 0.402$^\dag$& 0.975$^\dag$& +9.8  \\
                %\hline
                %\multicolumn{8}{c}{OPQ M=64. Embedding space  0.6 GB}\\
%, Report S+*
                % S $+$ IVFOPQ-5\% & 0.389 & 0.981 & 0.389 & 0.980 & 0.370 & 0.975 & 23.7 \\
                %S $+$ HNSWOPQ & & & & & & &  \\
                %S $+$ \bf{CS} & 0.402& 0.981& 0.402& 0.981& 0.380& 0.973& 10.2 \\
            \hline\hline
		\end{tabular}
		}
	\caption{CluSD performance  under  other  sparse models}

\vspace*{-5mm}
	\label{tab:sparse}
\end{table}
% For all three sparse models, we use the same dense model configuration so for each row we only report one latency number. 
}

\comment{
\begin{table}[htbp]
	\centering
		\resizebox{\columnwidth}{!}{%
		\begin{tabular}{ r r r r r  r r r}
			\hline\hline
			& \multicolumn{2}{c}{MSMARCO Dev}& \multicolumn{2}{c}{DL19}& 
\multicolumn{2}{c}{DL20} \\
			& \% n& MRR@10 & R@1K & NDCG@10 & R@1K &  NDCG@10 & R@1K\\
   			\hline
 D& -- & 0.416& 0.988& 0.720& 0.744& 0.703&0.755\\
            $\blacktriangle$  S $+$ D & -- & 0.425 & 0.988 &  0.740& 0.816&   0.731& 0.819\\
            \bf S $+$ \bf{CluSD} & 0.5 &  0.426 & 0.987 &  0.744&  0.820& 0.734&  0.818\\
            \hline
            \multicolumn{8}{c}{OPQ M=128 setting, Storage 1.1GB, Report S+*}\\
            \hline
            IVFOPQ &10 & 0.404 & 0.987 & 0.713 & 0.818 & 0.722 & 0.817 \\
            & 5 & 0.394 & 0.987 & 0.687 & 0.817 & 0.706 & 0.817 \\
            & 2 & 0.374 & 0.986 & 0.656 & 0.815 & 0.700 & 0.817 \\
            HNSWOPQ & & & & & & \\
            \bf{CS} & 0.5 & 0.417& 0.986& 0.742 & 0.818 & 0.735  &0.815 \\
            \hline
            \multicolumn{8}{c}{OPQ M=64, Storage 0.6 GB, Report S+*}\\
            \hline
            IVFOPQ & 10 & 0.393 & 0.986 & 0.676 & 0.814 & 0.730 & 0.818 \\
            & 5 & 0.384 & 0.985 & 0.659 & 0.814 & 0.717 & 0.817 \\
            & 2 & 0.368 & 0.985 & 0.643 & 0.814 & 0.707 & 0.816 \\
            HNSWOPQ & & & & & & & \\
            \bf{CS} & 0.5  & 0.403& 0.987& 0.729 & 0.812 &0.724 & 0.814 \\           
			\hline\hline
		\end{tabular}
		}
	\caption{RetroMAE
%For quantization methods on top of ColBERT, we also report \% degradation from ColBERT.
}
	\label{tab:retromae}
\end{table}
}

%Added for KDD 2024

\begin{table}[htbp]
	\centering
		\resizebox{\columnwidth}{!}{%
		\begin{tabular}{ r |l l  |ll |ll |r }
			\hline\hline
                Sparse model& \multicolumn{2}{c|}{\bf{LexMAE}} & \multicolumn{2}{c|}{\bf{uniCOIL}}   & \multicolumn{2}{c|}{\bf{BM25T5}} & \bf{Dense}\\ 
%\cline{1-7}
                % & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{}   & \multicolumn{2}{c|}{} & Latency\\ 
\cline{1-7}
			& {MRR} & {R@1K}  & {MRR} & {R@1K}   & {MRR} & R@1K  & \bf{latency}\\
   \hline
   \multicolumn{8}{c}{\bf{Uncompressed SimLM  embeddings  with 27.2 GB space}}\\
			\hline
			S & 0.425& 0.988& 0.347$^\dag$ & 0.957$^\dag$& 0.259$^\dag$ &  0.935$^\dag$& -\\
                $\blacktriangle$  S $+$ D &    0.430& 0.990& 0.413 & 0.985& 0.415& 0.985& 1674ms\\
                S $+$ Rerank& 0.432& 0.988& 0.415& 0.957$^\dag$& 0.409& 0.935$^\dag$& 21.9ms\\
                %S $+$ LADR& 0.430& 0.990& 0.414& 0.983& 0.412& 0.983& 21.9ms\\
                {\textbf{S $+$ CluSD}} & 0.431& 0.989& 0.414 &  0.980&  0.410&  0.980& 12.1ms\\
                \hline
                \multicolumn{8}{c}{\bf{OPQ m=128. SimLM embedding space  1.1 GB}}\\
%, Report S+*
\hline
                S $+$ D-IVFOPQ & 0.383$^\dag$& 0.988& 0.354$^\dag$& 0.961$^\dag$& 0.369$^\dag$& 0.975$^\dag$& 21.9ms\\
                %S $+$ D=HNSWOPQ & & & & & & &  \\
                \bf{S $+$ CluSD} & 0.429& 0.989& 0.404 & 0.980&  0.402$^\dag$& 0.975$^\dag$& 9.8ms\\
                %\hline
                %\multicolumn{8}{c}{OPQ M=64. Embedding space  0.6 GB}\\
%, Report S+*
                % S $+$ IVFOPQ-5\% & 0.389 & 0.981 & 0.389 & 0.980 & 0.370 & 0.975 & 23.7 \\
                %S $+$ HNSWOPQ & & & & & & &  \\
                %S $+$ \bf{CS} & 0.402& 0.981& 0.402& 0.981& 0.380& 0.973& 10.2 \\
            \hline\hline
		\end{tabular}
		}
	\caption{ CluSD with  LexMAE, uniCOIL \& BM25  sparse models}
\vspace*{-6mm}
	\label{tab:sparse}
\end{table}


==> cikmintro.tex <==


\section{Introduction}

\label{sect:intro}
Dense and sparse retrievers are two main categories of retrieval techniques for text  document search.
%It can be time-consuming to compute query-document similarities for the whole corpus on a CPU-only platform. The cost is often mitigated through approximate nearest neighbor search techniques. However, this reduction in latency comes with a tradeoff in relevance effectiveness. 
Traditional sparse retrieval models, such as BM25, use lexical text matching and run
%to retrieve results from the collection 
efficiently by traversing  an inverted index on an inexpensive  CPU platform.
Recently, sparse retrieval studies have exploited deep learning models~\cite{Dai2020deepct,
Mallia2021deepimpact, Lin2021unicoil,2021NAACL-Gao-COIL, Formal2021SPLADE, shen2023lexmae} to learn lexical representations of documents for better matching.
Dense retrieval 
exploits a dual encoder architecture to produce single document representations, 
e.g. ~\cite{gao-2021-condenser,2021SIGIR-Zhan-ADORE-dense,Ren2021RocketQAv2, 
Lin2021tctcolbert, Santhanam2021ColBERTv2,  Wang2022SimLM,  Liu2022RetroMAE}.
This paper is focused on the efficiency optimization to combine the above  two retrieval approaches on a low-cost CPU-only platform.
This  is important in a large-scale  search system  which employs  a multi-stage search architecture, and 
runs partitioned first-stage retrieval in parallel  on a massive number of inexpensive machines. 
Single-GPU memory size is limited and insufficient to host a large language model for dense retrieval.
Since GPU servers tend to be an order 
of magnitude more expensive than CPU-only platforms,
using multiple GPUs for retrieval and replicating them in many data centers can cost 
billions of dollars and consume much more energy for a large and busy search engine. 
%For instance, AWS EC2 charges 
%High cost can be seen from AWS EC2 which charges a GPU instance one or two magnitute more than a strong CPU instance.  
%23x more for a GPU instance than CPU one for RepLLaMA retrieval.

%and SPLADE~\cite{Formal2021SPLADE, Formal2021SPLADEV2} has demonstrated the strong relevance performance among these models. 
\comments{
Recent studies have found that combining  sparse and dense retrieval scores  can further boost
retrieval recall and relevance~\cite{Lin2021unicoil,2022LinearInterpolationJimLin,kuzi2020leveraging},
suggest  that both categories  of retrievers tend to capture  different relevant signals. 
These studies  make an assumption that  a search platform has to run two retrievers separately and a dense retriever.
%delivers   its maximum effectiveness, and the impact of compression and IVF clustering is not considered. 
There is an imbalance of computing platform requirements for running  these two retrievers.

dense retrieval typically requires GPU support unless significant  
%We study the use of dense retrieval results to argument sparse retrieval. 
Sparse retrieval with an inverted index has the advantage that a low-cost CPU server can run the online inference  without GPU.
A judicious tradeoff consideration of retrieval  effectiveness and efficiency is critical on  a low-cost CPU-friendly search platform. 
The importance of CPU-friendly search is recognized 
in neural ranking studies~\cite{Yang2021WSDM-BECR,2022WWWforwardIndex,2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
For a large-scale  dataset (e.g. with billions of documents), a practical search system often employs  a multi-stage 
search architecture, which divides the dataset into many partitions so that  a fast first-stage  retrieval 
method  can  search these partitions in parallel.  Such a system  prefers low-cost
CPU-only servers for first-stage retrieval, and both time and memory space complexity of retrieval should be considered 
so that  each server can host as many documents as possible
to reduce the total number of servers to support a large data size and high query traffic. 
%Thus the challenge for retrieval on such an architecture needs to consider both time and space complexity. 
% small search index needs to be as small as possible.
%and the in-memory footprint size of 
%server  needs to host documents in memory as many as possible 
%given a large number  of data partitions involved for parallel search.
%Each server employs multiple CPU cores and is replicated with many copies  for dealing high traffic of  concurrent 
%search requests, and thus 
}

%which run  efficiently  on a single CPU without hardware accelerators  GPU
%which re  retaining strong relevance effectiveness
%%Another development in learned sparse retrieval is that
%sparse retrieval with a learned representation
\comments{
There are several recent efficiency studies advancing the
inverted index implementation for sparse retrieval with learned neural 
representations~\cite{Lassance2022SPLADE-efficient,mallia2022faster,qiao2023optimizing,2023SIGIR-Qiao, 2023SIGIR-SPLADE-pruning}.
which accelerates learned sparse retrieval with BM25-guided traversal or index pruning.

For example, Row 3 of Table~\ref{tab:costbudget} shows the latency, memory space cost, and  MRR@10  of
the latest efficient SPLADE retriever for searching 8.8 million 
MS MARCO passages~\cite{2023SIGIR-Qiao} on a CPU-only server.
% with a single thread on  a 2.25GHz AMD EPYC 7742  CPU server.
Row 2 is performance of a BM25-based retriever after document expansion. 
%There is a tradeoff  in relevance effectiveness if BM25 guidance or threshold-based pruning  is too aggressive.
%and dense retrieval can boost if it does not add much overhead. 
}

As shown in previous literature~\cite{Lin2021unicoil,2022LinearInterpolationJimLin, kuzi2020leveraging}, combining  sparse and dense retrieval scores with linear interpolation
can boost relevance. 
However, none of above studies has considered to exploit the relationship of sparse and dense retrieval results for selective fusion. 
Dense retrieval is expensive, typically requiring GPUs. 
The cost of dense retrieval can be greatly reduced  by using  approximate nearest neighbor (ANN) search with 
partial IVF cluster search~\cite{johnson2019billion, 2021Facebook-DrBoost-Lewis} and proximity graph based navigation (HNSW)~\cite{2020TPAMI-HNSW}.
%2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
However, there is a  relevance tradeoff for a  reduced search cost in these efforts. For example,
Table~\ref{tab:costbudget} shows that  
while RetroMAE~\cite{Liu2022RetroMAE}, a state-of-the-art  dense retriever,  is slow on CPU without compression, the use of
5\% IVF cluster search reduces CPU time substantially  but there is a 7.5\% drop in MRR@10.
The use  of  OPQ quantization~\cite{Ge_2013_CVPR} implemented in FAISS~\cite{johnson2019billion}
 further reduces memory space  to 1.2GB but causes an extra 4.6\% MRR@10 drop.

\begin{table}[htbp]
        \centering      
         \resizebox{0.82\columnwidth}{!}{ 
                \begin{tabular}{ r | r  rr}
                        \hline\hline
Dense methods  & Latency & Memory & MRR@10\\ 
\hline
%BM25/DocT5Query & 9.2ms & 1.2GB & 0.261\\  
%SPLADE/HT1 & 31.2ms & 3.9GB & 0.396 \\ 
RetroMAE/Uncompressed & 1677ms & 27.2GB & 0.416 \\ 
%RetroMAE/IVF SimLM perhaps 3\% & 49.6ms  & 27.2GB & 0.389 \\ 
RetroMAE/IVF 5\% & 107ms  & 27.2GB & 0.387 \\ 
%SimLM /OPQ             & 225-1579ms & 0.57-2.3GB & $<$ 40.2 \\
RetroMAE /IVF 5\% OPQ  & 38ms & 1.2GB  & 0.370 \\ 
%RetroMAE SimLM? /IVF  OPQ  & 38-339ms & 1.2-2.3GB  & 0.37-0.401\\ 
                        \hline\hline
\end{tabular}
}
\caption{Latency, relevance, and space  tradeoff  in a dense model for passage retrieval with MS MARCO Dev set}
 \vspace*{-6mm}
\label{tab:costbudget}
\end{table}


%Quantization~\cite{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ} is another orthorgonal cost reduction technique.

LADR~\cite{2023SIGIR-LADR}, as a follow-up study of  GAR~\cite{2022CIKM-MacAvaneyGraphReRank},
has investigated partial dense retrieval by  
%pioneering in
taking  the results of a sparse retriever as a seed to select embeddings
%That takes an approach of augmenting sparse retrieval results using graph-based navigation based on
based on a document-to-document proximity graph. This strategy  follows  the previous graph-based ANN approach~\cite{2020TPAMI-HNSW,2021KDDgraphANN}. 
Using  sparse retrieval results as a seed  allows quick narrowing of  the search scope at a low CPU cost. 
While LADR and HNSW have demonstrated their high efficiency  to search within a time budget,
use  of a document-wise similarity graph adds a significant online space requirement  on a low-cost computing platform. 
%document-level  proximity graph  construction is  expensive for a large dataset during offline processing. 
For example, the proximity graph  can take an extra 4.3GB memory space~\cite{2023SIGIR-LADR} for an 8.8M  MS MARCO passage dataset.
% to keep top 128 top neighbors per document.  
%The above studies focus on  a standalone dense search task given seed candidates, and our work
%exploits  the overlap degree  of sparse and dense retrieval, which yields additional  optimization benefits.


Another limitation of LADR and  HSNW is the assumption of in-memory access to proximity graphs and dense vectors. 
% PARKER's suggestion:
For large datasets or higher-dimension embedding vectors, some or all of the embeddings and proximity graphs will have to 
be stored on disk, especially when such  applications desire uncompressed embeddings for  better  relevance. 
For example, the embedding dimension of the recent RepLLaMA dense retriever~\cite{ma2023finetuning} is 4096
based on LLaMA-2~\cite{touvron2023llama}, which leads to 145GB storage space for MS MARCO passages.
It is possible that more advanced dense models may be developed to take advantages of  
large language models in the future with  a higher  embedding dimensionality (e.g. up to 12,288~\cite{NEURIPS2020_GPT3}) for 
better relevance. 
For on-disk large data search, random access of dense embeddings and/or a document-level proximity graph can incur substantial 
fine-grained I/O overhead.
DiskANN~\cite{NEURIPS2019_DiskANN} and SPANN~\cite{chen2021spann} are
two on-disk ANN search algorithms for general data applications and they do not  leverage sparse retrieval.
They have not been studied in the context of text document retrieval
where the importance of semantic text matching presents a unique challenge and requires new design considerations.

% to replace: 
%When the dense embeddings or its proximity graph of a large dataset cannot fit into memory, this approach that access can suffer 
%large random fine-grained I/O access overhead. 
%Nevertheless, random access of dense embeddings and/or graph nodes, as necessitated by document-level proximity graph navigation, can incur substantial
%fine-grained I/O overhead.  

%In contrast, cluster-based structuring captures  similar documents from  statically-formed  groups and enables faster  block-level I/O.
%DiskANN  and its variant study on-disk graph navigation for ANN search~\cite{NEURIPS2019_DiskANN,2023Web-Filtered-DiskANN},
%and SPANN is an effort on cluster-based ANN search. They are targeted for a stand-alone and geneal ANN problem while our 
%work takes an advange of sparse retrieval for better relevance  in the context of text document search.

%None of above studies has considered to exploit the relationship  of sparse and dense retrieval results for selective fusion. 

\comments{
That is true also with the  navigation of  a  proximity graph based on inter-document similarity distances called HNSW~\cite{2020TPAMI-HNSW}. 
The proximity graph approach to guide dense retrieval is revisited recently in GAR~\cite{2022CIKM-MacAvaneyGraphReRank}, which is furthered improved by
%LADR Kulkarni  et al.~\cite{2023SIGIR-LADR} improves HNSW.
LADR~\cite{2023SIGIR-LADR}.
%~\cite{2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
The weakness of  the  proximity graph approach is that its graph  construction requires a quadratic computing complexity, which is expensive
for a large dataset and the online hosting of such a graph also adds a significant space requirement  on a low-cost
computing platform. For example, LADR takes an extra 4.3GB memory space for 8.8M  passages in the MS MARCO dataset to keep top 128 
top neighbors per document. 
%Similarily HNSW also incurs a high space cost for graph connections.  
%In comparison, cluster-based selective dense retrieval can achieve in a comparable time complexity
%while adding  insignificant extra  space  overhead.
}



  
%with a latency controled within 4 to 8 milliseconds on a single CPU, but with a significant tradeoff in relevance effectiveness.
%For example, MRR@10 for MS MARCO Dev set drops from RetroMAE has dropped from  0.416 to 0.356.
%This paper does not impose 4-8 millisecond latency, but rather looks for a solution that can leverage both dense and sparse retrieval
%and relax the latency constraint in some degree while maximizing its relevance effectiveness as much possible.
%a range below or around  100 milliseconds 

%The response time  for such a system for an interactive service needs to be fast enough a
%and thus search needs to be completed within a few hundred milliseconds. 

%which only requires triggering of dense embedding  computation for a relaively small subset of documents.
%The proposed scheme called cluster-based selective dense  retrieval


This paper proposes a lightweight approach called CluSD to 
conduct Cluster-based Selective Dense retrieval at a low CPU-time and space cost after sparse retrieval. 
%and  combine its results  with  sparse retrieval. 
%It exploits the relationship  of sparse and dense retrieval results to conduct  selective fusion. 
%To accomplish that, 
CluSD limits query-document similarity computations through a two-stage cluster selection algorithm via an LSTM model, which  
exploits inter-cluster distances and the overlapping degree between top sparse retrieval results and dense clusters.
%CluSD leverages IVF clustering and does not require an extra document similarity graph. 
%and then make a decision to determine which document clusters should be selected  to conduct dense retrieval computation.
%The extra memory space overhead required to assist CluSD is negligible, and it  works well when embedding vectors are highly compressed.
%  and  the extra memory required for hosting dense embeddings can be limited  after compression. 
When dense clusters are not available in memory, CluSD selects and loads a limited number of clusters with efficient disk block I/O.
Thus, it can handle a large dataset with high-dimension embeddings that cannot fit in memory, with less I/O overhead compared to a
graph-based ANN approach.  % TODO: second comma? split into two sentences? come back later Parker
This paper evaluates  the effectiveness of CluSD  under time and space constraints on a CPU-only server in searching 
the MS MARCO and BEIR  datasets  when they fit or do not fit into memory.
%We compare against other baseline methods, including in a case in which the dataset does not fit into memory.
Our goal is to show that CluSD reaches state-of-the-art relevance levels at a much lower space and/or time cost including I/O if needed.



%0.419 by RocketQAv2~\cite{Ren2021RocketQAv2}, 
%which are the two latest state-of-the-art retrieval-reranker pipelines using cross-encoder based rerankers.
%Re-ranking in  recent dense retrieval work SimLM~\cite{Wang2022SimLM} has  used an expensive cross-encoder to
%achieve impressive MRR score 0.437 
%Re-ranking in RocketQAv2~\cite{Ren2021RocketQAv2} achieves 0.419 with a similar strategy.  



%Our evaluation also compares DiskANN~\cite{NEURIPS2019_DiskANN,2023Web-Filtered-DiskANN} and SPANN~\cite{chen2021spann}
%that conduct on-disk  ANN search, and these studies are targeted for general ANN search without considering the leverage of
%sparse retrieval.
%and  shows that CluSD can effectively identify a small number of document clusters to 
%for  a stronger relevance  even though such a sparse retriever is fast with a relevance tradeoff. 
 
%provides a flexibility and reduces  the relevance requirement of sparse retrieval.
%Namely protentially we can choose a relatively fast sparse retrival with the slightly lower accuracy/recall,
%and  let dense retrivsal make up the loss. Our design needs to  adapt to  sparse retrieval quality and plans

%CSDR in improving the effectiveness of sparse retrieval with limited dense  retrieval
%traversal for low-cost search.  Our emprial findings suggest that SRF  can consistently outperform other baselines on a single CPU server 
%without GPUs 
% and achieve a strong tradeoff of effectiveness and efficiency compared to an exhausitve dense retrieval search.


%from pretrained language models to provide effective semantic text matching between a query and a document.



==> cikmmethod.tex <==
%\section{SRF with Query-Specific Cluster Skipping }
%\section{CluSD: Selective Dense Retrieval}

  
%\section{Selective Dense Cluster Retrieval}
%%%%%%%%%\label{sec:clusd}

\comments{
It is common practice to interpolate the results from a sparse system and a dense system. We propose two directions to improve the latency of such system by avoiding the unnecessary dense evaluation on query level and per query level. We envision a hybrid system where sparse retrieval runs first and partial query and documents are evaluated by the dense retrieval system. 

The proposed CluSD method contains two components  during runtime inference to 
decide if  dense retrieval augmentation  can be skipped for a query and which  top dense document clusters should be selected  during supplemental retrieval.
}

%Per-query inference latency depends on the number of document evaluated and how per query-document evaluate is approximated. We do not touch per-query-document approximation in this paper and focus on reducing the number of documents evaluated. We cluster document using kmeans as IVF and would like to intelligently select a few most promising clusters to retrieve candidate results. 
\comments{
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.9]{lstm.png}
    \caption{LSTM prediction for each query}
    \label{fig:lstm}
\end{figure}
}
\comments{
As discussed earlier, documents with embedding vectors are clustered based on their similarity to the cluster centroids. 
Our experiments take an advantage of the FAISS library which  provides such a support such as k-mean clustering.
Once a query is determined by CluSD to trigger  partial dense retrieval that selects and visits a subset of dense clusters. 
% online inference  will  visit the dense clusters one by one in
%an incresing order of   their centroid distance to the input query.
%A decision procedure is invoked to decide if a cluster to be visited should be skipped or not. 
Our objective is to examine the features of each cluster and  incrementally decide if this cluster should  be visited or not.
This section will first describe the overall flow of CluSD in online inference for selective fusion of sparse and dense retrieval,
 then present an LSTM-based  cluster selection algorithm. 
}


\subsection{ Online inference}
\label{sect:online}
\begin{figure}[htbp]
    \includegraphics[scale=0.79]{sparse_dense_flow_lout.drawio.pdf}
 \vspace*{-2mm}
    \caption{The flow of cluster-based selective dense retrieval}  
 \vspace*{-3mm}
    \label{fig:flow}

\end{figure}





%Step 3. Call the LSTM selection (Section 4.1)  to choose a small number of dense clusters. That is about 25 in our MS MARCO evaluation.





The online inference algorithm of CluSD has the following steps:

\textbf{Step 1}:   Conduct sparse retrieval to obtain top-$k$ results.

%\item Conduct the query filter  to determine if the cluster-based dense retrieval is necessary.If needed, 
%Step 2:  Sort clusters based on the overlap degree of dense clusters and top sparse retrieval results and their  centroid-to-query  distances.

\textbf{Step 2}:  Conduct a two-stage selection process. 
Stage I selects the top-$n$ clusters from  the given $N$ dense embedding clusters, discussed in detail in Section~\ref{sect:stage1}.
%The  key  features collected include the overlap degree of dense clusters and top sparse retrieval results and their centroid-to-query distances.
Stage II  applies an LSTM model to the $n$ top clusters
to choose  a limited number of dense clusters to evaluate, discussed in Section~\ref{sect:lstm}. 

\textbf{Step 3}: Expand the top-$k$ sparse retrieval results to include the documents vectors of these dense clusters and
merge their sparse and dense scores with linear interpolation.  

%During the above linear interpolation, only top $k$ of sparese retrieval contains a lexical score,
%and thus we  impute the lexical scores of other documents expanded by cluster-based selective dense retrieval 
%as the bottom document score in the top $k$ sparse retrieval list scalled by a factor. We use 0.95 in our evaluation.
\comments{
Notice that  the two ranked lists from two retrievers are usually not fully overlapped and  some documents only exist in one list. While
different  treatments on these documents affect fusion performance,
we resort  to imputing the score of such a document using  the top $k+1$ score   in the missed rank list scaled by 
a factor.
%While there are options to We consider a few options
For example,  we  impute the lexical scores of new documents added  by dense retrieval
using  the scaled lexical score of  top $(k+1)$ in the sparse retrieval list. We use scale $0.95$  in our evaluation.
}
%\item Remove the documents when they only exist in one ranked list
%    \item  Take the document and compute the score for only one ranked list

%When we have access to a relatively strong sparse retrieval system and a dense retrieval system, it is feasible to selectively choose queries that requires evaluation of both systems. We hypothesize that the sparse system is economical and we can afford to run it for every query. The problem boils down to dynamically select queries to evaluate by dense retrieval.

{\bf Time  and space  cost for CluSD.} 
%We only consider the cost of  online partial dense retrieval. 
The embedding space is $O(D)$  for a corpus with $D$ vectors.
For MS MARCO, this  cost is around 27GB without compression. Quantization can reduce the total size to about  0.5GB  to 1GB, depending on codebook parameters.
Then this cost becomes a fraction of sparse retrieval index cost.  
Excluding embeddings, the extra space overhead for CluSD is to maintain  the similarity among centroids of $N$ clusters.
We only maintain top $m$ cluster neighbors for each cluster in terms of their centroid similarity. 
For our evaluation, $m=128$ and this reduces the extra space overhead as $O(N)$, which
is negligible compared  to the embedding space with $N << D$. 
For example,  with $N=8192$,  the inter-cluster graph for MS MARCO passages takes about 5MB with quantization.
%In our evaluation, %we use  $N=8192$ or  $4096$.
%the inter-cluster similar graph for MS MARCO passages with $N=8192$ takes about 32MB with quantization.

Excluding sparse retrieval cost, the time  cost of 
CluSD is dominated by the cost of cluster selection and  dense similarity computation of selected dense clusters.
The former is about $O(n)$ while the latter is
proportional to the number of clusters selected, which is capped by $O(\frac{D}{N} n)$. 
In  our evaluation of MS MARCO and BEIR, $n$ is chosen to be 32, and
the actual number of clusters selected and visited is about 22.3.
%Given the short time added by the pruned LSTM model, 
Thus, the overall latency overhead introduced by CluSD is fairly small. 


\subsection{ Stage I: Selection of  top $n$ candidate clusters} 
\label{sect:stage1}
\comments{
As discussed earlier,  we control 
the input length  of the above  LSTM model  to be  $n$  as 
the number of top candidates clusters to be examined, and then the inference 
}

Given  $N$ clusters grouped using dense document embeddings, 
we devise a strategy below to conduct a preliminary selection that
prunes low-scoring clusters that contain  only less relevant documents.
%prunes low-scoring clusters that may not provide a meaningful boosting of relevance quality,
%and  choose  top $n$ candidate clusters for Stage II for further refinement.
The two-stage approach is motivated by the fact that the LSTM model used in the second stage is time consuming to examine all clusters. 
%Thus, we truncate the sequence of clusters to maximum length $n$ and then take a sequence of top $n$ clusters as the input to this LSTM. 
Thus, we choose the top-$n$ candidate clusters first.
\comments{
There are  $n$ nodes corresponding to these clusters in the LSTM model.
We will discuss how to truncate with a prioritization shortly below.
%Because this decision procedure uses the document scoring information  of each cluster visted 
}
\comments{
Table ~\ref{tab:LSTMclustertime} shows that the number of clusters to be examined
varies from 32 to 512, the LSTM inference time increases from  2.8ms to 33.9ms.
As we would like to make a quick decision given the overall  time budget,
we devise another strategy to prune clusters that may not provide a meaningful boosting
of relevance quality. 

% dependent on the length of the sequence input. 

\begin{table}[h]
	\centering
		\resizebox{0.68\columnwidth}{!}{ 
%		\begin{small}
		\begin{tabular}{r | rrrrr}
			\hline\hline
			  \#Clusters examined & 512 & 256 & 128 & 64 & 32 \\
\hline
            Time (ms) & 33.9 & 16.2 & 6.2 & 3.8 & 2.8\\
                \hline\hline
		\end{tabular}
%		\end{small}
	}
	\caption{LSTM inference time with different input lengths.}
	\label{tab:LSTMclustertime}
% \vspace{-4mm} 
\end{table}

\comments{
\begin{figure}[htbp]

    \includegraphics[scale=0.27]{dist.pdf}
    \caption{Distribution of Good Documents }
    \label{fig:dist}
%\vspace{-1em} 
\end{figure}
}
}

To prioritize clusters, one idea is to adopt their query-centroid distance used
in IVF cluster selection.  We find this does not work well for CluSD.
For example, if we rank clusters based on the query-centroid distance for MS MARCO passages, 
around 10\% of top-10 dense results reside in clusters ranked beyond the 175th cluster, which means we would have to 
select 175 clusters in order to recover 90\% of top-10 documents. Visiting all of these clusters is still too slow
and as evaluated later in Section~\ref{sect:threshold}, CluSD only visits about 22.3 clusters on average for MS MARCO Dev set. 
  
\comments{
Table~\ref{tab:dist} shows the distribution of top 10 documents from the full dense retrieval  
in embedding clusters under the different query percentile when searching an MS MARCO passage dataset using queries from its  Dev set. 
Row 2 of Table~\ref{tab:dist} shows the number of top clusters needed to cover  top 10 
documents from the full dense retrieval  when clusters are sorted by sorted by  the query-centroid distance.
This row shows that to cover top 10 dense results, $n$ needs  to be larger than 175.
%On the other hand, Row 2 is  the number of lusters decided by the LSTM to visit  under the different query percentiles. 
%At most  66 clusters are  selected  by the LSTM model for all queries.
%We further propose to skip unnecessary clusters. 
\begin{table}[h]
% \vspace*{-1mm}
	\centering
		\resizebox{0.78\columnwidth}{!}{ 
%		\begin{small}
		\begin{tabular}{r |r  r r r r}
			\hline\hline
			  Query percentile & 10\% & 50\% & 75\% & 90\% & 95\% \\
            \hline
%            \#clusters selected by  LSTM & 1 & 4 & 14 & 40 & 66\\
            %Relevant doc coverage & 1 & 2 & 7 & 29 & 69\\
             Top 10 dense result coverage & 1 & 6 & 25 & 92 & 175\\
                \hline\hline
		\end{tabular}
%		\end{small}
	}
	\caption{ Distribution of  top 10 dense results in sorted clusters 
% \% of Good Documents Among Clusters Sorted by Query-Centroid Distance
}
% \vspace*{-5mm}
	\label{tab:dist}
\end{table}
}


%provides an explanation.  evidence on the effectivness of the above LSTM model.
%After searching an MS MARCO passage dataset using queries from the MAMARCO dev set, 
%under the different query percentile shown in Row 2 is  the number of clusters decided by the LSTM to visit.
%Row 3 is  the number of clusters needed to 
%For a lot of queries, the top 5 or even top 10 clusters do not contain enough information, for example, around 10\% of queries need more than 92 top clusters to recover the top results from the full dense retrieval. It demonstrates the necessity of doing cluster selection and skipping.  
%On the other hand, there is a reasonable distribution resemblance between  Row 2 and  Row 3, which shows the LSTM model provides a reasonable guidance on where relevance results are.
%%While it does not exactly follow the distribution of top 10 results of sparse retrieval, the feature 
%From  Table~\ref{tab:dist}, we observe that
%the distribution of top 10 results from a sparse are contained is not necessarily concentrated in the top  clusters.
%With the above design consideration,  we propose to use the following strategy to 
%sort the candidate clusters based their feature vectors from Group  (3).


Our method   for the preliminary selection at this stage is to rely on
the degree of overlap between dense clusters and the top sparse retrieval results. 
Specifically, we divide $k$ top sparse retrieval results into $v$ top sparse result bins denoted $B_1, \cdots, B_v$,  
as depicted in Figure~\ref{fig:LSTMfeaturegroup}(b).
We  assign each embedding cluster $C_i$ with a priority vector $(P(C_i, B_1), \cdots, P(C_i, B_v))$ where
\[
P(C_i, B_j)=  |C_i  \cap  B_j|.
\]
Namely, $P(C_i, B_j)$ is the number of documents in top sparse bin $B_j$ included in cluster $C_i$.
A larger $P(C_i, B_j)$ value indicates a higher priority for $C_i$ with respect to sparse result position bin $B_j$.
In our evaluation with  retrieval depth $k = 1000$ for the MS MARCO and BEIR datasets,
we use $v=6$ result bins, divided into the top-10 results, top 11-25, top 26-50, top 51-100, top 101-200, top 201-500, and top 501 to $k$ documents.
The main reason to divide sparse results into bins is to reduce the time complexity of LSTM for cluster selection with 
a shorter sequence. The reason to have a non-uniform bin size is that the importance of rank positions derived by sparse 
retrieval is nonlinear. For example, the top 1 to 50 results are much more important than the results 
ranked from 50 to 1,000, requiring finer grained partitioning.

%top $k$ sparse results are divided into $v$ result bins where $v=6$, and these bins are top 10, top 11 to 25,  and so on.
%top 26-50, top 51-100, top 101-200, top 201-top 500, and 
%top 501 to k documents.  
    %\item $\{  AvgScore (c_i  \cap  B_j)    \}^{6}_{j=1} $: 
% bin 
%top 10/25/50/100/200/500/1000 documents  in the sparse retrival results.

Then, we sort clusters based on the lexicographic ordering of cluster priority vectors $(P(C_i, B_1), \cdots, P(C_i, B_v))$.
%$(P_1, \cdots, P_v)$. A higher value for each dimension entry represents a higher priority and is prefered.
If there is a tie between two clusters, then we rank them by their centroid distance to the query.
%We first use a simple heuristic to reorder the clusters, refered as Top K heuristic. 
%We order the clusters based the six features then 
%followed by q-c-orders. 
%Then, the  top $n$ ranked candidate cluster list is used as the input sequence to the LSTM model. 
The top-$n$ ranked candidate clusters will be  the  input for the LSTM model described below.
%We will stop the LSTM computation of  this list
%after visiting $\tau$ clusters and when the predicted $f(c_i)$  values of a few consecutive clusters are all below a threshold. 
%For our evaluation in MS MARCO and BEIR datasets, $\tau=20$. 

\comments{
Section~\ref{sect:evalLSTM} studies the effectiveness of features used in Stage II, and explains our choice of features for preliminary cluster selection. 
For the choice of $n$,
our evaluation finds  that a relatively small number of candidate clusters, such as $n=32$, yields competitive results  for our
evaluations when $k=1000$.
%As a result, the LSTM computation for cluster selection can be completed within  1.8 milliseconds. 
%The number of clusters selected varies from a few to 20 on average, which yields a quick argumentation with dense cluster results.
%Features marked with Hexgos 1 and 4 are used for a boosting tree to make a decision if cluster selection should be triggered or not.

}
\subsection{Stage II: Selection with LSTM}
\label{sect:lstm}

%{\bf LSTM design.}

\begin{figure}[htbp]
    \includegraphics[scale=0.9]{dense_separse_feature_lout.drawio.pdf}
    \vspace*{-1mm}
    \caption{Illustration of CluSD and its features.}
    \label{fig:features}
     \vspace*{-3mm}
\end{figure}


\comments{
The LSTM model outputs 1 for each cluster node if this cluster should be visited to perform the corresponding dense retrieval.
The goal of this procedure  is to visit  dense clusters as few as possible while still delivering a competitive fusion performance.
The number of predicted clusters are different across queries and the overall budget is controlled by the prediction threshold.
}
%  a few clusters as possible to recover the top results from the original dense retrieval. 
%The label of each query-cluster is 1 when the cluster contains the top k results of the query in the exact full search of dense retrieval.  
%The input is the a sequence of cluster nodes in the order of the centroid-query distance. 
%The feature of each input include: statistics on query-centroid distance, centroid-to-centroid distances, distribution of sparse top results across clusters. 
%The model will predict for each query which clusters to choose. 
%The input features of our proposed LSTM model are listed below.
%These clusters are sorted by the the similarity distance of the given query with the  centroid of each cluster.

To select which dense clusters we visit, we adopt a simple LSTM model~\cite{hochreiter1997long}
which takes a sequence of clusters as input along with their features. We choose LSTM because it can 
capture cluster selection order as a sequence. Selected clusters can influence what will be selected next based on 
their semantic distance and other features. This allows CluSD to select cluster accurately to 
minimize I/O and computing cost.
The time complexity of the LSTM model is limited by $O(n)$,
where the $n$ top clusters are  given from  Stage I.
%We denote $n$ as the  input length  to our LSTM  throughout the rest of this paper.

The LSTM sequentially visits each cluster, denoted $C_1$ to $C_{n}$. 
For each cluster $C_i$, the LSTM predicts a score $f(C_i)$ such that $0\leq f(C_i) \leq 1$.
If $f(C_i) \ge \Theta$, where $\Theta$ is a set prediction threshold, then cluster  $C_i$ should be visited. 
$\Theta$ controls the tradeoff between efficiency and relevance; in practice, $\Theta$ can be tuned based on the overall latency requirement.
Section~\ref{sect:threshold} 
evaluates the impact of varying this threshold on the number of clusters selected.

%In practice, the strictness on selecting a cluster to evaluate is controlled by $\Theta$ and it can be determined based on the overall latency requirement. 

\comments{
When the dense vectors of all documents are grouped into $N$ clusters, 
we limit our cluster search scope to top $n$ clusters in terms of query and cluster centroid similarities. 
we limit $n=128$ in our evaluation out of 1000 clusters.
%Query-specific information derived from  dense clusters:
}

As depicted in Figure~\ref{fig:features}, the feature input vector for the current cluster  $C_i$ for the above LSTM computation to produce $f(C_i)$
%$f(q, c_i)$  
is composed of the following three groups of features:


\comments{
\[ sim(q,c_i),   
\{ AvgDist(sim(c_i, c_l) \mbox{ for } c_l \in A_j) \}^u_{j=1}, 
\]
\[ 
     \{  |c_i  \cap  B_j|    \}^{v}_{j=1},  
\{  AvgScore (c_i  \cap  B_j)    \}^{v}_{j=1}. 
\] 
}
%\begin{enumerate}[leftmargin=*]
%KDD style does not recognize leftmargin
\begin{itemize}[leftmargin=*]
\item \textbf{Query-cluster similarity:} $sim(q,c_i)$.
The similarity distance of this query $q$ with the centroid $c_i$ of cluster $C_i$.  
%\item $sim(q,c_i)$: The similarity distance of this query $q$ with the centroid $c_i$ of cluster $C_i$.  
%\item  $\{ sim(c_i, c_j) \}^{n-1}_{j=0}$: The distance vector between the centroid $c_i$ of cluster $C_i$ to  all other clusters.
%the top  clusters that have been visited (or skipped).  We limit this number as $K=128$.
%other top k centroids for this query (k=128)??
  

%\item  $\{ AvgDist(sim(c_i, c_l)) \mbox{ for } c_l \in A_j \}^u_{j=1}$: 

\item \textbf{Inter-cluster similarity:} $AvgDist(C_i, Aj)$ for $1 \leq j \le u$.

%\item  $AvgDist(C_i, Aj)$ for $1 \leq j \le u$.
As depicted in   Figure~\ref{fig:LSTMfeaturegroup}(a),
given the $n$ sorted clusters derived from Stage I, we uniformly partition  these $n$ consecutive  clusters into $u$ consecutive cluster bins:
$\{ A_1, A_2, \cdots, A_u\}$. Then we define
\[
AvgDist(C_i, Aj) = \frac{1}{|A_j|} \sum_{ c_l \in A_j}
 sim(c_i, c_l) 
\]
where  $c_l$ is the centroid representing cluster $C_l$ in bin $A_j$.
The above formula computes the mean distance between centroid $c_i$ and the centroid of each cluster within  Bin $A_j$.


%These six bins  are formed by partitioning all clusters into consecutive position bins.
%For example, $A_1$ contains clusters from Postions  1 to 5, Positions 6-10, 
%$A_2$  contains clusters from Postions  6 to 10, and so on.   Bin $A_6$ contains the rest of uncovered clusters.  
%After all the $N$ centroids are ordered based on a criterion discussed shortly, we partition the sequence of sorted clusters into $u$ consecutive 
%cluster bins.

The purpose of this feature group is to capture the distances of a cluster to previously examined clusters and unexamined clusters 
following the LSTM flow. 
When the mean distance  between cluster $c_i$  and clusters in a previously-examined  bin is close, if  
many clusters in that bin have been selected, cluster 
$c_i$ may have a good  chance to  be selected.
In our evaluation with MS MARCO and BEIR datasets, we found that $u=6$ is appropriate.
% these 6 cluster bins respectively contain clusters in Positions  1-5, Positions 6-10, Positions 11-20, Positions 21-50, Positions 51-100, and the rest of N clusters. 
%Since the clusters are processed from a lower position to a higher position one by  one,
%these features represent the distance to the groups 
As discussed earlier in Section~\ref{sect:online}, to reduce the extra space cost, 
we only maintain top-$m$ cluster neighbors of each cluster where $m$ is not large  (128 in our evaluation).
    
%\item $ \{  |c_i  \cap  B_j|    \}^{v}_{j=1} $ and $\{  AvgScore (c_i  \cap  B_j)    \}^{v}_{j=1} $: 

\item \textbf{Cluster overlap:} $P(C_i, B_j)$ and $Q(C_i,   B_j)$     for $1 \leq j \le v$.
%\item $P(C_i, B_j)$ and $Q(C_i,   B_j)$     for $1 \leq j \le v$.

As shown in   Figure~\ref{fig:LSTMfeaturegroup}(b),
this group of features captures the position-weighted and score-weighted overlap degree of this embedding cluster $C_i$ with the top sparse results.
Stage I in Section~\ref{sect:stage1} divided the top-$k$ sparse retrieval results into $v$ position bins
$B_1, \cdots B_v$ and defined   $P (C_i, B_j)$ as  the count-based overlap measure.
Now, we define a score-weighted overlap degree $Q (C_i,   B_j)$     
as the average sparse rank score of documents that  are in both $C_i$ and sparse position bin $B_j$.  
Namely,
\[
Q (C_i,   B_j) = \frac{ \sum_{d \in C_i \cap B_j} SparseRankScore(d)} { |C_i  \cap  B_j|}.    
\]


%With a high score from this feature, a cluster that contains many top sparse results may be selected.
Clusters with high $Q$ scores for the top bins contain many top sparse results and may be selected.

%In our evaluation with  retrieval depth $k = 1000$ for MS MARCO and BEIR datasets,
%top $k$ sparse results are divided into $v$ bins where $v=6$, and 
%these bints are top 10, top 11 to 25, top 26-50, top 51-100, top 101-200, top 201-top 500, and 
%top 501 to k documents.  

    %\item $\{  AvgScore (c_i  \cap  B_j)    \}^{6}_{j=1} $: 

% bin 
%top 10/25/50/100/200/500/1000 documents  in the sparse retrival results.

\end{itemize}

In total, we extract $1+u+2v$ features for each top-$n$ cluster.



\begin{figure}[htbp]
    \includegraphics[scale=0.85]{LSTM\_feature.drawio.pdf}
    \vspace*{-2mm}
    \caption{Cluster distance   and result  overlap features } 
\vspace*{-3mm}
    \label{fig:LSTMfeaturegroup}
\end{figure}

%Section~\ref{sect:evaluation} provides more details on the effectiveness 
 

\comments{
\subsection{Query filtering}
%When computing the embedding of each query token or the whole  original query, we use 
%the denser retriever's encoder. 


We also exploit the possibility to skip dense retrieval completely.
Modifying the above LSTM-based decision mechanism does not yield a satisfactory result.
We sort to add a classifier with  boosted decision trees with supervised learning
to make an earlier  determination before triggering the LSTM computation.
}
\comments{

a query needs an argumentation from dense retrieval 
%A challenge is to identify features and infer based on such features with supervised learning.
Given that sparse retrieval is conducted first,
our idea is to predict the quality of sparse retrieval and its relative strength  compared to unexecuted
dense retrieval based on quality of query token expansion by the sparse model,
the statistical behavior of  sparse retrieval results, and
the relationship between dense document embedding summary and sparse retrieval scoring structure.

}


\comments{
\begin{table}[ht]       
    \centering          
%    \resizebox{1.05\columnwidth}{!}{

\begin{small}                        

    \begin{tabular}{l |l}
        \hline
    Query    & "how long nyquil kicks in"\\
    \hline
 Query Expanded&["in", 36],  ["time", 74], ["years", 71], ["long", 97], \\
 & ["total", 60],\textcolor{red}{["move", 23]}, ["effect", 22], \textcolor{red}{["weapon", 21]}, \\
 & \textcolor{red}{["jump", 24]}, ["kick", 100], ["ny", 111], ["timing", 34], \\
 & ["kicks", 76], ["\#\#quil", 139]\\
    \hline  
Relevance Doc &["\#\#quil", 410.1], ["ny", 301.0], ["long", 216.7], \\
& ["time", 134.7], ["years", 131.5], ["total", 87.4],\\
& ["effect", 34.4], ["timing", 17.4]\\
\hline
Top 5 Doc & ["\#\#quil", 392.6], ["ny", 295.7], ["kick", 236.1], \\
& ["long", 198.3], ["time", 141.2], ["years", 116.9], \\ 
& ["kicks", 101.8], ["total", 86.3],\\
& ["in", 35.3], ["effect", 24.1], ["timing", 23.6],\\
& \textcolor{red}{["jump", 10.0], ["move", 6.0]}\\
        \hline
    \end{tabular}
\end{small}                        
%}     

\caption{An example of weak query expansion in SPLADE} 
\label{tab:queryencoder}
\end{table} 
}

\comments{
\begin{table*}[ht]       
    \centering          
%    \resizebox{1.05\columnwidth}{!}{

\begin{small}                        

    \begin{tabular}{l  l l}
        \hline\hline
    Query   &  \multicolumn{2}{l}{ "why do we push others away"}\\
    \cline{2-3}
&  \multicolumn{2}{l}{('push', 105), ('away', 104), ('because', 97), ('others', 94), ('people', 44), ('why', 44), ('purpose', 43), ('cause', 42), (',', 40), ('we', 38),} \\
&\multicolumn{2}{l}{ ('other', 38), ('effect', 33), ('them', 29), \boldred{('responsibility', 28),} ('help', 20), \boldred{('move', 19), ('severe', 17),}  ('step', 17), ('do', 16),...}\\
%& & ('things', 15)， ('fear', 15), ('method', 10), ('to', 6), ('language', 5), ('anger', 5), ('when', 2), ('feeling', 2), ('\#\#ness', 1), ('dangerous', 1)]\\
    \hline  \hline
   Doc Relevant? & \ rank & Text and Expanded Tokens \\
\hline
\comments{
Yes & 17 & From a psychological standpoint, pushing away the people you love the most is a very basic and common, defense mechanism.\\
&& As the relationship develops, people become inundated with their own fears and insecurities that they will not be accepted\\
&& and therefore hurt by their loved one.\\
\cline{3-3}
& & [('push', 198), ('away', 196), ('fear', 127), ('people', 104), ('effect', 81), ('because', 70), ('severe', 67), (',', 61), ('method', 61),
\\
& &  ('when', 59), ('anger', 58), ('dangerous', 55), ('feeling', 53), ('purpose', 53), ('responsibility', 53), ('move', 44), ('cause', 43),... \\
%& & ('them', 37), ('things', 31), ('\#\#ness', 27), ('step', 23), ('why', 13), ('help', 9), ('to', 3), ('do', 1), ('language', 0)]\\
\specialrule{.1em}{.05em}{.05em} 
}
No & 10 & Different types of push factors can be seen further below. A push factor is a flaw or distress that drives a person away from \\
&&  a certain place. A pull factor is something concerning the country to which a person migrates. It is generally a benefit that  \\
&&attracts people to  a certain place. Push and pull factors are usually considered as north and south poles on a magnet.\\
\cline{3-3}
&& [('push', 283), ('away', 162), \boldred{('move', 80),} \boldred{('severe', 74)}, ('people', 70), ('because', 68), ('effect', 58), ('cause', 44), ('purpose', 43),\\
& & \boldred{('responsibility', 41),} (',', 36), ('method', 35), ('\#\#ness', 33), ('step', 23), ('them', 22), ('to', 18), ('when', 13), ...\\ 
%& &  ('things', 11), ('anger', 9), ('dangerous', 8), ('fear', 3), ('do', 0)]\\
\specialrule{.1em}{.05em}{.05em} 
No & 8& Most of the universe is rushing away from us. It\textbackslash{}'s not that we\textbackslash{}'re particularly repellent; it\textbackslash{}'s just that the universe is\\
&&  expanding, pushing most other galaxies away. Light from distant galaxies travels toward us through this \\
&& expanding space, which stretches their light to longer, or redder, wavelengths.\\
\cline{3-3}
&& [('away', 184), ('push', 158), ('other', 111), \boldred{('move', 103)}, ('we', 101), ('effect', 83), (',', 73), ('because', 66), ('method', 53),\\
&&  ('others', 39), ('cause', 39), ('severe', 39), ('them', 36), ('do', 29), ('things', 29), ('dangerous', 29), ('feeling', 28), ... \\
% & & ('when', 27), ('help', 19), ('purpose', 13), ('to', 4), ('why', 2)]\\
         \hline\hline
    \end{tabular}
\end{small}                        
%}     

\caption{An example of weak SPLADE query expansion that boosts  irrelevant documents  } 
\label{tab:queryencoder}
\end{table*} 

Our consideration 
%is that the necessity of invoking a dense retrieval model after running a sparse model depends on 
%\begin{enumerate}
%the relative strength of results scored by this sparse retriever. If a
    is that  if a chosen
sparse retriever has  well-performed, the benefit of addition of dense scoring  is limited. 
Notice that a learned neural sparse retriever expands the original query with a transformer-based encoder
We found that the quality of query encoding with expansion in SPLADE impacts the quality of sparse retrieval. 
%and we form features using both the original query  and the expanded query.
When  there is a low similarity value  between the original query and the tokens of 
its expanded  query, the confidence for  strong sparse retrieval can be low.
Table~\ref{tab:queryencoder} gives such an example and lists an original query and its expanded query tokens
sorted by token weights.  Expanded query words  in red color
not highly relevant to the original query and they are weighted high in two irrelevant documents, which boosts their ranking.  
Thus    excessive presence of un-similar  query tokens  after expansion  can misrank irrelevant documents. 
Another consideration is that the alignment of sparse retrieval ranking  with the 
query-cluster based similarity can shed light  on the necessity of  dense retrieval.
When top sparse retrieval results are concentrated in a few top  ordered dense clusters, dense retrieval may bear
a resemblance  in  ranking.


With the above consideration  in mind, we use the  following categories of features
to train a boosted decision tree model.

}
% with these featuers an input by using the xgboost package. 
\comments{
To evaluate the performance of the sparse system, we design some features to describe the quality of sparse encoder. 
For example, the length of expanded query, distribution of token impact scores and their corresponding matching scores with top k documents.

To evaluate the discrepancy between the performance of sparse and dense system. We encode the original query with the dense retrieval encode and each expanded token and generate distributional features around the similarity between them. 


%We take a supervised approach to the construction of a query filter that classifies  a query after sparse retrieval 
%needs an argumentation from  dense retrieval or not. We consider the following two categories of the feautres.
}
\comments{
\begin{itemize}[leftmargin=*]
\item Quality of query expansion by the sparse retriever model.
    For example, the query-level matching score, define as the similarity  between the CLS embeddings of the original query and the expanded query.
    Another one is the token-based matching histogram vector between the expanded query and the original query. 
For each query token in the expanded query, we evaluate the matching score in terms of similarity
 between its token embedding and  the original query embedding. 
We map  these values into five bins with  ranges <0.5, 0.5-0.6, 0.6-0.7, 0.7-0.8, >0.8.
Then derive a matching histgram count  vector for each bin.
}

\comments{
{\bf WILL DELETE THIS LIST.}
\begin{enumerate}
    \item The length of the original query and the expanded query in terms of  the  number of words or tokens, respectively. 
    \item The token-based matching  vector between the expanded query and the original query. 
For each query token in the expanded query, we evaluate the matching score in terms of similarity
 between its token embedding and  the original query embedding. 
We map  these values into five bins with  ranges <0.5, 0.5-0.6, 0.6-0.7, 0.7-0.8, >0.8.
Then derive a matching count vector based on this bin mapping???
    \item The query-level matching score, define as the similarity  between the CLS embeddings of the original query and the expanded query.
    \item The sum of matching scores within each of above token similarity bin, divided by
the  query-level matching score. 
%The token groups are the tokens with similarities in each bin.
    \item The sum of matching scores of tokens not in NLTK English corpus, divided by  the query-level matching score. 
    \item The number of overlapping tokens between expanded and original query / number of all unique queries in both expanded and original query.
    \item number of  tokens only in expanded query / number of all unique queries in both expanded and original query.
    \item overall/mean/max of token weight of overlapping tokens between expanded and original query in the expanded query.
    \item max/min/mean of token weights of expanded query tokens.
\end{enumerate}

}
%\item
\comments{
Ranking characteristics of documents scored by sparse retrieval.
We compute  the mean sparse retrieval score of top 10-20/20-30/30-40/40-50/50-100/100-400/400-700/700-1000 documents.

%Sparse  retrieval score distribution:
\begin{enumerate}
    \item Sparse retrieval scores of top 10 results
    \item The mean sparse retrieval score of top 10-20/20-30/30-40/40-50/50-100/100-400/400-700/700-1000 documents.
\end{enumerate}
%Sparse and Dense relational features:
\item Overlapping degree of sparse retrieval with dense clusters:
\begin{enumerate}
    \item The number of dense clusters containing top 5/10/20/50/100/1000 results from the sparse system
\end{enumerate}
}

%\end{itemize}


%\subsection{Partial Document Evaluation}
{\bf Training of LSTM.} 
We assume that the training data  contains
a set of queries and relevance-labeled documents,  that allows the computation of a ranking metric such as MRR or NDCG.
For example, from MS MARCO training set we randomly sample 5000 training instances, where each training instance contains a query and  one or more  relevant documents. 
%Then we run a sparse retriever this instance, and seperately run a fusion with a dense retriever. If the result of sparse retriever results merged with dense results  exceeds the standalone sparse retrival,  we label consider training instance as an positive example for dense retrieval, otherwise consider this as a negative example. The converted training isntances are used for training In this way, we convert a set of training instances for ranking as a set of training instances for fusion.
To train the LSTM for cluster selection, 
for each training instance, we mark the positive and negative examples for  top cluster selection.
If a cluster contains one of top-10 dense retrieval results, we mark this cluster as positive otherwise negative.
This approximately indicates that such an embedding cluster should be visited for a fusion.

 
\comments{
We convert We define the labels as 
\begin{equation}
       y(q)= 
\begin{cases}
    1,& \text{if } U(s(q), d(q)) > U(s(q))\\
    0,              & \text{otherwise,}
\end{cases}
\end{equation}
where $U(.)$ is a evaluation metric we choose, for example, NDCG@10 or MRR. $s(q)$ is the scoring of a sparse system of query $q$ and $d(q)$ represents the scoring of a dense system.
}

\comments{
\subsection{How to combine two ranked lists}
There are two commonly used methods to combine the sparse and dense ranked lists:
\begin{enumerate}
    \item linear combination
    \item reciprocal rank fusion
\end{enumerate}
For linear combination, the final ranking score of a document is the weighted sum of the ranking score of two systems respectively. The weight on each system can be determined through grid search on a left-out training set or just use 1:1 combination. In this case, rescaling of the two ranked lists is necessary as it largely affects the impact of a ranked list on the merged ranked list. 

On the other hand, reciprocal rank fusion alleviates the scoring distribution difference by only considering the ranking positions when merging. 
  Another consideration is the missing values. The two ranked lists usually do not fully overlap. Some documents only exist in one ranked list. Thus 
the treatment on these documents affects model performance. We consider a few options
\begin{enumerate}
    \item Remove the documents when they only exist in one ranked list
    \item  Take the document and compute the score for only one ranked list
    \item Impute the missing document with rank K+1 or score as 0.95 * min(score) in the ranked list.
\end{enumerate}

}




==> cikmproblem.tex <==
\vspace*{-1em}
\section{Background and Related Work }
%\section{Problem Definition}
\label{sect:background}

\comments{
\begin{table}[h]
	\centering
		%\resizebox{1.02\columnwidth}{!}{ 
		\begin{small}
		\begin{tabular}{l l}
			\hline
			Symbol & Def. \\
                \hline
                %$\mathcal{D}$ & A set of documents in a dataset\\
                %$N$ & Total number of documents in a dataset \\
                $Q$ & A query \\
                $d_i$ & A document \\
                $\mathcal{D}^{+}$, $\mathcal{D}^{-}$ & Positive/negative document subsets corresponding to $Q$  \\
                $|.|$ &  The size of a set\\
		$\Theta$& Parameters of a scoring model\\
		$S(Q,d_i, \Theta)$ & The rank score of a document for a query using a model\\
%			& based on a model with parameters $\Theta$. \\
                $p_i$ & Teacher's top one probability of document $d_i$,\\
			& standing for  $P(d_i|Q, \mathcal{D}^+, \mathcal{D}^-, \Theta$) \\
                $q_i$ & Student's top one probability of document $d_i$\\
                $\pi(.)$ & The rank position of a document for a query\\
                $\beta_i$ & Exponent weight bias for negative  document $d_i$\\
                $\gamma, \alpha$ & CKL hyper-parameters\\
                \hline
		\end{tabular}
		\end{small}
	%}
	\caption{Table of Symbols}

	\label{tab:data}
\end{table}
}

\textbf{Problem definition.}
Given query $q$ for searching a collection of $D$ text documents:   $ \{d_i\}^D_{i=1}$, 
retrieval  obtains the top $k$ relevant documents from this collection based on
the similarity between query $q$ and document  $d_i$ using  their
representation vectors.

With a lexical representation, each  representation vector of a document or a query is sparse.
Sparse retrieval uses  the dot product of their lexical representation vectors as the similarity function
and implements its search efficiently using an inverted index: 
%\begin{equation}
%\label{eq:sparseretrieval}
$L(q) \cdot  L(d_i)$
%\end{equation}
%L(q,d_i ) = 
where $L(.)$ is a lexical representation   which is a vector of weighted term tokens for a document or a query.
For BM25 based lexical representation~\cite{Robertson2009BM25}, 
$L(.)$ treats each document or a query as a bag of terms.
% Q: do we want to keep referring to everything as bag of terms?
%and term weights  are scaled based on   frequency of terms within a bag and  across all bags involved.
Term weights are scaled based on the frequency of terms within a document and across all documents in the collection.
For a learned sparse representation~\cite{Dai2020deepct, Mallia2021deepimpact, Lin2021unicoil,2021NAACL-Gao-COIL}, 
a document or a query is encoded using  a trained neural ranking model, which
%produces a bag which may contain original  and  expanded terms.
produces modified representations of document or query containing both original and expanded terms.
The encoding functions for a query and document can be different. Without the loss of generality, we assume they are the same in this paper.

With a single-vector dense  representation, each  representation vector of a document or a query is a dense vector. 
Dense retrieval computes the following rank score: 
%\begin{equation}
%\label{eq:denseretrieval}
$R(q) \cdot  R(d_i)$
%\end{equation}
%D(q,d_i) 
where $R(.)$ is a dense representation vector  of a fixed size~\cite{Karpukhin2020DPR}.


  %revises the SparTerm model~\cite{Bai2020SparTerm} to predict the weight 
%The weights of these terms evaluated in this paper use the SPLADE model as discussed below while other options are possible.
%(e.g., a bag of words or a neural encoder). 
%The implementation of such a dot product for a sparse retriever uses the inverted index data structure.
\comments{
%{\bf Learned term weights with SPLADE}.
For each document, the SPLADE term weighting revises the SparTerm model~\cite{Bai2020SparTerm} to predict the weight 
score $w_j$ of $j$-th token term in BERT WordPiece vocabulary.
\begin{equation}
\label{eq:splade}
w_j = \sum_{i \in d}  log (1 + ReLU ( H(h_i)^T E_j + b_j)) 
\end{equation}
where document $d$ consists of a sequence of BERT last layer's embeddings $(h_1, h_2, $
$\cdots, h_n)$.
$E_j$ is the BERT input embedding of the $j$-th token and $b_j$ is a token level bias.
$H(.)$ is a linear layer with activation and layer normalization. 
% (In SPLADE GeLU activation is used). 

{\bf Combining the results of a dense retriever and a sparse retriever.}
}
Following the work of~\cite{kuzi2020leveraging, 2022LinearInterpolationJimLin, Gao2020ComplementingLR}, 
linear interpolation is used  to  ensemble  dense and sparse retrieval scores. 
%Let $S$ be the set of top results obtained by a sparse retriever, and $D$ be
%be the set of results obtained by dense retrieval. 
%For any document $d_i \in S \cup D$, its  
The fused rank score for document $d_i$ in responding  query $q$ is:
\begin{equation}
\label{eq:fusion}
\alpha L(q) \cdot  L(d_i) +
(1-\alpha) R(q) \cdot  R(d_i) 
\end{equation}
where $\alpha$ is a coefficient in a range between 0 and 1.

\comments{
Notice that   the two ranked lists $S$ and $D$ are usually not fully overlapped and  some documents only exist in one list. While 
different  treatments on these documents affect fusion performance,
we take an option to  impute the score of such a document score   using $\beta * score (top \  k+1) $  in the missed  ranklist where $\beta$
is a scaling factor.
%While there are options to We consider a few options
For example,  we  impute the lexical scores of documents expanded by dense retrieval
as the top-$(k+1)$ lexical  score scaled by a factor. We use $\beta=0.95$  in our evaluation.
 
%\item Remove the documents when they only exist in one ranked list
%    \item  Take the document and compute the score for only one ranked list
}


Our goal is to maintain a relevance competitive to full dense retrieval, while minimizing the time and memory overhead of cluster-based dense retrieval,
guided by sparse retrieval results.
%to minimize the scope of dense clusters to visit.
% Parker: below is awkard, and a bit of a run-on sentence. Above I reworked it, but it's still not great
%Our optimization goal is to minimize the scope of cluster-based dense retrieval and extra memory space overhead by leveraging sparse retrieval 
%while maintaining a relevance competitive to full dense retrieval.  
%In this way, limited dense retrieval that augments sparse retrieval is fast with minimum space consumption  on a CPU server. 
\comments{
The ensembling method used in our evaluation is 
%The final ranking of the top $K$ documents is 
the reciprocal rank fusion (RRF) following Cormack et al.~\cite{Cormack2009RRF}, considering ranking positions of each candidate 
generated by a retriever and by a re-ranker. 
We use RRF
% above reciprocal rank fusion 
instead of linear interpolation as it has a similar performance with a simplified combination of two scoring models. 
%We choose RRF because it is easily applicable to multiple ranked lists ignoring the score distribution differences. 
\begin{equation}
     %RRF(Q,d) =  \sum_{r \in {rt, rr,}} \frac{1}{k_r + r(d)},
     RRF(Q,d) =  
\frac{1}{c_1 + \pi_1(d)} + 
\frac{1}{c_{2} + \pi_2(d)},
     \label{eq:score}
\end{equation}
where $c_{1}$ and $c_{2}$ are fixed smoothing constants. $\pi_2(d)$ is the rank position based  a re-ranker formula
while $\pi_1(d)$ is the rank position based on a retriever.
}



==> clustabs.tex <==
%Dense and sparse retrievers are two main categories of the
%first-stage search techniques for text  documents, and both of them have benefited 
%from pretrained language models to provide effective semantic text matching between a query and a document.
Previous work has shown that  ranking of documents from dense and sparse retrievers could be combined for higher relevance effectiveness. 
The downside is that dense retrieval is time consuming on a CPU-only server platform.
This paper considers the optimization of dense and sparse retrieval fusion and 
 proposes a cluster-based selective dense retrieval scheme called CluSD which only requires triggering of dense retrieval 
computation for a relatively small subset of documents after  fast sparse retrieval. 
CluSD takes an advantage of clustering under an advanced  dense retrieval model and
detects clusters of documents that can boost sparse retrieval with  embedding  computation.
This paper provides a detailed evaluation with MS MARCO and BEIR  datasets  
on the usefulness of CluSD in improving the effectiveness of sparse retrieval with limited dense  retrieval
traversal.  Our empirical findings suggest that CluSD can outperform other baselines on a single CPU server 
without GPUs, and achieve a strong tradeoff of effectiveness and efficiency compared to an exhaustive dense retrieval search.



==> clustconcl.tex <==
%\section{Limitations and Future Work}
\section{Concluding Remarks}

The contribution of this work is a cluster-based dense retrieval selection scheme  
to augment sparse retrieval with minimal space overhead and a small amount of extra latency  time.
CluSD optimizes an LSTM based model with cluster prioritization and pruning
to effectively identify  a small number of clusters that can supplement and boost  sparse retrieval. 
With this lightweight low-cost design,  
CluSD can deliver a strong in-domain and out-of-domain relevance  efficiently when searching  MS MARCO and BEIR datasets
on a CPU only server. %even though the sparse retriever used has its relevance tradeoff under a time efficiency constraint.
For example, CluSD delivers 0.423 MRR@10  for searching 8.8M MS MARCO passages 
with 11.4ms  latency and  1.13GB space mainly for compressed dense embeddings, to augment sparse retrieval under
a fraction of its  cost. The same  CluSD version  reaches  0.514 average NDCG@10 for BEIR with compression.

Compared to re-ranking approach, CluSD outperforms for recall in MS MARCO while having a marginal improvement for MRR@10 numbers 
while  CluSD’s average NDCG number is 7.2\% and 4\% higher than re-ranking with RetroMAE and SimLM, respectively for BEIR.
%It is attractive to run such an algorithm on a first-stage retrieval low-cost machine
%to host  as many documents as possible and 
%that can  significantly reduce the overall infrastructure cost when scaling  data size and  search traffic. 

\comments{
 While IVF does not add extra space cost,
the relevance  of IVF top cluster search under the time budget performs  worse than others.
Simple re-ranking ``D-rerank'' achieves good MRR@10 but under-performs on recall. 
When the recall of a sparse retriever is relatively low, it cannot boost further as seen in the case of $m=64$.
}

Compared to a  graph navigation based approach, the main advantage of CluSD is its capability in delivering 
a similar or higher relevance under the same time budget with negligible extra space overhead. 
HNSW and LADR perform comparably, at the cost of extra online memory overhead  and extra complexity to compute offline in advance.
HNSW requires extra 9.2GB and LADR requires extra 4.3GB to store graph data in memory.
When we  try to reduce their graph size by decreasing  the number of neighbors for HNSW and LADR, their  MRR@10 and/or  recall@1000 numbers drop visibly. For example,
using the default 32 neighbors for the HNSW graph results in 2.4GB graph space, however  MRR@10 drops from 0.407 to 0.4 under the 25ms time budget.



\comments{
Our evaluation uses OPQ in FAISS to compress embeddings. 
Switching to a different quantization affects the compression ratio and  the relevance outcome.  
However, we expect that our findings remain similar because  the recent  quantization 
methods~\cite{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ}
also have  a significant relevance drop pattern when the compression ratio increases.
%A limitation of the current  CluSD work is that the training of the LSTM model has a dependence on the sparse retrieval model used. 
While  CluSD can  boost the relevance of a weaker sparse retriever model such as BM25, the augmented relevance still has not reached a level
comparable  to the one where CluSD is coupled with a stronger sparse retriever. There is room for improvement in future work.
}
%the dependency on a training dataset. Unlike rule-based or unsupervised pipelines, our pipeline requires labeled data on at least one search task. However, the number of queries with labels is not large and a trained model is robust on never-seen corpus and tasks. 
%
%Another limitation is the dependency on the sparse retrieval model performance. CluSD benefit from a good sparse retrieval top results. When using a BM25 based retrieval, the quality of the clusters selected degrades slightly. 


==> clustdesign.tex <==

\comments{
Sparse retrieval with a learned representation  is much slower than BM25
        Guided sparse retrieval can speedup, but there is a trade in  effectiveness
        Agumenting sparse retrieval with dense retrieval through fusion can make up the loss
        Selective dense  retrieval can make up the loss argument sparse retiieval more effective with limited extra computing cost.

Points to market: Option 2

                New dense retrieval algorithms have been developed every year that beat new performance records.
                New fast  sparse retrieval algorithms are developed.
                Fusion of  sparse retrieval and dense retrieval is helpful, but slow on a CPU server, dominating by dense computation.
                There is a clear redudance of computation as both retrievers scan the same dataset with different representation
                        for push for the same top documents.
                How to avoid redudant computation?
                        1) Select dense retrieval. We donot need to scan all dense documents. We can take advanrage of
                clusters of dense documents
                        and only  need to visit top clusters which are similar to a query.
                        2) The use of dense retrieval reduces the relevance reqirement of sparse retrieval. We can use a fast sparse
retrieval BM25-guided sparse retrieval or effient SPLADE version, which quickly retrieves top results. Selective dense retrieval
                can augment  a weaker but faster sparse retriever by only adding limited  extra computing cost
to  improve the recall and relevance metric.

                Challenges:
                        1) How to accomplish  selective clusetrs.
                        Which clusters  can make most contributions
                        2) What queries definitely need dense retrieval boosting?

}
%\section{Design Considerations}
\label{sect:design}

\comments{
The availability of a dense retriever model, possibly  trained separately by a different language model,
offers opportunities to re-confirm and adjust the ranking of top quality documents in  the initial
candidate pool and improve the  recall by introducing more diversified
candidates.  On the other hand, there is a clear redundancy of computation as both retrievers visit the same dataset 
with different representation, possibly  pursing the  same subset of top documents.
}
 
%{\bf Yingrui, please add a table or figure which shows the distribution of training
%queries if possible, otherise the Dev set of MS MARCOS,  that has the various level of MRR increase.
%I remeber you show us some data you collected during summer or spring.} 
%Table~\ref{tab:fusionanalysis} shows 



%We found that among 33\% of queries in the MSMARCO training set, there is no increase in terms of the MRR@10 when dense retrieval results are added to sparse retrieval results. Namely there are many queries that do not actually benefit from the use of dense retrieval after sparse retrieval.
% two retrievers, and explicitly skipping some of fusion can avoid the unnecessary computing cost.
%Motivated by the above data, 

%Our design considerations are:

%of selective dense retrieval  
%has  the following considerations.
%\begin{itemize} [leftmargin=*]
\comments{
\item  {\bf Partial dense retrieval after  full sparse retrieval.}
The experience with the SPLADE model ~\cite{Formal2021SPLADE, Formal2021SPLADEV2} showed that
learned sparse representations from  BERT can be very effective.
For example, without optimization in language model pretraining, SPLADE's MRR performance is on par to
the dense retriever by RocketQA~\ref{Ren2021RocketQAv2}. 
Thus there is an opportunity to skip some of scoring computation in dense or sparse retrieval.
Since it is not easy to recognize and separate part of an inverted index  that contains high scoring documents,
our design choice is  to run a sparse retriever completely first and steer partial dense  retrieval. 

%and also there are several techniques developed recently to accelerate learned sparse retrieval,
}

%\item {Inter-cluster vs. inter-document similarity.}
{\bf Cluster-based  dense retrieval.}
\comments{
After the  fusion option is determined for a  query,
there is an option to follow LADR~\cite{2023SIGIR-LADR} and select documents that are similar to
the top sparse retrieval results  using a similarity graph.
These similar documents form candidates  for partial dense retrieval and  rest of un-selected
documents in a dataset can be skipped.  
Maintaining a large inter-document similarity graph online is quite expensive from
offline  data collection, online storage space, and   inference time.
}
There are two ways  to select documents for dense retrieval.
One way is to take a graph navigation approach such as HNSW~\cite{2020TPAMI-HNSW}, GAR~\cite{2022CIKM-MacAvaneyGraphReRank} and LADR~\cite{2023SIGIR-LADR}, 
exploiting  document-to-document similarity links during inference time.
Another way is to follow a clustering  approach to group  documents based on their embedding similarity at offline 
time~\cite{johnson2019billion} and select a small set of  clusters.
%~\cite{2020TPAMI-HNSW,2022CIKM-MacAvaneyGraphReRank, 2023SIGIR-LADR}.
% is viewed as  a modern instantiation
%of the clustering hypothesis to revisit these ideas in a new context.  
We opt to take  the clustering based approach with two reasons.
1) Maintaing a large document-to-document similarity graph with a qudradical complexity is not scalable for  a large  data collection size. 
%As illustrated in  Table~\ref{tab:costbudget}, compression with embedding  quantization is necessary to meet the space constraint.
%due to the memory usage of stroing  embedding vectors. 
%For 8.8M MS MACRO passages, that takes  about 27GB space.
%Fortunately the quantization techniques can significantly compress this space into 1-2GB or even 0.5GB depending on the configuration. 
%Our feature design does not opt for  inter-document similarity since it is space-consuming, but  plans to exploit cluster-based summary information, 
%which  only adds  insignificant  space overhead.  
%\end{itemize}
%, and set a limit on the number of dense clusters used.
2) Embedding vectors of a large dataset with a high dimension per vector may not fit into the memory.
Cluster-based on selection exploits the block-level disk I/O for lower access overhead and higher bandwidth. 
In comparison, random access of selected documents in a graph based approach can suffer higher I/O overhead. 
\comments{
We intend to exploit coarse grain cluster-level similarity to reduce the complexity in selective dense retrieval with two reasons.
%The challenge is to how to select clusters  which can make most contributions.
%We opt to take a cluster-level skipping approach with two reasons.
1) Documents can be clustered in advance during offline processing 
%Documents within a cluster similar to a query can provide a large variety of strong candidates to supplement sparse retrieval results.  
2) Cluster-level computation allows  aggregation of  similarity computation for query-document dot products as a fast matrix operation 
to fully  utilize on-chip CPU caches. 
%In comparsion, there is a less chance for online inference to fully benefit from  CPU cache based on an irregular  graph structure.
%During offline processing, it is computationally expensive to drive document-level similarity for all pairs for documents in a large datset.
A research problem  is how to adaptively identify a subset of clusters  which yield sufficient relevance benefits.
% benefitial fusion if  sparse retrieval scoring may be sufficient. In addition to the influence of sparse retrieval results,
% a dynamically-visited dense cluster may provide sufficient high quality documents, reducing the necessarity of visiting
%the remaining dense clusters.   
%Thus we will develop a dynamic feature-driven decision scheme based the results of sparse retrieval.
%and incremtentally navigated  dense document clusters  as input. 
}
\comments{
Another consideration is that there are various relevance and efficiency tradeoff in selecting  a sparse retrieval 
model~\cite{Lassance2022SPLADE-efficient,mallia2022faster,Qiao20222GT,2023SIGIR-Qiao,2023SIGIR-SPLADE-pruning}.
For example, BM25 guided-sparse retrieval can greatly speedup, but lose some recall or precision
 when this guidance is weighted aggressively.
The use of dense retrieval provides a flexibility and reduces  the relevance requirement of sparse retrieval.
Namely potentially we can choose a relatively fast sparse retrieval with the slightly lower accuracy/recall,
and  let dense retrieval make up the loss. Our design
needs to  adapt to  sparse retrieval quality and plans
We plan to exploit features that reveal  the overlapping degree of top sparse retrieval results with  dense clusters
to guide the selection in addition to query-cluster distances. 
}

\comments{
\item  {\bf Query filtering for skipping dense retrieval}
We want an online system to make an earlier  determination if a query needs an argumentation from dense retrieval with supervised learning.
%A challenge is to identify features and infer based on such features with supervised learning.
Given that sparse retrieval is conducted first,
our idea is to predict the quality of sparse retrieval and its relative strength  compared to unexecuted
dense retrieval based on quality of query token expansion by the sparse model,
the statistical behavior of  sparse retrieval results, and
the relationship between dense document embedding summary and sparse retrieval scoring structure.

}



{\bf Latency budget.}
%Our heuristic-based fusion selection may suffer from an effectiveness tradeoff
%as full dense retrieval execution likely offers the maximum relevance benefits.
For search latency, our goal is to minimize the relevance effectiveness loss to a small degree while still accomplishing  a fast response time
acceptable to the interactive search system requirement.
In a search system running as an interactive  web service,  a query with multi-stage processing
needs to be completed within a few hundred milliseconds.
%Considering the multi-stage search nature  and other service overhead involved, 
A first-stage retriever operation  for a data partition needs to be completed within several tens of milliseconds without query caching (e.g. 200ms). 
Our targeted time budget to augment sparse retrieval cannot be too high     compared to  sparse retrieval cost.
We will evaluate the latency budget in two settings: around 50ms  and 25ms, including the  sparse retrieval time.
%For the example of Table~\ref{tab:costbudget},
%The studies from~\cite{Lassance2022SPLADE-efficientmallia2022GTI,Qiao20222GT,2023SIGIR-Qiao},
If sparse retrieval can complete  in 30 ms on an  average CPU and the total latency
target is around 50ms,  the cost of dense retrieval is targeted under around  20ms.
% At most the total sparse and dense retrieval cannot be more than 100ms.
%Accuracy of above query-specific cluster skipping while retaining a competiitve relevance is the key to accomplish this latency goal. 
%Notice that the latency target in the  LADR paper~\cite{2023SIGIR-LADR} is in a 4ms-8ms range
%and 
%This latency budget choice is reasonable because for 
%Also our evaluation is conducted in a low-end CPU server and a faster CPU can further accelerate. 
%CPU latency reported in~\cite{2022WWWforwardIndex} is at 11

\comments{
For the memory space cost,  our target budget for  dense retrieval augmentation is controlled in  the same level or some fraction of  sparse retrieval cost.
As illustrated in  Table~\ref{tab:costbudget}, compression with embedding  quantization is necessary to meet the space constraint.
%due to the memory usage of stroing  embedding vectors. 
%For 8.8M MS MACRO passages, that takes  about 27GB space.
%Fortunately the quantization techniques can significantly compress this space into 1-2GB or even 0.5GB depending on the configuration. 
Our feature design does not opt for  
inter-document similarity since it is space-consuming,
but  plans to exploit cluster-based summary information, 
which  only adds  insignificant  space overhead.  
%, and set a limit on the number of dense clusters used.
}



==> clustexp.tex <==
\section{Evaluations}


\comments{
Our evaluation answers  the following research questions around our proposed techniques and the correspond subsection are marked.

\textbf{RQ1} (Section~\ref{sect:eval0space}): 
How does CluSD compare against other low-cost baselines when space is constrained?
%extra space overhead is minimized by augmentation under different compression configurations? 

\textbf{RQ2} (Section~\ref{sect:evaltimebudget}): 
How does CluSD  perform under a retrieval latency time budget when there is no space restriction?

\textbf{RQ3} (Section~\ref{sect:evalbeir}): 
How does CluSD  perform in searching  out-of-domain text content?
Zero-shot retrieval performance is important since a large dataset can contain documents from many domains. 


\textbf{RQ4} (Section~\ref{sect:evalLSTM}): 
Is  LSTM with cluster pruning preferred compared to other design options?
Are  features designed for LSTM useful?

\textbf{RQ5} 
(Section~\ref{sect:clusterno}): 
How does the number of clusters used in dataset partitioning 
affect the relevance and latency of CluSD? 

\textbf{RQ6} 
(Section~\ref{sect:threshold}):
How does the choice of selection threshold value in LSTM affect the average number of clusters selected?
%Does the cluster selection model dynamically select different number of clusters for different queries? How the selection differs for different datasets?

\textbf{RQ7}
(Section~\ref{sect:evalsparse}):
How does CluSD perform in augmenting  different sparse retrievers with different efficiency and relevance characteristics?


}

{\bf Datasets and measures.}
Our evaluation uses the MS MARCO datasets with 8.8 million passages for full passage ranking~\cite{Campos2016MSMARCO,Craswell2020OverviewOT}. 
%MS MARCO contains  8.8 million passages and about 1.1  judgment label per query. 
The test query sets are the Dev set with 6980 queries and TREC deep learning (DL)  2019/2020 tracks with 43 and 54 queries.
%The average number of WordPiece~\cite{wordpiece} tokens per passage is 67.5.
%The development (Dev) query set contains  6980 test queries. %with about 1.1  judgment label per query. 
%The test sets in  TREC deep learning (DL)  2019 and 2020 tracks 
%provide 43 and 54 queries, respectively, with many judgment labels per query.
%which provide 54 and 43 test queries, repsectively,  
Following the common practice for Dev, 
%official leader-board standard, 
we report mean reciprocal rank at 10 (MRR@10) and recall at 1000 (recall@1K) 
which is the percentage of relevant-labeled results appeared in the final top-1000 results.
%we report mean reciprocal rank (MRR@10) for relevance instead of
%Normalized discounted cumulative gain (NDCG)~\cite{NDCG}  is not used because such a set has about 1.1 judgment label per query, which is too sparse to use NDCG.
For DL19 and DL20 sets, we report NDCG@10.
%which have many judgment labels per query, we report the commonly used NDCG@10 score.
% when space allowed, we also report the recall@1k. 
%If space allows,
%In addition, we also report recall at 50 (recall@50) 
%as if we use large language model as a reranker, it is common practice to take less than 100 documents from retrieval model for evaluation.
%For TREC DL test sets which have many judgment labels per query, we report the commonly used NDCG@10 score.
%When space allows, we also report the recall ratio at 1000 
We report average NDCG@10 for the 13 publically available BEIR datasets~\cite{thakur2021beir} 
to evaluate  zero-shot retrieval performance. 
\comments{
BEIR is a heterogeneous benchmark containing a variety of IR tasks, 
including search tasks (e.g.  question-answering, bio-medical IR, and entity retrieval)  
and semantic relatedness tasks (e.g.  duplicate question retrieval). 
The size of these data sets ranges from 3,633 to 5.4M.
%Their average query length ranges from 5.39 to 192.98, 
%and  their average document length ranges from 11.44 to 634.79. 
%Each dataset has binary or three-level relevance labels.
}

{\bf Models and parameters.}
For sparse retrieval, we adopt 3 SPLADE-based  models and one BM25 based model with different relevance and efficiency  tradeoffs:
1) SPLADE-HT1 is based on   a recent SPLADE model optimized by  hybrid thresholding~\cite{2023SIGIR-Qiao}
and BM25-guided traversal~\cite{mallia2022faster,qiao2023optimizing} with index space 3.9GB
and 31.2 ms retrieval latency. 2) SPLADE-HT1-fast is a variation of SPLADE-HT1 with a different parameter setting, which has 
3.9GB index space and 22.4 ms latency. 
3) SPLADE-effi-HT3 is the SPLADE-efficient model~\cite{Lassance2022SPLADE-efficient} with 3GB space
and  12.4ms latency due to use of hybrid thresholding and BM25 guided traversal techniques. 
4) BM25-T5 applies  the BM25 lexical model on expanded documents using DocT5Query~\cite{Cheriton2019doct5query}. 
BM25-T5 uses 1.2GB index space with latency 9.2ms. 
For dense retrieval, we adopt the recently published   dense models
SimLM~\cite{Wang2022SimLM} and RetroMAE~\cite{Liu2022RetroMAE}. 
We use their   checkpoints from the Huggingface library to generate document and query embeddings 
and  use  K-means in the FAISS library~\cite{johnson2019billion} to derive dense embedding clusters.
Our evaluation implementation uses C++ and Python and the
related code will be released to the public after publication of this paper. 
\comments{
%Note that SimLM model's embeddings are normalized while RetroMAE's embeddings are not. 
For sparse retrieval, we use two fast versions of SPLADE and a SPLADE-efficient model, as well as BM25-T5. 
The implementation of SPLADE models follows 2GTI optimization~\cite{qiao2023optimizing}. %its official release~\cite{spladeRepo}. 
SPLADE-HT1 is the SPLADE model trained with hybrid thresholding scheme~\cite{2023SIGIR-Qiao} using $\lambda_{t}=1$, 
SPLADE-effi-HT3
is the SPLADE-efficient model~\cite{Lassance2022SPLADE-efficient} trained with hybrid thresholding scheme using $\lambda_{t}=3$. Both of these two models are using the "accurate" configuration in 2GTI during retrieval, while SPLADE-HT1-fast uses the "fast" configuration.
The sparse retrieval code for Splade and BM25-T5 uses the code from PISA~\cite{mallia2019pisa}
with some optimization~\cite{Lassance2022SPLADE-efficient,2023SIGIR-Qiao}.
}

To train the CluSD model, we sample 5000 queries from the MS MARCO training set 
%and use the LSTM unit in Pyytorch. 
and the hidden dimension for LSTM is 32. The models are trained for 150 epochs. 
%The input documents are sorted based on the distance between the centroids the documents belong to and  the query. 
For sparse and dense model interpolation, we use min-max normalization to rescale the top results per query. 
%Then we use linear combination with equal weights to combine two ranked lists. 
For  BM25-T5, the interpolation  weights are  0.05 and 0.95 for sparse  and  dense scores, respectively. 
For SPLADE, they are  0.5 and  0.5, respectively. 
%In terms of missing document in either ranked list, as the smallest value from each normalized list is 0, there is no missing imputation needed as we 
%can view the missing  documents taking the value of the worst document in the ranked list automatically. 
For CluSD, the default setting of number of clusters is $N=8192$, and the input sequence length to the LSTM model is truncated at $n=32$.  
To report the mean single-query latency and 99 percentile latency in milliseconds,
we  run test queries multiple times  from MS MARCO Dev set using a single thread on  a 2.25GHz AMD EPYC 7742  CPU server. 

%{\bf Baselines and notations.}
%We select two groups of baselines under space and time constraints respectively.
%\label{sect:eval0space}

\begin{table*}[htbp]
	\centering
		\resizebox{1.9\columnwidth}{!}{
		\begin{tabular}{ r r l |l l ll l |llll l|r}
			\hline\hline
			 & & & \multicolumn{2}{c}{ 
{\bf MSMARCO Dev} }& {\bf DL19}& {\bf DL20} & {\bf BEIR} 
& \multicolumn{2}{c} { {\bf MSMARCO Dev} }& {\bf DL19}& {\bf DL20} & {\bf BEIR} 
& {\bf  Latency}    \\
			& &\% D& {MRR@10}& R@1k& {NDCG@10}&  {NDCG@10}& {NDCG@10}& {MRR@10}& {R@1k}& {NDCG@10}&{NDCG@10}& {NDCG@10}& ms \\
    \hline
 1. & S={\bf SPLADE-HT1} & --& 0.396& 0.980 & 0.732   & 0.721    & 0.500 & -- & --& --& --& --&31.2  \\
 & & & \multicolumn{5}{c|}{D=\textbf{SimLM}}& \multicolumn{5}{c|}{D=\textbf{RetroMAE}}&\\
   \hline
   &&& \multicolumn{10}{c}{\bf{Uncompressed flat setting. Embedding space  27.2GB}}\\
     \hline
          2. &   D  & 100 & 0.411$^\dag$ & 0.985$^\dag$& 0.714 &  0.697  & 0.429 & 0.416$^\dag$& 0.988& 0.720&0.703& 0.482 & 1674.1 \\
            3. &   $\blacktriangle$ S $+$ D   &100 & 0.424 & 0.989 & 0.740 & 0.726  & 0.518 & 0.425& 0.988& 0.740&0731& 0.520~& $+$1674.1 \\
           4. &    \bf S $+$ CluSD &0.3& 0.425 & 0.987 & 0.744 & 0.724  & 0.516 & 0.426& 0.987& 0.744&0.734 & 0.518 & $+$13.2 \\
              \hline
            &&& \multicolumn{10}{c}{\bf{OPQ $m=128$. Embedding space  1.1GB}}\\
              \hline
            5. &   $\blacktriangle$  S $+$ D-OPQ &100 & 0.420 & 0.988 & 0.735 &  0.719  & 0.508 & 0.416 & 0.988 & 0.737 & 0.732 & 0.515& $+$568.9 \\
            6. &  S $+$ D-IVFOPQ &10& 0.414$^\dag$& 0.987 & 0.726 & 0.734  & 0.505 & 0.404$^\dag$& 0.987& 0.713&0.722& 0.513 &  $+$95.2 \\
           7. &   &5& 0.407$^\dag$& 0.987 & 0.717 & 0.733  & 0.499  & 0.394$^\dag$& 0.987& 0.687&0.817&0.507&$+$ 48.8 \\
           8. &   &2& 0.392$^\dag$& 0.986$^\dag$& 0.691 & 0.738  & 0.467 & 0.374$^\dag$& 0.986$^\dag$& 0.656&0.815& 0.499&$+$21.3 \\
           9. &   \textbf{S $+$ CluSD}  &0.3& 0.423 & 0.987 & 0.739& 0.725 &0.514 & 0.417& 0.986& 0.742&0.735& 0.514  & $+$11.4  \\
             \hline
           & & & \multicolumn{10}{c}{\bf{OPQ $m=64$. Embedding space 0.6GB}}\\
            \hline
           10. & $\blacktriangle$  S $+$ D-OPQ  &100 & 0.409 & 0.986 & 0.718 &  0.721  &0.501 & 0.402 & 0.986 & 0.717 &  0.719 & 0.508 &$+$ 290.4 \\
           11. &   S $+$ D-IVFOPQ &10& 0.405 & 0.986 & 0.716 & 0.734 & 0.502 & 0.393$^\dag$& 0.986& 0.676&0.730& 0.505& $+$44.4 \\
           12. &   &5& 0.397$^\dag$& 0.986 & 0.704 & 0.733  & 0.497 & 0.384$^\dag$& 0.985& 0.659&0.717& 0.500& $+$23.8 \\ 
            13. &  &2& 0.383$^\dag$& 0.985 & 0.680 & 0.738 & 0.487 & 0.368$^\dag$& 0.985 & 0.643&0.707& 0.493 & $+$11.2 \\
            14. &  \textbf{S $+$ CluSD}  &0.3& 0.414 & 0.986 & 0.743& 0.726 & 0.511 & 0.403 & 0.987& 0.729&0.724 & 0.506 & $+$9.6 \\
              \hline\hline
		\end{tabular}
		}
	\caption{
Sparse retrieval argumentation with minimum extra space overhead.
%no  with compressed or uncompressed dense emebddings S=SPLADE-HT1, D=SimLM or RetroMAE. 
%Model relevance and latency under compressed or uncompressed dense emebddings S=SPLADE-HT1, D=SimLM or RetroMAE. 
%Row  ``S $+$ D'' marked with $\blacktriangle$ indicates the oracle setting of sparse model interpolated with full dense retrieval. 
For MSMARCO Dev set, $^\dag$ is tagged when statistically significant drop is observed from the oracle $\blacktriangle$ at 5\% confidence level. 
}
\vspace*{-5mm}
	\label{tab:mainspace}
\end{table*}
	%\caption{Model relevance and latency under different configurations with storage constraints. S=SPLADE-HT1, D=SimLM or RetroMAE. The row  ``S $+$ D'' marked with $\blacktriangle$ indicates the oracle setting of sparse model interpolated with full flat dense search model. For MSMARCO Dev set, $^\dag$ is marked when statistically significant drop is observed from the oracle $\blacktriangle$ at 5\% confidence level.



{\bf Fast search with minimized space overhead}
Table~\ref{tab:mainspace} 
Table~\ref{tab:mainspace} compares   CluSD and the baselines in searching MS MARCO and BEIR datasets with memory space constraint. 
It uses two quantization  configurations and the uncompressed setting. 
The sparse model used is SPLADE-HT1 while the dense models are SimLM and RetroMAE.
%The top portion of this table reports the performance when compression is not used, which captures a peak possible performance.
IVFOPQ is compared, which use some percentage of top dense clusters sorted by query to centroid clusters.
%against CluSD as it selects only top clusters and does not incur extra space overhead. 
We include dense retrieval with quantization option OPQ and  IVFOPQ with IVF clustering available in FAISS.
OPQ quantization  is configured with  the number of codebooks as $m=$ 128 or 64.  
We report performance of IVF clustering using top 10\%, 5\%, 2\% clusters respectively
as a standard approach which performs   limited top cluster retrieval. 
CluSD execution is also based on the the same OPQ or  IVFOPQ index from  FAISS but clusters are  selected  by our LSTM model. 


Notation ``S+D'' in Table~\ref{tab:mainspace} (and Table~\ref{tab:sparse} later) 
reports the fused performance of a sparse model and a dense model with linear interpolation. 
Column marked with  ``\%D'' means the percentage of dense embeddings  evaluated. 
Last column on ``Latency'' is the average single-query time using SimLM for MS MARCO Dev set.  
We only report SimLM latency because the latency of SimLM and RetroMAE are similar. 
When 	prefix `+' is marked for a latency entry, it indicates  the extra milliseconds is spent 
for full or selective dense retrieval without counting   sparse retrieval time.
CluSD uses setting $n=32$
% Tables~\ref{tab:mainspace} and~\ref{tab:maintime} use 
which results in  selection of 22.3 clusters on average per query 
and allows CluSD to meet  the latency requirement.
%Switching a quantization different  from OPQ  is might result in an improvement in relevance, but it is orthogonal to our proposal. 
%The reported CluSD performance on the flat index uses the exact same IVF index. 
% for CluSD uses on average 20-25 (0.25 - 0.3\%) clusters per query. 
%For re-ranking, we report the results of re-ranking top 1000 results from the sparse model using the dense model.  
The mean latency and 99 percentile latency of CluSD are 13.2 ms and 18.1 ms for searching uncompressed flat index, respectively; 
11.4 ms and 14.6ms for searching OPQ m=128 index;  9.6 ms and 11.1ms for searching OPQ m=128 index.

For MS MARCO Dev set, the result of a method is marked with  tag $^\dag$ when 
statistically significant drop is observed compared to  an oracle baseline
tagged with $\blacktriangle$ at 5\% confidence level.  This oracle
is sparse retrieval fused with full dense retrieval marked as ``S+D'', which typically delivers the highest relevance  
using all uncompressed or quantized dense embeddings ($m=128$ or $m=64$).

Table ~\ref{tab:mainspace} 
shows that
selective dense  to augment sparse retrieval by top IVF clusters sorted by query-centroid distances 
can be fast below  100ms  when the percentage of clusters searched  drops from 100\% to 10\%. But the relevance drop is significant. 
Moreover, CluSD is as  fast  as IVFOPQ  top 2\% search at m=64 and 2x fast at m=128 while
its relevance is much higher.
CluSD  performs  closely as the oracle at each compression setting, which  
indicates CluSD effectively minimizes visitation of unnecessary  dense clusters. 

 

{\bf Search with no memory space constraints}.
%\label{sect:evaltimebudget}
Table~\ref{tab:maintime} compares  CluSD with  several baselines under two time budgets when memory space restriction is removed.
%Uncompressed dense embeddings  are used to exclude the relevance impact by quantization.
The last two columns report the total latency time in milliseconds including sparse retrieval when needed,
and data space cost. Extra memory space on the top of sparse retrieval is marked with prefix `+'. 
``MRR'' means  MRR@10 and ``NDCG'' means  NDCG@10.
The extra space for quantized inter-cluster distances for CluSD takes about 32MB. 
%Table~\ref{tab:maintime} compares  baselines  without  memory space constraint. 
For proximity graph-based dense retrieval which incurs additional graph space overhead,
we include  HNSW~\cite{2020TPAMI-HNSW} and  LADR~\cite{2023SIGIR-LADR} as shown in Table~\ref{tab:maintime}. 
%For HNSW, we fix the number of neighbors to be 128 and vary the expansion factor(ef) to meet the latency constraint. 
%For LADR, we use its default setting with seed = 200, number of neighbor = 128 and use the exploration depth as 50 to meet the latency requirements in 
%Table~\ref{tab:maintime}.
%Uncompressed dense embeddings (marked as "flat") are used
%to exclude the impact due to quantization.
We also compare  a simple re-ranking method,  denoted as ``D-rerank'' or ``rrk'', 
that fetches the dense scores of top 1000 of sparse retrieval to re-rank with interpolation. 
%We use the same clustering setting for IVF and CluSD. 




%As discussed in Section~\ref{sect:design}, the overall latency budget is set as 50ms and 25ms respectively. 
We allow some time for budget relaxation since it is difficult to tune parameters of all baselines to meet the constraints exactly. 
For IVF, we use 1.5$\%$ and 3$\%$ top clusters for ``S+IVF'' and ``IVF''.
%  but we allow some variation for some baselines because it is difficult to find parameters that exactly control the latency under this budget. 
%In this case, we choose the dense configuration such that the overall latency is within 70 or 30 milliseconds. 
For HNSW under 50ms time budget, we set its expansion factor parameter (ef) as 1024, 
2048 for S$+$D-HNSW and D-HNSW. 
Under 30ms time constraint, the expansion factor (ef) is  512 and  1024 respectively. 
%We include option ``S+Re-rank" which uses the top 1,000 sparse retrieval results and only compute dense scores of these top results, and merge the score with an interpolation.
%For HNSW, we fix the number of neighbors to be 128 and vary the expansion factor(ef) to meet the latency constraint.
For LADR, we use its default setting with seed = 200, number of neighbor = 128 and use the exploration depth as  50 to meet the latency budget.
%Table~\ref{tab:maintime}.
\comments{
Under time budget 50ms, 
model  SPLADE-HT1 is used and it has a latency of 31.2 ms in sparse retrieval.  
Under  time budget 25ms, model SPLADE-effi-HT3 is used and it is more aggressive in  efficiency 
with a 12.4ms latency at the cost of a relevance degradation. 

%using the dense model only, We also include sparse retriever 
%IVFOPQ, IVF, OPQ and HNSW using the dense model only, We also include sparse retriever 
%with reranking top 1000 results using the dense model. We also include the results of document evaluation using LADR algorithm. 
Note that when ``S$+$'' is in the row, it means we use the sparse model and the reported results are interpolated. 

}
%[DISCUSS TABLE 4 RESULTS.]
\comments{
The takeaways from this table are:

\textbullet\ While IVF does not add extra space cost,
the relevance  of IVF top cluster search under the time budget performs  worse than others.
Simple re-ranking ``D-rerank'' achieves good MRR@10 but under-performs on recall.
When the recall of a sparse retriever is relatively low, it cannot boost further as seen in the case of $m=64$.

\textbullet\ HNSW and LADR perform comparably, at the cost of extra online memory overhead  and extra complexity to compute offline in advance.
HNSW requires extra 9.2GB and LADR requires extra 4.3GB to store graph data in memory. 
When we  try to reduce their graph size by decreasing  the number of neighbors for HNSW and LADR, their  MRR@10 and/or  recall@1000 numbers drop visibly. For example, 
using the default 32 neighbors for the HNSW graph results in 2.4GB graph space, however  MRR@10 drops from 0.407 to 0.4 under the 25ms time budget. 

\textbullet\ CluSD incurs negligible extra space cost other than hosting embeddings, compared to HNSW and LADR.
For $m=128$,  CluSD has a higher MRR@10 while its DL19 and DL20 numbers are higher than HNSW, but comparable as LADR.
CluSD has more  advantages in relevance when $m=64$. 

\textbullet\ The time budget setting is discussed in Section~\ref{sect:design}.
Even when we relax the latency requirements for the baselines, CluSD still maintains its advantages in different datasets. 
For instance, if we double the time budget to around  110ms
for 	``S+D-HNSW'' after  SPLADE-HT1 retrieval, its MRR@10 for MS MARCO Dev is 0.422, which is still below S$+$CluSD with 46.3ms.


}

 

\begin{table}[htbp]
	\centering
 \resizebox{0.9\columnwidth}{!}{
		\begin{tabular}{r |llll|rr}
			\hline\hline
			& \multicolumn{2}{|c}{\bf{MSMARCO Dev}}& \bf{DL19}& 
\bf{DL20}& \bf{Latency}& \bf{Space}\\
			 & {MRR}& {R@1k}& \smaller{NDCG} &   \smaller{NDCG} & Total& GB\\
			\hline
        \multicolumn{7}{c}{\bf{Time Budget = 50 ms, S=SPLADE-HT1}}\\
        \hline
            D=SimLM & 0.411 & 0.985$^\dag$& 0.714 &  0.697 & 1674.1 & 27.2 \\
          S& 0.396$^\dag$& 0.980$^\dag$& 0.732   & 0.721    &   31.2 & 3.9 \\
           S $+$ D-rerank &  0.421 & 0.980$^\dag$& 0.745 & 0.728 & 34.6 & 31.1 \\
             $\blacktriangle$  S $+$ D  & 0.424 & 0.989 & 0.740 & 0.726 & 1705.0 & 31.1 \\
              \hline
              % D-IVF & 0.398$^\dag$& 0.935$^\dag$& 0.690 & 0.693 & 81.4 & $+$0.0\\
            D-IVF & 0.389$^\dag$& 0.907$^\dag$& 0.671 & 0.676 & 49.5 & $+\sim$0\\
            S $+$ D-IVF & 0.393$^\dag$& 0.987  & 0.678 & 0.715 & 56.5 & $+\sim$0\\
            %D-OPQ& 0.314$^\dag$& 0.957$^\dag$& 0.619 & 0.608 & 109.1 & 0.3 \\
           % D-IVFOPQ & 0.386$^\dag$& 0.929$^\dag$& 0.680 & 0.697 & 48.8 & 1.2\\
             D-HNSW & 0.409$^\dag$& 0.978$^\dag$& 0.669 & 0.695 & 54.4 & $+$9.2\\
            %S $+$ rerank-D &  0.412 & 0.980    &0.715  & 0.811 & 0.698 & 0.815 & $+$2.3 \\
            S $+$ D-LADR & 0.422& 0.984$^\dag$& 0.743&0.728& 43.6& $+$4.3\\
%           7.1 &  S $+$ D-LADR & 0.423 & 0.987$^\dag$& 0.745 &0.728& 53.0 & $+$4.3\\
           % S $+$ D-IVF & 0.398$^\dag$& 0.987  & 0.674 & 0.720 & 64.7 & $+$0.0\\
           %S $+$ D-IVFOPQ & 0.392$^\dag$& 0.987 & 0.656 & 0.700 &  52.5 & 4.0\\
           S $+$ D-HNSW & 0.420 & 0.987 & 0.718 & 0.723 & 59.6 & $+$9.2\\
            \bf S $+$ CluSD & 0.426 & 0.987 & 0.744 & 0.724 &46.3& $+$0.03\\
       \hline       
            \multicolumn{7}{c}{\bf{Time Budget = 25 ms, S=SPLADE-effi-HT3}}\\
            \hline
            S& 0.380$^\dag$& 0.944$^\dag$& 0.721 &  0.726 & 12.4 & 3.0 \\
             S + D-rerank & 0.406 & 0.944$^\dag$& 0.728 & 0.738 & 15.1 & 30.2 \\
            $\blacktriangle$  S + D & 0.413 & 0.984 & 0.721 &0.729 & 1654.2& 30.2  \\
            \hline
            D-HNSW & 0.406 & 0.971$^\dag$& 0.672 & 0.694 & 28.4 & $+$9.2\\
             S $+$ D-HNSW & 0.407 & 0.984 & 0.706 & 0.724 & 28.7 & $+$9.2\\
            S $+$ D-LADR & 0.404$^\dag$& 0.984 & 0.728 &  0.736 & 24.2 & $+$4.3\\
%           16.1 & S $+$ D-LADR & 0.409 & 0.987 & 0.744 &  0.728  & 41.1 & $+$4.3\\
            \bf S $+$ CluSD & 0.412 & 0.984 & 0.733 & 0.728 & 25.4 & $+$0.03\\
			\hline\hline
		\end{tabular}  }
	\caption{Search under time budget but  no memory constraints 
}
  \vspace*{-10mm}
	\label{tab:maintime}
\end{table}
%For pipelines with a time budget, we report the additional overhead in the Storage (GB) column. 






==> clustexp_ab.tex <==
\vspace*{-5mm}
\subsection{Fast search with minimized space overhead}
\label{sect:eval0space}

\begin{table*}[htbp]
	\centering
		\resizebox{1.9\columnwidth}{!}{
		\begin{tabular}{ r r l |l l ll l |llll l|r}
			\hline\hline
			 & & & \multicolumn{2}{c}{ 
{\bf MSMARCO Dev} }& {\bf DL19}& {\bf DL20} & {\bf BEIR} 
& \multicolumn{2}{c} { {\bf MSMARCO Dev} }& {\bf DL19}& {\bf DL20} & {\bf BEIR} 
& {\bf  Latency}    \\
			& &\% D& {MRR@10}& R@1k& {NDCG@10}&  {NDCG@10}& {NDCG@10}& {MRR@10}& {R@1k}& {NDCG@10}&{NDCG@10}& {NDCG@10}& ms \\
    \hline
 1. & S={\bf SPLADE-HT1} & --& 0.396& 0.980 & 0.732   & 0.721    & 0.500 & -- & --& --& --& --&31.2  \\
 & & & \multicolumn{5}{c|}{D=\textbf{SimLM}}& \multicolumn{5}{c|}{D=\textbf{RetroMAE}}&\\
   \hline
   &&& \multicolumn{10}{c}{\bf{Uncompressed flat setting. Embedding space  27.2GB}}\\
     \hline
          2. &   D  & 100 & 0.411$^\dag$ & 0.985$^\dag$& 0.714 &  0.697  & 0.429 & 0.416$^\dag$& 0.988& 0.720&0.703& 0.482 & 1674.1 \\
            3. &   $\blacktriangle$ S $+$ D   &100 & 0.424 & 0.989 & 0.740 & 0.726  & 0.518 & 0.425& 0.988& 0.740&0731& 0.520~& $+$1674.1 \\
           4. &    \bf S $+$ CluSD &0.3& 0.425 & 0.987 & 0.744 & 0.724  & 0.516 & 0.426& 0.987& 0.744&0.734 & 0.518 & $+$13.2 \\
              \hline
            &&& \multicolumn{10}{c}{\bf{OPQ $m=128$. Embedding space  1.1GB}}\\
              \hline
            5. &   $\blacktriangle$  S $+$ D-OPQ &100 & 0.420 & 0.988 & 0.735 &  0.719  & 0.508 & 0.416 & 0.988 & 0.737 & 0.732 & 0.515& $+$568.9 \\
            6. &  S $+$ D-IVFOPQ &10& 0.414$^\dag$& 0.987 & 0.726 & 0.734  & 0.505 & 0.404$^\dag$& 0.987& 0.713&0.722& 0.513 &  $+$95.2 \\
           7. &   &5& 0.407$^\dag$& 0.987 & 0.717 & 0.733  & 0.499  & 0.394$^\dag$& 0.987& 0.687&0.817&0.507&$+$ 48.8 \\
           8. &   &2& 0.392$^\dag$& 0.986$^\dag$& 0.691 & 0.738  & 0.467 & 0.374$^\dag$& 0.986$^\dag$& 0.656&0.815& 0.499&$+$21.3 \\
           9. &   \textbf{S $+$ CluSD}  &0.3& 0.423 & 0.987 & 0.739& 0.725 &0.514 & 0.417& 0.986& 0.742&0.735& 0.514  & $+$11.4  \\
             \hline
           & & & \multicolumn{10}{c}{\bf{OPQ $m=64$. Embedding space 0.6GB}}\\
            \hline
           10. & $\blacktriangle$  S $+$ D-OPQ  &100 & 0.409 & 0.986 & 0.718 &  0.721  &0.501 & 0.402 & 0.986 & 0.717 &  0.719 & 0.508 &$+$ 290.4 \\
           11. &   S $+$ D-IVFOPQ &10& 0.405 & 0.986 & 0.716 & 0.734 & 0.502 & 0.393$^\dag$& 0.986& 0.676&0.730& 0.505& $+$44.4 \\
           12. &   &5& 0.397$^\dag$& 0.986 & 0.704 & 0.733  & 0.497 & 0.384$^\dag$& 0.985& 0.659&0.717& 0.500& $+$23.8 \\ 
            13. &  &2& 0.383$^\dag$& 0.985 & 0.680 & 0.738 & 0.487 & 0.368$^\dag$& 0.985 & 0.643&0.707& 0.493 & $+$11.2 \\
            14. &  \textbf{S $+$ CluSD}  &0.3& 0.414 & 0.986 & 0.743& 0.726 & 0.511 & 0.403 & 0.987& 0.729&0.724 & 0.506 & $+$9.6 \\
              \hline\hline
		\end{tabular}
		}
	\caption{
Sparse retrieval argumentation with minimum extra space overhead.
%no  with compressed or uncompressed dense emebddings S=SPLADE-HT1, D=SimLM or RetroMAE. 
%Model relevance and latency under compressed or uncompressed dense emebddings S=SPLADE-HT1, D=SimLM or RetroMAE. 
%Row  ``S $+$ D'' marked with $\blacktriangle$ indicates the oracle setting of sparse model interpolated with full dense retrieval. 
For MSMARCO Dev set, $^\dag$ is tagged when statistically significant drop is observed from the oracle $\blacktriangle$ at 5\% confidence level. 
}
\vspace*{-5mm}
	\label{tab:mainspace}
\end{table*}
	%\caption{Model relevance and latency under different configurations with storage constraints. S=SPLADE-HT1, D=SimLM or RetroMAE. The row  ``S $+$ D'' marked with $\blacktriangle$ indicates the oracle setting of sparse model interpolated with full flat dense search model. For MSMARCO Dev set, $^\dag$ is marked when statistically significant drop is observed from the oracle $\blacktriangle$ at 5\% confidence level.



Table~\ref{tab:mainspace} demonstrates  the effectiveness  of CluSD in searching MS MARCO and BEIR datasets under
two quantization  configurations and the uncompressed setting. 
IVFOPQ is compared against CluSD as it selects only top clusters and does not incur extra space overhead. 
%is compared, which use some percentage of top dense clusters sorted by query to centroid clusters.
The sparse model used is SPLADE-HT1 while the dense models are SimLM and RetroMAE.
%The top portion of this table reports the performance when compression is not used, which captures a peak possible performance.
Column marked with  ``\%D'' means the percentage of dense embeddings  evaluated. 
Last column on ``Latency'' is the average single-query time using SimLM for MS MARCO Dev set.  We only report SimLM latency because the latency of SimLM and RetroMAE are similar. 
When 	prefix `+' is marked for a latency entry, it indicates  the extra milliseconds is spent 
for full or selective dense retrieval without counting   sparse retrieval time.

Tables~\ref{tab:mainspace} and~\ref{tab:maintime} use the same CluSD setting with $n=32$, which results in  selection of
22.3 clusters on average per query. 
The mean latency and 99 percentile latency of CluSD are 13.2 ms and 18.1 ms for searching uncompressed flat index, respectively; 
11.4 ms and 14.6ms for searching OPQ m=128 index;  9.6 ms and 11.1ms for searching OPQ m=128 index.

\comments{
%In realistic settings, a flat dense index is usually not affordable when corpus size is not small. Certain compression technique need to be used. 
The top portion of this table reports the performance of  SimLM dense model marked as ``D'' in Row 2.
In Row 1, ``S'' denotes sparse retrieval using  a variation of SPLADE with hard thresholding called HT1~\cite{2023SIGIR-Qiao}.
Sparse results merged with full  dense retrieval  results  are marked in Row 3, ``S $+$ D''.  
Our pipeline is reported in Row 4,``S $+$ CluSD''. 
The second and third portions of this table reports
the search performance   with  two compression configurations using OPQ implemented in FAISS:
1) ``m128'' that compresses dense embeddings from about 27GB into 1.1GB with 128 quantization codebooks.
2) ``m64'' that  yields 0.6GB compressed embeddings with 64 codebooks. 
%Setting where the storage for dense index is 1.1GB and 0.6GB. 
Under these two configurations, we report the Sparse model interpolated with dense retrieval under
IVFOPQ or OPQ using the default FAISS setting.


%In the first section of the table, we include the full dense retrieval SimLM (denoted as D in the table), 
%and full sparse retrieval SPLADE-HT1 (denoted as S in the table), 
%and 
%We then report dense retrieval with two compression configurations, using OPQ 
%with m=128 and m=64 respectively, resulting in an index 
%with 1.1GB and 0.6GB. These compressed configuration result in a 96\% and 97.8\% reduction in storage compared to flat index.
% and compare them against our pipeline.
}
 This table shows that
selective dense  to augment sparse retrieval by top IVF clusters sorted by query-centroid distances 
can be fast below  100ms  when the percentage of clusters searched  drops from 100\% to 10\%. But the relevance drop is significant. 
Moreover, CluSD is as  fast  as IVFOPQ  top 2\% search at m=64 and 2x fast at m=128 while
its relevance is much higher.
CluSD  performs  closely as the oracle at each compression setting, which  
indicates CluSD effectively minimizes visitation of unnecessary  dense clusters. 

 



\comments{
 with full dense retrieval can reach a high relevance in all datasets and thus are marked as an oracle sign with or without compression.   
1. Almost no performance degradation when do S+CluSD.  Sometimes S+CluSD achieves slightly higher performance than S+D. It could be due to the fact that when we limit the search scope a lot of noisy documents are not considered by the dense model.

2. Under m=128 setting the performance degradation is acceptable especially on DL19 and 20. 

3. SimLM performs better under compression. This could be due to the fact that SimLM trained embedding is normalized while RetroMAE is not.

4. If we compare S+D-IVFOPQ with S+CluSD, given the same IVFPQ index, S+D-IVFOPQ represents the case where we use default order, even if we use 50x more clusters, the performance is not as good as CluSD. 
}


% table with skipping, 40ms for dense
\comment{
\begin{table}[htbp]
	\centering
		\resizebox{1.05\columnwidth}{!}{
		\begin{tabular}{ r l l l |r r  |r r  |r}
			\hline\hline
			 &\% & \multicolumn{2}{c|}{{MSMARCO Dev}}& \multicolumn{2}{c|}{DL19}& 
\multicolumn{2}{c|}{DL20}& Latency    \\
			 &n& {MRR@10}& {R@1k}& {N@10}& {R@1k}&  {N@10}& {R@1k}& ms \\
			\hline
            D  &--& 0.411$^\dag$ & 0.985 & 0.714 & 0.767 &  0.697 & 0.773 & 1674.1  \\
          S  &--& 0.396$^\dag$ & 0.980 & 0.732   &  0.811 & 0.721    &  0.815  &   31.2  \\
              $\blacktriangle$ S $+$ D   &--& 0.424 & 0.989 & 0.740 & 0.822 & 0.726 & 0.824 & 1705.0 \\
              \bf S $+$ CluSD  &0.2& 0.425 & 0.987 & 0.744 & 0.823 & 0.724 & 0.819 & 14.4 \\
              \hline
            \multicolumn{9}{c}{\bf{OPQ M=128 setting, Storage 1.1GB}}\\
            \hline
             S $+$ D-IVFOPQ&10& 0.414 & 0.987 & 0.726 & 0.820 & 0.734 & 0.818 & 95.2 \\
             &5& 0.407 & 0.987 & 0.717 & 0.820 & 0.733 & 0.817 & 48.8 \\
             &2& 0.392 & 0.869 & 0.691 & 0.815 & 0.738 & 0.815 & 21.3 \\
             S $+$ OPQ &--& 0.420 & 0.988 & 0.735 & 0.816 & 0.719 & 0.821 &  568.9 \\
             HNSW+OPQ && &  &  & & & &   \\
             \textbf{S $+$ CluSD}  &0.2& 0.422 & 0.986 & 0.739& 0.822& 0.725& 0.818& 14.2  \\
             \hline
          \multicolumn{9}{c}{\bf{OPQ M=64 setting, 0.6GB}}\\
          \hline
             S $+$ IVFOPQ&10& 0.405 & 0.986 & 0.716 & 0.814 & 0.734 & 0.818 & 44.4 \\
             &5& 0.397 & 0.986 & 0.704 & 0.814 & 0.733 & 0.817 & 23.8 \\ 
             &2& 0.383 & 0.985 & 0.680 & 0.813 & 0.738 & 0.815 & 11.2 \\
             S $+$ OPQ  &--& 0.409 & 0.986 & 0.718 & 0.815 & 0.721 & 0.821 & 290.4 \\
             HNSW+OPQ && &  &  & & & &   \\
             \textbf{S $+$ CluSD}  &0.2& 0.411 & 0.985 & 0.743& 0.823& 0.726& 0.816& 11.5 \\
              \hline\hline
		\end{tabular}
		}
	\caption{Model relevance and latency under different configurations with storage constraints. S=SPLADE-HT1, D=SimLM. The row  ``S $+$ D'' marked with $\blacktriangle$ indicates the oracle setting of sparse model interpolated with full flat dense search model. For MSMARCO Dev set, $^\dag$ is marked when statistically significant drop is observed from the oracle $\blacktriangle$ at 5\% confidence level.
}
	\label{tab:mainspace}
\end{table}

}



\subsection{Search with no memory space constraints}
\label{sect:evaltimebudget}
Table~\ref{tab:maintime} compares  CluSD with  several baselines under two time budgets when memory space restriction is removed.
Uncompressed dense embeddings  are used to exclude the relevance impact by quantization.
The last two columns report the total latency time in milliseconds including sparse retrieval when needed,
and data space cost. Extra memory space on the top of sparse retrieval is marked with prefix `+'. 
``MRR'' means  MRR@10 and ``NDCG'' means  NDCG@10.
The extra space for quantized inter-cluster distances for CluSD takes about 32MB. 

%As discussed in Section~\ref{sect:design}, the overall latency budget is set as 50ms and 25ms respectively. 
We allow some time for budget relaxation since it is difficult to tune parameters of all baselines to meet the constraints exactly. 
For IVF, we use 1.5$\%$ and 3$\%$ top clusters for ``S+IVF'' and ``IVF''.
%  but we allow some variation for some baselines because it is difficult to find parameters that exactly control the latency under this budget. 
%In this case, we choose the dense configuration such that the overall latency is within 70 or 30 milliseconds. 
For HNSW under 50ms time budget, we set its expansion factor parameter (ef) as 1024, 
2048 for S$+$D-HNSW and D-HNSW. 
Under 30ms time constraint, the expansion factor (ef) is  512 and  1024 respectively. 
%We include option ``S+Re-rank" which uses the top 1,000 sparse retrieval results and only compute dense scores of these top results, and merge the score with an interpolation.
%For HNSW, we fix the number of neighbors to be 128 and vary the expansion factor(ef) to meet the latency constraint.
For LADR, we use its default setting with seed = 200, number of neighbor = 128 and use the exploration depth as  50 to meet the latency budget.
%Table~\ref{tab:maintime}.
\comments{
Under time budget 50ms, 
model  SPLADE-HT1 is used and it has a latency of 31.2 ms in sparse retrieval.  
Under  time budget 25ms, model SPLADE-effi-HT3 is used and it is more aggressive in  efficiency 
with a 12.4ms latency at the cost of a relevance degradation. 

%using the dense model only, We also include sparse retriever 
%IVFOPQ, IVF, OPQ and HNSW using the dense model only, We also include sparse retriever 
%with reranking top 1000 results using the dense model. We also include the results of document evaluation using LADR algorithm. 
Note that when ``S$+$'' is in the row, it means we use the sparse model and the reported results are interpolated. 

}
%[DISCUSS TABLE 4 RESULTS.]
The takeaways from this table are:

\textbullet\ While IVF does not add extra space cost,
the relevance  of IVF top cluster search under the time budget performs  worse than others.
Simple re-ranking ``D-rerank'' achieves good MRR@10 but under-performs on recall.
When the recall of a sparse retriever is relatively low, it cannot boost further as seen in the case of $m=64$.

\textbullet\ HNSW and LADR perform comparably, at the cost of extra online memory overhead  and extra complexity to compute offline in advance.
HNSW requires extra 9.2GB and LADR requires extra 4.3GB to store graph data in memory. 
When we  try to reduce their graph size by decreasing  the number of neighbors for HNSW and LADR, their  MRR@10 and/or  recall@1000 numbers drop visibly. For example, 
using the default 32 neighbors for the HNSW graph results in 2.4GB graph space, however  MRR@10 drops from 0.407 to 0.4 under the 25ms time budget. 

\textbullet\ CluSD incurs negligible extra space cost other than hosting embeddings, compared to HNSW and LADR.
For $m=128$,  CluSD has a higher MRR@10 while its DL19 and DL20 numbers are higher than HNSW, but comparable as LADR.
CluSD has more  advantages in relevance when $m=64$. 

\textbullet\ The time budget setting is discussed in Section~\ref{sect:design}.
Even when we relax the latency requirements for the baselines, CluSD still maintains its advantages in different datasets. 
For instance, if we double the time budget to around  110ms
for 	``S+D-HNSW'' after  SPLADE-HT1 retrieval, its MRR@10 for MS MARCO Dev is 0.422, which is still below S$+$CluSD with 46.3ms.




 

\begin{table}[htbp]
	\centering
 \resizebox{0.9\columnwidth}{!}{
		\begin{tabular}{r |llll|rr}
			\hline\hline
			& \multicolumn{2}{|c}{\bf{MSMARCO Dev}}& \bf{DL19}& 
\bf{DL20}& \bf{Latency}& \bf{Space}\\
			 & {MRR}& {R@1k}& \smaller{NDCG} &   \smaller{NDCG} & Total& GB\\
			\hline
        \multicolumn{7}{c}{\bf{Time Budget = 50 ms, S=SPLADE-HT1}}\\
        \hline
            D=SimLM & 0.411 & 0.985$^\dag$& 0.714 &  0.697 & 1674.1 & 27.2 \\
          S& 0.396$^\dag$& 0.980$^\dag$& 0.732   & 0.721    &   31.2 & 3.9 \\
           S $+$ D-rerank &  0.421 & 0.980$^\dag$& 0.745 & 0.728 & 34.6 & 31.1 \\
             $\blacktriangle$  S $+$ D  & 0.424 & 0.989 & 0.740 & 0.726 & 1705.0 & 31.1 \\
              \hline
              % D-IVF & 0.398$^\dag$& 0.935$^\dag$& 0.690 & 0.693 & 81.4 & $+$0.0\\
            D-IVF & 0.389$^\dag$& 0.907$^\dag$& 0.671 & 0.676 & 49.5 & $+\sim$0\\
            S $+$ D-IVF & 0.393$^\dag$& 0.987  & 0.678 & 0.715 & 56.5 & $+\sim$0\\
            %D-OPQ& 0.314$^\dag$& 0.957$^\dag$& 0.619 & 0.608 & 109.1 & 0.3 \\
           % D-IVFOPQ & 0.386$^\dag$& 0.929$^\dag$& 0.680 & 0.697 & 48.8 & 1.2\\
             D-HNSW & 0.409$^\dag$& 0.978$^\dag$& 0.669 & 0.695 & 54.4 & $+$9.2\\
            %S $+$ rerank-D &  0.412 & 0.980    &0.715  & 0.811 & 0.698 & 0.815 & $+$2.3 \\
            S $+$ D-LADR & 0.422& 0.984$^\dag$& 0.743&0.728& 43.6& $+$4.3\\
%           7.1 &  S $+$ D-LADR & 0.423 & 0.987$^\dag$& 0.745 &0.728& 53.0 & $+$4.3\\
           % S $+$ D-IVF & 0.398$^\dag$& 0.987  & 0.674 & 0.720 & 64.7 & $+$0.0\\
           %S $+$ D-IVFOPQ & 0.392$^\dag$& 0.987 & 0.656 & 0.700 &  52.5 & 4.0\\
           S $+$ D-HNSW & 0.420 & 0.987 & 0.718 & 0.723 & 59.6 & $+$9.2\\
            \bf S $+$ CluSD & 0.426 & 0.987 & 0.744 & 0.724 &46.3& $+$0.03\\
       \hline       
            \multicolumn{7}{c}{\bf{Time Budget = 25 ms, S=SPLADE-effi-HT3}}\\
            \hline
            S& 0.380$^\dag$& 0.944$^\dag$& 0.721 &  0.726 & 12.4 & 3.0 \\
             S + D-rerank & 0.406 & 0.944$^\dag$& 0.728 & 0.738 & 15.1 & 30.2 \\
            $\blacktriangle$  S + D & 0.413 & 0.984 & 0.721 &0.729 & 1654.2& 30.2  \\
            \hline
            D-HNSW & 0.406 & 0.971$^\dag$& 0.672 & 0.694 & 28.4 & $+$9.2\\
             S $+$ D-HNSW & 0.407 & 0.984 & 0.706 & 0.724 & 28.7 & $+$9.2\\
            S $+$ D-LADR & 0.404$^\dag$& 0.984 & 0.728 &  0.736 & 24.2 & $+$4.3\\
%           16.1 & S $+$ D-LADR & 0.409 & 0.987 & 0.744 &  0.728  & 41.1 & $+$4.3\\
            \bf S $+$ CluSD & 0.412 & 0.984 & 0.733 & 0.728 & 25.4 & $+$0.03\\
			\hline\hline
		\end{tabular}  }
	\caption{Search under time budget but  no memory constraints 
}
  \vspace*{-10mm}
	\label{tab:maintime}
\end{table}
%For pipelines with a time budget, we report the additional overhead in the Storage (GB) column. 






==> clustexp_beir.tex <==

\begin{table*}[h]
	\centering
		\resizebox{1.9\columnwidth}{!}{
		%\begin{small}
		\begin{tabular}{r r r lr  |lllll|lllll}
			\hline\hline
                 &  & &  & &  \multicolumn{5}{c|}{SPLADE-HT1+SimLM} & \multicolumn{5}{c}{SPLADE-HT1+RetroMAE}\\
                  &  & &  & {SPLADE}  &  & &  \textbf{CluSD} & \textbf{CluSD} & \textbf{CluSD} & & & \textbf{CluSD} & \textbf{CluSD} & \textbf{CluSD}\\
		    Dataset & \smaller{BM25} &{SimLM}  &  {RetroMAE} &{-HT1} & \smaller{$\blacktriangle$ 
 flat} &rrk&\textbf{flat}& \textbf{m=128}& \textbf{m=64}& \smaller{$\blacktriangle$ flat} &rrk &\textbf{flat}& \textbf{m=128}& \textbf{m=64}\\
              \hline
              \multicolumn{15}{c}{\bf{Search Tasks}}\\
               \hline
                {DBPedia}	& 0.313	& 0.351 &  0.390&0.447	& 0.426 &0.442& 0.429 & 0.425 & 0.422 & 0.446 & 0.411 & 0.446 & 0.445&0.436 \\
                                {FiQA} &	0.236	& 0.298 &  0.316&0.355 & 0.355 &0.355 &0.365 & 0.361 &0.359 & 0.365 & 0.333 & 0.366 & 0.359& 0.353\\
                {NQ}	& 0.329   & 0.502  &	 0.518&0.550 & 0.568 &0.549&0.568 & 0.566 & 0.560 & 0.563 & 0.520 & 0.564 & 0.553& 0.538\\
                {HotpotQA} & 0.603 & 0.568 &  0.635& {0.681} & 0.672 &0.668&  0.672 & 0.669 & 0.661 & 0.702 & 0.642 & 0.702 & 0.693&0.672 \\
                {NFCorpus}  & 0.325 & 0.318  &  0.308&0.351 & 0.353 &0.347&  0.360 & 0.358 & 0.359 & 0.345 &0.331 & 0.351 & 0.349& 0.346 \\
                {T-COVID}	& 0.656 & 0.515  &  0.772&0.705 & 0.726 &0.692&  0.745 & 0.741 & 0.725 & 0.780 & 0.699 &0.747 &0.740& 0.726\\
                {Torche}	& {0.367}  & 0.292  &  0.237&0.291 & 0.336 &0.292 &0.333 & 0.336 & 0.332 & 0.292 &0.316 & 0.295 &0.288& 0.283\\
                \hline
                \multicolumn{15}{c}{\bf{Semantic Relatedness Tasks}}\\
                 \hline
                {ArguAna} & 0.315 & 0.376  &  0.433&0.446 & 0.481 &0.427&  0.492 & 0.489 & 0.486 & 0.459 & 0.434 & 0.455 &0.455 & 0.451\\
                {C-Fever}	& 0.213 & 0.171  &  0.232&0.234 & {0.239} &0.236&  0.241 & 0.250 & 0.242 & 0.260 &0.198 &0.260 &0.267& 0.262\\
                {Fever} & 0.753  &0.689  &	 0.774& {0.781} & 0.793 &0.784&  0.794 & 0.783 & 0.789 & 0.820 &0.774 &0.820 &0.814& 0.800\\
                {Quora} & 0.789 & 0.797  &	 0.847&0.817 &	0.847 &0.816&  0.847 & 0.849 &0.848 & 0.856 &0.814 &0.855 &0.854& 0.849\\
                {Scidocs}	& 0.158 &0.137  &	 0.15&0.155 &	{0.165} &0.152&  0.166 & 0.166 & 0.165 & 0.167 &0.142 &0.169&0.166& 0.164\\
                {SciFact}	& 0.665 & 0.559  &  0.653& {0.682} & 0.674 &0.682&  0.694 & 0.689 & 0.693 & 0.706  &0.661 &0.703 &0.699& 0.694\\
                            \hline
                \textbf{Avg.} & 0.440 & 0.429  &  0.482&0.500 & 0.518 &0.496&  0.516 & 0.514 & 0.511 & 0.520 &0.483 &0.518 &0.514& 0.506\\
                %\textbf{BM25 Diff} & -- & -2.6\%  &	13.6\% &17.7\% &  6.1\%&12.7\%&14.8\% &  \textbf{15.7\%} \\
                \textbf{{Splade Diff}} & -12.0 \% &  -14.2\%  &	 -3.6\% &-- & 3.6\% & -0.8\% &3.2\% & 2.8\% & 2.2\% &4.0\%& -3.5\%& 3.5\%&2.8\%&1.2\%\\
            \hline\hline
		\end{tabular}
		%\end{small}
		}
%\vspace*{-5mm}
	\caption{Zero-shot performance in average NDCG@10 on BEIR datasets. 
%Row ``SPLADE Diff.'' is the mean relative performance compared to the SPLADE-HT1 performance.
}
  \vspace*{-5mm}
%For quantization approaches, we adopt M=16, K=256, i.e. compression rate 32$\times$ compared to ColBERT.
	\label{tab:beir}

\end{table*}


{\bf Zero-shot retrieval performance with BEIR}.
\label{sect:evalbeir}
Table~\ref{tab:beir} lists  details on how  CluSD  performs when supplementing sparse SPLADE-HT1 with either SimLM or RetroMAE results in
searching one of  13 BEIR datasets that contain out-of-domain documents.
The LSTM model of CluSD  is trained with the  MS MARCO training set,
and it is directly applied to each of the BEIR  datasets to select clusters without any change. 
%Zero-shot out-of-domain performance is important since a large dataset can contain document content from many domains.
% to unseen models and datasets, we evaluate the pipeline on out-domain data. For this experiment, we use the BEIR benchmarks which consists 13 released document 
%sets on various semantic relatedness tasks. 
%We directly apply the CluSD model trained on MSMARCO training set to predict the clusters on the BEIR queries and BEIR specific clusters. 


As a baseline, column ``$\blacktriangle$ flat'' is to merge  the uncompressed full dense retrieval results with SPLADE-HT1 sparse  retrieval.
Column marked ``rrk'' is to rerank   top 1,000  sparse retrieval results interpolated with their dense scores. 
%The final score are the interpolation of the sparse ranked list and dense re-ranked list. 
Columns with ``CluSD-flat'', ``CluSD-m128'' and ``CluSD-m64''  are  CluSD results  using uncompressed or compressed embeddings with
m=128 or m=64. 
%\begin{itemize} [leftmargin=*]
%\item 
Even SimLM and RetroMAE  underperform SPLADE retriever for BEIR,  the relevance after sparse and dense  result fusion
is still higher than each individual retriever.
CluSD with limited dense retrieval   performs  closely to   oracle ``$\blacktriangle$ flat''.
While embedding compression affects relevance,  CluSD still performs reasonably well.  
%\end{itemize}
  


==> clustintro.tex <==


\section{Introduction and Related Work}



\comments{
Sparse and dense retrievers are two main categories of retrieval techniques for text  document search.
Traditional sparse retrieval models, such as BM25, use lexical text matching and run
%to retrieve results from the collection 
efficiently by traversing  an inverted index on an inexpensive  CPU platform.
Recently sparse retrieval studies have exploited learned neural representations~\cite{Dai2020deepct,
Mallia2021deepimpact, Lin2021unicoil,2021NAACL-Gao-COIL, Formal2021SPLADE, Formal2021SPLADEV2} for better semantic matching. 
%and SPLADE~\cite{Formal2021SPLADE, Formal2021SPLADEV2} has demonstrated the strong relevance performance among these models. 
The second category of document retrieval 
exploits a pre-trained language model with a dual encoder architecture to produce a dense document representation, 
e.g. ~\cite{gao-2021-condenser,2021SIGIR-Zhan-ADORE-dense,Ren2021RocketQAv2, 
%e.g. ~\cite{Lin2021tctcolbert, 2021CIKM-JPQ-Zhan, xiong2021-ANCE, gao-2021-condenser,2021SIGIR-Zhan-ADORE-dense,Ren2021RocketQAv2}. 
%There are numerious studies recently to enhance  dense retrieval with knowledge distillation
%and  improved  langage model pretraining~\cite
Lin2021tctcolbert, Santhanam2021ColBERTv2,  Wang2022SimLM,  Liu2022RetroMAE}.
}

Recent studies have found that combining  sparse and dense retrieval scores  can further boost
retrieval recall and relevance~\cite{Lin2021unicoil,2022LinearInterpolationJimLin,kuzi2020leveraging},
suggest  that both categories  of retrievers tend to capture  different relevant signals. 
These studies  make an assumption that  a search platform has to run two retrievers separately and a dense retriever.
%delivers   its maximum effectiveness, and the impact of compression and IVF clustering is not considered. 
There is an imbalance of computing platform requirement for running  these two retrievers.
dense retrieval typically requires GPU support unless significant  
%We study the use of dense retrieval results to argument sparse retrieval. 
Sparse retrieval with an inverted index has an advantage that a low-cost CPU server can run the online inference  without GPU.
This paper is targted at a low-cost CPU-friendly retrieval design.
%A judicious tradeoff consideration of retrieval  effectiveness and efficiency is critical on  a low-cost CPU-friendly search platform. 
%The importance of CPU-friendly search is recognized 
%in neural ranking studies~\cite{Yang2021WSDM-BECR,2022WWWforwardIndex,2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
For a large-scale  dataset (e.g. with billions of documents), a practical search system often employs  a multi-stage 
search architecture, which divides the dataset into many partitions so that  a fast first-stage  retrieval 
method  can  search these partitions in parallel.  Such a system  prefers low-cost
CPU-only servers for first-stage retrieval, and both time and memory space complexity of retrieval should be considered 
so that  each server can host as many documents as possible
to reduce the total number of servers to support a large data size and high query traffic. 
%Thus the challenge for retrieval on such an architecture needs to consider both time and space complexity. 
% small search index needs to be as small as possible.
%and the in-memory footprint size of 
%server  needs to host documents in memory as many as possible 
%given a large number  of data partitions involved for parallel search.
%Each server employs multiple CPU cores and is replicated with many copies  for dealing high traffic of  concurrent 
%search requests, and thus 


\comments{
There are recent efficiency studies 
for 
%advancing the inverted index implementation for 
fast sparse retrieval with learned neural 
representations~\cite{Lassance2022SPLADE-efficient,mallia2022faster,qiao2023optimizing,2023SIGIR-Qiao, 2023SIGIR-SPLADE-pruning},
%which run  efficiently  on a single CPU without hardware accelerators  GPU
%which re  retaining strong relevance effectiveness
%%Another development in learned sparse retrieval is that
%sparse retrieval with a learned representation
which accelerates learned sparse retrieval with BM25-guided traversal or index pruning.
For example, Row 3 of Table~\ref{tab:costbudget} shows the latency, memory space cost, and  MRR@10  of
a latest efficient SPLADE retriever for searching 8.8 million 
MS MARCO passages~\cite{2023SIGIR-Qiao} on a CPU only server.
% with a single thread on  a 2.25GHz AMD EPYC 7742  CPU server.
Row 2 is performance of a BM25 based retriever after document expansion. 
%There is a tradeoff  in relevance effectiveness if BM25 guidance or threshold-based pruning  is too aggressive.
%and dense retrieval can boost if it does not add much overhead. 
}

%There are recent efficiency studies on
%fast  sparse retrieval with learned
%representations~\cite{Lassance2022SPLADE-efficient,mallia2022faster,qiao2023optimizing,2023SIGIR-Qiao, 2023SIGIR-SPLADE-pruning}.
Dense retrieval can be accelerated  by approximate nearest neighbor  search with 
IVF clustering~\cite{johnson2019billion, 2021Facebook-DrBoost-Lewis}, quantization~\cite{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ},
%and hierachical navigable  small world graphs (HNSW)
and  proximity graph based navigation~\cite{2020TPAMI-HNSW,2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
Limited IVF cluster search and quantization can lead to  a significant  relevance drop while 
%For example, RetroMAE~\cite{Liu2022RetroMAE} dense retrieval without compression is slow, use of
%IVF clustering and OPQ quantization substantially accelerates but leads to a significant drop  of   MRR@10 score when searching up-to 20\%  
%of top dense clusters. 
%There is also a cost-relevance tradeoff  with proximity graph based search  using inter-document similarity distances~\cite{2020TPAMI-HNSW, 
%2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}.  
%Construction of a large document-level  graph   is  expensive
%during offline processing. 
online hosting of a document similarity graph  for graph navigation adds a large space cost.
%For example, the proximity graph  can take extra 4.3GB memory space~\cite{2023SIGIR-LADR} for 8.8M  MS MARCO passages. 
None of above studies has considered to exploit the selective fusion of dense and sparse  retrievers. 
\comments{
That is true also with the  navigation of  a  proximity graph based on inter-document similarity distances called HNSW~\cite{2020TPAMI-HNSW}. 
The proximity graph approach to guide dense retrieval is revisited recently in GAR~\cite{2022CIKM-MacAvaneyGraphReRank}, which is furthered improved by
%LADR Kulkarni  et al.~\cite{2023SIGIR-LADR} improves HNSW.
LADR~\cite{2023SIGIR-LADR}.
%~\cite{2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
The weakness of  the  proximity graph approach is that its graph  construction requires a quadratic computing complexity, which is expensive
for a large dataset and the online hosting of such a graph also adds a significant space requirement  on a low-cost
computing platform. For example, LADR takes extra 4.3GB memory space for 8.8M  passages in the MS MARCO dataset to keep top 128 
top neighbors per document. 
%Similarily HNSW also incurs a high space cost for graph connections.  
%In comparison, cluster-based selective dense retrieval can achieve in a comparable time complexity
%while adding  insignificant extra  space  overhead.

\begin{table}[htbp]
        \centering      
         \resizebox{0.82\columnwidth}{!}{ 
                \begin{tabular}{ r | r  rr}
                        \hline\hline
Sparse or dense methods  & Latency & Memory & MRR@10\\ 
\hline
BM25/DocT5Query & 9.2ms & 1.2GB & 0.261\\  
SPLADE/HT1 & 31.2ms & 3.9GB & 0.396 \\ 
RetroMAE/Uncompressed & 1677ms & 27.2GB & 0.419 \\ 
%SimLM /OPQ             & 225-1579ms & 0.57-2.3GB & $<$ 40.2 \\
RetroMAE /IVFOPQ  & 38-339ms & 1.2-2.3GB  & 0.37-0.401\\ 
                        \hline\hline
\end{tabular}
}
\caption{Latency and space cost of sampled sparse and dense models for MS MARCO passages with Dev query  set}
 \vspace*{-5mm}
\label{tab:costbudget}
\end{table}



  
%with a latency controled within 4 to 8 milliseconds on a single CPU, but with a significant tradeoff in relevance effectiveness.
%For example, MRR@10 for MS MARCO Dev set drops from RetroMAE has dropped from  0.416 to 0.356.
%This paper does not impose 4-8 millisecond latency, but rather looks for a solution that can leverage both dense and sparse retrieval
%and relax the latency constraint in some degree while maximizing its relevance effectiveness as much possible.
%a range below or around  100 milliseconds 

%The response time  for such a system for an interactive service needs to be fast enough a
%and thus search needs to be completed within a few hundred milliseconds. 

%which only requires triggering of dense embedding  computation for a relaively small subset of documents.
%The proposed scheme called cluster-based selective dense  retrieval

}

This paper proposes  a selective fusion of dense and sparse retrieval results 
%Because sparse retrieval is fast on CPU-only servers, this paper 
%augmenting sparse retrieval with 
called CluSD to argument  sparse retrieval with limited cluster-based dense retrieval results.
CluSD includes an LSTM based model with cluster prioritization and pruning to trigger limited dense computation. 
CluSD exploits inter-cluster and query-to-cluster distances and   the overlapping degree between top sparse retrieval results and dense clusters
to optimize cluster selection. 
%and then make a decision to determine which document clusters should be selected  to conduct dense retrieval computation.
The extra memory space overhead required to assist CluSD is negligible, and it  
works well when embedding vectors are highly compressed.
%  and  the extra memory required for hosting dense embeddings can be limited  after compression. 

\comments{
This paper evaluates  the usefulness   of CluSD  under a time and space constraint on a CPU only server when
 searching MS MARCO and BEIR  datasets  and provides a comparison with other baselines.
The evaluation  shows that CluSD can effectively identify a small number of document clusters to augment sparse retrieval results efficiently 
for  a stronger relevance  even though such a  sparse retriever is fast with  a relevance tradeoff. 
} 
%provides a flexibility and reduces  the relevance reqirement of sparse retrieval.
%Namely protentially we can choose a relatively fast sparse retrival with the slightly lower accuracy/recall,
%and  let dense retrivsal make up the loss. Our design needs to  adapt to  sparse retrieval quality and plans

%CSDR in improving the effectiveness of sparse retrieval with limited dense  retrieval
%traversal for low-cost search.  Our emprial findings suggest that SRF  can consistently outperform other baselines on a single CPU server 
%without GPUs 
% and achieve a strong tradeoff of effectiveness and efficiency compared to an exhausitve dense retrieval search.


%from pretrained language models to provide effective semantic text matching between a query and a document.





%0.419 by RocketQAv2~\cite{Ren2021RocketQAv2}, 
%which are the two latest state-of-the-art retrieval-reranker pipelines using cross-encoder based rerankers.
%Re-ranking in  recent dense retrieval work SimLM~\cite{Wang2022SimLM} has  used an expensive cross-encoder to
%achieve impressive MRR score 0.437 
%Re-ranking in RocketQAv2~\cite{Ren2021RocketQAv2} achieves 0.419 with a similar strategy.  



\comments{Modern search engines for text documents
typically employ two-stage ranking design. 
The first retrieval stage extracts top candidate
documents matching a query from a large search index with a fast ranking method. 
The second stage uses a more complex algorithm to 
re-rank top results thoroughly.
Recently neural ranking techniques from transformer-based architectures
have achieved impressive relevance scores 
for both retrieval and top $k$ document re-ranking. 
However, many recent work treats retrieval and reranking stage as two independent tasks and optimize them separately. Only a few works take into consideration the interplay of a retriever and a reranker. RocketQAv2 trains a cross encoder reranker and dual encoder retriever jointly with a strong reranker as teacher and train the retriever by dynamically distilling from reranker. Leonhardt (2022)\footnote{https://arxiv.org/pdf/2110.06051.pdf} uses a linear combination of the semantic similarity scores from the re-ranking phase and lexical matching scores from the retrieval phase with respect to the query for query evaluation.  

These methods either uses the reranker as a teacher to train the re-retriever, or consider the shallow combination of the results from two stages. In these training strategies, both the retriever and reranker are trained towards the same goal. In real application, as the two stages work jointly, either model does not need to perform perfectly by itself. Instead, by taking a more integrated view of the two stages in training and inference, the joint performance of the two stage models will be more efficient and effective. 

Moreover, these approaches typically requires a reranker (such as a cross-encoder in the case of RocketQA). In text retrieval applications, efficient rerankers with low online inference latency are often favored. In recent years, the late interaction reranking model ColBERT, TILDE, BECR provide reasonable performance with low query latency. We demonstrate that pipelines with such efficient models can be improved using our training strategy. 


In our work, we train the efficient reranker and retriever iteratively to improve the integrated performance of the two stage pipeline through a process termed dynamic integrated training.
 To achieve optimal performance under such setting, when training the reranker, we upweight the poorly ranked samples in the joint pipeline through a soft-hard loss. In the meanwhile we gradually update the training set with the top combined ranked results from pipeline during training. With these shifts, the model will automatically be geared towards the weak point of the joint ranking results of the pipeline. In addition, we employ the top documents retrieved by the retriever to provide additional ranking signal in both training and evaluation in the reranking stage. 


During inference, the retriever would return top documents and their corresponding rank order to formulate a pseudo query. The reranker then matches both the original query and the pseudo query with top documents to get two ranking scores for each query-document pair. As the reranker is trained as a booster, the final ranking order from the pipeline naturally becomes the combination of the retrieval and reranking ranked lists. The final top-k ranking scores is determined by the reciprocal ranked fusion~\footnote{https://plg.uwaterloo.ca/~gvcormac/cormacksigir09-rrf.pdf} of ranks given by both the retrieval and reranking models.

We find that the propose integrated strategy enjoys several advantages. First, under same model setting and training condition, the dynamic integrated training strategy improves the relevance of the two stage pipeline under both scenarios where reranker is an efficient one or reranker strongly outperforms retriever on MS MARCO passage dataset and TREC19 and TREC20 datasets. This indicates that the integrated training strategy is generally applicable.  Secondly, as the two models learn slightly different goals, the joint performance of the two is less likely to overfit. Indeed, we observe a good zero-shot performance of the pipeline on the BEIR dataset. Lastly, we find that our training strategy can be applicable to the currently popular sparse and dense retrieval pipeline where two retrieval models jointly determine the final ranking list. 

}


==> clustmethod.tex <==
%\section{SRF with Query-Specific Cluster Skipping }
%\section{CluSD: Selective Dense Retrieval}

  
\section{Selective Dense Cluster Retrieval}
\label{sec:clusd}
\comments{
It is common practice to interpolate the results from a sparse system and a dense system. We propose two directions to improve the latency of such system by avoiding the unnecessary dense evaluation on query level and per query level. We envision a hybrid system where sparse retrieval runs first and partial query and documents are evaluated by the dense retrieval system. 

The proposed CluSD method contains two components  during runtime inference to 
decide if  dense retrieval augmentation  can be skipped for a query and which  top dense document clusters should be selected  during supplemental retrieval.
}

%Per-query inference latency depends on the number of document evaluated and how per query-document evaluate is approximated. We do not touch per-query-document approximation in this paper and focus on reducing the number of documents evaluated. We cluster document using kmeans as IVF and would like to intelligently select a few most promising clusters to retrieve candidate results. 
\comments{
\begin{figure}[h!]
    \centering
    \includegraphics[scale=1.0]{lstm.png}
    \caption{LSTM prediction for each query}
    \label{fig:lstm}
\end{figure}
}
As discussed earlier, documents with embedding vectors are clustered based on their similarity to the cluster centroids. 
\comments{
Our experiments take an advantage of the FAISS library which  provides such a support such as k-mean clustering.
Once a query is determined by CluSD to trigger  partial dense retrieval that selects and visits a subset of dense clusters. 
% online inference  will  visit the dense clusters one by one in
%an incresing order of   their centroid distance to the input query.
%A decision procedure is invoked to decide if a cluster to be visited should be skipped or not. 
}
Our objective is to examine the features of each cluster and  incrementally decide if this cluster should  be visited or not.
This section will first describe the overall flow of CluSD in online inference for selective fusion of sparse and dense retrieval,
 then present an LSTM-based  cluster selection algorithm. 


\subsection{ Online inference}
\begin{figure}[htbp]
    \includegraphics[scale=0.75]{sparse_dense_flow_lout.drawio.pdf}
    \caption{The flow of cluster-based selective dense retrieval}  
% \vspace*{-1mm}
    \label{fig:flow}

\end{figure}





%Step 3. Call the LSTM selection (Section 4.1)  to choose a small number of dense clusters. That is about 25 in our MS MARCO evaluation.





The online inference algorithm of CluSD has the following steps.

Step 1:   Conduct sparse retrieval to obtain top $k$ results.

%\item Condcut the query filter  to determine if the cluster-based dense retrieval is necessary.If needed, 
%Step 2:  Sort clusters based on the overlap degree of dense clusters and top sparse retrieval results and their  centroid-to-query  distances.

Step 2:  Collect key features for all clusters. These features include the overlap degree of dense clusters and top sparse retrieval results and their centroid-to-query distances.

Step 3: Select top $n$ of the above clusters and call an LSTM procedure to choose  a limited and small
 number of dense clusters as discussed in Section~\ref{sect:lstm}. 

Step 4: Expand top $k$ sparse retrieval results to include the document vectors of these dense clusters and
merge their sparse and dense scores with a linear interpolation.  

%During the above linear interpolation, only top $k$ of sparese retrieval contains a lexical score,
%and thus we  impute the lexical scores of other documents expanded by cluster-based selective dense retrieval 
%as the bottom document score in the top $k$ sparse retrieval list scalled by a factor. We use 0.95 in our evaluation.
\comments{
Notice that  the two ranked lists from two retrievers are usually not fully overlapped and  some documents only exist in one list. While
different  treatments on these documents affect fusion performance,
we resort  to  impute the score of such a document using  the top $k+1$ score   in the missed rank list scaled by 
a factor.
%While there are options to We consider a few options
For example,  we  impute the lexical scores of new documents added  by dense retrieval
using  the scaled lexical score of  top $(k+1)$ in the sparse retrieval list. We use scale $0.95$  in our evaluation.
}
%\item Remove the documents when they only exist in one ranked list
%    \item  Take the document and compute the score for only one ranked list

%When we have access to a relatively strong sparse retrieval system and a dense retrieval system, it is feasible to selectively choose queries that requires evaluation of both systems. We hypothesize that the sparse system is economical and we can afford to run it for every query. The problem boils down to dynamically select queries to evaluate by dense retrieval.

{\bf Online computing and space  cost for augmentation.} We only consider cost of  augmenting sparse retrieval results with dense retrieval during online inference. 
The space cost of dense retrieval is $O(D)$  for a corpus with $D$ vectors.
For MS MARCOS, the cost is around 27GB without compression. Quantization can  reduce that  0.5GB  to 1GB or less based on codebook parameters.
Then this cost becomes a fraction of sparse retrieval index cost.  
Excluding dense embeddings, the extra space overhead  for CluSD is to maintain  the similarity among centroids of $N$ clusters, which is  $O(N^2)$.
This cost is  negligible compared  to the embedding space with $N << D$.  In our evaluation, 
%we use  $N=8192$ or  $4096$.
the inter-cluster similar graph for MS MARCO passages with $N=8192$ takes about 32MB with quantization.

The time  cost of CluSD is dominated by the cost of cluster selection and  dense similarity computation of selected dense clusters.
The former is about $O(n)$ while the later is
proportional to the number of clusters selected, which is capped by $O(\frac{D}{N} n)$. 
In  our evaluation of MS MARCO and BEIR, $n$ is chosen to be 32, and
the actual number of clusters selected and visited is about 25.
%Given the short time added by the pruned LSTM model, 
The overall latency overhead introduced by CluSD is fairly small. 




\subsection{Selection of dense clusters with LSTM}
\label{sect:lstm}

%{\bf LSTM design.}
%Because this decision procedure uses the document scoring information  of each cluster visted 
We adopt a simple LSTM model based on  a recurrent neural network~\cite{hochreiter1997long}, 
taking a sequence  of clusters as an input along with their features.
Assume there are $N$ document clusters grouped using dense document embeddings, and 
it is time consuming for the LSTM model to examine all clusters. Thus
 we truncate the sequence of clusters at maximum length $n$ and then take a sequence of top $n$ clusters as the input to this LSTM. 
There are  $n$ nodes corresponding to these clusters in the LSTM model.
We will discuss how to truncate with a prioritization shortly below.

\begin{figure}[htbp]
    \includegraphics[scale=0.75]{dense_separse_feature_lout.drawio.pdf}
    \vspace*{-1mm}
    \caption{Illustration of CluSD and its features.}
    \label{fig:features}
%     \vspace*{-5mm}
\end{figure}


\comments{
The LSTM model outputs 1 for each cluster node if this cluster should be visited to perform the corresponding dense retrieval.
The goal of this procedure  is to visit  dense clusters as few as possible while still delivering a competitive fusion performance.
The number of predicted clusters are different across queries and the overall budget is controlled by the prediction threshold.
}
%  a few clusters as possible to recover the top results from the original dense retrieval. 
%The label of each query-cluster is 1 when the cluster contains the top k results of the query in the exact full search of dense retrieval.  
%The input is the a sequence of cluster nodes in the order of the centroid-query distance. 
%The feature of each input include: statistics on query-centroid distance, centroid-to-centroid distances, distribution of sparse top results across clusters. 
%The model will predict for each query which clusters to choose. 
%The input features of our proposed LSTM model are listed below.
%These clusters are sorted by the the similarity distance of the given query with the  centroid of each cluster.



Given the above  $n$ top clusters,
 the LSTM computation flow goes from the left most cluster called $c_1$ to the right most $c_{n}$.
Assume the current cluster is $c_i$,  
the LSTM computation outputs a predicted value $f(c_i)$ where $0\leq f(c_i) \leq 1$.
If $f(c_i) \ge \Theta$, where $\Theta$ is a predefined prediction threshold, then cluster  $c_i$ should be visited. In practice, the strictness on selecting a cluster to evaluate is controlled by $\Theta$ and it can be determined based on the overall latency requirement. 

\comments{
When the dense vectors of all documents are grouped into $N$ clusters, 
we limit our cluster search scope into top $n$ clusters in terms of query and cluster centroid similarities. 
we limit $n=128$ in our evaluation out of 1000 clusters.
%Query-specific information derived from  dense clusters:
}

As shown in Figure~\ref{fig:features}, the feature input vector for the current cluster  $c_i$ for the above LSTM computation to produce $f(c_i)$
%$f(q, c_i)$  
is composed of:
\[
[ sim(q,c_i),   
\{ AvgDist(sim(c_i, c_l) \text{ for } c_l \in A_j) \}^u_{j=1}, 
\]
\[ 
     \{  |c_i  \cap  B_j|    \}^{v}_{j=1},  
\{  AvgScore (c_i  \cap  B_j)    \}^{v}_{j=1} 
]. 
\] 
\begin{enumerate}[leftmargin=*]
    \item $sim(q,c_i)$: The similarity distance of this query $q$ with the centroid of cluster $c_i$.  
  %\item  $\{ sim(c_i, c_j) \}^{n-1}_{j=0}$: The distance vector between the centroid of $c_i$ to  all other clusters.
%the top  clusters that have been visited (or skipped).  We limit this number as $K=128$.
%other top k centroids for this query (k=128)??
  
\item  \{  $AvgDist(sim(c_i, c_l)) \text{for } c_l \in A_j \}^u_{j=1}$: 
The mean distance between this centroid and the centroids in each of $u$ position bins $A_j$.
%These six bins  are formed by partitioning all clusters into consecutive position bins.
%For example, $A_1$ contains clusters from Postions  1 to 5, Positions 6-10, 
%$A_2$  contains clusters from Postions  6 to 10, and so on.   Bin $A_6$ contains the rest of uncovered clusters.  
These $u$ position bins  are formed by cluster centriods. 
After all the $N$ centroids are ordered based on a criterion discussed shortly, we partition the sequence of sorted clusters into $u$ consecutive position bins.

The purpose of this feature group is to capture the distances of a cluster to previously examined clusters and unexamined clusters following the LSTM flow. 
When the mean distance  between cluster $c_i$  and clusters in a previously-examined  bin is close, if  many clusters in that bin have been selected, cluster 
$c_i$ may have a good  chance to  be selected.
In our evaluation with MS MARCO and BEIR datasets, we found that $u=6$ is appropriate and 
these 6 bins respectively contain clusters in Positions  1-5, Positions 6-10, 
Positions 11-20, Positions 21-50, Positions 51-100, and the rest of N clusters. 

%Since the clusters are processed from a lower position to a higher position one by  one,
%these features represent the distance to the groups 
    
    \item $ \{  |c_i  \cap  B_j|    \}^{v}_{j=1} $ and $\{  AvgScore (c_i  \cap  B_j)    \}^{v}_{j=1} $: 
The number of documents and average sparse ranking score from this  cluster contained in each of   the $v$ bins $B_j$  formed by
top $k$ sparse retrival results.
These bins are called $B_j$ where $1\leq j \leq v$. 
The purpose of this feature group is to capture the overlap degree  of a cluster with the top results of sparse retrieval.
A cluster that contains many top sparse results may be selected.

In our evaluation with  retrieval depth $k = 1000$ for MS MARCO and BEIR datasets,
top $k$ sparse results are divided into $v$ bins where $v=6$, and these bints are top 10, top 11 to 25, top 26-50, top 51-100, top 101-200, top 201-top 500, and 
top 501 to k documents.  

    %\item $\{  AvgScore (c_i  \cap  B_j)    \}^{6}_{j=1} $: 

% bin 
%top 10/25/50/100/200/500/1000 documents  in the sparse retrival results.
\end{enumerate}



%Section~\ref{sect:evaluation} provides more details on the effectiveness 
 

\textbf{Pruning to obtain top $n$ candidate clusters.} 
As discussed earlier,  we control 
the input length  of the above  LSTM model  to be  $n$  as 
the number of top candidates clusters to be examineds, and then the inference 
time complexity of the LSTM model is limited by $O(n)$.
%We denote $n$ as the  input length  to our LSTM  throughout the rest of this paper.
We devise a strategy below to select top $n$ candidate clusters 
from  the $N$ total number of clusters.
Namely we prune clusters that may not provide a meaningful boosting of relevance quality. 

\comments{
Table ~\ref{tab:LSTMclustertime} shows that as the number of clusters to be examined
varies from 32 to 512, the LSTM inference time increases from  2.8ms to 33.9ms.
As we would like to make a quick decision given the overall  time budget,
we devise another strategy to prune clusters that may not provide a meaningful boosting
of relevance quality. 

% dependent on the length of the sequence input. 

\begin{table}[h]
	\centering
		\resizebox{0.68\columnwidth}{!}{ 
%		\begin{small}
		\begin{tabular}{r | rrrrr}
			\hline\hline
			  \#Clusters examined & 512 & 256 & 128 & 64 & 32 \\
\hline
            Time (ms) & 33.9 & 16.2 & 6.2 & 3.8 & 2.8\\
                \hline\hline
		\end{tabular}
%		\end{small}
	}
	\caption{LSTM inference time with different input length.}
	\label{tab:LSTMclustertime}
 \vspace{-7mm} 
\end{table}

\comments{
\begin{figure}[htbp]

    \includegraphics[scale=0.27]{dist.pdf}
    \caption{Distribution of Good Documents }
    \label{fig:dist}
%\vspace{-1em} 
\end{figure}
}
}

To prune clusters, one may prioritize a few top clusters sorted by the query-centroid distance.
We find this does not work well in the context of augmenting sparse retrieval results for MS MARCO passages.
For example, if we rank clusters based on the query-centroid distance, many of top 10 dense results reside
in clusters ranked beyond 175. 
  

\comments{
Table~\ref{tab:dist} shows the distribution of top 10 documents from the full dense retrieval  
in embedding clusters under the different query percentile when searching an MS MARCO passage dataset using queries from its  Dev set. 
Row 2 of Table~\ref{tab:dist} shows the number of top clusters needed to cover  top 10 
documents from the full dense retrieval  when clusters are sorted by sorted by  the query-centroid distance.
This row shows that to cover top 10 dense results, $n$ needs  to be larger than 175.
%On the other hand, Row 2 is  the number of lusters decided by the LSTM to visit  under the different query percentiles. 
%At most  66 clusters are  selected  by the LSTM model for all queries.
%We further propose to skip unnecessary clusters. 
\begin{table}[h]
 \vspace*{-1mm}
	\centering
		\resizebox{0.78\columnwidth}{!}{ 
%		\begin{small}
		\begin{tabular}{r |r  r r r r}
			\hline\hline
			  Query percentile & 10\% & 50\% & 75\% & 90\% & 95\% \\
            \hline
%            \#clusters selected by  LSTM & 1 & 4 & 14 & 40 & 66\\
            %Relevant doc coverage & 1 & 2 & 7 & 29 & 69\\
             Top 10 dense result coverage & 1 & 6 & 25 & 92 & 175\\
                \hline\hline
		\end{tabular}
%		\end{small}
	}
	\caption{ Distribution of  top 10 dense results in sorted clusters 
% \% of Good Documents Among Clusters Sorted by Query-Centroid Distance
}
 \vspace*{-5mm}
	\label{tab:dist}
\end{table}
}


%provides an explanation.  evidence on the effectivness of the above LSTM model.
%After searching an MS MARCO passage dataset using queries from the MAMARCO dev set, 
%under the different query percentile shown in Row 2 is  the number of clusters decided by the LSTM to visit.
%Row 3 is  the number of clusters needed to 
%For a lot of queries, the top 5 or even top 10 clusters do not contain enough information, for example, around 10\% of queries need more than 92 top clusters to recover the top results from the full dense retrieval. It demonstrates the necessity of doing cluster selection and skipping.  
%On the other hand, there is a reasonable distribution resemblance between  Row 2 and  Row 3, which shows the LSTM model provides a reasonable guidance on where relevance results are.
%%While it does not exactly follow the distribution of top 10 results of sparse retrieval, the feature 
%From  Table~\ref{tab:dist}, we observe that
%the distribution of top 10 results from a sparse are contained is not necessarily concentrated in the top  clusters.
Since our ablation  analysis finds that Group  (3) of the above feature list
is important for the accuracy of LSTM to make a sound cluster selection, we resort to this feature group in making 
a preliminary selection of  necessary clusters. 
%With the above design consideration,  we propose to use the following strategy to 
%sort the candidate clusters based their feature vectors from Group  (3).
Specifically we rank candidate clusters by   the overlap degree of a cluster with the $v$ top sparse retrival result bins. 
If there is a tie between two clusters, then we rank them by their centroid distance to the query.
%We first use a simple heuristic to reorder the clusters, refered as Top K heuristic. 
%We order the clusters based the six features then 
%followed by q-c-orders. 
Then, the  top $n$ ranked candidate cluster list is used as the input sequence to the LSTM model. 
%We will stop the LSTM computation of  this list
%after visiting $\tau$ clusters and when the predicted $f(c_i)$  values of a few consecutive clusters are all below a threshold. 
%For our evaluation in MS MARCO and BEIR datasets, $\tau=20$. 
In our evaluation, we find that a relatively small number such as $n=32$ is a solid choice  to yield competitive results  after the above cluster sorting and prioritization.
%As a result, the LSTM computation for cluster selection can be completed within  1.8 milliseconds. 
%The number of clusters selected varies from a few to 20 on average, which yields a quick argumentation with dense cluster results.


%Features marked with Hexgos 1 and 4 are used for a boosting tree to make a decision if cluster selection should be triggered or not.
\comments{
\subsection{Query filtering}
%When computing the embedding of each query token or the whole  original query, we use 
%the denser retriever's encoder. 


We also exploit the possibility to skip dense retrieval completely.
Modifying the above LSTM-based decision mechanism does not yield a satisfied result.
We sort to add a classifier with  boosted decision trees with supervised learning
to make an earlier  determination before triggering the LSTM computation.
}
\comments{

a query needs an argumentation from dense retrieval 
%A challenge is to identify features and infer based on such features with supervised learning.
Given that sparse retrieval is conducted first,
our idea is to predict the quality of sparse retrieval and its relative strength  compared to unexecuted
dense retrieval based on quality of query token expansion by the sparse model,
the statistical behavior of  sparse retrieval results, and
the relationship between dense document embedding summary and sparse retrieval scoring structure.

}


\comments{
\begin{table}[ht]       
    \centering          
%    \resizebox{1.05\columnwidth}{!}{

\begin{small}                        

    \begin{tabular}{l |l}
        \hline
    Query    & "how long nyquil kicks in"\\
    \hline
 Query Expanded&["in", 36],  ["time", 74], ["years", 71], ["long", 97], \\
 & ["total", 60],\textcolor{red}{["move", 23]}, ["effect", 22], \textcolor{red}{["weapon", 21]}, \\
 & \textcolor{red}{["jump", 24]}, ["kick", 100], ["ny", 111], ["timing", 34], \\
 & ["kicks", 76], ["\#\#quil", 139]\\
    \hline  
Relevance Doc &["\#\#quil", 410.1], ["ny", 301.0], ["long", 216.7], \\
& ["time", 134.7], ["years", 131.5], ["total", 87.4],\\
& ["effect", 34.4], ["timing", 17.4]\\
\hline
Top 5 Doc & ["\#\#quil", 392.6], ["ny", 295.7], ["kick", 236.1], \\
& ["long", 198.3], ["time", 141.2], ["years", 116.9], \\ 
& ["kicks", 101.8], ["total", 86.3],\\
& ["in", 35.3], ["effect", 24.1], ["timing", 23.6],\\
& \textcolor{red}{["jump", 10.0], ["move", 6.0]}\\
        \hline
    \end{tabular}
\end{small}                        
%}     

\caption{An example of weak query expansion in SPLADE} 
\label{tab:queryencoder}
\end{table} 
}

\comments{
\begin{table*}[ht]       
    \centering          
%    \resizebox{1.05\columnwidth}{!}{

\begin{small}                        

    \begin{tabular}{l  l l}
        \hline\hline
    Query   &  \multicolumn{2}{l}{ "why do we push others away"}\\
    \cline{2-3}
&  \multicolumn{2}{l}{('push', 105), ('away', 104), ('because', 97), ('others', 94), ('people', 44), ('why', 44), ('purpose', 43), ('cause', 42), (',', 40), ('we', 38),} \\
&\multicolumn{2}{l}{ ('other', 38), ('effect', 33), ('them', 29), \boldred{('responsibility', 28),} ('help', 20), \boldred{('move', 19), ('severe', 17),}  ('step', 17), ('do', 16),...}\\
%& & ('things', 15)， ('fear', 15), ('method', 10), ('to', 6), ('language', 5), ('anger', 5), ('when', 2), ('feeling', 2), ('\#\#ness', 1), ('dangerous', 1)]\\
    \hline  \hline
   Doc Relevant? & \ rank & Text and Expanded Tokens \\
\hline
\comments{
Yes & 17 & From a psychological standpoint, pushing away the people you love the most is a very basic and common, defense mechanism.\\
&& As the relationship develops, people become inundated with their own fears and insecurities that they will not be accepted\\
&& and therefore hurt by their loved one.\\
\cline{3-3}
& & [('push', 198), ('away', 196), ('fear', 127), ('people', 104), ('effect', 81), ('because', 70), ('severe', 67), (',', 61), ('method', 61),
\\
& &  ('when', 59), ('anger', 58), ('dangerous', 55), ('feeling', 53), ('purpose', 53), ('responsibility', 53), ('move', 44), ('cause', 43),... \\
%& & ('them', 37), ('things', 31), ('\#\#ness', 27), ('step', 23), ('why', 13), ('help', 9), ('to', 3), ('do', 1), ('language', 0)]\\
\specialrule{.1em}{.05em}{.05em} 
}
No & 10 & Different types of push factors can be seen further below. A push factor is a flaw or distress that drives a person away from \\
&&  a certain place. A pull factor is something concerning the country to which a person migrates. It is generally a benefit that  \\
&&attracts people to  a certain place. Push and pull factors are usually considered as north and south poles on a magnet.\\
\cline{3-3}
&& [('push', 283), ('away', 162), \boldred{('move', 80),} \boldred{('severe', 74)}, ('people', 70), ('because', 68), ('effect', 58), ('cause', 44), ('purpose', 43),\\
& & \boldred{('responsibility', 41),} (',', 36), ('method', 35), ('\#\#ness', 33), ('step', 23), ('them', 22), ('to', 18), ('when', 13), ...\\ 
%& &  ('things', 11), ('anger', 9), ('dangerous', 8), ('fear', 3), ('do', 0)]\\
\specialrule{.1em}{.05em}{.05em} 
No & 8& Most of the universe is rushing away from us. It\textbackslash{}'s not that we\textbackslash{}'re particularly repellent; it\textbackslash{}'s just that the universe is\\
&&  expanding, pushing most other galaxies away. Light from distant galaxies travels toward us through this \\
&& expanding space, which stretches their light to longer, or redder, wavelengths.\\
\cline{3-3}
&& [('away', 184), ('push', 158), ('other', 111), \boldred{('move', 103)}, ('we', 101), ('effect', 83), (',', 73), ('because', 66), ('method', 53),\\
&&  ('others', 39), ('cause', 39), ('severe', 39), ('them', 36), ('do', 29), ('things', 29), ('dangerous', 29), ('feeling', 28), ... \\
% & & ('when', 27), ('help', 19), ('purpose', 13), ('to', 4), ('why', 2)]\\
         \hline\hline
    \end{tabular}
\end{small}                        
%}     

\caption{An example of weak SPLADE query expansion that boosts  irrelevant documents  } 
\label{tab:queryencoder}
\end{table*} 

Our consideration 
%is that the necessity of invoking a dense retrieval model after running a sparse model depends on 
%\begin{enumerate}
%the relative strength of results scored by this sparse retriever. If a
    is that  if a chosen
sparse retriever has  well-performed, the benefit of addition of dense scoring  is limited. 
Notice that a learned neural sparse retriever expands the original query with a transformer-based encoder
We found that the quality of query encoding with expansion in SPLADE impacts the quality of sparse retrieval. 
%and we form features using both the original query  and the expanded query.
When  there is a low similarity value  between the original query and the tokens of 
its expanded  query, the confidence for  strong sparse retrieval can be low.
Table~\ref{tab:queryencoder} gives such an example and lists an original query and its expanded query tokens
sorted by token weights.  Expanded query words  in red color
not highly relevant to the original query and they are weighted high in two irrelevant documents, which boosts their ranking.  
Thus    excessive presence of un-similar  query tokens  after expansion  can misrank irrelevant documents. 
Another consideration is that the alignment of sparse retrieval ranking  with the 
query-cluster based similarity can shed light  on the necessity of  dense retrieval.
When top sparse retrieval results are concentrated in a few top  ordered dense clusters, dense retrieval may bear
a resemblance  in  ranking.


With the above consideration  in mind, we use the  following categories of features
to train a boosted decision tree model.

}
% with these featuers an input by using the xgboost package. 
\comments{
To evaluate the performance of the sparse system, we design some features to describe the quality of sparse encoder. 
For example, the length of expanded query, distribution of token impact scores and their corresponding matching scores with top k documents.

To evaluate the discrepancy between the performance of sparse and dense system. We encode the original query with the dense retrieval encode and each expanded token and generate distributional features around the similarity between them. 


%We take a supervised approach to the construction of a query filter that classifies  a query after sparse retrieval 
%needs an argumentation from  dense retrieval or not. We consider the following two categories of the feautres.
}
\comments{
\begin{itemize}[leftmargin=*]
\item Quality of query expansion by the sparse retriever model.
    For example, the query-level matching score, define as the similarity  between the CLS embeddings of the orginal query and the expanded query.
    Another one is the token-based matching histogram vector between the expanded query and the original query. 
For each query token in the expanded query, we evaluate the matching score in terms of similarity
 between its token embedding and  the oringal query embedding. 
We map  these values into five bins with  ranges <0.5, 0.5-0.6, 0.6-0.7, 0.7-0.8, >0.8.
Then derive a matching histgram count  vector for each bin.
}

\comments{
{\bf WILL DELETE THIS LIST.}
\begin{enumerate}
    \item The length of the original query and the expanded query in terms of  the  number of words or tokens, respectively. 
    \item The token-based matching  vector between the expanded query and the original query. 
For each query token in the expanded query, we evaluate the matching score in terms of similarity
 between its token embedding and  the original query embedding. 
We map  these values into five bins with  ranges <0.5, 0.5-0.6, 0.6-0.7, 0.7-0.8, >0.8.
Then derive a matching count vector based on this bin mapping???
    \item The query-level matching score, define as the similarity  between the CLS embeddings of the original query and the expanded query.
    \item The sum of matching scores within each of above token similarity bin, divided by
the  query-level matching score. 
%The token groups are the tokens with similarities in each bin.
    \item The sum of matching scores of tokens not in NLTK English corpus, divided by  the query-level matching score. 
    \item The number of overlapping tokens between expanded and original query / number of all unique queries in both expanded and original query.
    \item number of  tokens only in expanded query / number of all unique queries in both expanded and original query.
    \item overall/mean/max of token weight of overlapping tokens between expanded and original query in the expanded query.
    \item max/min/mean of token weights of expanded query tokens.
\end{enumerate}

}
%\item
\comments{
Ranking characteristics of documents scored by sparse retrieval.
We compute  the mean sparse retrieval score of top 10-20/20-30/30-40/40-50/50-100/100-400/400-700/700-1000 documents.

%Sparse  retrival score distribution:
\begin{enumerate}
    \item Sparse retrieval scores of top 10 results
    \item The mean sparse retrieval score of top 10-20/20-30/30-40/40-50/50-100/100-400/400-700/700-1000 documents.
\end{enumerate}
%Sparse and Dense relational features:
\item Overlapping degree of sparse retrieval with dense clusters:
\begin{enumerate}
    \item The number of dense clusters containing top 5/10/20/50/100/1000 results from sparse system
\end{enumerate}
}

%\end{itemize}


%\subsection{Partial Document Evaluation}
{\bf Training of LSTM.} 
We assume that the training data  contains
a set of queries and relevance-labeled documents,  that allows the computation of a ranking metric such as MRR or NDCG.
For example, from MS MARCO training set we randomly sample 5000 training instances, where each training instance contains a query and  one or more  relevant documents. 
%Then we run a sparse retriever this instance, and seperately run a fusion with a dense retriever. If the result of sparse retriever results merged with dense results  exceeds the standalone sparse retrival,  we label consider training instance as an positive example for dense retrieval, otherwise consider this as a negative example. The converted training isntances are used for training In this way, we convert a set of training instances for ranking as a set of training instances for fusion.
To train the LSTM for cluster selection, 
for each training instance, we mark the positive and negative examples for  top clusters.
If a cluster contains one of top 10 sparse retrieval results, we mark this cluster should be visited.
Otherwise this cluster should not be visited.


 
\comments{
We convert We define the labels as 
\begin{equation}
       y(q)= 
\begin{cases}
    1,& \text{if } U(s(q), d(q)) > U(s(q))\\
    0,              & \text{otherwise,}
\end{cases}
\end{equation}
where $U(.)$ is a evaluation metric we choose, for example, NDCG@10 or MRR. $s(q)$ is the scoring of a sparse system of query $q$ and $d(q)$ represents the scoring of a dense system.
}

\comments{
\subsection{How to combine two ranked list}
There are two commonly used method to combine the sparse and dense ranked lists:
\begin{enumerate}
    \item linear combination
    \item reciprocal rank fusion
\end{enumerate}
For linear combination, the final ranking score of a document is the weighted sum of the ranking score of two systems respectively. The weight on each system can be determined through grid search on a left-out training set or just use 1:1 combination. In this case, rescaling of the two ranked lists are necessary as the it largely affects the impact of a ranked list to the merged ranked list. 

On the other hand, reciprocal rank fusion alleviate the scoring distribution difference by only considering the ranking positions when merging. 
  Another consideration is on the missing values. The two ranked lists are usually not fully overlap. Some documents only exists in one ranked lists. Thus 
the treatment on these documents affects model performance. We consider a few options
\begin{enumerate}
    \item Remove the documents when they only exist in one ranked list
    \item  Take the document and compute the score for only one ranked list
    \item Impute the missing document with rank K+1 or score as 0.95 * min(score) in the ranked list.
\end{enumerate}

}




==> clustprob.tex <==

%\section{Problem Definition}
%\section{Background and  Design Considerations}
\section{Design Considerations}
\label{sect:background}

\comments{
\begin{table}[h]
	\centering
		%\resizebox{1.02\columnwidth}{!}{ 
		\begin{small}
		\begin{tabular}{l l}
			\hline
			Symbol & Def. \\
                \hline
                %$\mathcal{D}$ & A set of documents in a dataset\\
                %$N$ & Total number of documents in a dataset \\
                $Q$ & A query \\
                $d_i$ & A document \\
                $\mathcal{D}^{+}$, $\mathcal{D}^{-}$ & Positive/negative document subsets corresponding to $Q$  \\
                $|.|$ &  The size of a set\\
		$\Theta$& Parameters of a scoring model\\
		$S(Q,d_i, \Theta)$ & The rank score of a document for a query using a model\\
%			& based on a model with parameters $\Theta$. \\
                $p_i$ & Teacher's top one probability of document $d_i$,\\
			& standing for  $P(d_i|Q, \mathcal{D}^+, \mathcal{D}^-, \Theta$) \\
                $q_i$ & Student's top one probability of document $d_i$\\
                $\pi(.)$ & The rank position of a document for a query\\
                $\beta_i$ & Exponent weight bias for negative  document $d_i$\\
                $\gamma, \alpha$ & CKL hyper-parameters\\
                \hline
		\end{tabular}
		\end{small}
	%}
	\caption{Table of Symbols}

	\label{tab:data}
\end{table}
}


{\bf Problem definition.}
Given query $q$ for searching a collection of $D$ text documents:   $ \{d_i\}^D_{i=1}$, 
retrieval  obtains the top $k$ relevant documents from this collection based on
the similarity between query $q$ and a candidate document  $d_i$ using  their
representation vectors.
Sparse retrieval uses  the dot product of their lexical or learned representation vectors as the similarity function
and implements its search efficiently using an inverted index. 
%\begin{equation}
%\label{eq:sparseretrieval}
$L(q) \cdot  L(d_i)$
%\end{equation}
%L(q,d_i ) = 
where $L(.)$ is a a vector of weighted term tokens for a document or a 
query~\cite{Robertson2009BM25, Dai2020deepct, Mallia2021deepimpact, Lin2021unicoil,2021NAACL-Gao-COIL}. 
\comments{
For BM25 based lexical representation~\cite{Robertson2009BM25}, 
$L(.)$ treats each document or a query as a bag of terms
and term weights  are scaled based on   frequency of terms within a bag and  across all bags involved.
For a learned sparse representation~\cite{Dai2020deepct, Mallia2021deepimpact, Lin2021unicoil,2021NAACL-Gao-COIL}, 
a document or a query is encoded using  a learned neural model, which
produces a bag which may contain original  and  expanded terms.
The encoding functions for a query and document can be different. Without the loss of generality, we assume they are the same in this paper.
}
Dense retrieval with a single vector representation computes the following rank score
%\begin{equation}
%\label{eq:denseretrieval}
$R(q) \cdot  R(d_i)$
%\end{equation}
%D(q,d_i) 
where $R(.)$ is a dense representation vector  of a fixed size~\cite{Karpukhin2020DPR}.
%In a single-vector dense  representation, each  representation vector of a document or a query is a dense vector. 


  %revises the SparTerm model~\cite{Bai2020SparTerm} to predict the weight 
%The weights of these terms evaluated in this paper use the SPLADE model as discussed below while other options are possible.
%(e.g., a bag of words or a neural encoder). 
%The implementation of such a dot product for a sparse retriever uses the inverted index data structure.
\comments{
%{\bf Learned term weights with SPLADE}.
For each document, the SPLADE term weighting revises the SparTerm model~\cite{Bai2020SparTerm} to predict the weight 
score $w_j$ of $j$-th token term in BERT WordPiece vocabulary as
%\begin{equation}
%\label{eq:splade}
$w_j = \sum_{i \in d}  log (1 + ReLU ( H(h_i)^T E_j + b_j)) $
%\end{equation}
where document $d$ consists of a sequence of BERT last layer's embeddings $(h_1, h_2, $
$\cdots, h_n)$.
$E_j$ is the BERT input embedding of the $j$-th token and $b_j$ is a token level bias.
$H(.)$ is a linear layer with activation and layer normalization. 
% (In SPLADE GeLU activation is used). 

{\bf Combining the results of a dense retriever and a sparse retriever.}
}
Following the work of~\cite{kuzi2020leveraging, 2022LinearInterpolationJimLin, Gao2020ComplementingLR}, 
linear interpolation is used  to  ensemble  dense and sparse retrieval scores. 
%Let $S$ be the set of top results obtained by a sparse retriever, and $D$ be
%be the set of results obtained by dense retrieval. 
%For any document $d_i \in S \cup D$, its  
The fused rank score for document $d_i$ in responding  query $q$ is:
%\begin{equation}
%\label{eq:fusion}
$\alpha L(q) \cdot  L(d_i) +
(1-\alpha) R(q) \cdot  R(d_i) $
%\end{equation}
where $\alpha$ is a coefficient in a range between 0 and 1.
\comments{
Notice that   the two ranked lists $S$ and $D$ are usually not fully overlapped and  some documents only exist in one list. While 
different  treatments on these documents affect fusion performance,
we take an option to  impute the score of such a document score   using $\beta * score (top \  k+1) $  in the missed  ranklist where $\beta$
is a scaling factor.
%While there are options to We consider a few options
For example,  we  impute the lexical scores of documents expanded by dense retrieval
as the top-$(k+1)$ lexical  score scaled by a factor. We use $\beta=0.95$  in our evaluation.
 
%\item Remove the documents when they only exist in one ranked list
%    \item  Take the document and compute the score for only one ranked list
}
Our optimization goal is to select a small number of dense vectors to fuse after sparse retrieval 
while maintaining a relevance competitive to the full dense retrieval  which searches  the entire document set. 
\comments{
In this way, limited dense retrieval that augments sparse retrieval is fast with minimum space consumption  on a CPU server. 
The ensembling method used in our evaluation is 
%The final ranking of the top $K$ documents is 
the reciprocal rank fusion (RRF) following Cormack et al.~\cite{Cormack2009RRF}, considering ranking positions of each candidate 
generated by a retriever and by a re-ranker. 
We use RRF
% above reciprocal rank fusion 
instead of linear interpolation as it has a similar performance with a simplified combination of two scoring models. 
%We choose RRF because it is easily applicable to multiple ranked lists ignoring the score distribution differences. 
\begin{equation}
     %RRF(Q,d) =  \sum_{r \in {rt, rr,}} \frac{1}{k_r + r(d)},
     RRF(Q,d) =  
\frac{1}{c_1 + \pi_1(d)} + 
\frac{1}{c_{2} + \pi_2(d)},
     \label{eq:score}
\end{equation}
where $c_{1}$ and $c_{2}$ are fixed smoothing constants. $\pi_2(d)$ is the rank position based  a re-ranker formula
while $\pi_1(d)$ is the rank position based on a retriever.
}



==> concl.tex <==
%\section{Limitations and Future Work}
\section{Concluding Remarks}

The contribution of this work is a cluster-based dense retrieval selection scheme  
to augment sparse retrieval with minimal space overhead and a small amount of extra latency  time.
CluSD optimizes an LSTM based model with cluster prioritization and pruning
to effectively identify  a small number of clusters that can supplement and boost  sparse retrieval. 
With this lightweight low-cost design,  
CluSD can deliver a strong in-domain and out-of-domain relevance  efficiently when searching  MS MARCO and BEIR datasets
on a CPU only server. %even though the sparse retriever used has its relevance tradeoff under a time efficiency constraint.
For example, CluSD delivers 0.423 MRR@10  for searching 8.8M MS MARCO passages 
with 11.4ms  latency and  1.13GB space mainly for compressed dense embeddings, to augment sparse retrieval under
a fraction of its  cost. The same  CluSD version  reaches  0.514 average NDCG@10 for BEIR with compression.

Compared to other baselines, the main advantage of CluSD is its capability in delivering the similar 
%or higher
relevance under the same time budget
with negligible extra space overhead. It is attractive to run such an algorithm on a first-stage retrieval low-cost machine
%to host  as many documents as possible and 
that can  significantly reduce the overall infrastructure cost when scaling  data size and  search traffic. 


Our evaluation uses OPQ in FAISS to compress embeddings. 
Switching to a different quantization affects the compression ratio and  the relevance outcome.  
However, we expect that our findings remain similar because  the recent  quantization 
methods~\cite{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ}
also have  a significant relevance drop pattern when the compression ratio increases.
%A limitation of the current  CluSD work is that the training of the LSTM model has a dependence on the sparse retrieval model used. 
While  CluSD can  boost the relevance of a weaker sparse retriever model such as BM25, the augmented relevance still has not reached a level
comparable  to the one where CluSD is coupled with a stronger sparse retriever. There is room for improvement in future work.

%the dependency on a training dataset. Unlike rule-based or unsupervised pipelines, our pipeline requires labeled data on at least one search task. However, the number of queries with labels is not large and a trained model is robust on never-seen corpus and tasks. 
%
%Another limitation is the dependency on the sparse retrieval model performance. CluSD benefit from a good sparse retrieval top results. When using a BM25 based retrieval, the quality of the clusters selected degrades slightly. 


==> design.tex <==

\comments{
Sparse retrieval with a learned representation  is much slower than BM25
        Guided sparse retrieval can speedup, but there is a trade in  effectiveness
        Agumenting sparse retrieval with dense retrieval through fusion can make up the loss
        Selective dense  retrieval can make up the loss argument sparse retiieval more effective with limited extra computing cost.

Points to market: Option 2

                New dense retrieval algorithms have been developed every year that beat new performance records.
                New fast  sparse retrieval algorithms are developed.
                Fusion of  sparse retrieval and dense retrieval is helpful, but slow on a CPU server, dominating by dense computation.
                There is a clear redudance of computation as both retrievers scan the same dataset with different representation
                        for push for the same top documents.
                How to avoid redudant computation?
                        1) Select dense retrieval. We donot need to scan all dense documents. We can take advanrage of
                clusters of dense documents
                        and only  need to visit top clusters which are similar to a query.
                        2) The use of dense retrieval reduces the relevance reqirement of sparse retrieval. We can use a fast sparse
retrieval BM25-guided sparse retrieval or effient SPLADE version, which quickly retrieves top results. Selective dense retrieval
                can augment  a weaker but faster sparse retriever by only adding limited  extra computing cost
to  improve the recall and relevance metric.

                Challenges:
                        1) How to accomplish  selective clusetrs.
                        Which clusters  can make most contributions
                        2) What queries definitely need dense retrieval boosting?

}
\section{Design Considerations}
\label{sect:design}

\comments{
The availability of a dense retriever model, possibly  trained separately by a different language model,
offers opportunities to re-confirm and adjust the ranking of top quality documents in  the initial
candidate pool and improve the  recall by introducing more diversified
candidates.  On the other hand, there is a clear redundancy of computation as both retrievers visit the same dataset 
with different representation, possibly  pursing the  same subset of top documents.
}
 
%{\bf Yingrui, please add a table or figure which shows the distribution of training
%queries if possible, otherise the Dev set of MS MARCOS,  that has the various level of MRR increase.
%I remeber you show us some data you collected during summer or spring.} 
%Table~\ref{tab:fusionanalysis} shows 



%We found that among 33\% of queries in the MSMARCO training set, there is no increase in terms of the MRR@10 when dense retrieval results are added to sparse retrieval results. Namely there are many queries that do not actually benefit from the use of dense retrieval after sparse retrieval.
% two retrievers, and explicitly skipping some of fusion can avoid the unnecessary computing cost.
%Motivated by the above data, 

%Our design considerations are:

%of selective dense retrieval  
%has  the following considerations.
%\begin{itemize} [leftmargin=*]
\comments{
\item  {\bf Partial dense retrieval after  full sparse retrieval.}
The experience with the SPLADE model ~\cite{Formal2021SPLADE, Formal2021SPLADEV2} showed that
learned sparse representations from  BERT can be very effective.
For example, without optimization in language model pretraining, SPLADE's MRR performance is on par to
the dense retriever by RocketQA~\ref{Ren2021RocketQAv2}. 
Thus there is an opportunity to skip some of scoring computation in dense or sparse retrieval.
Since it is not easy to recognize and separate part of an inverted index  that contains high scoring documents,
our design choice is  to run a sparse retriever completely first and steer partial dense  retrieval. 

%and also there are several techniques developed recently to accelerate learned sparse retrieval,
}

%\item {Inter-cluster vs. inter-document similarity.}
{\bf Cluster-based  augmentation.}
\comments{
After the  fusion option is determined for a  query,
there is an option to follow LADR~\cite{2023SIGIR-LADR} and select documents that are similar to
the top sparse retrieval results  using a similarity graph.
These similar documents form candidates  for partial dense retrieval and  rest of un-selected
documents in a dataset can be skipped.  
Maintaining a large inter-document similarity graph online is quite expensive from
offline  data collection, online storage space, and   inference time.
}
We intend to exploit coarse grain cluster-level similarity to reduce the complexity in selective dense retrieval with two reasons.
%The challenge is to how to select clusters  which can make most contributions.
%We opt to take a cluster-level skipping approach with two reasons.
1) Documents can be clustered in advance during offline processing based on their embedding similarity where mature clustering techniques 
(e.g.  ~\cite{johnson2019billion}) have  been well developed
and can be leveraged. 
%Documents within a cluster similar to a query can provide a large variety of strong candidates to supplement sparse retrieval results.  
2) Cluster-level computation allows  aggregation of  similarity computation for query-document dot products as a fast matrix operation 
to fully  utilize on-chip CPU caches. 
%In comparsion, there is a less chance for online inference to fully benefit from  CPU cache based on an irregular  graph structure.
%During offline processing, it is computationally expensive to drive document-level similarity for all pairs for documents in a large datset.
A research problem  is how to adaptively identify a subset of clusters  which yield sufficient relevance benefits.
% benefitial fusion if  sparse retrieval scoring may be sufficient. In addition to the influence of sparse retrieval results,
% a dynamically-visited dense cluster may provide sufficient high quality documents, reducing the necessarity of visiting
%the remaining dense clusters.   
%Thus we will develop a dynamic feature-driven decision scheme based the results of sparse retrieval.
%and incremtentally navigated  dense document clusters  as input. 
\comments{
Another consideration is that there are various relevance and efficiency tradeoff in selecting  a sparse retrieval 
model~\cite{Lassance2022SPLADE-efficient,mallia2022faster,Qiao20222GT,2023SIGIR-Qiao,2023SIGIR-SPLADE-pruning}.
For example, BM25 guided-sparse retrieval can greatly speedup, but lose some recall or precision
 when this guidance is weighted aggressively.
The use of dense retrieval provides a flexibility and reduces  the relevance requirement of sparse retrieval.
Namely potentially we can choose a relatively fast sparse retrieval with the slightly lower accuracy/recall,
and  let dense retrieval make up the loss. Our design
needs to  adapt to  sparse retrieval quality and plans
}
We plan to exploit features that reveal  the overlapping degree of top sparse retrieval results with  dense clusters
to guide the selection in addition to query-cluster distances. 

\comments{
\item  {\bf Query filtering for skipping dense retrieval}
We want an online system to make an earlier  determination if a query needs an argumentation from dense retrieval with supervised learning.
%A challenge is to identify features and infer based on such features with supervised learning.
Given that sparse retrieval is conducted first,
our idea is to predict the quality of sparse retrieval and its relative strength  compared to unexecuted
dense retrieval based on quality of query token expansion by the sparse model,
the statistical behavior of  sparse retrieval results, and
the relationship between dense document embedding summary and sparse retrieval scoring structure.

}



{\bf Low-cost budget for balanced effectiveness and efficiency.}
%Our heuristic-based fusion selection may suffer from an effectiveness tradeoff
%as full dense retrieval execution likely offers the maximum relevance benefits.
For time latency, our goal is to minimize the relevance effectiveness loss to a small degree while still accomplishing  a fast response time
acceptable to the interactive search system requirement.
In a search system running as an interactive  web service,  a query with multi-stage processing
needs to be completed within a few hundred milliseconds.
%Considering the multi-stage search nature  and other service overhead involved, 
A first-stage retriever operation  for a data partition needs to be completed within several tens of milliseconds without query caching (e.g. 200ms). 
Our targeted time budget to augment sparse retrieval cannot be too high     compared to  sparse retrieval cost.
We will evaluate the latency budget in two settings: around 50ms  and 25ms, including the  sparse retrieval time.
For the example of Table~\ref{tab:costbudget},
%The studies from~\cite{Lassance2022SPLADE-efficientmallia2022GTI,Qiao20222GT,2023SIGIR-Qiao},
if SPLADE sparse retrieval can complete  in 31 ms on an  average CPU and the total latency
target is around 50ms,  the cost of dense retrieval is targeted under around  19ms.
% At most the total sparse and dense retrieval cannot be more than 100ms.
%Accuracy of above query-specific cluster skipping while retaining a competiitve relevance is the key to accomplish this latency goal. 
%Notice that the latency target in the  LADR paper~\cite{2023SIGIR-LADR} is in a 4ms-8ms range
%and 
%This latency budget choice is reasonable because for 
%Also our evaluation is conducted in a low-end CPU server and a faster CPU can further accelerate. 
%CPU latency reported in~\cite{2022WWWforwardIndex} is at 11

For the memory space cost,  our target budget for  dense retrieval augmentation is controlled in  the same level or some fraction of  sparse retrieval cost.
As illustrated in  Table~\ref{tab:costbudget}, compression with embedding  quantization is necessary to meet the space constraint.
%due to the memory usage of stroing  embedding vectors. 
%For 8.8M MS MACRO passages, that takes  about 27GB space.
%Fortunately the quantization techniques can significantly compress this space into 1-2GB or even 0.5GB depending on the configuration. 
Our feature design does not opt for  
inter-document similarity since it is space-consuming,
but  plans to exploit cluster-based summary information, 
which  only adds  insignificant  space overhead.  
%\end{itemize}
%, and set a limit on the number of dense clusters used.



==> expe_ablation.tex <==
\vspace*{-5mm}
\subsection{Fast search with minimized space overhead}
\label{sect:eval0space}

\begin{table*}[htbp]
	\centering
		\resizebox{1.9\columnwidth}{!}{
		\begin{tabular}{ r r l |l l ll l |llll l|r}
			\hline\hline
			 & & & \multicolumn{2}{c}{ 
{\bf MSMARCO Dev} }& {\bf DL19}& {\bf DL20} & {\bf BEIR} 
& \multicolumn{2}{c} { {\bf MSMARCO Dev} }& {\bf DL19}& {\bf DL20} & {\bf BEIR} 
& {\bf  Latency}    \\
			& &\% D& {MRR@10}& R@1k& {NDCG@10}&  {NDCG@10}& {NDCG@10}& {MRR@10}& {R@1k}& {NDCG@10}&{NDCG@10}& {NDCG@10}& ms \\
    \hline
 1. & S={\bf SPLADE-HT1} & --& 0.396& 0.980 & 0.732   & 0.721    & 0.500 & -- & --& --& --& --&31.2  \\
 & & & \multicolumn{5}{c|}{D=\textbf{SimLM}}& \multicolumn{5}{c|}{D=\textbf{RetroMAE}}&\\
   \hline
   &&& \multicolumn{10}{c}{\bf{Uncompressed flat setting. Embedding space  27.2GB}}\\
     \hline
          2. &   D  & 100 & 0.411$^\dag$ & 0.985$^\dag$& 0.714 &  0.697  & 0.429 & 0.416$^\dag$& 0.988& 0.720&0.703& 0.482 & 1674.1 \\
            3. &   $\blacktriangle$ S $+$ D   &100 & 0.424 & 0.989 & 0.740 & 0.726  & 0.518 & 0.425& 0.988& 0.740&0731& 0.520~& $+$1674.1 \\
           4. &    \bf S $+$ CluSD &0.3& 0.425 & 0.987 & 0.744 & 0.724  & 0.516 & 0.426& 0.987& 0.744&0.734 & 0.518 & $+$13.2 \\
              \hline
            &&& \multicolumn{10}{c}{\bf{OPQ $m=128$. Embedding space  1.1GB}}\\
              \hline
            5. &   $\blacktriangle$  S $+$ D-OPQ &100 & 0.420 & 0.988 & 0.735 &  0.719  & 0.508 & 0.416 & 0.988 & 0.737 & 0.732 & 0.515& $+$568.9 \\
            6. &  S $+$ D-IVFOPQ &10& 0.414$^\dag$& 0.987 & 0.726 & 0.734  & 0.505 & 0.404$^\dag$& 0.987& 0.713&0.722& 0.513 &  $+$95.2 \\
           7. &   &5& 0.407$^\dag$& 0.987 & 0.717 & 0.733  & 0.499  & 0.394$^\dag$& 0.987& 0.687&0.817&0.507&$+$ 48.8 \\
           8. &   &2& 0.392$^\dag$& 0.986$^\dag$& 0.691 & 0.738  & 0.467 & 0.374$^\dag$& 0.986$^\dag$& 0.656&0.815& 0.499&$+$21.3 \\
           9. &   \textbf{S $+$ CluSD}  &0.3& 0.423 & 0.987 & 0.739& 0.725 &0.514 & 0.417& 0.986& 0.742&0.735& 0.514  & $+$11.4  \\
             \hline
           & & & \multicolumn{10}{c}{\bf{OPQ $m=64$. Embedding space 0.6GB}}\\
            \hline
           10. & $\blacktriangle$  S $+$ D-OPQ  &100 & 0.409 & 0.986 & 0.718 &  0.721  &0.501 & 0.402 & 0.986 & 0.717 &  0.719 & 0.508 &$+$ 290.4 \\
           11. &   S $+$ D-IVFOPQ &10& 0.405 & 0.986 & 0.716 & 0.734 & 0.502 & 0.393$^\dag$& 0.986& 0.676&0.730& 0.505& $+$44.4 \\
           12. &   &5& 0.397$^\dag$& 0.986 & 0.704 & 0.733  & 0.497 & 0.384$^\dag$& 0.985& 0.659&0.717& 0.500& $+$23.8 \\ 
            13. &  &2& 0.383$^\dag$& 0.985 & 0.680 & 0.738 & 0.487 & 0.368$^\dag$& 0.985 & 0.643&0.707& 0.493 & $+$11.2 \\
            14. &  \textbf{S $+$ CluSD}  &0.3& 0.414 & 0.986 & 0.743& 0.726 & 0.511 & 0.403 & 0.987& 0.729&0.724 & 0.506 & $+$9.6 \\
              \hline\hline
		\end{tabular}
		}
	\caption{
Sparse retrieval argumentation with minimum extra space overhead.
%no  with compressed or uncompressed dense emebddings S=SPLADE-HT1, D=SimLM or RetroMAE. 
%Model relevance and latency under compressed or uncompressed dense emebddings S=SPLADE-HT1, D=SimLM or RetroMAE. 
%Row  ``S $+$ D'' marked with $\blacktriangle$ indicates the oracle setting of sparse model interpolated with full dense retrieval. 
For MSMARCO Dev set, $^\dag$ is tagged when statistically significant drop is observed from the oracle $\blacktriangle$ at 5\% confidence level. 
}
\vspace*{-5mm}
	\label{tab:mainspace}
\end{table*}
	%\caption{Model relevance and latency under different configurations with storage constraints. S=SPLADE-HT1, D=SimLM or RetroMAE. The row  ``S $+$ D'' marked with $\blacktriangle$ indicates the oracle setting of sparse model interpolated with full flat dense search model. For MSMARCO Dev set, $^\dag$ is marked when statistically significant drop is observed from the oracle $\blacktriangle$ at 5\% confidence level.



Table~\ref{tab:mainspace} demonstrates  the effectiveness  of CluSD in searching MS MARCO and BEIR datasets under
two quantization  configurations and the uncompressed setting. 
IVFOPQ is compared against CluSD as it selects only top clusters and does not incur extra space overhead. 
%is compared, which use some percentage of top dense clusters sorted by query to centroid clusters.
The sparse model used is SPLADE-HT1 while the dense models are SimLM and RetroMAE.
%The top portion of this table reports the performance when compression is not used, which captures a peak possible performance.
Column marked with  ``\%D'' means the percentage of dense embeddings  evaluated. 
Last column on ``Latency'' is the average single-query time using SimLM for MS MARCO Dev set.  We only report SimLM latency because the latency of SimLM and RetroMAE are similar. 
When 	prefix `+' is marked for a latency entry, it indicates  the extra milliseconds is spent 
for full or selective dense retrieval without counting   sparse retrieval time.

Tables~\ref{tab:mainspace} and~\ref{tab:maintime} use the same CluSD setting with $n=32$, which results in  selection of
22.3 clusters on average per query. 
The mean latency and 99 percentile latency of CluSD are 13.2 ms and 18.1 ms for searching uncompressed flat index, respectively; 
11.4 ms and 14.6ms for searching OPQ m=128 index;  9.6 ms and 11.1ms for searching OPQ m=128 index.

\comments{
%In realistic settings, a flat dense index is usually not affordable when corpus size is not small. Certain compression technique need to be used. 
The top portion of this table reports the performance of  SimLM dense model marked as ``D'' in Row 2.
In Row 1, ``S'' denotes sparse retrieval using  a variation of SPLADE with hard thresholding called HT1~\cite{2023SIGIR-Qiao}.
Sparse results merged with full  dense retrieval  results  are marked in Row 3, ``S $+$ D''.  
Our pipeline is reported in Row 4,``S $+$ CluSD''. 
The second and third portions of this table reports
the search performance   with  two compression configurations using OPQ implemented in FAISS:
1) ``m128'' that compresses dense embeddings from about 27GB into 1.1GB with 128 quantization codebooks.
2) ``m64'' that  yields 0.6GB compressed embeddings with 64 codebooks. 
%Setting where the storage for dense index is 1.1GB and 0.6GB. 
Under these two configurations, we report the Sparse model interpolated with dense retrieval under
IVFOPQ or OPQ using the default FAISS setting.


%In the first section of the table, we include the full dense retrieval SimLM (denoted as D in the table), 
%and full sparse retrieval SPLADE-HT1 (denoted as S in the table), 
%and 
%We then report dense retrieval with two compression configurations, using OPQ 
%with m=128 and m=64 respectively, resulting in an index 
%with 1.1GB and 0.6GB. These compressed configuration result in a 96\% and 97.8\% reduction in storage compared to flat index.
% and compare them against our pipeline.
}
 This table shows that
selective dense  to augment sparse retrieval by top IVF clusters sorted by query-centroid distances 
can be fast below  100ms  when the percentage of clusters searched  drops from 100\% to 10\%. But the relevance drop is significant. 
Moreover, CluSD is as  fast  as IVFOPQ  top 2\% search at m=64 and 2x fast at m=128 while
its relevance is much higher.
CluSD  performs  closely as the oracle at each compression setting, which  
indicates CluSD effectively minimizes visitation of unnecessary  dense clusters. 

 



\comments{
 with full dense retrieval can reach a high relevance in all datasets and thus are marked as an oracle sign with or without compression.   
1. Almost no performance degradation when do S+CluSD.  Sometimes S+CluSD achieves slightly higher performance than S+D. It could be due to the fact that when we limit the search scope a lot of noisy documents are not considered by the dense model.

2. Under m=128 setting the performance degradation is acceptable especially on DL19 and 20. 

3. SimLM performs better under compression. This could be due to the fact that SimLM trained embedding is normalized while RetroMAE is not.

4. If we compare S+D-IVFOPQ with S+CluSD, given the same IVFPQ index, S+D-IVFOPQ represents the case where we use default order, even if we use 50x more clusters, the performance is not as good as CluSD. 
}


% table with skipping, 40ms for dense
\comment{
\begin{table}[htbp]
	\centering
		\resizebox{1.05\columnwidth}{!}{
		\begin{tabular}{ r l l l |r r  |r r  |r}
			\hline\hline
			 &\% & \multicolumn{2}{c|}{{MSMARCO Dev}}& \multicolumn{2}{c|}{DL19}& 
\multicolumn{2}{c|}{DL20}& Latency    \\
			 &n& {MRR@10}& {R@1k}& {N@10}& {R@1k}&  {N@10}& {R@1k}& ms \\
			\hline
            D  &--& 0.411$^\dag$ & 0.985 & 0.714 & 0.767 &  0.697 & 0.773 & 1674.1  \\
          S  &--& 0.396$^\dag$ & 0.980 & 0.732   &  0.811 & 0.721    &  0.815  &   31.2  \\
              $\blacktriangle$ S $+$ D   &--& 0.424 & 0.989 & 0.740 & 0.822 & 0.726 & 0.824 & 1705.0 \\
              \bf S $+$ CluSD  &0.2& 0.425 & 0.987 & 0.744 & 0.823 & 0.724 & 0.819 & 14.4 \\
              \hline
            \multicolumn{9}{c}{\bf{OPQ M=128 setting, Storage 1.1GB}}\\
            \hline
             S $+$ D-IVFOPQ&10& 0.414 & 0.987 & 0.726 & 0.820 & 0.734 & 0.818 & 95.2 \\
             &5& 0.407 & 0.987 & 0.717 & 0.820 & 0.733 & 0.817 & 48.8 \\
             &2& 0.392 & 0.869 & 0.691 & 0.815 & 0.738 & 0.815 & 21.3 \\
             S $+$ OPQ &--& 0.420 & 0.988 & 0.735 & 0.816 & 0.719 & 0.821 &  568.9 \\
             HNSW+OPQ && &  &  & & & &   \\
             \textbf{S $+$ CluSD}  &0.2& 0.422 & 0.986 & 0.739& 0.822& 0.725& 0.818& 14.2  \\
             \hline
          \multicolumn{9}{c}{\bf{OPQ M=64 setting, 0.6GB}}\\
          \hline
             S $+$ IVFOPQ&10& 0.405 & 0.986 & 0.716 & 0.814 & 0.734 & 0.818 & 44.4 \\
             &5& 0.397 & 0.986 & 0.704 & 0.814 & 0.733 & 0.817 & 23.8 \\ 
             &2& 0.383 & 0.985 & 0.680 & 0.813 & 0.738 & 0.815 & 11.2 \\
             S $+$ OPQ  &--& 0.409 & 0.986 & 0.718 & 0.815 & 0.721 & 0.821 & 290.4 \\
             HNSW+OPQ && &  &  & & & &   \\
             \textbf{S $+$ CluSD}  &0.2& 0.411 & 0.985 & 0.743& 0.823& 0.726& 0.816& 11.5 \\
              \hline\hline
		\end{tabular}
		}
	\caption{Model relevance and latency under different configurations with storage constraints. S=SPLADE-HT1, D=SimLM. The row  ``S $+$ D'' marked with $\blacktriangle$ indicates the oracle setting of sparse model interpolated with full flat dense search model. For MSMARCO Dev set, $^\dag$ is marked when statistically significant drop is observed from the oracle $\blacktriangle$ at 5\% confidence level.
}
	\label{tab:mainspace}
\end{table}

}



\subsection{Search with no memory space constraints}
\label{sect:evaltimebudget}
Table~\ref{tab:maintime} compares  CluSD with  several baselines under two time budgets when memory space restriction is removed.
Uncompressed dense embeddings  are used to exclude the relevance impact by quantization.
The last two columns report the total latency time in milliseconds including sparse retrieval when needed,
and data space cost. Extra memory space on the top of sparse retrieval is marked with prefix `+'. 
``MRR'' means  MRR@10 and ``NDCG'' means  NDCG@10.
The extra space for quantized inter-cluster distances for CluSD takes about 32MB. 

%As discussed in Section~\ref{sect:design}, the overall latency budget is set as 50ms and 25ms respectively. 
We allow some time for budget relaxation since it is difficult to tune parameters of all baselines to meet the constraints exactly. 
For IVF, we use 1.5$\%$ and 3$\%$ top clusters for ``S+IVF'' and ``IVF''.
%  but we allow some variation for some baselines because it is difficult to find parameters that exactly control the latency under this budget. 
%In this case, we choose the dense configuration such that the overall latency is within 70 or 30 milliseconds. 
For HNSW under 50ms time budget, we set its expansion factor parameter (ef) as 1024, 
2048 for S$+$D-HNSW and D-HNSW. 
Under 30ms time constraint, the expansion factor (ef) is  512 and  1024 respectively. 
%We include option ``S+Re-rank" which uses the top 1,000 sparse retrieval results and only compute dense scores of these top results, and merge the score with an interpolation.
%For HNSW, we fix the number of neighbors to be 128 and vary the expansion factor(ef) to meet the latency constraint.
For LADR, we use its default setting with seed = 200, number of neighbor = 128 and use the exploration depth as  50 to meet the latency budget.
%Table~\ref{tab:maintime}.
\comments{
Under time budget 50ms, 
model  SPLADE-HT1 is used and it has a latency of 31.2 ms in sparse retrieval.  
Under  time budget 25ms, model SPLADE-effi-HT3 is used and it is more aggressive in  efficiency 
with a 12.4ms latency at the cost of a relevance degradation. 

%using the dense model only, We also include sparse retriever 
%IVFOPQ, IVF, OPQ and HNSW using the dense model only, We also include sparse retriever 
%with reranking top 1000 results using the dense model. We also include the results of document evaluation using LADR algorithm. 
Note that when ``S$+$'' is in the row, it means we use the sparse model and the reported results are interpolated. 

}
%[DISCUSS TABLE 4 RESULTS.]
The takeaways from this table are:

\textbullet\ While IVF does not add extra space cost,
the relevance  of IVF top cluster search under the time budget performs  worse than others.
Simple re-ranking ``D-rerank'' achieves good MRR@10 but under-performs on recall.
When the recall of a sparse retriever is relatively low, it cannot boost further as seen in the case of $m=64$.

\textbullet\ HNSW and LADR perform comparably, at the cost of extra online memory overhead  and extra complexity to compute offline in advance.
HNSW requires extra 9.2GB and LADR requires extra 4.3GB to store graph data in memory. 
When we  try to reduce their graph size by decreasing  the number of neighbors for HNSW and LADR, their  MRR@10 and/or  recall@1000 numbers drop visibly. For example, 
using the default 32 neighbors for the HNSW graph results in 2.4GB graph space, however  MRR@10 drops from 0.407 to 0.4 under the 25ms time budget. 

\textbullet\ CluSD incurs negligible extra space cost other than hosting embeddings, compared to HNSW and LADR.
For $m=128$,  CluSD has a higher MRR@10 while its DL19 and DL20 numbers are higher than HNSW, but comparable as LADR.
CluSD has more  advantages in relevance when $m=64$. 

\textbullet\ The time budget setting is discussed in Section~\ref{sect:design}.
Even when we relax the latency requirements for the baselines, CluSD still maintains its advantages in different datasets. 
For instance, if we double the time budget to around  110ms
for 	``S+D-HNSW'' after  SPLADE-HT1 retrieval, its MRR@10 for MS MARCO Dev is 0.422, which is still below S$+$CluSD with 46.3ms.




 

\begin{table}[htbp]
	\centering
 \resizebox{0.9\columnwidth}{!}{
		\begin{tabular}{r |llll|rr}
			\hline\hline
			& \multicolumn{2}{|c}{\bf{MSMARCO Dev}}& \bf{DL19}& 
\bf{DL20}& \bf{Latency}& \bf{Space}\\
			 & {MRR}& {R@1k}& \smaller{NDCG} &   \smaller{NDCG} & Total& GB\\
			\hline
        \multicolumn{7}{c}{\bf{Time Budget = 50 ms, S=SPLADE-HT1}}\\
        \hline
            D=SimLM & 0.411 & 0.985$^\dag$& 0.714 &  0.697 & 1674.1 & 27.2 \\
          S& 0.396$^\dag$& 0.980$^\dag$& 0.732   & 0.721    &   31.2 & 3.9 \\
           S $+$ D-rerank &  0.421 & 0.980$^\dag$& 0.745 & 0.728 & 34.6 & 31.1 \\
             $\blacktriangle$  S $+$ D  & 0.424 & 0.989 & 0.740 & 0.726 & 1705.0 & 31.1 \\
              \hline
              % D-IVF & 0.398$^\dag$& 0.935$^\dag$& 0.690 & 0.693 & 81.4 & $+$0.0\\
            D-IVF & 0.389$^\dag$& 0.907$^\dag$& 0.671 & 0.676 & 49.5 & $+\sim$0\\
            S $+$ D-IVF & 0.393$^\dag$& 0.987  & 0.678 & 0.715 & 56.5 & $+\sim$0\\
            %D-OPQ& 0.314$^\dag$& 0.957$^\dag$& 0.619 & 0.608 & 109.1 & 0.3 \\
           % D-IVFOPQ & 0.386$^\dag$& 0.929$^\dag$& 0.680 & 0.697 & 48.8 & 1.2\\
             D-HNSW & 0.409$^\dag$& 0.978$^\dag$& 0.669 & 0.695 & 54.4 & $+$9.2\\
            %S $+$ rerank-D &  0.412 & 0.980    &0.715  & 0.811 & 0.698 & 0.815 & $+$2.3 \\
            S $+$ D-LADR & 0.422& 0.984$^\dag$& 0.743&0.728& 43.6& $+$4.3\\
%           7.1 &  S $+$ D-LADR & 0.423 & 0.987$^\dag$& 0.745 &0.728& 53.0 & $+$4.3\\
           % S $+$ D-IVF & 0.398$^\dag$& 0.987  & 0.674 & 0.720 & 64.7 & $+$0.0\\
           %S $+$ D-IVFOPQ & 0.392$^\dag$& 0.987 & 0.656 & 0.700 &  52.5 & 4.0\\
           S $+$ D-HNSW & 0.420 & 0.987 & 0.718 & 0.723 & 59.6 & $+$9.2\\
            \bf S $+$ CluSD & 0.426 & 0.987 & 0.744 & 0.724 &46.3& $+$0.03\\
       \hline       
            \multicolumn{7}{c}{\bf{Time Budget = 25 ms, S=SPLADE-effi-HT3}}\\
            \hline
            S& 0.380$^\dag$& 0.944$^\dag$& 0.721 &  0.726 & 12.4 & 3.0 \\
             S + D-rerank & 0.406 & 0.944$^\dag$& 0.728 & 0.738 & 15.1 & 30.2 \\
            $\blacktriangle$  S + D & 0.413 & 0.984 & 0.721 &0.729 & 1654.2& 30.2  \\
            \hline
            D-HNSW & 0.406 & 0.971$^\dag$& 0.672 & 0.694 & 28.4 & $+$9.2\\
             S $+$ D-HNSW & 0.407 & 0.984 & 0.706 & 0.724 & 28.7 & $+$9.2\\
            S $+$ D-LADR & 0.404$^\dag$& 0.984 & 0.728 &  0.736 & 24.2 & $+$4.3\\
%           16.1 & S $+$ D-LADR & 0.409 & 0.987 & 0.744 &  0.728  & 41.1 & $+$4.3\\
            \bf S $+$ CluSD & 0.412 & 0.984 & 0.733 & 0.728 & 25.4 & $+$0.03\\
			\hline\hline
		\end{tabular}  }
	\caption{Search under time budget but  no memory constraints 
}
  \vspace*{-10mm}
	\label{tab:maintime}
\end{table}
%For pipelines with a time budget, we report the additional overhead in the Storage (GB) column. 






==> expe_beir.tex <==
\subsection{Zero-shot retrieval performance with BEIR}
\label{sect:evalbeir}

\begin{table*}[h]
	\centering
		\resizebox{1.9\columnwidth}{!}{
		%\begin{small}
		\begin{tabular}{r r r lr  |lllll|lllll}
			\hline\hline
                 &  & &  & &  \multicolumn{5}{c|}{SPLADE-HT1+SimLM} & \multicolumn{5}{c}{SPLADE-HT1+RetroMAE}\\
                  &  & &  & {SPLADE}  &  & &  \textbf{CluSD} & \textbf{CluSD} & \textbf{CluSD} & & & \textbf{CluSD} & \textbf{CluSD} & \textbf{CluSD}\\
		    Dataset & \smaller{BM25} &{SimLM}  &  {RetroMAE} &{-HT1} & \smaller{$\blacktriangle$ 
 flat} &rrk&\textbf{flat}& \textbf{m=128}& \textbf{m=64}& \smaller{$\blacktriangle$ flat} &rrk &\textbf{flat}& \textbf{m=128}& \textbf{m=64}\\
              \hline
              \multicolumn{15}{c}{\bf{Search Tasks}}\\
               \hline
                {DBPedia}	& 0.313	& 0.351 &  0.390&0.447	& 0.426 &0.442& 0.429 & 0.425 & 0.422 & 0.446 & 0.411 & 0.446 & 0.445&0.436 \\
                                {FiQA} &	0.236	& 0.298 &  0.316&0.355 & 0.355 &0.355 &0.365 & 0.361 &0.359 & 0.365 & 0.333 & 0.366 & 0.359& 0.353\\
                {NQ}	& 0.329   & 0.502  &	 0.518&0.550 & 0.568 &0.549&0.568 & 0.566 & 0.560 & 0.563 & 0.520 & 0.564 & 0.553& 0.538\\
                {HotpotQA} & 0.603 & 0.568 &  0.635& {0.681} & 0.672 &0.668&  0.672 & 0.669 & 0.661 & 0.702 & 0.642 & 0.702 & 0.693&0.672 \\
                {NFCorpus}  & 0.325 & 0.318  &  0.308&0.351 & 0.353 &0.347&  0.360 & 0.358 & 0.359 & 0.345 &0.331 & 0.351 & 0.349& 0.346 \\
                {T-COVID}	& 0.656 & 0.515  &  0.772&0.705 & 0.726 &0.692&  0.745 & 0.741 & 0.725 & 0.780 & 0.699 &0.747 &0.740& 0.726\\
                {Torche}	& {0.367}  & 0.292  &  0.237&0.291 & 0.336 &0.292 &0.333 & 0.336 & 0.332 & 0.292 &0.316 & 0.295 &0.288& 0.283\\
                \hline
                \multicolumn{15}{c}{\bf{Semantic Relatedness Tasks}}\\
                 \hline
                {ArguAna} & 0.315 & 0.376  &  0.433&0.446 & 0.481 &0.427&  0.492 & 0.489 & 0.486 & 0.459 & 0.434 & 0.455 &0.455 & 0.451\\
                {C-Fever}	& 0.213 & 0.171  &  0.232&0.234 & {0.239} &0.236&  0.241 & 0.250 & 0.242 & 0.260 &0.198 &0.260 &0.267& 0.262\\
                {Fever} & 0.753  &0.689  &	 0.774& {0.781} & 0.793 &0.784&  0.794 & 0.783 & 0.789 & 0.820 &0.774 &0.820 &0.814& 0.800\\
                {Quora} & 0.789 & 0.797  &	 0.847&0.817 &	0.847 &0.816&  0.847 & 0.849 &0.848 & 0.856 &0.814 &0.855 &0.854& 0.849\\
                {Scidocs}	& 0.158 &0.137  &	 0.15&0.155 &	{0.165} &0.152&  0.166 & 0.166 & 0.165 & 0.167 &0.142 &0.169&0.166& 0.164\\
                {SciFact}	& 0.665 & 0.559  &  0.653& {0.682} & 0.674 &0.682&  0.694 & 0.689 & 0.693 & 0.706  &0.661 &0.703 &0.699& 0.694\\
                            \hline
                \textbf{Avg.} & 0.440 & 0.429  &  0.482&0.500 & 0.518 &0.496&  0.516 & 0.514 & 0.511 & 0.520 &0.483 &0.518 &0.514& 0.506\\
                %\textbf{BM25 Diff} & -- & -2.6\%  &	13.6\% &17.7\% &  6.1\%&12.7\%&14.8\% &  \textbf{15.7\%} \\
                \textbf{{Splade Diff}} & -12.0 \% &  -14.2\%  &	 -3.6\% &-- & 3.6\% & -0.8\% &3.2\% & 2.8\% & 2.2\% &4.0\%& -3.5\%& 3.5\%&2.8\%&1.2\%\\
            \hline\hline
		\end{tabular}
		%\end{small}
		}
%\vspace*{-5mm}
	\caption{Zero-shot performance in average NDCG@10 on BEIR datasets. 
%Row ``SPLADE Diff.'' is the mean relative performance compared to the SPLADE-HT1 performance.
}
  \vspace*{-5mm}
%For quantization approaches, we adopt M=16, K=256, i.e. compression rate 32$\times$ compared to ColBERT.
	\label{tab:beir}

\end{table*}


Table~\ref{tab:beir} lists  details on how  CluSD  performs when supplementing sparse SPLADE-HT1 with either SimLM or RetroMAE results in
searching one of  13 BEIR datasets that contain out-of-domain documents.
The LSTM model of CluSD  is trained with the  MS MARCO training set,
and it is directly applied to each of the BEIR  datasets to select clusters without any change. 
%Zero-shot out-of-domain performance is important since a large dataset can contain document content from many domains.
% to unseen models and datasets, we evaluate the pipeline on out-domain data. For this experiment, we use the BEIR benchmarks which consists 13 released document 
%sets on various semantic relatedness tasks. 
%We directly apply the CluSD model trained on MSMARCO training set to predict the clusters on the BEIR queries and BEIR specific clusters. 


As a baseline, column ``$\blacktriangle$ flat'' is to merge  the uncompressed full dense retrieval results with SPLADE-HT1 sparse  retrieval.
Column marked ``rrk'' is to rerank   top 1,000  sparse retrieval results interpolated with their dense scores. 
%The final score are the interpolation of the sparse ranked list and dense re-ranked list. 
Columns with ``CluSD-flat'', ``CluSD-m128'' and ``CluSD-m64''  are  CluSD results  using uncompressed or compressed embeddings with
m=128 or m=64. 
%\begin{itemize} [leftmargin=*]
%\item 
Even SimLM and RetroMAE  underperform SPLADE retriever for BEIR,  the relevance after sparse and dense  result fusion
is still higher than each individual retriever.
CluSD with limited dense retrieval   performs  closely to   oracle ``$\blacktriangle$ flat''.
While embedding compression affects relevance,  CluSD still performs reasonably well.  
%\end{itemize}
  


==> expe_feature.tex <==
\subsection{Design options for LSTM}
\label{sect:evalLSTM}

% In this section, we discuss \textbf{RQ3} and \textbf{RQ4}.
Table~\ref{tab:cluster_feat} investigates the following five design options 
for cluster selection in CluSD. 
\begin{enumerate}[leftmargin=*]
    \item TopByDistance: Choose top clusters sorted by the distance of their  centroids to  the  query embedding.
% as implemented in the faiss IVF index.
    \item TopByOverlap:  Choose top  clusters sorted  by Group (3) features discussed in Section~\ref{sec:clusd}.
Namely use the overlap degree of clusters with top result bins of sparse retrieval.  

% select  the centroids based on the number of top10/25/100 sparse retrieval results in the clusters. This is the purning technique we propose in the method section.
    \item XGBoost: Use the boosting tree XGBoost model to detect if a cluster should be visited.
The features used are the same ones discussed in Section~\ref{sec:clusd}. This is a pointwise approach as we view query-cluster pairs as independent samples and the decision on one clusters doesn't affect other clusters for the same query.
% excluding inter-cluster distances.
%for each query-centroid pair to predict whether the centroid should be evaluted. This is a pointwise approach.
    \item RNN: Use a vanilla RNN model to predict. The feature and sequence setup is the same as our LSTM model. 
    \item Unpruned LSTM: Sort clusters  by the distance of their  centroids to  the  query embedding and feed into the LSTM model.
    \item Pruned LSTM: That is the final version used by CluSD with  cluster pruning.
\end{enumerate}
To have a fair comparison, this table assumes on average either 3 or 5 clusters are targeted by CluSD.
%We compare the performance of different strategies to select dense clusters.  
For XGBoost, RNN or LSTM, we set their prediction threshold so that 
the average number of clusters is close to the targeted number.
The last column of this table is the time spent by cluster selection.
%chosen depends  on the model prediction thresholds. 
%where top 3 or 5 clusters are selected. 
%In order to compare under same budget, we set the thresholds where on average around 3 or 5 clusters are used averaged over all queries. 
Table~\ref{tab:cluster_feat} shows that  the RNN or LSTM based prediction achieves much higher MRR@10 and recall compared to 
XGBoost. 
%point-wise tree based model. 
%It is reasonable as the tree model doesn't take  into account of incremental the inter-cluster relationships.
%Row  marked ``LSTM+prune'' of Table~\ref{tab:cluster_feat}, we 
Candidate pruning before using LSTM in CluSD can significantly 
decrease  the decision time by reducing the length of input cluster sequence, and can  actually lead a visible relevance increase in all cases.

 

\comments{
%\textbf{Effect of Model Options}
For k-means and topk heuristics, we report the performance where top 3 or 5 clusters are selected. For XGBoost, RNN or LSTM, the number of clusters chosen is dependent on the model prediction thresholds. In order to compare under same budget, we set the thresholds where on average around 3 or 5 clusters are used averaged over all queries. 
As we can see in Table~\ref{tab:cluster_feat}, RNN or LSTM based prediction achieves much higher MRR and Recall compared to point-wise tree based model. It is reasonable as the tree based model doesn't take into account the relationships between centroids when making predictions. 
}


%\textbf{Impact of feature groups}.  
The last two rows of Table~\ref{tab:cluster_feat} show
the {\bf positive impact  of feature groups}  used in the LSTM model.
That is done by 
removing  the inter-cluster distance feature group marked as ``w/o inter-cluster dist'' 
or by removing  the overlap degree of top sparse results and each cluster marked as  
`` w/o S-C overlap''.
The results indicate that the overlap degree is important for  cluster selection
while the inter-cluster feature group is also useful. 

%  vs. Dense'' has a visible drop in relevance, indicating that the features we use are useful. Especially the sparse vs. dense feature, model performance has a significant drop without the feature group.

\begin{table}
\resizebox{1.0\columnwidth}{!}{
  \begin{tabular}{ r r r r r r }
			\hline\hline
			 Avg \#clusters targeted  & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{5} & Time \\
			& MRR@10 & R@1k& MRR@10 & R@1k & ms\\
                   \hline
                 \multicolumn{6}{l}{\it{Model options}}\\
%                 Kmeans 
TopByDistance
& 0.297 & 0.655 & 0.331 & 0.740  & 0 \\
%                 TopK Heuristic
TopByOverlap
& 0.384 & 0.867 & 0.401 & 0.917 & 0.2 \\
                 XGBoost& 0.398 & 0.888 & 0.404 & 0.929 & 192 \\
                 RNN & 0.404 & 0.908 & 0.406 & 0.938 & 2.8 \\
                 %RNN+prune & 0.401 & 0.919 & 0.411 & 0.961 & 2.8 \\
                 Unpruned LSTM & 0.406 & 0.923 & 0.406 &0.943 & 2.8\\
            \textbf{Pruned LSTM}  &  0.408 & 0.943 & 0.410 & 0.953 & 2.8 \\
              \hline
             \multicolumn{5}{l}{\it{Feature group removal}}\\
             w/o inter-cluster  dist& 0.402 & 0.915 & 0.406 & 0.941 & --\\
             %w/o Centroid Distance& 0.389 & 0.898 & 0.410 & 0.959 & --\\
             %w/o Sparse vs. Dense& 0.378 & 0.866 & 0.404 & 0.943 & --\\
             w/o  S-C overlap& 0.289 & 0.638 & 0.325 & 0.730 & --\\
             %$-$ Query vs. Centroid & 0.405 & 0.925 & 0.406 & 0.941 & --\\
              \hline\hline
		\end{tabular}
}
	\caption{Design options for  CluSD and the impact of  features }
	 \vspace*{-5mm}
        \label{tab:cluster_feat}
\end{table}

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.4]{ncluster2.pdf}
    \caption{CluSD performance and latency with respect to a different average  number of visited clusters}
     \vspace*{-4mm}
    \label{fig:ncluster}
\end{figure}


\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.45]{threshold.pdf}
    \caption{Left: Distribution  of \#visited clusters under different selection threshold $\Theta$.
Right: Mean \#visited clusters on MSMARCO Dev set and BEIR datasets.}
     %\vspace*{-5mm}
    \label{fig:thresholds}
\end{figure}

\subsection{Impact of  cluster partitioning size}
\label{sect:clusterno}

%The cluster selection technique is built on top of a group of defined clusters. It is important to understand how the cluster selection works and a good rule of thumb to 
%determine the model prediction threshold given different number of clusters. 
CluSD assumes the embeddings are  pre-partitioned into $N$ clusters.  Figure~\ref{fig:ncluster} shows the impact of CluSD when
$N$ is  4096 and  8192.
% we plot three scenarios where the total number of clusters is 1024, 4096 and 8192 respectively. 
We use $n=128$ in this figure to depict the impact of selecting different numbers of clusters on average in a wider range.
A  solid line refers to the use of uncompressed dense embeddings while  a dash-dot line refers to the quantization with OPQ M=128, 
and a dotted line refers to the quantization  with OPQ m=64. X-axis is the average number of clusters selected by CluSD when $n=128$.
We vary the selection threshold parameter $\Theta$ in CluSD to achieve the different average number of clusters selected. 

Figure~\ref{fig:ncluster} shows that with both $N$,
%MRR@10 reaches above 0.420 when above    $<$ 10 clusters 
MRR@10 reaches above 0.420 when above 10 clusters 
are selected.
As more clusters are selected,  the recall ratio does  increase. 
%Note that when total number of clusters increases, the percentage of documents search will be different given a fixed number of clusters are selected. 
%Given a fixed number of selected clusters,  the latency impact is different with different $n$ values.
%This result in difference in average latency. 
Looking at  a fixed average number of selected clusters, 
different $N$ values imply different latencies.
For example, when 10 clusters are selected on average, 
CluSD  scans through 0.1\% and  0.2\% of embeddings corresponding to N=4096 and 8192, respectively. 
%As we can see in the bottom two sub-figures, 
When $N= 8192$, its latency in milliseconds is smaller  with a  smaller size per cluster
as the CluSD time complexity is proportional  to  the size per cluster and the number of clusters selected.
With $N$ becomes much bigger,  the sorting overhead of clusters in pruning optimization starts to offset or outweigh latency benefits
of small clusters. 
% while the overall CluSD time is still  
\comments{
In this case, given a 20 
%(35 ms for 99\%) 
millisecond mean latency constraint, 
CluSD  with flat index can achieve 0.425 and 0.988 in MRR@10 and recall@10 by visiting  about 50 clusters (0.6\% of documents), 
which is the same performance compared to the full index search. 
This is observation is logical, as for each cluster, there are possible only tens or a few hundred relatively important documents to be evaluated for 
a given query. Majority of the documents in the clusters are not worth exploring. As the size of each clusters decreases, we are able to see more top important documents. 
}

Lastly, as CluSD makes a query-specific decision to dynamically select  clusters, each query has  a  different number of clusters visited
given a fixed threshold value and query latency can vary. 
The bottom right subfigure shows that the 99th percentile latency is around 2x longer than the mean latency, which is reasonable by
looking at the previous retrieval latency studies (e.g. ~\cite{mallia2019pisa, mackenzie2021anytime}). 




\subsection{Impact of  selection threshold $\Theta$}
\label{sect:threshold}
\comments{
\textbf{RQ6}: does the cluster selection model dynamically select different number of clusters for different queries? How the selection differs for different datasets?
For the first question, we plot out the distribution of number of clusters selected for each query as a boxplot in 
}
The left portion of Figure~\ref{fig:thresholds} shows
the average number of SimLM dense clusters selected by CluSD for MS MARCO Dev set under a different value of threshold $\Theta$ when
the input sequence length $n$ is 32.
%Model prediction threshold refers to the threshold which we use to determine the selection of a cluster. 
The threshold can be determined based on the time budget. 
%As we can see, there is a variety in the number of clusters selected. 
While the median number of clusters selected is  10 clusters, 75th percentile is around 18 clusters. 

The right portion of Figure~\ref{fig:thresholds} 
shows  the mean number of clusters selected for MS MARCO Dev set and averaged over 
the zero-shot BEIR datasets.
This subfigure shows that for a fixed $\Theta$ value, CluSD  chooses a fewer number of clusters for a
BEIR dataset compared to the MS MARCO Dev set.  
%This aligns with our expectation that  
This is because
SimLM underperforms SPLADE on the BEIR datasets in general. Thus, it is unnecessary to evaluate a lot of clusters. 
CluSD adaptively selects fewer clusters to conduct selective dense retrieval.



==> expe_old.tex <==
\comment{
\begin{table*}[htbp]
	\centering
		\begin{small}
		\begin{tabular}{ r r r |r r  |r r  |r r}
			\hline\hline
			& \multicolumn{2}{c|}{MSMARCO Dev}& \multicolumn{2}{c|}{DL19}& 
\multicolumn{2}{c|}{DL20}& Latency  & Storage  \\
			& MRR@10 & R@1k & NDCG@10 & R@1k &  NDCG@10 & R@1k & ms & GB\\
			\hline
            \multicolumn{9}{c}{Retrieval Depth = 1000}\\
           D=SimLM & 0.411 & 0.985 & 0.714 & 0.767 &  0.697 & 0.773 & 1674.1 & 27.2 \\
            D-IVF-6\% & 0.400  & 0.942 & 0.673 & 0.679 & 0.694 & 0.684 &  100.4 & 27.2 \\
            D-OPQ-m32 & 0.314 & 0.957  & 0.619 & 0.671 & 0.608 & 0.683 & 109.1 & 0.3 \\
            D-IVFOPQ-m128-15\% & 0.397 & 0.965 & 0.699 & 0.708 & 0.699 &0.720 &102.4 & 1.2 \\
            D-HNSW & 0.409 & 0.978 & 0.669 & 0.722 & 0.695 & 0.760 & 127.8 & 36.4 \\
            S=SPLADE-HT1 & 0.396 & 0.980 & 0.732   &  0.811 & 0.721    &  0.815  &   62.3 & \\
            S $+$ rerank-D &  0.412 & 0.980    &0.715  & 0.811 & 0.698 & 0.815 & $+$2.3 \\
            LADR & 0.412 & 0.983 & 0.714 &  0.785 &0.697  & 0.799& $+$ 19.1 & \\
            S $+$ D  & 0.424 & 0.989 & 0.740 & 0.767  & 0.726 & 0.773 & $+$ 1674.1 & \\
           S $+$ D-IVF-2\% & 0.398 & 0.987  & 0.674 & 0.816 & 0.720 & 0.813 &  $+$ 33.5 & \\
           S $+$ D-IVFOPQ-m128-5\% & 0.407 & 0.987 & 0.717 & 0.820 & 0.733 & 0.817 &  $+$ 38.1 & \\
            %\bf S $+$ CS-D &  0.420 & 0.985 & 0.734 & 0.816 & 0.722 & 0.818 & +19.4 & \\
             %\bf S $+$ QF-CS-D &  0.415 & 0.983 & 0.735 & 0.815 & 0.722 & 0.817 & $+$ 11.6 & \\
             \bf S $+$ CS-D $+$  rrk10 & 0.425 & 0.986 & 0.740 & 0.815 & 0.727 & 0.819 & $+$ 20.5 & \\
            \bf S $+$ CS-D $+$  rrk10 & 0.425 & 0.985 & 0.739 & 0.817 & 0.726 & 0.819 & $+$ 15.9 & \\
       \bf S $+$ QF-CS-D + rrk10 &  0.417 & 0.983 &  0.738 & 0.815 & 0.722 & 0.818 & $+$ 10.3 & \\
       \bf S $+$ QF-CS-D + rrk10 &  0.417 & 0.983 &  0.738 & 0.813 & 0.722 & 0.817 & $+$ 12.7 & \\
       \hline
       \multicolumn{9}{c}{Retrieval Depth = 10}\\
       D=SimLM & 0.411 & 0.696 & 0.714 & 0.169 &  0.697 &        0.225 &  \\
            D-IVF-6\% &  0.400 & 0.671 & 0.673 & 0.145 & 0.694 & 0.223 & 100.4 & 27.2 \\
            D-OPQ-m32 & 0.314 & 0.571 & 0.619 & 0.134 & 0.608 & 0.207 & 109.1 & 0.3 \\
            D-IVFOPQ-m128-15\% & 0.397 & 0.675 & 0.699 & 0.158 & 0.699 & 0.221 & 102.4 & 1.2 \\
            D-HNSW & 0.409 & 0.691 & 0.669 & 0.142 & 0.695 & 0.225 & 127.8 & 36.4  \\
            LADR & 0.412 & 0.696 & 0.722 & 0.701 & 0.697 & 0.696 & splade 200T $+$ 3.9 &  \\
           S=SPLADE-HT1 & 0.396 & 0.514 &  0.732   &  0.175 & 0.721    & 0.245 &  \\
          S $+$ D  & 0.421 & 0.704 & 0.732 & 0.175 & 0.721 & 0.245 & & \\
            S $+$ rerank-D &  0.410 & 0.674 & 0.733 & 0.175 & 0.726 & 0.245  &  \\
            %S $+$ rerank-D-itp &  0.413 & 0.674 & 0.736 & 0.175 & 0.726 & 0.245 &   \\
            S $+$ D-IVF-2\% & 0.399 & 0.682  & 0.676 & 0.153 & 0.693 & 0.213 &  $+$ 33.5 & \\
           S $+$ D-IVFOPQ-m128-5\% & 0.404 & 0.682 & 0.695 & 0.149 & 0.707 & 0.220 &  $+$ 38.1 & \\
            %\bf S $+$ CS-D &  0.418 &0.701&0.724&0.172&0.725&0.247 & \\
             %\bf S $+$ QF-CS-D &  0.413 &0.695&0.729 &0.173&0.731&0.249&\\
            \bf S $+$ CS-D $+$  rrk10 & 0.418 & 0.703 & 0.722 & 0.173 & 0.710 & 0.228 & $+$ 15.9 &  \\
       \bf S $+$ QF-CS-D + rrk10 &  0.413 & 0.695 & 0.726 & 0.173 & 0.719 & 0.244 & $+$ 10.3 & \\

			\hline\hline
		\end{tabular}
		\end{small}
	\caption{Model relevance and Latency Under Different Search Settings with Retrieval Depth 1000 and 10
%For quantization methods on top of ColBERT, we also report \% degradation from ColBERT.
}
	\label{tab:main1k}
\end{table*}
}

\comment{
\begin{table*}[htbp]
	\centering
		\begin{small}
		\begin{tabular}{ r r r |r r  |r r  |r}
			\hline\hline
			& \multicolumn{2}{c}{MSMARCO Dev}& \multicolumn{2}{c}{DL19}& 
\multicolumn{2}{c}{DL20}& Latency   \\
			& MRR@10 & R@1k & NDCG@10 & R@1k &  NDCG@10 & R@1k & ms \\
			\hline
              \multicolumn{7}{l}{\it S: BM25-T5-B, D: SimLM}&  \\
            S & 0.259 & 0.935 & 0.578 & 0.755 & 0.588 &       0.761 & 9.2 \\
              S $+$ flat-D  & 0.415 & 0.985 & 0.718 & 0.808 & 0.705 & 0.813 & $+$ 1674.1 \\
             S $+$  rerank-D &  0.409 & 0.935  & 0.714 & 0.755 & 0.698 & 0.761 & $+$ 2.3\\
             S $+$  rerank-D-itp & 0.413 & 0.935 & 0.721 & 0.755 & 0.705 & 0.761 & $+$ 2.3\\
           %S $+$ LADR& 0.412& 0.983& 0.712& 0.788& 0.692& 0.787& $+$ 19.1 \\
  %S $+$ LADR-itp& & & & & & &\\
            S $+$ LADR& 0.412& 0.983& 0.712& 0.788& 0.692& 0.787& $+$ 19.1 \\
           S \textbf{ $+$ CS-D} &0.408 & 0.977 & 0.713 & & 0.689 & 0.797  & $+$ 18.2 \\
           S \textbf{ $+$ CS-D + rrk10} &0.412 & 0.977 & 0.713 & 0.801 & 0.699 & 0.796  & $+$ 18.2 \\
           \multicolumn{7}{l}{\it S: BM25-T5-B, D: RetroMAE}&  \\
     S $+$ flat-D  & 0.416 & 0.986 &  & & &  & $+$ 1677.9 \\
           S $+$  rerank-D &  0.413 & 0.935  &  & & & & $+$ 2.3\\
            S $+$  rerank-D-itp &  0.416 & 0.935  &  & & & & $+$ 2.3\\
            S \textbf{$+$ CS-D} & 0.404 & 0.978  &&  && & $+$ 21.4 \\
            S  \textbf{$+$ CS-D $+$ rrk10} & 0.415 & 0.978  &&  && & $+$ 21.4 \\
            \hline
   %        \multicolumn{11}{l}{\it  S: SPLADE-effi-HT3-2GT,  D: SimLM}  \\
    %        S & 0.391 & 0.846 &  0.976 & 0.724 &     0.429  & 0.813  & 0.731  &  0.505   &  0.805  & 14.2 \\
    %       S $+$ flat-D  & 0.421 & 0.860 & 0.985 & 0.724 & 0.432 & 0.815 & 0.735 & 0.516 & 0.775 & $+$ 1674.1 \\
    %       S + rerank-D &  0.411 & 0.879 & 0.976   & 0.713 & 0.422 & 0.813 & 0.686 & 0.493 & 0.805 & $+$23.4 \\
    %         S $+$ IVF-D & 0.380 & 0.771 & 0.985 & & & & & & &  $+$ 25.6\\
    %     \bf S  $+$ CS-D & 0.415 & 0.874 & 0.985 & 0.728 & 0.430 & 0.818 & 0.726 & 0.505 & 0.811 & $+$ 18.1 \\
    %        \bf S $+$ QF-CS-D & 0.407 & 0.866 & 0.982 & 0.715 & 0.438 & 0.817 & 0.720 & 0.496 & 0.807 & 15.3  \\
    %        \multicolumn{11}{l}{\it  S: SPLADE-effi-HT3-2GT,  D: RetroMAE}  \\
     %      S $+$ flat-D  & 0.425 & 0.891 & 0.988 &  & & & & &  & $+$ 1677.9 \\
     %      S + rerank-D &  0.416 & 0.883 & 0.976   &  & & &  & &  & $+$23.4 \\
     %       S $+$ IVF-D & 0.350 & 0.716 & 0.985 & & & & & & &  $+$ 37.2\\
     %       \bf  $+$ CS-D & 0.413 & 0.877 & 0.986 &&&  &&& & $+$ 22.2 \\
      %      \bf $+$ QF-CS-D & 0.404 & 0.866 & 0.981 &&&  &&& & $+$ 16.8  \\
      %      \hline
            \multicolumn{7}{l}{\it  S: SPLADE-HT1, D: SimLM}&  \\
            S & 0.396 & 0.980 & 0.732   &  0.811 & 0.721    &  0.815  &   62.3 \\
          S $+$ flat-D-itp  & 0.424 & 0.989 & 0.740 & 0.767  & 0.726 & 0.773 & $+$ 1674.1 \\
            S $+$ rerank-D &  0.412 & 0.980    &0.715  & 0.811 & 0.698 & 0.815 & $+$2.3 \\
            S $+$ rerank-D-itp &  0.421 & 0.980 & 0.745 & 0.811 & 0.728 & 0.815 & $+$2.3 \\
           S $+$ IVF-D & 0.384 & 0.987 & & & & &  $+$ 25.6\\
           S  $+$ LADR & 0.412& 0.983& 0.697&0.799&& & $+$42.8 \\
 S $+$ LADR-itp& 0.422& 0.969& & & & &\\
            \bf S $+$ CS-D &  0.420 & 0.985 & 0.734 & 0.816 & 0.722 & 0.818 & +17.2 \\
             \bf S $+$ QF-CS-D &  0.415 & 0.983 & 0.735 & 0.815 & 0.722 & 0.817 & $+$ 8.9 \\
            \bf S $+$ CS-D $+$  rrk10 & 0.425 & 0.985 & 0.739 & 0.817 & 0.726 & 0.819 & $+$ 17.2 \\
       \bf S $+$ QF-CS-D + rrk10 &  0.417 & 0.983 &  0.738 & 0.815 & 0.722 & 0.818 & $+$ 9.9 \\
            \it  S: SPLADE-HT1, D: RetroMAE&&&&&&&  \\
            S $+$ flat-D-itp  & 0.425 & 0.988 &  & & &  & $+$ 1677.9 \\
            S $+$ rerank-D &  0.416 & 0.980    & & & &  & $+$2.3 \\
            S $+$ rerank-D-itp &  0.422 & 0.980    & & & &  & $+$2.3 \\
            S $+$ IVF-D & 0.350 & 0.987 & & & & &  $+$ 37.2\\
            \bf $+$ CS-D &  0.414 & 0.987 &  &  & & & $+$ 19.7 \\
            \bf $+$ QF-CS-D &  0.410 & 0.985 &  & & &  & $+$ 9.8 \\
           \bf $+$ CS-D $+$ rrk10 &  0.424 & 0.987 &  &  & & & $+$ 20.7 \\
            \bf $+$ QF-CS-D $+$ rrk10 &  0.412 & 0.985 &  & & &  & $+$ 10.2 \\
            \hline
           \multicolumn{7}{l}{\it  Dense Retrieval Options}&  \\
             SimLM-flat & 0.411 & 0.985 & 0.714 & 0.767 &  0.697 & 0.773 & 1674.1\\
             SimLM-IVF-2\% &  0.388 &  &&  && &33.5 \\
             SimLM-IVF-10\% &  0.403 &  &&  && &164.3 \\
             SimLM-OPQ-m16 & 0.221 &  &&  && & 59.0 \\
             SimLM-OPQ-m32 & 0.325 &  &&  && & 109.1 \\
            SimLM-IVFOPQ-m128-5\% & 0.379 &  &&  && &13.7 \\
            SimLM-IVFOPQ-m256,10\% & 0.399 &  &&  && & 143.8 \\
              RetroMAE-flat & 0.416 & 0.988 &&  && & 1677.9 \\
               RetroMAE-IVF-2\% &  0.367 &  &&  && &48.1 \\
              RetroMAE-IVF-10\% &  0.406 &  &&  && &299.0 \\
              RetroMAE-OPQ-m16 & 0.171 &  &&  && & 59.4 \\
             SimLM-OPQ-m256 & 0.404 &  &&  && & 1586.5 \\
             RetroMAE-IVFOPQ-m256,10\% & 0.395 &  &&  && & 180.5 \\
			\hline\hline
		\end{tabular}
		\end{small}
	\caption{Model relevance and Latency Under Different Search Settings with Retrieval Depth 1000
%For quantization methods on top of ColBERT, we also report \% degradation from ColBERT.
}
	\label{tab:main1k}
\end{table*}
}
\comment{
\begin{table*}[htbp]
	\centering
		\begin{small}
		\begin{tabular}{ r r r | r r | r r | r}
			\hline\hline
			& \multicolumn{2}{c|}{MSMARCO Dev} & \multicolumn{2}{c|}{DL19 } & 
\multicolumn{2}{c}{DL20} & Latency   \\
			& MRR@10 & R@10 & NDCG@10 & R@10 & NDCG@10 & R@10  & ms \\
			\hline
              \multicolumn{8}{l}{\it S: BM25-T5-B, D: SimLM}  \\
            S & 0.259 &  0.514  & 0.578 &  & 0.588 &      &  \\
              S $+$ flat-D  &0.411 & 0.686 & 0.724 & 0.171 & 0.730 & 0.246 & \\
             S $+$  rerank-D &  0.354 & 0.514 & 0.622 & 0.152 & 0.630 & 0.209 & \\
             S $+$  rerank-D-itp &0.355 & 0.514 & 0.623 & 0.152 & 0.629 & 0.209 &  \\
           S $+$ LADR & 0.408 & 0.689 & & & & & \\
           S \textbf{ $+$ CS-D} & &&&&&&\\
           S \textbf{ $+$ CS-D + rrk10} &&&&&&&\\
           \multicolumn{8}{l}{\it S: BM25-T5-B, D: RetroMAE}  \\
     S $+$ flat-D  & 0.416 & 0.710 &   & & & & \\
           S $+$  rerank-D &  0.356 & 0.514 & &&&&  \\
             S $+$  rerank-D-itp &  0.356 & 0.514 & &&&& \\
            S \textbf{$+$ CS-D} & &&&&&&\\
            S  \textbf{$+$ CS-D $+$ rrk10} &&&&&&&\\
            \hline
            \multicolumn{8}{l}{\it  S: SPLADE-HT1, D: SimLM}  \\
            S & 0.396 & 0.514 &  0.732   &  & 0.721    &        &  \\
          S $+$ flat-D-itp  & 0.421 & 0.704 & 0.732 & 0.175 & 0.721 & 0.245 & 
\\
            S $+$ rerank-D &  0.410 & 0.674 & 0.733 & 0.175 & 0.726 & 0.245  &  \\
            S $+$ rerank-D-itp &  0.413 & 0.674 & 0.736 & 0.175 & 0.726 & 0.245 &   \\
            S $+$ LADR & 0.412 & & &&&& 2.2 \\
            \bf S $+$ CS-D &  0.418 &0.701&0.724&0.172&0.725&0.247 & \\
             \bf S $+$ QF-CS-D &  0.413 &0.695&0.729 &0.173&0.731&0.249&\\
            \bf S $+$ CS-D $+$  rrk10 & 0.418 & 0.703 & 0.722 & 0.173 & 0.710 & 0.228 &  \\
       \bf S $+$ QF-CS-D + rrk10 &  0.413 & 0.695 & 0.726 & 0.173 & 0.719 & 0.244 & \\
 \multicolumn{ 8}{l}{\it  S: SPLADE-HT1, D: RetroMAE}  \\
            S $+$ flat-D-itp  & 0.422 & 0.706 & &&&& \\
            S $+$ rerank-D &  0.412 & 0.674 &&&&&  \\
            S $+$ rerank-D-itp &  0.413 & 0.674 &&&&&  \\
            \bf $+$ CS-D &  0.418 & 0.701 &  &  &  & & \\
            \bf $+$ QF-CS-D &  0.413 & 0.695 &  &   & & & \\
           \bf $+$ CS-D $+$ rrk10 &  0.418 & 0.703 &  &  & &  & \\
            \bf $+$ QF-CS-D $+$ rrk10 &  0.413 & 0.695 &&&&& \\
            \hline
			\hline\hline
		\end{tabular}
		\end{small}
	\caption{Model relevance and Latency Under Different Search Settings with Retrieval Depth 10
%For quantization methods on top of ColBERT, we also report \% degradation from ColBERT.
}
	\label{tab:main10}
\end{table*}
}

\comment{
\begin{table*}[htbp]
	\centering
		\begin{tabular}{ r r r |r r  |r r  |r r}
			\hline\hline
			& \multicolumn{2}{c|}{MSMARCO Dev}& \multicolumn{2}{c|}{DL19}& 
\multicolumn{2}{c|}{DL20}& Latency  & Storage  \\
			& MRR@10 & R@1k & NDCG@10 & R@1k &  NDCG@10 & R@1k & ms & GB\\
			\hline
        \multicolumn{9}{c}{Time Budget = 70 ms}\\
        \hline
            D=SimLM & 0.411 & 0.985 & 0.714 & 0.767 &  0.697 & 0.773 & 1674.1 & 27.2 \\
          S=SPLADE-HT1 & 0.396 & 0.980 & 0.732   &  0.811 & 0.721    &  0.815  &   31.2 & 2.8 \\
           S $+$ rerank-D &  0.421 & 0.980 & 0.745 & 0.811 & 0.728 & 0.815 & 34.6 & 30.0 \\
             $\blacktriangle$  S $+$ D  & 0.424 & 0.989 & 0.740 & 0.767  & 0.726 & 0.773 & 1705.0 & 30.0 \\
              \hline
            D-IVF-6\% & 0.398  & 0.938 & 0.673 & 0.679 & 0.694 & 0.684 &  100.3& 27.2 \\
            D-OPQ-m32 & 0.314 & 0.957  & 0.619 & 0.671 & 0.608 & 0.683 & 109.1 & 0.3 \\
            D-IVFOPQ-m128-15\% & 0.397 & 0.965 & 0.699 & 0.708 & 0.699 &0.720 &102.4 & 1.2 \\
            D-HNSW & 0.409 & 0.978 & 0.669 & 0.722 & 0.695 & 0.760 & 127.8 & 36.4 \\
            %S $+$ rerank-D &  0.412 & 0.980    &0.715  & 0.811 & 0.698 & 0.815 & $+$2.3 \\
            S $+$ LADR & 0.423& 0.987 & 0.745 &  0.804&0.724  & 0.815 & 59.9& 34.3 \\
           S $+$ D-IVF-2\% & 0.398 & 0.987  & 0.674 & 0.816 & 0.720 & 0.813 & 70.2& 30.0 \\
           S $+$ D-IVFOPQ-m128-5\% & 0.407 & 0.987 & 0.717 & 0.820 & 0.733 & 0.817 &  70.8& 4.0 \\
             \bf S $+$ CS-D & 0.426& 0.987 & 0.744 & 0.823 & 0.724 & 0.819 &47.3& 45.6 \\
       \hline       
            %\multicolumn{9}{c}{Time Budget = 30 ms}\\
            %s=SPLADE-HT1-fast & 0.385 & 0.949 & 0.730& 0.806&  0.722&0.793& 22.4 & 3.0 \\
            %$\blacktriangle$  S + D & 0.416 & 0.986 & 0.743& 0.827&  0.724&0.830& 22.4 & 30.2  \\
            %S + rerank-D & 0.409 & 0.949 & & &  && 25.1 & 30.2 \\
            %D-HNSW & 0.403 & 0.965 & 0.675 & 0.723 & 0.694 & 0.752 & 34.3 & 36.4 \\
            %S $+$ LADR & 0.409 & 0.986 & \boldred{0.745} & \boldred{0.837} & \boldred{0.729} & \boldred{0.834} & 32.2 & 34.5 \\
            %\bf S $+$ CS-D & 0.415 & 0.982 & 0.725 & 0.816 & 0.733 & 0.828 & 32.1 & 30.2 \\
            %\hline
            \multicolumn{9}{c}{Time Budget = 30 ms}\\
            \hline
            s=SPLADE-effi-HT3 & 0.380 & 0.944 & 0.721 & 0.806 &  0.726 &0.790& 12.4 & 3.0 \\
             S + rerank-D & 0.406 & 0.944 & 0.728 &  0.806 & 0.738 & 0.790 & 15.1 & 30.2 \\
            $\blacktriangle$  S + D & 0.413 & 0.984 & 0.721 & 0.806 &0.729 & 0.824 & -- & 30.2  \\
            \hline
            D-HNSW & 0.403 & 0.965 & 0.675 & 0.723 & 0.694 & 0.752 & 34.3 & 36.4 \\
            S $+$ LADR & 0.404 & 0.984 & 0.728 & \boldred{0.838} &  \boldred{0.736} & \boldred{0.829} & 24.2 & 34.5 \\
            \bf S $+$ CS-D & 0.412 & 0.984 & 0.733 & 0.833 & 0.728 & 0.822 & 23.1 & 30.2 \\
			\hline\hline
		\end{tabular}
	\caption{Comparing Dense Options Under Time Budget 70 and 30 ms}
	\label{tab:main1k}
\end{table*}
}


\comments{\textbf{Query Selective Fusion}
For query selection model we plot the relevance against the \% of query used for Different Feature Options against random baseline in Table~\ref{tab:query_level}. For fair comparison, instead of using the same model prediction thresholds, we report the result where around 50\% of queries and 75\% of queries are evaluated. For queries using dense model, we calculate the fusion results. For queries without dense evaluation, we use the splade only ranked list. 

The row ``w/o Query Quality" refers to the model trained without query quality features. The row ``w/o Sparse vs Dense" refers to the model trained without features describing the distribution of sparse results in the dense clusters. 


\textbf{Cluster Selection Model}
For cluster selection model we plot the relevance against the \% of query used for different feature options against random baseline in Table~\ref{tab:cluster_feat}. In this table, we only report the dense evaluation without interpolation with SPLADE to get a clear picture on the performance differences. 

The row ``w/o Centroid Distance" refers to the model trained without inter centroid distance features. The row ``w/o Sparse vs. Dense" refers to the model trained without features describing the distribution of sparse results in the dense clusters. 

We also report the LSTM model trained with different length of input. We train a model that only consider top 64, 84, 128 or 256 top clusters. In the Time column, we report the model inference time with different input sequence length. Longer sequence with bigger candidate sets generally yield better performance.
}

\comment{
\begin{table*}[h]
	\centering
		%\resizebox{1.07\columnwidth}{!}{
		%\begin{small}
		\begin{tabular}{r r r r  |r r r llr }
			\hline\hline
                 &  & & &  \multicolumn{6}{c}{SPLADE-HT1+SimLM}\\
		    Dataset & \smaller{BM25} &\footnotesize{SimLM}  & \footnotesize{SPLADE-HT1} & \smaller{$\blacktriangle$ 
 flat} &  rrk &rrk-itp&  LADR&LADR-itp&{CS} \\
              \hline
              \multicolumn{10}{c}{Search Tasks}\\
                DBPedia	& 0.313	& 0.351 & 0.447	& 0.426 &  0.413 &0.442&  0.351&0.429&0.429\\
                FiQA &	0.236	& 0.298 & 0.355 & 0.355 &   0.335&0.355&  0.297&0.358&0.365\\
                NQ	& 0.329   & 0.502  &	0.550 & 0.568 &	  0.535&0.549&  0.503&0.568&0.568\\
                HotpotQA & 0.603 & 0.568 & \textbf{0.681} & 0.672 &   0.605&0.668&  0.569&0.674&0.672\\
                NFCorpus  & 0.325 & 0.318  & 0.351 & 0.353 &	  0.332&0.347&  0.319&0.352&0.360\\
                T-COVID	& 0.656 & 0.515  & 0.705 & 0.726 &  0.597&0.692&  0.533&0.732&0.745\\
                Torche-2020	& \textbf{0.367}  & 0.292  & 0.291 & 0.336 &   0.277&0.292&  0.292&0.335&0.333\\
                \hline
                \multicolumn{10}{c}{Semantic Relatedness Tasks}\\
                ArguAna & 0.315 & 0.376  & 0.446 & 0.481 &   0.388&0.427&  0.283&0.487&0.492\\
                C-FEVER	& 0.213 & 0.171  & 0.234 & \textbf{0.239} &   0.214&0.236&  0.173&0.243&0.241\\
                FEVER & 0.753  &0.689  &	\textbf{0.781} & 0.793 &   0.771&0.784&  0.692&0.796&0.794\\
                Quora & 0.789 & 0.797  &	0.817 &	0.847 &   0.801&0.816&  0.800&0.847&0.847\\
                SCIDOCS	& 0.158 &0.137  &	0.155 &	\textbf{0.165} &   0.138&0.152&  0.137&0.165&0.166\\
                SciFact	& 0.665 & 0.559  & \textbf{0.682} & 0.674 &   0.668&0.682&  0.559&0.675&0.694\\
                            \hline
                \textbf{Avg.} & 0.440 & 0.429  & 0.500 & 0.511 &    0.467&0.496&  0.424&0.512&0.516\\
                %\textbf{BM25 Diff} & -- & -2.6\%  &	13.6\% &17.7\% &  6.1\%&12.7\%&14.8\% &  \textbf{15.7\%} \\
                \textbf{SPLADE Diff} & -12.0 \% &  -14.2\%  &	-- & 2.2\% &  -6.6\%& -0.8\%&   -15.3\%&2.5\%&3.2\%\\
            \hline\hline
		\end{tabular}
		%\end{small}
		%}
%\vspace{-0.5em}
	\caption{Zero-shot performance (NDCG@10) on BEIR }
%For quantization approaches, we adopt M=16, K=256, i.e. compression rate 32$\times$ compared to ColBERT.
	\label{tab:zero-shot}
\vspace{-1em}
\end{table*}

}

\comment{
\textbf{In-domain Data, Different Sparse Model}
\begin{table}
  \begin{tabular}{ r r r r r }
			\hline\hline
	          & \multicolumn{2}{c}{Zero-shot} & \multicolumn{2}{c}{Trained} \\
			& MRR@10 & R@10 & MRR@10 & R@10\\
              \hline
             \multicolumn{5}{c}{Splade-HT1-fast} \\
             S $+$ QF & 0.410 & 0.981 & 0.412  & 0.976 \\ %0.3 / 0.1, % = 0.730
             CS-D & & &  & \\ %0.1, 4.7 cluster
             S $+$ CS-D & & & 0.415 & 0.981 \\
             S $+$ QF-CS-D & & & 0.410 & 0.972 \\
             \multicolumn{5}{c}{Splade-effi-HT3} \\
             S $+$ QF & 0.407 & 0.977 & 0.407 & 0.975 \\%0.05, %0.79
             CS-D & & & & \\
             S $+$ CS-D & & & 0.411 & 0.978\\ % 
             S $+$ QF-CS-D & & & 0.406 & 0.969\\ 
             \multicolumn{5}{c}{BM25-T5} \\
             CS-D & & & 0.403 & 0.927 \\ %0.1, 5.6
             S $+$ CS-D & & & 0.406 & 0.967 \\
              \hline\hline
		\end{tabular}
	\caption{S $+$ D relevance using partial queries evaluated by D.}
	\label{tab:zero-shot}
\end{table}
}


\comments{
\begin{table}
      \begin{tabular}{ r r r r r  }
			\hline\hline
			\% Queries Kept & \multicolumn{2}{c}{50\%} & \multicolumn{2}{c}{75\%} \\
			& MRR@10 & R@10 & MRR@10 & R@10\\
              \hline
             \multicolumn{5}{l}{\it{Feature Group Removal}}\\
             default & 0.417 & 0.702 & 0.422 & 0.709 \\
             w/o Sparse vs. Dense & 0.413 & 0.697 & 0.419 & 0.706 \\
 w/t sparse/dense score& 0.414& 0.700& 0.420&0.706\\
 w/t sparse/dense number& 0.416& 0.704& 0.421&0.708\\ %0.0.2
             w/o Query Quality& 0.414 & 0.700 & 0.422& 0.707 \\ % 0.0.1
             Random Removal & 0.411 & 0.693 & 0.418 &0.700 \\
              \hline\hline
		\end{tabular}
	\caption{S $+$ D relevance using partial queries evaluated by D.}
	\label{tab:query_level}
\end{table}
}
\comments{
\subsection{Effect of Merging}




\subsection{Feature List Query-level Model}

We compute the following features based on the orginal query and its expanded query using a sparse retriever's  encoder. 
When computing the embedding of each token or the original query, we use the denser retriever's encoder. 
\begin{enumerate}
    \item The length of the original query and the expanded query in terms of  the  number of words or tokens, respectively. 
    \item The token-based similarity between the expanded query and the original query. 
For each query token in the expanded query, we evaluate the similarity between its token embedding and  the oringal query embedding. 
Based on their similarity to the query, we map these tokens into five bins with  ranges <0.5, 0.5-0.6, 0.6-0.7, 0.7-0.8, >0.8.
We derive a similarity count vector after this mapping?
    \item The matching score of the whole query.??? The similarity between the CLS embeddings of the orginal query and the expanded query.
    \item The sum of matching scores of a token group/  The matching score of whole query. The token groups are the tokens with similarities in each bin.
    \item The sum of matching scores of tokens not in NLTK english corpus /  The matching score of whole query. 
    \item number of overlapping tokens between expanded and original query / number of all unique queries in both expanded and original query.
    \item number of  tokens only in expanded query / number of all unique queries in both expanded and original query.
    \item overall/mean/max of token weight of overlapping tokens between expanded and original query in the expanded query.
    \item max/min/mean of token weights of expanded query tokens.
\end{enumerate}

Sparse Matching score distribution:
\begin{enumerate}
    \item sparse scores of top 1-10 results
    \item mean sparse score of top 10-20/20-30/30-40/40-50/50-100/100-400/400-700/700-1000 documents.
\end{enumerate}


Sparse and Dense relational features:
\begin{enumerate}
    \item The number of dense clusters containing top 5/10/20/50/100/1000 results from sparse system
\end{enumerate}


\subsection{Feature List for Each Centroid in Cluster-Select Model}

\begin{enumerate}
    \item query-centroid similarities
    \item the distance between this centroid and the other top k centroids for this query (k=128)
    \item mean distance between this centroid and the rest of centroids (top 129+)
    \item Number of clusters containing top 10/25/50/100/200/500/1k documents in the sparse results
    \item mean sparse scores of top 10/25/50/100/200/500/1k documents 
\end{enumerate}

\begin{table}[ht]
    \centering
    \resizebox{1.05\columnwidth}{!}{

    \begin{tabular}{l |l}
        \hline
    Query    & "what is mechanical advantages in science terms"\\
    \hline
Relevance Doc & ["mechanical", 414.8], ["advantage", 226.3], ["advantages", 163.9], ["benefit", 97.9], \\
& ["definition", 82.2], [",", 64.1], ["is", 43.1], ["purpose", 15.5]  \\
Top 5 Doc & ["mechanical", 423.1], ["advantage", 228.9], ["advantages", 170.0], ["benefit", 95.3], \\
& ["definition", 83.4], [",", 65.0], ["is", 45.4], ["science", 24.6], ["purpose", 23.5], \\
& ["scientific", 15.0] \\
        \hline
    \end{tabular}
    }
\caption{Splade Expansion Example on Query Quality}
\label{tab:example}
\end{table}

\subsection{How to combine two ranked list}
There are two commonly used method to combine the sparse and dense ranked lists:
\begin{enumerate}
    \item linear combination
    \item reciprocal rank fusion
\end{enumerate}
For linear combination, the final ranking score of a document is the weighted sum of the ranking score of two systems perspectively. The weight on each system can be determined through grid search on a left-out training set or just use 1:1 combination. In this case, rescaling of the two ranked lists are necessary as the it largely affects the impact of a ranked list to the merged ranked list. 

On the other hand, reciprocal rank fusion alleviate the scoring distribution difference by only considering the ranking positions when merging. 

Another consideration is on the missing values. The two ranked lists are usually not fully overlap. Some documents only exists in one ranked lists. Thus the treatment on these documents affects model performance. We consider a few options
\begin{enumerate}
    \item Remove the documents when they only exist in one ranked list
    \item  Take the document and compute the score for only one ranked list
    \item Impute the missing document with rank K+1 or score as 0.95 * min(score) in the ranked list.
\end{enumerate}
}



==> expe_sparse.tex <==
\subsection{CluSD under  different sparse models}
\label{sect:evalsparse}

%We explore the model performance when we interpolate different sparse model with SimLM with cluster selection in 
Table~\ref{tab:sparse} examines the outcome  of CluSD when employing
three sparse retrievers with different efficiency/relevance tradeoffs. 
These sparse models accomplish  different relevance  scores: 
the fastest BM25 model 
delivers the lowest MRR number
while the slowest Splade-HT1 takes more time but has a higher MRR@10 number.
For all three models, CluSD supplements sparse results and boosts the overall retrieval relevance.
The final relevance outcome of using two SPLADE models is better  than that for BM25 retriever.
%That is partially caused by dependence of LSTM training where  the positive clusters are identified by the overlap of top 10 SPLADE results with these  clusters.
It is because the LSTM model uses  the overlap feature  of top sparse results with dense clusters,
the quality of top sparse results still has an impact on the final outcome.  
%consists of the distribution of sparse top results into clusters. 
%When the sparse model doesn't identify good top candidates, the input features to the LSTM model becomes more noisy which affect performance. 
\comments{
From left to right, the model performance degrades. 
We can observe that when sparse model performance degrades, 
the performance of S + CluSD degrades as well on the flat index. 
For example, on Splade-HT1-fast, the relevance is around the same as S $+$ D on MRR@10, and 0.6\% degradation on recall@1k. 
When we use BM25-T5 model, the degradation is 1.7\% and 1.5\% respectively on MRR@10 and recall@1k. 
This indicates that when the Splade model model does not perform well, CluSD becomes less effective. 
It is expected because the input to the LSTM model consists of the distribution of sparse top results into clusters. 
When the sparse model does not identify good top candidates, the input features to the LSTM model become more noisy which affects performance.
}

\begin{table}[htbp]
	\centering
		\resizebox{\columnwidth}{!}{%
		\begin{tabular}{ r l l  |ll |ll |r }
			\hline\hline
                Sparse Model& \multicolumn{2}{c|}{\bf{Splade-HT1-fast}} & \multicolumn{2}{c|}{\bf{Splade\_effi-HT3}}   & \multicolumn{2}{c|}{\bf{BM25-T5}} & Extra\\ 
%\cline{1-7}
                Latency & \multicolumn{2}{c|}{22.4ms} & \multicolumn{2}{c|}{12.4 ms}   & \multicolumn{2}{c|}{9.2 ms} & Latency\\ 
\cline{1-7}
			& {MRR@10} & {R@1k}  & {MRR@10} & {R@1k}   & {MRR@10} & R@1k  & ms \\
   \hline
   \multicolumn{8}{c}{\bf{uncompressed flat embedding. Embedding space  27.2 GB}}\\
			\hline
			S & 0.385$^\dag$& 0.949$^\dag$& 0.380$^\dag$& 0.944$^\dag$& 0.259$^\dag$& 0.935$^\dag$& -\\
                $\blacktriangle$  S $+$ D & 0.416 & 0.986 & 0.413 & 0.984 & 0.415 & 0.985  & +1674.1\\
                {\textbf{S $+$ CluSD}} & 0.415 & 0.981$^\dag$& 0.411 & 0.979$^\dag$& 0.408& 0.970$^\dag$& +12.1 \\
                \hline
                \multicolumn{8}{c}{\bf{OPQ m=128. Embedding space  1.1 GB}}\\
%, Report S+*
\hline
                S $+$ D-IVFOPQ & 0.384$^\dag$& 0.981$^\dag$& 0.381$^\dag$& 0.978$^\dag$& 0.369$^\dag$& 0.975$^\dag$& +21.9 \\
                %S $+$ D=HNSWOPQ & & & & & & &  \\
                \bf{S $+$ CluSD} & 0.413& 0.984& 0.412& 0.984& 0.402$^\dag$& 0.975$^\dag$& +9.8  \\
                %\hline
                %\multicolumn{8}{c}{OPQ M=64. Embedding space  0.6 GB}\\
%, Report S+*
                % S $+$ IVFOPQ-5\% & 0.389 & 0.981 & 0.389 & 0.980 & 0.370 & 0.975 & 23.7 \\
                %S $+$ HNSWOPQ & & & & & & &  \\
                %S $+$ \bf{CS} & 0.402& 0.981& 0.402& 0.981& 0.380& 0.973& 10.2 \\
            \hline\hline
		\end{tabular}
		}
	\caption{CluSD performance  under  three  sparse models}

\vspace*{-5mm}
	\label{tab:sparse}
\end{table}
% For all three sparse models, we use the same dense model configuration so for each row we only report one latency number. 


\comment{
\begin{table}[htbp]
	\centering
		\resizebox{\columnwidth}{!}{%
		\begin{tabular}{ r r r r r  r r r}
			\hline\hline
			& \multicolumn{2}{c}{MSMARCO Dev}& \multicolumn{2}{c}{DL19}& 
\multicolumn{2}{c}{DL20} \\
			& \% n& MRR@10 & R@1k & NDCG@10 & R@1k &  NDCG@10 & R@1k\\
   			\hline
 D& -- & 0.416& 0.988& 0.720& 0.744& 0.703&0.755\\
            $\blacktriangle$  S $+$ D & -- & 0.425 & 0.988 &  0.740& 0.816&   0.731& 0.819\\
            \bf S $+$ \bf{CluSD} & 0.5 &  0.426 & 0.987 &  0.744&  0.820& 0.734&  0.818\\
            \hline
            \multicolumn{8}{c}{OPQ M=128 setting, Storage 1.1GB, Report S+*}\\
            \hline
            IVFOPQ &10 & 0.404 & 0.987 & 0.713 & 0.818 & 0.722 & 0.817 \\
            & 5 & 0.394 & 0.987 & 0.687 & 0.817 & 0.706 & 0.817 \\
            & 2 & 0.374 & 0.986 & 0.656 & 0.815 & 0.700 & 0.817 \\
            HNSWOPQ & & & & & & \\
            \bf{CS} & 0.5 & 0.417& 0.986& 0.742 & 0.818 & 0.735  &0.815 \\
            \hline
            \multicolumn{8}{c}{OPQ M=64, Storage 0.6 GB, Report S+*}\\
            \hline
            IVFOPQ & 10 & 0.393 & 0.986 & 0.676 & 0.814 & 0.730 & 0.818 \\
            & 5 & 0.384 & 0.985 & 0.659 & 0.814 & 0.717 & 0.817 \\
            & 2 & 0.368 & 0.985 & 0.643 & 0.814 & 0.707 & 0.816 \\
            HNSWOPQ & & & & & & & \\
            \bf{CS} & 0.5  & 0.403& 0.987& 0.729 & 0.812 &0.724 & 0.814 \\           
			\hline\hline
		\end{tabular}
		}
	\caption{RetroMAE
%For quantization methods on top of ColBERT, we also report \% degradation from ColBERT.
}
	\label{tab:retromae}
\end{table}
}



==> experiments.tex <==
\section{Evaluations}

Our evaluation answers  the following research questions around our proposed techniques and the correspond subsection are marked.

\textbf{RQ1} (Section~\ref{sect:eval0space}): 
How does CluSD compare against other low-cost baselines when space is constrained?
%extra space overhead is minimized by augmentation under different compression configurations? 

\textbf{RQ2} (Section~\ref{sect:evaltimebudget}): 
How does CluSD  perform under a retrieval latency time budget when there is no space restriction?

\textbf{RQ3} (Section~\ref{sect:evalbeir}): 
How does CluSD  perform in searching  out-of-domain text content?
Zero-shot retrieval performance is important since a large dataset can contain documents from many domains. 


\textbf{RQ4} (Section~\ref{sect:evalLSTM}): 
Is  LSTM with cluster pruning preferred compared to other design options?
Are  features designed for LSTM useful?

\textbf{RQ5} 
(Section~\ref{sect:clusterno}): 
How does the number of clusters used in dataset partitioning 
affect the relevance and latency of CluSD? 

\textbf{RQ6} 
(Section~\ref{sect:threshold}):
How does the choice of selection threshold value in LSTM affect the average number of clusters selected?
%Does the cluster selection model dynamically select different number of clusters for different queries? How the selection differs for different datasets?

\textbf{RQ7}
(Section~\ref{sect:evalsparse}):
How does CluSD perform in augmenting  different sparse retrievers with different efficiency and relevance characteristics?


\comments{
To answer \textbf{RQ1},  we compare our proposed approach on the in domain test set, MSMARCO passage dev, DL 19, 20 with other commonly used techniques under storage (Table~\ref{tab:mainspace}) and latency constraints (Tabel~\ref{tab:maintime}).  
For \textbf{RQ2}, as our cluster selection technique requires training, we would like to understand how the approach would work on our domain dataset. In Table~\ref{tab:beir}, we use our cluster selection model trained on MS MARCO datasets on the 13 datasets from BEIR on a zero-shot manner and observe promising performance on all 13 out-domain datasets. 
For \textbf{RQ3} and \textbf{RQ4}, We compare the different cluster selection techniques, including heuristic approaches, a point-wise prediction model xgboost and a vanilla RNN prediction model against the proposed LSTM model (Table~\ref{tab:cluster_feat}).
To answer \textbf{RQ5}, we take two scenarios where the number of clusters is 4096, and 8192. Then we present the relevance in MRR@10, recall@1000, and the latency in terms of mean and 99 percentile time under three settings: when the flat index is used without compression, when we use OPQ to compress with m=128 or 64. Results are shown in Figure~\ref{fig:ncluster}.
For \textbf{RQ6}, we first plot the distribution of the number of clusters selected for each query under different model prediction thresholds. We also plot the average number of clusters for MSMARCO dev set and BEIR in Figure~\ref{fig:thresholds}.
For \textbf{RQ7}, we report the performance using three weaker sparse retrievers in Table~\ref{tab:sparse}. 
}

\subsection{Datasets and measures}
Our evaluation uses the MS MARCO datasets for full passage ranking~\cite{Campos2016MSMARCO,Craswell2020OverviewOT}. 
MS MARCO contains  8.8 million passages and about 1.1  judgment label per query. 
%The average number of WordPiece~\cite{wordpiece} tokens per passage is 67.5.
The development (Dev) query set contains  6980 test queries. %with about 1.1  judgment label per query. 
The test sets in  TREC deep learning (DL)  2019 and 2020 tracks 
provide 43 and 54 queries, respectively, with many judgment labels per query.
%which provide 54 and 43 test queries, repsectively,  
Following the common practice for the Dev set of MS MARCO,
%official leader-board standard, 
we report mean reciprocal rank at 10 (MRR@10) and recall at 1000 (recall@1K) 
which is the percentage of relevant-labeled results appeared in the final top-1000 results.
%we report mean reciprocal rank (MRR@10) for relevance instead of
%Normalized discounted cumulative gain (NDCG)~\cite{NDCG}  is not used because such a set has about 1.1 judgment label per query, which is too sparse to use NDCG.
For TREC DL test sets which have many judgment labels per query, we report the commonly used NDCG@10 score.
% when space allowed, we also report the recall@1k. 

%If space allows,
%In addition, we also report recall at 50 (recall@50) 
%as if we use large language model as a reranker, it is common practice to take less than 100 documents from retrieval model for evaluation.
%For TREC DL test sets which have many judgment labels per query, we report the commonly used NDCG@10 score.
%When space allows, we also report the recall ratio at 1000 

We also we use a collection called BEIR which contains the 13 publicly available datasets~\cite{thakur2021beir} 
for evaluating zero-shot retrieval performance. 
BEIR is a heterogeneous benchmark containing a variety of IR tasks, 
including search tasks (e.g.  question-answering, bio-medical IR, and entity retrieval)  
and semantic relatedness tasks (e.g.  duplicate question retrieval). 
The size of these data sets ranges from 3,633 to 5.4M.
%Their average query length ranges from 5.39 to 192.98, 
%and  their average document length ranges from 11.44 to 634.79. 
%Each dataset has binary or three-level relevance labels.
We report average NDCG@10 for the BEIR datasets. 

\subsection{Models and parameters}
For sparse retrieval, we adopt 3 SPLADE-based  models and one BM25 based model with different relevance/efficiency  tradeoffs:
1) SPLADE-HT1 is based on   a recent SPLADE model optimized by  hybrid thresholding~\cite{2023SIGIR-Qiao}
and BM25-guided traversal~\cite{mallia2022faster,qiao2023optimizing} with index space 3.9GB
and 31.2 ms retrieval latency. 2) SPLADE-HT1-fast is a variation of SPLADE-HT1 with a different parameter setting, which has 
3.9GB index space and 22.4 ms latency. 
3) SPLADE-effi-HT3 is the SPLADE-efficient model~\cite{Lassance2022SPLADE-efficient} with 3GB space
and  12.4ms latency due to use of hybrid thresholding and BM25 guided traversal techniques. 
4) BM25-T5 applies  the BM25 lexical model on expanded documents using DocT5Query~\cite{Cheriton2019doct5query}. 
BM25-T5 uses 1.2GB index space with latency 9.2ms. 
For dense retrieval, we adopt the recently published   dense models
SimLM~\cite{Wang2022SimLM} and RetroMAE~\cite{Liu2022RetroMAE}. 
We use their   checkpoints from the Huggingface library to generate document and query embeddings 
and  use  K-means in the FAISS library~\cite{johnson2019billion} to derive dense embedding clusters.
Our evaluation implementation uses C++ and Python and the
related code will be released to the public after publication of this paper. 
\comments{
%Note that SimLM model's embeddings are normalized while RetroMAE's embeddings are not. 
For sparse retrieval, we use two fast versions of SPLADE and a SPLADE-efficient model, as well as BM25-T5. 
The implementation of SPLADE models follows 2GTI optimization~\cite{qiao2023optimizing}. %its official release~\cite{spladeRepo}. 
SPLADE-HT1 is the SPLADE model trained with hybrid thresholding scheme~\cite{2023SIGIR-Qiao} using $\lambda_{t}=1$, 
SPLADE-effi-HT3
is the SPLADE-efficient model~\cite{Lassance2022SPLADE-efficient} trained with hybrid thresholding scheme using $\lambda_{t}=3$. Both of these two models are using the "accurate" configuration in 2GTI during retrieval, while SPLADE-HT1-fast uses the "fast" configuration.
The sparse retrieval code for Splade and BM25-T5 uses the code from PISA~\cite{mallia2019pisa}
with some optimization~\cite{Lassance2022SPLADE-efficient,2023SIGIR-Qiao}.
}

To train the CluSD model, we sample 5000 queries from the MS MARCO training set 
%and use the LSTM unit in Pyytorch. 
and the hidden dimension for LSTM is 32. The models are trained for 150 epochs. 
%The input documents are sorted based on the distance between the centroids the documents belong to and  the query. 
For sparse and dense model interpolation, we use min-max normalization to rescale the top results per query. 
%Then we use linear combination with equal weights to combine two ranked lists. 
For  BM25-T5, the interpolation  weights are  0.05 and 0.95 for sparse  and  dense scores, respectively. 
For SPLADE, they are  0.5 and  0.5, respectively. 
%In terms of missing document in either ranked list, as the smallest value from each normalized list is 0, there is no missing imputation needed as we 
%can view the missing  documents taking the value of the worst document in the ranked list automatically. 
For CluSD, the default setting of number of clusters is $N=8192$, and the input sequence length to the LSTM model is truncated at $n=32$.  
To report the mean single-query latency and 99 percentile latency in milliseconds,
we  run test queries multiple times  from MS MARCO Dev set using a single thread on  a 2.25GHz AMD EPYC 7742  CPU server. 

\subsection{Baselines and notations}
%We select two groups of baselines under space and time constraints respectively.

Table~\ref{tab:mainspace} compares  baselines  with memory space constraint. 
We include dense retrieval with quantization option OPQ and  IVFOPQ with IVF clustering available in FAISS.
OPQ quantization  is configured with  the number of codebooks as $m=$ 128 or 64.  
When IVF clustering is used,  we report its performance  using top 10\%, 5\%, 2\% clusters respectively
as a standard approach which performs   limited top cluster retrieval. 
CluSD execution is also based on the the same OPQ or  IVFOPQ index from  FAISS but clusters are  selected  by our LSTM model. 
%Switching a quantization different  from OPQ  is might result in an improvement in relevance, but it is orthogonal to our proposal. 
We use notation ``S+D'' to report the interpolated performance of a sparse model and a dense model in Table~\ref{tab:mainspace} and Table~\ref{tab:sparse}.

Table~\ref{tab:maintime} compares  baselines  without  memory space constraint. 
For proximity graph-based dense retrieval which incurs additional graph space overhead,
we include  HNSW~\cite{2020TPAMI-HNSW} and  LADR~\cite{2023SIGIR-LADR} as shown in Table~\ref{tab:maintime}. 
%For HNSW, we fix the number of neighbors to be 128 and vary the expansion factor(ef) to meet the latency constraint. 
%For LADR, we use its default setting with seed = 200, number of neighbor = 128 and use the exploration depth as 50 to meet the latency requirements in 
%Table~\ref{tab:maintime}.
%Uncompressed dense embeddings (marked as "flat") are used
%to exclude the impact due to quantization.
We also compare  a simple re-ranking method,  denoted as ``D-rerank'' or ``rrk'', 
that fetches the dense scores of top 1000 of sparse retrieval to re-rank with interpolation. 
%We use the same clustering setting for IVF and CluSD. 

%The reported CluSD performance on the flat index uses the exact same IVF index. 
The configuration we selected to meet the latency requirement for CluSD uses on average 20-25 (0.25 - 0.3\%) clusters per query. 
%For re-ranking, we report the results of re-ranking top 1000 results from the sparse model using the dense model.  

For MS MARCO Dev set, the result of a method is marked with  tag $^\dag$ when 
statistically significant drop is observed compared to  an oracle baseline
tagged with $\blacktriangle$ at 5\% confidence level.  This oracle
is sparse retrieval fused with full dense retrieval marked as ``S+D'', which typically delivers the highest relevance  
using all uncompressed or quantized dense embeddings ($m=128$ or $m=64$).


==> intro.tex <==


\section{Introduction}



Sparse and dense retrievers are two main categories of retrieval techniques for text  document search.
Traditional sparse retrieval models, such as BM25, use lexical text matching and run
%to retrieve results from the collection 
efficiently by traversing  an inverted index on an inexpensive  CPU platform.
Recently sparse retrieval studies have exploited learned neural representations~\cite{Dai2020deepct,
Mallia2021deepimpact, Lin2021unicoil,2021NAACL-Gao-COIL, Formal2021SPLADE, Formal2021SPLADEV2} for better semantic matching. 
%and SPLADE~\cite{Formal2021SPLADE, Formal2021SPLADEV2} has demonstrated the strong relevance performance among these models. 
The second category of document retrieval 
exploits a pre-trained language model with a dual encoder architecture to produce a dense document representation, 
e.g. ~\cite{gao-2021-condenser,2021SIGIR-Zhan-ADORE-dense,Ren2021RocketQAv2, 
%e.g. ~\cite{Lin2021tctcolbert, 2021CIKM-JPQ-Zhan, xiong2021-ANCE, gao-2021-condenser,2021SIGIR-Zhan-ADORE-dense,Ren2021RocketQAv2}. 
%There are numerious studies recently to enhance  dense retrieval with knowledge distillation
%and  improved  langage model pretraining~\cite
Lin2021tctcolbert, Santhanam2021ColBERTv2,  Wang2022SimLM,  Liu2022RetroMAE}.

\comments{
Recent studies have found that combining  sparse and dense retrieval scores  can further boost
retrieval recall and relevance~\cite{Lin2021unicoil,2022LinearInterpolationJimLin,kuzi2020leveraging},
suggest  that both categories  of retrievers tend to capture  different relevant signals. 
These studies  make an assumption that  a search platform has to run two retrievers separately and a dense retriever.
%delivers   its maximum effectiveness, and the impact of compression and IVF clustering is not considered. 
There is an imbalance of computing platform requirement for running  these two retrievers.

dense retrieval typically requires GPU support unless significant  
%We study the use of dense retrieval results to argument sparse retrieval. 
Sparse retrieval with an inverted index has an advantage that a low-cost CPU server can run the online inference  without GPU.
}
A judicious tradeoff consideration of retrieval  effectiveness and efficiency is critical on  a low-cost CPU-friendly search platform. 
The importance of CPU-friendly search is recognized 
in neural ranking studies~\cite{Yang2021WSDM-BECR,2022WWWforwardIndex,2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
For a large-scale  dataset (e.g. with billions of documents), a practical search system often employs  a multi-stage 
search architecture, which divides the dataset into many partitions so that  a fast first-stage  retrieval 
method  can  search these partitions in parallel.  Such a system  prefers low-cost
CPU-only servers for first-stage retrieval, and both time and memory space complexity of retrieval should be considered 
so that  each server can host as many documents as possible
to reduce the total number of servers to support a large data size and high query traffic. 
%Thus the challenge for retrieval on such an architecture needs to consider both time and space complexity. 
% small search index needs to be as small as possible.
%and the in-memory footprint size of 
%server  needs to host documents in memory as many as possible 
%given a large number  of data partitions involved for parallel search.
%Each server employs multiple CPU cores and is replicated with many copies  for dealing high traffic of  concurrent 
%search requests, and thus 


There are several recent efficiency studies advancing the
inverted index implementation for sparse retrieval with learned neural 
representations~\cite{Lassance2022SPLADE-efficient,mallia2022faster,qiao2023optimizing,2023SIGIR-Qiao, 2023SIGIR-SPLADE-pruning},
%which run  efficiently  on a single CPU without hardware accelerators  GPU
%which re  retaining strong relevance effectiveness
%%Another development in learned sparse retrieval is that
%sparse retrieval with a learned representation
which accelerates learned sparse retrieval with BM25-guided traversal or index pruning.
For example, Row 3 of Table~\ref{tab:costbudget} shows the latency, memory space cost, and  MRR@10  of
a latest efficient SPLADE retriever for searching 8.8 million 
MS MARCO passages~\cite{2023SIGIR-Qiao} on a CPU only server.
% with a single thread on  a 2.25GHz AMD EPYC 7742  CPU server.
Row 2 is performance of a BM25 based retriever after document expansion. 
%There is a tradeoff  in relevance effectiveness if BM25 guidance or threshold-based pruning  is too aggressive.
%and dense retrieval can boost if it does not add much overhead. 
On the other hand, 
the cost  of dense retrieval can be greatly reduced  by using  approximate nearest neighbor (ANN) search with 
IVF clustering~\cite{johnson2019billion, 2021Facebook-DrBoost-Lewis}, quantization~\cite{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ},
%and hierachical navigable  small world graphs (HNSW)
and  proximity graph based navigation~\cite{2020TPAMI-HNSW,2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
However, there is a  relevance tradeoff for a  reduced search cost.
For the example in  Table~\ref{tab:costbudget},  
while RetroMAE~\cite{Liu2022RetroMAE} dense retrieval without compression is slow, use of
IVF clustering and OPQ quantization substantially accelerates but leads to a significant drop  of   MRR@10 score when searching up-to 20\%  
of top dense clusters. 
There is also a cost-relevance tradeoff  with proximity graph based search  using inter-document similarity distances~\cite{2020TPAMI-HNSW, 
2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}.  Document-level  graph  construction is  expensive
for a large dataset during offline processing. The online hosting of such a graph also adds a significant space requirement  on a low-cost
computing platform. For example, the proximity graph  can take extra 4.3GB memory space~\cite{2023SIGIR-LADR}
for 8.8M  passages in the MS MARCO dataset.
% to keep top 128 top neighbors per document. 
\comments{
That is true also with the  navigation of  a  proximity graph based on inter-document similarity distances called HNSW~\cite{2020TPAMI-HNSW}. 
The proximity graph approach to guide dense retrieval is revisited recently in GAR~\cite{2022CIKM-MacAvaneyGraphReRank}, which is furthered improved by
%LADR Kulkarni  et al.~\cite{2023SIGIR-LADR} improves HNSW.
LADR~\cite{2023SIGIR-LADR}.
%~\cite{2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
The weakness of  the  proximity graph approach is that its graph  construction requires a quadratic computing complexity, which is expensive
for a large dataset and the online hosting of such a graph also adds a significant space requirement  on a low-cost
computing platform. For example, LADR takes extra 4.3GB memory space for 8.8M  passages in the MS MARCO dataset to keep top 128 
top neighbors per document. 
%Similarily HNSW also incurs a high space cost for graph connections.  
%In comparison, cluster-based selective dense retrieval can achieve in a comparable time complexity
%while adding  insignificant extra  space  overhead.
}

\begin{table}[htbp]
        \centering      
         \resizebox{0.82\columnwidth}{!}{ 
                \begin{tabular}{ r | r  rr}
                        \hline\hline
Sparse or dense methods  & Latency & Memory & MRR@10\\ 
\hline
BM25/DocT5Query & 9.2ms & 1.2GB & 0.261\\  
SPLADE/HT1 & 31.2ms & 3.9GB & 0.396 \\ 
RetroMAE/Uncompressed & 1677ms & 27.2GB & 0.419 \\ 
%SimLM /OPQ             & 225-1579ms & 0.57-2.3GB & $<$ 40.2 \\
RetroMAE /IVFOPQ  & 38-339ms & 1.2-2.3GB  & 0.37-0.401\\ 
                        \hline\hline
\end{tabular}
}
\caption{Latency and space cost of sampled sparse and dense models for MS MARCO passages with Dev query  set}
 \vspace*{-5mm}
\label{tab:costbudget}
\end{table}



  
%with a latency controled within 4 to 8 milliseconds on a single CPU, but with a significant tradeoff in relevance effectiveness.
%For example, MRR@10 for MS MARCO Dev set drops from RetroMAE has dropped from  0.416 to 0.356.
%This paper does not impose 4-8 millisecond latency, but rather looks for a solution that can leverage both dense and sparse retrieval
%and relax the latency constraint in some degree while maximizing its relevance effectiveness as much possible.
%a range below or around  100 milliseconds 

%The response time  for such a system for an interactive service needs to be fast enough a
%and thus search needs to be completed within a few hundred milliseconds. 

%which only requires triggering of dense embedding  computation for a relaively small subset of documents.
%The proposed scheme called cluster-based selective dense  retrieval



This paper proposes  to  augment sparse retrieval with 
cluster-based selective dense retrieval called CluSD which
leverages the clustering of documents   under an advanced dense retrieval model after  a sparse retrieval phase.
CluSD includes an LSTM based model with cluster prioritization and pruning to 
trigger limited dense computation. 
CluSD exploits inter-cluster and query-to-cluster distances and   the overlapping degree between top sparse retrieval results and dense clusters
to optimize cluster selection. 
%and then make a decision to determine which document clusters should be selected  to conduct dense retrieval computation.
The extra memory space overhead required to assist CluSD is negligible, and it  
works well when embedding vectors are highly compressed.
%  and  the extra memory required for hosting dense embeddings can be limited  after compression. 

This paper evaluates  the usefulness   of CluSD  under a time and space constraint on a CPU only server when
 searching MS MARCO and BEIR  datasets  and provides a comparison with other baselines.
The evaluation  shows that CluSD can effectively identify a small number of document clusters to augment sparse retrieval results efficiently 
for  a stronger relevance  even though such a  sparse retriever is fast with  a relevance tradeoff. 
 
%provides a flexibility and reduces  the relevance reqirement of sparse retrieval.
%Namely protentially we can choose a relatively fast sparse retrival with the slightly lower accuracy/recall,
%and  let dense retrivsal make up the loss. Our design needs to  adapt to  sparse retrieval quality and plans

%CSDR in improving the effectiveness of sparse retrieval with limited dense  retrieval
%traversal for low-cost search.  Our emprial findings suggest that SRF  can consistently outperform other baselines on a single CPU server 
%without GPUs 
% and achieve a strong tradeoff of effectiveness and efficiency compared to an exhausitve dense retrieval search.


%from pretrained language models to provide effective semantic text matching between a query and a document.





%0.419 by RocketQAv2~\cite{Ren2021RocketQAv2}, 
%which are the two latest state-of-the-art retrieval-reranker pipelines using cross-encoder based rerankers.
%Re-ranking in  recent dense retrieval work SimLM~\cite{Wang2022SimLM} has  used an expensive cross-encoder to
%achieve impressive MRR score 0.437 
%Re-ranking in RocketQAv2~\cite{Ren2021RocketQAv2} achieves 0.419 with a similar strategy.  



\comments{Modern search engines for text documents
typically employ two-stage ranking design. 
The first retrieval stage extracts top candidate
documents matching a query from a large search index with a fast ranking method. 
The second stage uses a more complex algorithm to 
re-rank top results thoroughly.
Recently neural ranking techniques from transformer-based architectures
have achieved impressive relevance scores 
for both retrieval and top $k$ document re-ranking. 
However, many recent work treats retrieval and reranking stage as two independent tasks and optimize them separately. Only a few works take into consideration the interplay of a retriever and a reranker. RocketQAv2 trains a cross encoder reranker and dual encoder retriever jointly with a strong reranker as teacher and train the retriever by dynamically distilling from reranker. Leonhardt (2022)\footnote{https://arxiv.org/pdf/2110.06051.pdf} uses a linear combination of the semantic similarity scores from the re-ranking phase and lexical matching scores from the retrieval phase with respect to the query for query evaluation.  

These methods either uses the reranker as a teacher to train the re-retriever, or consider the shallow combination of the results from two stages. In these training strategies, both the retriever and reranker are trained towards the same goal. In real application, as the two stages work jointly, either model does not need to perform perfectly by itself. Instead, by taking a more integrated view of the two stages in training and inference, the joint performance of the two stage models will be more efficient and effective. 

Moreover, these approaches typically requires a reranker (such as a cross-encoder in the case of RocketQA). In text retrieval applications, efficient rerankers with low online inference latency are often favored. In recent years, the late interaction reranking model ColBERT, TILDE, BECR provide reasonable performance with low query latency. We demonstrate that pipelines with such efficient models can be improved using our training strategy. 


In our work, we train the efficient reranker and retriever iteratively to improve the integrated performance of the two stage pipeline through a process termed dynamic integrated training.
 To achieve optimal performance under such setting, when training the reranker, we upweight the poorly ranked samples in the joint pipeline through a soft-hard loss. In the meanwhile we gradually update the training set with the top combined ranked results from pipeline during training. With these shifts, the model will automatically be geared towards the weak point of the joint ranking results of the pipeline. In addition, we employ the top documents retrieved by the retriever to provide additional ranking signal in both training and evaluation in the reranking stage. 


During inference, the retriever would return top documents and their corresponding rank order to formulate a pseudo query. The reranker then matches both the original query and the pseudo query with top documents to get two ranking scores for each query-document pair. As the reranker is trained as a booster, the final ranking order from the pipeline naturally becomes the combination of the retrieval and reranking ranked lists. The final top-k ranking scores is determined by the reciprocal ranked fusion~\footnote{https://plg.uwaterloo.ca/~gvcormac/cormacksigir09-rrf.pdf} of ranks given by both the retrieval and reranking models.

We find that the propose integrated strategy enjoys several advantages. First, under same model setting and training condition, the dynamic integrated training strategy improves the relevance of the two stage pipeline under both scenarios where reranker is an efficient one or reranker strongly outperforms retriever on MS MARCO passage dataset and TREC19 and TREC20 datasets. This indicates that the integrated training strategy is generally applicable.  Secondly, as the two models learn slightly different goals, the joint performance of the two is less likely to overfit. Indeed, we observe a good zero-shot performance of the pipeline on the BEIR dataset. Lastly, we find that our training strategy can be applicable to the currently popular sparse and dense retrieval pipeline where two retrieval models jointly determine the final ranking list. 

}


==> kddabstract.tex <==



\comment{
{\bf Old abstract:}
Recent studies show that neural sparse retrieval for searching  text documents with a learned neural representation
can be greatly accelerated but there are  tradeoffs  in its relevance effectiveness.
This paper proposes a relevance augmentation scheme of fast sparse  document retrieval with cluster-based selective dense retrieval called CluSD
on  a CPU-only platform.
CluSD takes an advantage of clustering under an advanced  dense retrieval model and
detects clusters of neural embeddings  that can boost sparse retrieval with  limited  extra memory space overhead and embedding selection and computing time. 
This paper provides a detailed evaluation of CluSD for searching  MS MARCO and BEIR  datasets, 
and demonstrates its effectiveness in improving the relevance metric of sparse retrieval by scoring  selected dense embedding clusters 
at a low time and space cost.


{\bf New abstract:}
}
Dense retrievers and sparse lexical retrievers are two main categories of the
first-stage search techniques for text  documents, both of which have benefited from pretrained language models.
Dense document retrieval is attractive  in semantic  matching between queries and
text  documents, though it can be time-consuming on a CPU-only platform.
The cost of dense retrieval can be mitigated through approximate nearest neighbor search techniques, including IVF clustering, quantization, and/or 
proximity graph navigation. However, this reduction in latency comes with a tradeoff  in relevance effectiveness. 
This paper proposes a cluster-based selective dense retrieval called CluSD with an augmentation from sparse lexical retrieval 
at a low space and CPU time cost. 
CluSD takes a lightweight cluster-based approach and exploits the overlap of sparse retrieval results and embedding clusters
using an LSTM model to quickly identify relevant clusters  while incurring limited  extra memory space overhead. 
CluSD  triggers limited dense retrieval, and combines it with  sparse results to enhance relevance. 
%advantage of clustering of embeddings from an advanced dense retrieval model, 
This paper provides a comprehensive evaluation of CluSD on both in-domain (the MS MARCO dataset) and out-of-domain (BEIR  datasets) search tasks
and demonstrates its effectiveness in relevance and efficiency.




==> kddbackground.tex <==
%\section{Related Work}
%\label{sect:background}

\textbf{Sparse and dense retrieval}
%A traditional method for first-stage retrieval uses 
%BM25 based additive ranking with a bag-of-words sparse document representation~\cite{Robertson2009BM25}
%and fast retrieval can be designed  using the inverted index data structure to exploit this
%sparse representation.
To improve traditional BM25 lexical sparse retrieval, 
%Meanwhile, an advancement in sparse retrieval with inverted indices is to 
%adopt learned sparse representations with neural term weights, which has
%yielded in  a significant relevance gain. 
%severl studies  have developed  
learned sparse representations with neural term weights have been studied in 
DeepCT~\cite{Dai2020deepct},
DeepImpact~\cite{Mallia2021deepimpact}, uniCOIL~\cite{Lin2021unicoil,2021NAACL-Gao-COIL},
and SPLADE~\cite{Formal2021SPLADE, Formal2021SPLADEV2}. 
Pre-training optimization of a language model for SPLADE-like retrieval is studied in LexMAE~\cite{shen2023lexmae}. 
Retriever efficiency optimization techniques have been developed for learned
sparse representations~\cite{Lassance2022SPLADE-efficient,mallia2022faster,qiao2023optimizing,2023SIGIR-Qiao, 2023SIGIR-SPLADE-pruning,2022ACMTransAnytime, 2022EMNLP-mackenzie-clipping} at various  efficiency and relevance tradeoffs.

%following the pretraining optimization in SimLM~\cite{Wang2022SimLM} and RetroMAE~\cite{Liu2022RetroMAE}.
\comments{
The  evaluation of our work for the first-stage retrieval
centers on the SPLADE family of sparse retrieval~\cite{Formal2021SPLADE, Formal2021SPLADEV2} 
because it can deliver a strong relevance with maintaining low space and time costs during inference.
For instance, SPLADE++~\cite{Formal2022SPLADE++} 
delivers 0.38 MRR@10 for the MS MARCO passage Dev set and it is possible to improve this score 
to 0.394 as shown in Section~\ref{sect:evaluation}.  

We use SPLADE in our evaluation because it has been well studied by  
a number of papers  with various efficiency optimization options as discussed below
and LexMAE has not made its checkpoints available for evaluation. 
Besides, using a sparse model like LexMAE with better language model pretraining is orthogonal and complementary to our study.
% not sure if the last sentence is needed
}

\comments{
Initially there was a concern
that online traversal  of  a learned  inverted index is significantly slower than a BM25 based index,
the recent efficiency studies such as guided traversal and index pruning with sparsification 
show that the  latency of learned sparse retrieval  can be 
reduced dramatically~\cite{Lassance2022SPLADE-efficient,mallia2022faster,qiao2023optimizing,2023SIGIR-SPLADE-pruning}.
%In~\cite{Qiao20222GT}, the model retrieves top 1000 documents in 43ms with 0.394 MRR@10, 25ms with 0.388 MRR@10, or 
%15ms with 0.379 MRR@10, under different index sizes respectively.
}

% should be approximate search or approximate nearest neighbor search
\comments{
This performance score is very close to 0.395 produced by
AR2 dense retrieval with approximate search which requires 8 NVIDIA Tesla A100 GPUs.
AR2 dense retrieval with approximate search using faiss 
IndexFlatIP~\footnote{https://faiss.ai/cpp_api/struct/structfaiss_1_1IndexFlatIP.html} 
which uses a flat index with exhaustive search.  
%Qiao20222GT.
%takes about a few hundred milliseconds without GPA support and can be further reduced to  up-to 80ms with a small relevance 
%tradeoff~\cite{Lassance2022SPLADE-efficient,AskYifan}.
Meanwhile, avoiding exhaustive exact search in  dense retrieval with approximate search comes with a 
tradeoff of  a relevance drop~\cite{2021Facebook-DrBoost-Lewis, johnson2019billion, Xiao2022Distill-VQ}.
For instance, %AR2 dense retrieval with exact search yields an MRR@10 of 0.395 while 
with Distill-VQ~\cite{Xiao2022Distill-VQ} , a recent 
joint IVF and PQ based ANN search framework, AR2 has an MRR@10 of 0.361 as opposed to 0.395.
%, which still needs GPU support
%because a dense retriever has a significant relerence loss when using faster but 

Notice that for a large-scale search system containing billions of documents, 
the first-stage fast retrieval is typically executed in parallel across many index partitions hosted on
a large number of  machines. In such cases, efficient retrieval with inexpensive hardware could be preferred. 

}

Dense retrieval is an alternative approach for the first-stage search with a dual encoder architecture
%For example, TCT-ColBERT~\cite{Lin2021tctcolbert} and  JPQ~\cite{2021CIKM-JPQ-Zhan}
(e.g. ~\cite{xiong2021-ANCE,gao-2021-condenser}).
Since the representation  for a document and a query is a dense vector,
%Efficiency studies for dense retrieval have been conducted on
fast dense retrieval for a large dataset requires
approximate nearest neighbor (ANN) search~\cite{johnson2019billion},
%exhaustive exact search~\cite{2021Facebook-DrBoost-Lewis}  
%and ~\cite{Xiao2022Distill-VQ}, 
or  a more expensive GPU server.
%and quantization~\citep{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ},
%applying dense retrieval on  a large dataset requires requires an approximate nereast neighbor search a more expensive GPU 
%, which is more suitable for a GPU-based platform for fast processing.
There are numerous recent studies to enhance  dense retrieval with knowledge distillation
and  improved  language model pretraining~\cite{Lin2021tctcolbert, Santhanam2021ColBERTv2,  Ren2021RocketQAv2,
Wang2022SimLM,  Liu2022RetroMAE}.

\comments{
Retrieval that uses a dense representation of documents and a dual-encoder (or also called bi-encoder) architecture 
outperforms BM25 significantly in relevance at the cost of relatively more expensive similarity computation
%For example, TCT-ColBERT~\cite{Lin2021tctcolbert} and  JPQ~\cite{2021CIKM-JPQ-Zhan}
(e.g. ~\cite{Lin2021tctcolbert, 2021CIKM-JPQ-Zhan, xiong2021-ANCE,gao-2021-condenser,2021SIGIR-Zhan-ADORE-dense,Ren2021RocketQAv2}). 
Efficiency studies for dense retrieval have been conducted on
approximate nearest neighbor (ANN) search~\cite{johnson2019billion} to avoid
exhaustive exact search~\cite{2021Facebook-DrBoost-Lewis}  and  quantization~\citep{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ}, 
%Meanwhile, avoiding exhaustive exact search in  dense retrieval with approximate search 
and these optimizations come with a tradeoff of  a relevance drop.
}

\textbf{Combining  dense and sparse retrieval}
%The earlier IR studies use the term fusion to combine rankers, e.g.  the reciprocal rank fusion (RRF)~\cite{Cormack2009RRF}.
Previous neural IR studies  have  considered combining the traditional lexical ranking signals and neural semantic matching signals~\cite{Mitra2017LearningTM,Shao2019PrivacyawareDR,Gao2020ComplementingLR,Luan2020SparseDA,Yang2021WSDM-BECR}. 
Recent work has found that combining  sparse and dense retrieval scores  
can further boost recall and/or other relevance metrics~\cite{Lin2021unicoil,2022LinearInterpolationJimLin, kuzi2020leveraging}, which
suggests  that both categories  of retrievers tend to capture  different relevant signals. However, these studies do not address the high  latency  of
dense retrieval on a CPU-only server.
% and do not consider impact of data compression  in dense retrieval. 
%The focus of this paper follows ~\cite{Lin2021unicoil,2022LinearInterpolationJimLin,kuzi2020leveraging} to 
%to combine the ranking results of two retrievers with a linear interpolation,
%
\comments{
We adopt 
a simple fusion wit linear combination ~\cite{Lin2021unicoil,2022LinearInterpolationJimLin,kuzi2020leveraging}, 
which allows the proposed techniques to  easily adopt the latest dense or sparse retriever models.
Our query filtering work is motivated by
the dense and sparse retriever selection study~\cite{2021CIKM-PredictDenseSparse}
when to use BM25 retriever or a  dense retriever.
The difference is our work always assumes sparse retrieval is conducted first, and our selection focuses on how to choose part of dense clusters.
Another difference is that we exploit the characteristics of a learned lexical representation in query encoding and expansion in making a query-level decision.
% filtering exploits the SPLADE encoding as SPLADE is our primary targeted sparse retrieval, even 
%our work is applicable to other sparse retrivers such as BM25. 
}

\textbf{Re-ranking} 
There  are many studies that exploit advanced re-ranking in a multi-stage search pipeline with modern
neural IR techniques (e.g. ~\cite{MacAvaney2019SIGIR-cedr, MacAvaney2020SIGIR-prettr, 2023SIGIR-ZhuangRankT5,Yang2022CQ,Zhuang2021TILDEv2,2022WWWforwardIndex}),
possibly leveraging more expensive GPU platforms to conduct complex scoring.
These  re-ranking pipelines perform very well but are inherently limited by the recall of the first-stage retrieval,
as noted in  ~\cite{2022CIKM-MacAvaneyGraphReRank, 2023SIGIR-LADR}. 
A focus of this work is improving the relevance of fast sparse retrievers by expanding the candidate pool of first-stage retrieval using 
selective dense retrieval, a CPU-friendly optimization that incurs small or modest additional CPU and space cost.
% Parker: I reworked below into above. Still might need work, but let me come back to it
%A  focus of this work is to enhance the relevance of retrieval with CPU-friendly low-cost optimization by expanding the candidate pool of  
%fast sparse retrieval using selective  dense retrieval at a modest amount of extra CPU cost and without incurring significant  space cost.  

\comments{
{\bf Cluster based retrieval and proximity graph navigation based on inter-document similarity.}
%with lexical matching
There is a large body of work on cluster-based document retrieval  in traditional IR
throughout the past few decades (e.g.  ~\cite{liu2004cluster,2022SIGIR-KurlandClusterRank,kurland2008opposite}).
In most cases, it has been applied to re-rank an initial retrieved list by creating clusters of similar  documents in this list. 
Then, the clusters are ranked, which may be further transformed to document rankings.  
%{\bf Proximity graph navagation based on inter-document similarity.}
Search with  inter-document similarity has also been studied~\cite{2006NAACL-docExpan}.
The above studies follow traditional IR   with  lexical signals. 
Advances in neural representations introduce new opportunities and challenges, as studied in  
GAR~\cite{2022CIKM-MacAvaneyGraphReRank} and LADR~\cite{2023SIGIR-LADR}, following
HNSW~\cite{2020TPAMI-HNSW} and NAPG~\cite{2021KDDgraphANN}
for proximity graph based search with inter-document similarity.
%~\cite{2020TPAMI-HNSW,2022CIKM-MacAvaneyGraphReRank, 2023SIGIR-LADR}.
% is viewed as  a modern instantiation 
%of the clustering hypothesis to revisit these ideas in a new context.  

Motivated by such studies, our work emphasizes fast selective dense retrieval to augment sparse retrieval effectively
without introducing substantial memory overhead by exploiting inter-cluster similarity and query-cluster similarity at a coarse-grain level. 
%Result overlapping degree of sparse retrieval with the dense clusters also plays a key role in the low-cost selection  of dense clusters.
}

\textbf{Approximate nearest neighbor search}
In addition to the IVF cluster 
search~\cite{johnson2019billion}, and proximity graph navigation such as HNSW~\cite{2020TPAMI-HNSW}, NAPG~\cite{2021KDDgraphANN},
GAR~\cite{2022CIKM-MacAvaneyGraphReRank},  and LADR~\cite{2023SIGIR-LADR}, discussed in Section~\ref{sect:intro}, 
\comments{
Faster dense retrieval can be accomplished by approximate nearest neighbor search~\cite{2021Facebook-DrBoost-Lewis, johnson2019billion} with 
a small number of top clusters  (e.g. IVF-based), which can run efficiently on a CPU-only  server.
The memory space cost of dense retrieval can be reduced significantly by 
embedding  quantization (e.g.  ~\cite{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ}).
However, these techniques have a tradeoff: a significant drop in relevance, as shown in these previous studies.
%Using these techniques has a tradeoff with a significant relevance drop as shown in these previous studies. 
Our evaluation confirms  that sparse retrieval aided with top IVF-based dense clusters does not yield a competitive relevance 
under a tight time budget.  
}
there  are studies on  cluster-based earlier termination studies for nearest neighbor search over a large   
feature vector collection~\cite{2020SIGMOD-ANNadaptive,2023USENIX-ANNcluster, 2023VLDB-FARGO}.
The use of locality sensitive hashing  for high-dimensional ANN search 
is studied in~\cite{2020VLDB-ANN-LSH,2023VLDB-FARGO,2015KDD-LSH-ANN} to approximate in
a projected space, and the improvement of a proximity graph is studied in~\cite{2021KDDgraphANN}.
DiskANN, SPANN,  and other follow-up studies~\cite{NEURIPS2019_DiskANN,2023Web-Filtered-DiskANN,2020NIPS-HM-ANN, chen2021spann}
address ANN search when data cannot fit in memory. 
The above techniques are targeted at general data applications and have not been studied in the context of text document retrieval,
where the importance of semantic matching presents a unique challenge and requires new design considerations.
Another key difference is that the above studies assume a standalone search task,
whereas we exploit the interaction of sparse and dense retrieval, requiring additional optimization.
%The above techniques are targeted for general data applications and  have not investigated in the context of text document  retrieval where
%semantic  matching relevance presents   its unique ranking challenge and  
%requires new design considerations and model structuring.  Another key difference is that the above studies assume a standalone search task.
%in our context the interaction of sparse retreival and dense retrieval  is exploited, which demands new optimization. 



==> kddconcl.tex <==
%\section{Limitations and Future Work}
\section{Concluding Remarks}

The main contribution of this work is  to  show  how 
a lightweight cluster-based partial dense retrieval 
with competitive  relevance can be made possible
to deliver fast response time on affordable computing platforms, without the need of an expensive  document-wise  proximity graph.
%CluSD carries with minimal space overhead compared to the orginal dense retrieval
%and incurrs a small amount of CPU latency time due to the limited dense computation.
\comments{
CluSD uses  an LSTM-based  model and  leverages sparse retrieval results to effectively identify  a small number of 
clusters that can supplement and boost the relevance of partial dense  retrieval.  
With this lightweight low-cost design,  
CluSD is suitable for a CPU-only low-cost server while delivering  a fairly strong  in-domain and out-of-domain relevance.  
For example, CluSD delivers 0.423 MRR@10  for searching 8.8M MS MARCO passages 
with 11.4ms  latency and  1.13GB space mainly for compressed dense embeddings, to augment sparse retrieval under
a fraction of its  cost. The same  CluSD version  reaches  0.514 average NDCG@10 for BEIR with compression.
That represents state-of-the-art relevance performance for a retriever that  runs on a CPU-only server. 
}
Guided by sparse retrieval, CluSD  outperforms  previous cluster-based partial dense retrieval with IVF 
search significantly in relevance under the same time budget.
For example, CluSD delivers 0.431 MRR@10  for searching 8.8M MS MARCO passages on its Dev test set taking only tens of milliseconds on a low-end CPU server
and reaches  0.516 average NDCG@10 for BEIR.  That represents a state-of-the-art relevance performance for a retriever that  runs on 
a CPU-only server. 
%The othe recent efficient retrievers reported 0.426  for MS MARCO Dev, and 0.48 for BEIR by LexMAE.
Its MRR@10 number is close to one reported recently using an expensive cross-encoder RankT5 which reaches 0.434~\cite{2023SIGIR-ZhuangRankT5}. 
%ClusD's BEIR performance is close to  that  of  Promptagator++~\cite{dai2023promptagator}.  Both  RankT5 and Promptagtor++h employ an expensive cross-encoder.
Noted that user search experience is highly impacted by the ranking order and its relevance thus a relatively small percentage point increase  
in metrics for the standard public test benchmarks used in this paper is viewed to be hard and valuable in the IR research literature.

%For example,
%Table ~\ref{tab:mainspace} shows CluSD is as fast as IVFOPQ top 2\% search at m=64 and 2x fast at m=128 while its MRR@10  is 11.5\% and 9.5\% higher 
%that only use query-centroid distances to select clusters. 

Compared to LADR and HNSW, our evaluation demonstrates that without a document-levelproximity graph, CluSD can 
deliver a similar or higher 
relevance under the same time budget
with negligible extra space overhead when embeddings are available in memory  and  is  much faster by avoiding fine-grained document-level disk I/O
when embeddings do not fit in  memory.  
Thus the lightweight with low-space overhead  and low-I/O cost is the main advantage of CluSD compared to a graph navigation approach.
\comments{
For example, Table ~\ref{tab:maintime} shows
CluSD has 2\% higher MRR@10  than LADR and 1.2\% higher than HNSW under a time budget of 25ms.
%It is attractive to run such an algorithm on a first-stage retrieval low-cost machine
%that can significantly reduce the overall infrastructure cost when scaling  data size and search traffic. 
}
Compared to several on-disk nearest-search efforts  with DiskANN and SPANN~\cite{NEURIPS2019_DiskANN,2023Web-Filtered-DiskANN},
like HNSW, they are targeted for a stand-alone and general ANN problem while our
work takes advantage of sparse retrieval for much shorter latency and similar or better relevance in the context of text document search.

Simple re-ranking does surprisingly well if sparse results are strong. But as stated in~\cite{2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR},
when the sparse retriever doesn’t achieve high relevance, re-ranking is too 
restrictive and recall@1k does not increase as shown in Table 5. 
\comments{
For example, after 
sparse retrieval with SPLADE-effi-HT3 with 0.944 recall@1k, re-ranking does not increase it while CluSD increases it to 0.984.
While re-ranking restricts candidate documents to the top sparse results, CluSD adds more diversified results from selected dense clusters. 
}
CluSD’s advantage becomes more significant in zero-shot retrieval as shown in Table 6 with 13 BEIR datasets. CluSD’s average NDCG number is 
7.2\% higher than re-ranking with RetroMAE. With SimLM, CluSD is 4\% higher than re-ranking.
In addition to this, when embeddings are not available in memory, re-ranking becomes very slow with a large number of document-level random I/O operations. 

Our evaluation uses OPQ in FAISS. 
Switching to a different quantization affects the compression ratio and  the relevance outcome. 
However, we expect that our findings remain similar and  the recent  quantization 
methods~\cite{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ}
also have  a significant relevance drop pattern when the compression ratio increases.
%A limitation of the current  CluSD work is that the training of the LSTM model has a dependence on the sparse retrieval model used. 
%While  CluSD can  boost the relevance of a weaker sparse retriever model such as BM25, the augmented relevance still has not reached a level
%comparable  to the one where CluSD is coupled with a stronger sparse retriever. There is room for improvement in future work.
\comments{
}

%the dependency on a training dataset. Unlike rule-based or unsupervised pipelines, our pipeline requires labeled data on at least one search task. However, the number of queries with labels is not large and a trained model is robust on never-seen corpus and tasks. 
%
%Another limitation is the dependency on the sparse retrieval model performance. CluSD benefit from a good sparse retrieval top results. When using a BM25 based retrieval, the quality of the clusters selected degrades slightly. 


==> kdddesign.tex <==

\comments{
Sparse retrieval with a learned representation  is much slower than BM25
        Guided sparse retrieval can speedup, but there is a trade in  effectiveness
        Augmenting sparse retrieval with dense retrieval through fusion can make up the loss
        Selective dense  retrieval can make up the loss argument sparse retiieval more effective with limited extra computing cost.

Points to market: Option 2

                New dense retrieval algorithms have been developed every year that beat new performance records.
                New fast  sparse retrieval algorithms are developed.
                Fusion of  sparse retrieval and dense retrieval is helpful, but slow on a CPU server, dominating by dense computation.
                There is a clear redudance of computation as both retrievers scan the same dataset with different representation
                        for push for the same top documents.
                How to avoid redudant computation?
                        1) Select dense retrieval. We donot need to scan all dense documents. We can take advanrage of
                clusters of dense documents
                        and only  need to visit top clusters which are similar to a query.
                        2) The use of dense retrieval reduces the relevance reqirement of sparse retrieval. We can use a fast sparse
retrieval BM25-guided sparse retrieval or effient SPLADE version, which quickly retrieves top results. Selective dense retrieval
                can augment  a weaker but faster sparse retriever by only adding limited  extra computing cost
to  improve the recall and relevance metric.

                Challenges:
                        1) How to accomplish  selective clusetrs.
                        Which clusters  can make most contributions
                        2) What queries definitely need dense retrieval boosting?

}
%\section{Design Considerations}
%label{sect:design}
\section{Selective Dense Cluster Retrieval}
\label{sec:clusd}


\comments{
The availability of a dense retriever model, possibly  trained separately by a different language model,
offers opportunities to re-confirm and adjust the ranking of top quality documents in  the initial
candidate pool and improve the  recall by introducing more diversified
candidates.  On the other hand, there is a clear redundancy of computation as both retrievers visit the same dataset 
with different representation, possibly  pursing the  same subset of top documents.
}
 
%{\bf Yingrui, please add a table or figure which shows the distribution of training
%queries if possible, otherise the Dev set of MS MARCOS,  that has the various level of MRR increase.
%I remeber you show us some data you collected during summer or spring.} 
%Table~\ref{tab:fusionanalysis} shows 



%We found that among 33\% of queries in the MSMARCO training set, there is no increase in terms of the MRR@10 when dense retrieval results are added to sparse retrieval results. Namely there are many queries that do not actually benefit from the use of dense retrieval after sparse retrieval.
% two retrievers, and explicitly skipping some of fusion can avoid the unnecessary computing cost.
%Motivated by the above data, 

%Our design considerations are:

%of selective dense retrieval  
%has  the following considerations.
%\begin{itemize} [leftmargin=*]
\comments{
\item  {\bf Partial dense retrieval after  full sparse retrieval.}

%and also there are several techniques developed recently to accelerate learned sparse retrieval,
}

%\item {Inter-cluster vs. inter-document similarity.}
\comments{
{\bf Cluster-based  dense retrieval.}
After the  fusion option is determined for a  query,
there is an option to follow LADR~\cite{2023SIGIR-LADR} and select documents that are similar to
the top sparse retrieval results  using a similarity graph.
These similar documents form candidates  for partial dense retrieval and  rest of un-selected
documents in a dataset can be skipped.  
Maintaining a large inter-document similarity graph online is quite expensive from
offline  data collection, online storage space, and   inference time.


The experience with the learned sparse models such as SPLADE~\cite{Formal2021SPLADE, Formal2021SPLADEV2} showed that
learned sparse representations from  BERT can be very effective.
For example, without optimization in language model pretraining, SPLADE's MRR performance is on par to
the dense retriever by RocketQA~\ref{Ren2021RocketQAv2}. 
Thus there is an opportunity to skip some of scoring computation in dense or sparse retrieval.
Since it is not easy to recognize and separate part of an inverted index  that contains high scoring documents,
we follow the approach of LADR~\cite{2023SIGIR-LADR} and GAR~\cite{2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}
run a sparse retriever completely first and steer partial dense  retrieval. 
}

%Previous studies  with the learned sparse models~\cite{Mallia2021deepimpact, 
%Lin2021unicoil,2021NAACL-Gao-COIL, Formal2021SPLADE, Formal_etal_SIGIR2022_splade++, shen2023lexmae
%Formal2021SPLADE, Formal2021SPLADEV2} showed that
%the relevance resutls from learned sparse representations from  BERT can be  fairly strong.
We aim to identify the opportunity to skip a substantial portion of dense retrieval computation 
by exploiting the potential overlap of sparse and  dense retrieval results.
We take the IVF clustering approach~\cite{johnson2019billion} that  places similar documents within each cluster. 
However, unlike IVF cluster search, our selection goes beyond the similarity between the query and cluster centroids to select top clusters.
Instead, our work explicitly exploits the overlap of sparse retrieval results with the potential dense clusters for better efficiency and relevance.   

\comments{
As discussed in Section~\ref{sect:intro}, we do not take a document-to-document similarity graph approach~\cite{2020TPAMI-HNSW, 
2022CIKM-MacAvaneyGraphReRank,  2023SIGIR-LADR} to avoid both the large space requirement of hosting such a graph and the high cost of random fine-grained
disk I/O to 
either the dense embedding set or the graph when one of them is hosted on the disk.
}

%and also there are several techniques developed recently to accelerate learned sparse retrieval,
\comments{
There are two ways  to select documents for dense retrieval.
One way is to take a graph navigation approach such as HNSW~\cite{2020TPAMI-HNSW}, GAR~\cite{2022CIKM-MacAvaneyGraphReRank} and LADR~\cite{2023SIGIR-LADR}, 
exploiting  document-to-document similarity links during inference time.
Another way is to follow a clustering  approach to group  documents based on their embedding similarity at offline 
time~\cite{johnson2019billion} and select a small set of  clusters.
%~\cite{2020TPAMI-HNSW,2022CIKM-MacAvaneyGraphReRank, 2023SIGIR-LADR}.
% is viewed as  a modern instantiation
%of the clustering hypothesis to revisit these ideas in a new context.  
We opt to take  the clustering based approach with two reasons.
1) Maintaing a large document-to-document similarity graph with a qudradical complexity is not scalable for  a large  data collection size. 
%As illustrated in  Table~\ref{tab:costbudget}, compression with embedding  quantization is necessary to meet the space constraint.
%due to the memory usage of stroing  embedding vectors. 
%For 8.8M MS MACRO passages, that takes  about 27GB space.
%Fortunately the quantization techniques can significantly compress this space into 1-2GB or even 0.5GB depending on the configuration. 
%Our feature design does not opt for  inter-document similarity since it is space-consuming, but  plans to exploit cluster-based summary information, 
%which  only adds  insignificant  space overhead.  
%\end{itemize}
%, and set a limit on the number of dense clusters used.
2) Embedding vectors of a large dataset with a high dimension per vector may not fit into the memory.
Cluster-based on selection exploits the block-level disk I/O for lower access overhead and higher bandwidth. 
In comparison, random access of selected documents in a graph based approach can suffer higher I/O overhead. 

}
\comments{
We intend to exploit coarse grain cluster-level similarity to reduce the complexity in selective dense retrieval with two reasons.
%The challenge is to how to select clusters  which can make most contributions.
%We opt to take a cluster-level skipping approach with two reasons.
1) Documents can be clustered in advance during offline processing 
%Documents within a cluster similar to a query can provide a large variety of strong candidates to supplement sparse retrieval results.  
2) Cluster-level computation allows  aggregation of  similarity computation for query-document dot products as a fast matrix operation 
to fully  utilize on-chip CPU caches. 
%In comparsion, there is a less chance for online inference to fully benefit from  CPU cache based on an irregular  graph structure.
%During offline processing, it is computationally expensive to drive document-level similarity for all pairs for documents in a large datset.
A research problem  is how to adaptively identify a subset of clusters  which yield sufficient relevance benefits.
% benefitial fusion if  sparse retrieval scoring may be sufficient. In addition to the influence of sparse retrieval results,
% a dynamically-visited dense cluster may provide sufficient high quality documents, reducing the necessarity of visiting
%the remaining dense clusters.   
%Thus we will develop a dynamic feature-driven decision scheme based the results of sparse retrieval.
%and incremtentally navigated  dense document clusters  as input. 
}
\comments{
Another consideration is that there are various relevance and efficiency tradeoff in selecting  a sparse retrieval 
model~\cite{Lassance2022SPLADE-efficient,mallia2022faster,Qiao20222GT,2023SIGIR-Qiao,2023SIGIR-SPLADE-pruning}.
For example, BM25 guided-sparse retrieval can greatly speedup, but lose some recall or precision
 when this guidance is weighted aggressively.
The use of dense retrieval provides a flexibility and reduces  the relevance requirement of sparse retrieval.
Namely potentially we can choose a relatively fast sparse retrieval with the slightly lower accuracy/recall,
and  let dense retrieval make up the loss. Our design
needs to  adapt to  sparse retrieval quality and plans
We plan to exploit features that reveal  the overlapping degree of top sparse retrieval results with  dense clusters
to guide the selection in addition to query-cluster distances. 
}

\comments{
\item  {\bf Query filtering for skipping dense retrieval}
We want an online system to make an earlier  determination if a query needs an argumentation from dense retrieval with supervised learning.
%A challenge is to identify features and infer based on such features with supervised learning.
Given that sparse retrieval is conducted first,
our idea is to predict the quality of sparse retrieval and its relative strength  compared to unexecuted
dense retrieval based on quality of query token expansion by the sparse model,
the statistical behavior of  sparse retrieval results, and
the relationship between dense document embedding summary and sparse retrieval scoring structure.




{\bf Latency budget.}
%Our heuristic-based fusion selection may suffer from an effectiveness tradeoff
%as full dense retrieval execution likely offers the maximum relevance benefits.
For search latency, our goal is to minimize the relevance effectiveness loss to a small degree while still accomplishing  a fast response time
acceptable to the interactive search system requirement.
In a search system running as an interactive  web service,  a query with multi-stage processing
needs to be completed within a few hundred milliseconds.
%Considering the multi-stage search nature  and other service overhead involved, 
A first-stage retriever operation  for a data partition needs to be completed within several tens of milliseconds without query caching (e.g. 200ms). 
Our targeted time budget to augment sparse retrieval cannot be too high     compared to  sparse retrieval cost.
We will evaluate the latency budget in two settings: around 50ms  and 25ms, including the  sparse retrieval time.
%For the example of Table~\ref{tab:costbudget},
%The studies from~\cite{Lassance2022SPLADE-efficientmallia2022GTI,Qiao20222GT,2023SIGIR-Qiao},
If sparse retrieval can complete  in 30 ms on an  average CPU and the total latency
target is around 50ms,  the cost of dense retrieval is targeted under around  20ms.
% At most the total sparse and dense retrieval cannot be more than 100ms.
%Accuracy of above query-specific cluster skipping while retaining a competiitve relevance is the key to accomplish this latency goal. 
%Notice that the latency target in the  LADR paper~\cite{2023SIGIR-LADR} is in a 4ms-8ms range
%and 
%This latency budget choice is reasonable because for 
%Also our evaluation is conducted in a low-end CPU server and a faster CPU can further accelerate. 
%CPU latency reported in~\cite{2022WWWforwardIndex} is at 11

}
\comments{
For the memory space cost,  our target budget for  dense retrieval augmentation is controlled in  the same level or some fraction of  sparse retrieval cost.
As illustrated in  Table~\ref{tab:costbudget}, compression with embedding  quantization is necessary to meet the space constraint.
%due to the memory usage of stroing  embedding vectors. 
%For 8.8M MS MACRO passages, that takes  about 27GB space.
%Fortunately the quantization techniques can significantly compress this space into 1-2GB or even 0.5GB depending on the configuration. 
Our feature design does not opt for  
inter-document similarity since it is space-consuming,
but  plans to exploit cluster-based summary information, 
which  only adds  insignificant  space overhead.  
%, and set a limit on the number of dense clusters used.
}



==> kddexp.tex <==
\section{Evaluations}

\comments{
Our evaluation answers  the following research questions around our proposed techniques and the correspond subsection are marked.

\textbf{RQ1} (Section~\ref{sect:eval0space}): 
How does CluSD compare against other low-cost baselines when space is constrained?
%extra space overhead is minimized by augmentation under different compression configurations? 

\textbf{RQ2} (Section~\ref{sect:evaltimebudget}): 
How does CluSD  perform under a retrieval latency time budget when there is no space restriction?

\textbf{RQ3} (Section~\ref{sect:evalbeir}): 
How does CluSD  perform in searching  out-of-domain text content?
Zero-shot retrieval performance is important since a large dataset can contain documents from many domains. 


\textbf{RQ4} (Section~\ref{sect:evalLSTM}): 
Is  LSTM with cluster pruning preferred compared to other design options?
Are  features designed for LSTM useful?

\textbf{RQ5} 
(Section~\ref{sect:clusterno}): 
How does the number of clusters used in dataset partitioning 
affect the relevance and latency of CluSD? 

\textbf{RQ6} 
(Section~\ref{sect:threshold}):
How does the choice of selection threshold value in LSTM affect the average number of clusters selected?
%Does the cluster selection model dynamically select different number of clusters for different queries? How the selection differs for different datasets?

\textbf{RQ7}
(Section~\ref{sect:evalsparse}):
How does CluSD perform in augmenting  different sparse retrievers with different efficiency and relevance characteristics?
}

\comments{
To answer \textbf{RQ1},  we compare our proposed approach on the in domain test set, MSMARCO passage dev, DL 19, 20 with other commonly used techniques under storage (Table~\ref{tab:mainspace}) and latency constraints (Tabel~\ref{tab:maintime}).  
For \textbf{RQ2}, as our cluster selection technique requires training, we would like to understand how the approach would work on our domain dataset. In Table~\ref{tab:beir}, we use our cluster selection model trained on MS MARCO datasets on the 13 datasets from BEIR on a zero-shot manner and observe promising performance on all 13 out-domain datasets. 
For \textbf{RQ3} and \textbf{RQ4}, We compare the different cluster selection techniques, including heuristic approaches, a point-wise prediction model xgboost and a vanilla RNN prediction model against the proposed LSTM model (Table~\ref{tab:cluster_feat}).
To answer \textbf{RQ5}, we take two scenarios where the number of clusters is 4096, and 8192. Then we present the relevance in MRR@10, recall@1000, and the latency in terms of mean and 99 percentile time under three settings: when the flat index is used without compression, when we use OPQ to compress with m=128 or 64. Results are shown in Figure~\ref{fig:ncluster}.
For \textbf{RQ6}, we first plot the distribution of the number of clusters selected for each query under different model prediction thresholds. We also plot the average number of clusters for MSMARCO dev set and BEIR in Figure~\ref{fig:thresholds}.
For \textbf{RQ7}, we report the performance using three weaker sparse retrievers in Table~\ref{tab:sparse}. 
}

\subsection{Settings }
{\bf Datasets and measures}.
Our evaluation uses the MS MARCO dataset with 8.8 million passages for full passage ranking~\cite{Campos2016MSMARCO,Craswell2020OverviewOT}.
The test query sets are the Dev set with 6980 queries and TREC deep learning (DL)  2019/2020 tracks with 43 and 54 queries.
We report mean reciprocal rank at 10 (MRR@10) and recall at 1000 (recall@1K)
which is the percentage of relevant-labeled results appeared in the final top-1000 results.
For DL19 and DL20 sets, we report NDCG@10.
%We report average NDCG@10 for the 13 publically available BEIR datasets~\cite{thakur2021beir}
%to evaluate  zero-shot retrieval performance.  
We also report average NDCG@10 for 
the  BEIR  collection containing the 13 publicly available datasets~\cite{thakur2021beir} 
for evaluating zero-shot retrieval performance. 
%BEIR is a heterogeneous benchmark containing a variety of IR tasks, 
%including search tasks (e.g.  question-answering, bio-medical IR, and entity retrieval)  
%and semantic relatedness tasks (e.g.  duplicate question retrieval). 
The size of these data sets ranges from 3,633 to 5.4M.
%Their average query length ranges from 5.39 to 192.98, 
%and  their average document length ranges from 11.44 to 634.79. 
%Each dataset has binary or three-level relevance labels.
The above metrics follow the common practice in the information retrieval literature.

{\bf Models and parameters}.
For sparse retrieval, we adopt two variations of 
SPLADE~\cite{Formal2021SPLADE, Formal_etal_SIGIR2022_splade++,Lassance2022SPLADE-efficient} 
based on hybrid thresholding~\cite{2023SIGIR-Qiao} and  BM25-guided traversal~\cite{mallia2022faster,qiao2023optimizing}:
% and one BM25 based model with different relevance and efficiency  tradeoffs:
1) SPLADE-HT1 with index space 3.9GB and 31.2 ms retrieval latency; 
%2) SPLADE-HT1-fast is a variation of SPLADE-HT1 with a different parameter setting, which has 3.9GB index space and 22.4 ms latency. 
2) SPLADE-effi-HT3 with  3GB space and  12.4ms latency. 
We also test on three other sparse models:
% uniCOIL~\cite{Lin2021unicoil,2021NAACL-Gao-COIL}, and LexMAE~\cite{shen2023lexmae}.
%2) DeepImpact~\cite{Mallia2021deepimpact};
3) uniCOIL~\cite{ Lin2021unicoil,2021NAACL-Gao-COIL} with 1.2GB index and 35.5ms latency;
4) LexMAE~\cite{shen2023lexmae} with 3.7GB index and 180ms latency;
5) BM25-T5 that applies  BM25 with  DocT5Query document expansion~\cite{Cheriton2019doct5query}.  
BM25-T5 has 1.2GB index and  9.2ms latency. 
%Their index space varies from 1.2GB to  3.7GB.
% with 1.2GB index space.
% with latency 9.2ms.
%5) BM25 after T5-based document expansion~\cite{Cheriton2019doct5query}. 
They represent the state-of-the-art sparse retrievers.
% with the best relevance performance evaluated on MS MARCO.

For dense retrieval, we adopt the recent dense models
SimLM~\cite{Wang2022SimLM} and RetroMAE~\cite{Liu2022RetroMAE}. 
We use their checkpoints from the Huggingface library to generate document and query embeddings 
and  use  K-means in the FAISS library~\cite{johnson2019billion} to derive dense embedding clusters.
RetroMAE-2~\cite{liu-etal-2023-retromae} is not used because its checkpoint is not released.


Our evaluation implementation uses C++ and Python and the
related code will be released to the public after publication of this paper. 
\comments{
%Note that SimLM model's embeddings are normalized while RetroMAE's embeddings are not. 
For sparse retrieval, we use two fast versions of SPLADE and a SPLADE-efficient model, as well as BM25-T5. 
The implementation of SPLADE models follows 2GTI optimization~\cite{qiao2023optimizing}. %its official release~\cite{spladeRepo}. 
SPLADE-HT1 is the SPLADE model trained with hybrid thresholding scheme~\cite{2023SIGIR-Qiao} using $\lambda_{t}=1$, 
SPLADE-effi-HT3
is the SPLADE-efficient model~\cite{Lassance2022SPLADE-efficient} trained with hybrid thresholding scheme using $\lambda_{t}=3$. Both of these two models use the "accurate" configuration in 2GTI during retrieval, while SPLADE-HT1-fast uses the "fast" configuration.
The sparse retrieval code for Splade and BM25-T5 uses the code from PISA~\cite{mallia2019pisa}
with some optimization~\cite{Lassance2022SPLADE-efficient,2023SIGIR-Qiao}.
}
To train the CluSD model, we sample 5000 queries from the MS MARCO training set 
%and use the LSTM unit in Pyytorch. 
and the hidden dimension for LSTM is 32. The models are trained for 150 epochs. 
For sparse and dense model interpolation, we use min-max normalization to rescale the top results per query. 
%Then we use linear combination with equal weights to combine two ranked lists. 
For  BM25-T5, the interpolation  weights are  0.05 and 0.95 for sparse  and  dense scores, respectively. 
For other learned sparse retrieval models, they are  0.5 and  0.5, respectively. 
%In terms of missing document in either ranked list, as the smallest value from each normalized list is 0, there is no missing imputation needed as we 
%can view the missing  documents taking the value of the worst document in the ranked list automatically. 

%For CluSD, the default setting of number of clusters is $N=8192$, and the input sequence length to the Stage II LSTM model is $n=32$.  
To report the mean latency and 99 percentile latency, 
we  run test queries multiple times  from MS MARCO Dev set using a single thread on  a 2.25GHz AMD EPYC 7742  CPU server with PCIe SSD.
The reason to use a single thread is that each CPU server in a busy search site handles many queries in parallel, and thus we only take
one core resource with one thread from this server and leave other cores  for other queries.
That is the standard practice in many of the previous efficiency studies in the IR literature.

{\bf Time budget.}
%For search latency, our goal is to minimize the relevance effectiveness loss to a small degree while still accomplishing  a fast response time
%acceptable to the interactive search system requirement.
We use  two time budget settings: around 50ms  and 25ms, including the  sparse retrieval time.
We explain the reason as follows.
In a search system running as an interactive  web service,  a query with multi-stage processing
needs to be completed within a few hundred milliseconds.
%Considering the multi-stage search nature  and other service overhead involved,
A first-stage retriever operation  for a data partition needs to be completed within several tens of milliseconds without query caching.
Our targeted time budget to conduct dense retrieval cannot be too high     compared to  sparse retrieval cost.
%For the example of Table~\ref{tab:costbudget},
%The studies from~\cite{Lassance2022SPLADE-efficientmallia2022GTI,Qiao20222GT,2023SIGIR-Qiao},
For example, if sparse retrieval can complete  in 30 ms on an  average CPU and the total latency
target is around 50ms,  the cost of dense retrieval is targeted under around  20ms.
% At most the total sparse and dense retrieval cannot be more than 100ms.
%Accuracy of above query-specific cluster skipping while retaining a competiitve relevance is the key to accomplish this latency goal.
%Notice that the latency target in the  LADR paper~\cite{2023SIGIR-LADR} is in a 4ms-8ms range
%and
%This latency budget choice is reasonable because for
%Also our evaluation is conducted in a low-end CPU server and a faster CPU can further accelerate.
%CPU latency reported in~\cite{2022WWWforwardIndex} is at 11

\comments{
{\bf Baselines.}
We compare CluSD with two groups of baselines under space and time constraints respectively.
The first group compared in Section~\ref{sect:eval0space} 
is to fuse  sparse retrieval with cluster-based selective dense retrieval.
That includes  dense retrieval with quantization option OPQ and  IVFOPQ with IVF clustering available in FAISS.
The second group compared in Section~\ref{sect:evaltimebudget} 
is to fuse  sparse retrieval with re-ranking and graph-based selective dense retrieval such as HNSW~\cite{2020TPAMI-HNSW} and  LADR~\cite{2023SIGIR-LADR}. 
This group involves random access of embeddings and/or graph nodes, which  can incur high I/O cost when data is not on disk.
}


{\bf Statistical significance.}
For MS MARCO Dev set, the result of a method is marked with  tag $^\dag$ when 
statistically significant drop is observed compared to  an oracle baseline
tagged with $\blacktriangle$ at 95\% confidence level.  This oracle
is sparse retrieval fused with full dense retrieval marked as ``S+D'', which typically delivers the highest relevance  
using all uncompressed or quantized dense embeddings.


\comments{
{\bf Baselines and notations}
%We select two groups of baselines under space and time constraints respectively.
Table~\ref{tab:mainspace} compares  baselines  with memory space constraint. 
We include dense retrieval with quantization option OPQ and  IVFOPQ with IVF clustering available in FAISS.
OPQ quantization  is configured with  the number of codebooks as $m=$ 128 or 64.  
When IVF clustering is used,  we report its performance  using top 10\%, 5\%, 2\% clusters respectively
as a standard approach which performs   limited top cluster retrieval. 
CluSD execution is also based on the the same OPQ or  IVFOPQ index from  FAISS but clusters are  selected  by our LSTM model. 
%Switching a quantization different  from OPQ  is might result in an improvement in relevance, but it is orthogonal to our proposal. 
We use notation ``S+D'' to report the interpolated performance of a sparse model and a dense model in Table~\ref{tab:mainspace} and Table~\ref{tab:sparse}.

Table~\ref{tab:maintime} compares  baselines  without  memory space constraint. 
For proximity graph-based dense retrieval which incurs additional graph space overhead,
we include  HNSW~\cite{2020TPAMI-HNSW} and  LADR~\cite{2023SIGIR-LADR} as shown in Table~\ref{tab:maintime}. 
%For HNSW, we fix the number of neighbors to be 128 and vary the expansion factor(ef) to meet the latency constraint. 
%For LADR, we use its default setting with seed = 200, number of neighbor = 128 and use the exploration depth as 50 to meet the latency requirements in 
%Table~\ref{tab:maintime}.
%Uncompressed dense embeddings (marked as "flat") are used
%to exclude the impact due to quantization.
We also compare  a simple re-ranking method,  denoted as ``D-rerank'' or ``rrk'', 
that fetches the dense scores of top 1000 of sparse retrieval to re-rank with interpolation. 
%We use the same clustering setting for IVF and CluSD. 

%The reported CluSD performance on the flat index uses the exact same IVF index. 
The configuration we selected to meet the latency requirement for CluSD uses on average 20-25 (0.25 - 0.3\%) clusters per query. 
%For re-ranking, we report the results of re-ranking top 1000 results from the sparse model using the dense model.  

}



==> kddexpe_ablation.tex <==
%\vspace*{-5mm}
%\subsection{Fast search with minimized space overhead}
\begin{table*}[htbp]
	\centering
		\resizebox{1.98\columnwidth}{!}{
		\begin{tabular}{ r r l |l l ll l |llll l|r}
			\hline\hline
			 & & & \multicolumn{2}{c}{ 
{\bf MSMARCO Dev} }& {\bf DL19}& {\bf DL20} & {\bf BEIR} 
& \multicolumn{2}{c} { {\bf MSMARCO Dev} }& {\bf DL19}& {\bf DL20} & {\bf BEIR} 
& {\bf  Latency}    \\
			& &\% D& {MRR@10}& R@1k& {NDCG@10}&  {NDCG@10}& {NDCG@10}& {MRR@10}& {R@1k}& {NDCG@10}&{NDCG@10}& {NDCG@10}& ms \\
    \hline
 1. & S={\bf SPLADE-HT1} & --& 0.396& 0.980 & 0.732   & 0.721    & 0.500 & -- & --& --& --& --&31.2  \\
 & & & \multicolumn{5}{c|}{D=\textbf{SimLM}}& \multicolumn{5}{c|}{D=\textbf{RetroMAE}}&\\
   \hline
   &&& \multicolumn{10}{c}{\bf{Uncompressed flat setting. Embedding space  27.2GB}}\\
     \hline
          2. &   D  & 100 & 0.411$^\dag$ & 0.985$^\dag$& 0.714 &  0.697  & 0.429 & 0.416$^\dag$& 0.988& 0.720&0.703& 0.482 & 1674.1 \\
            3. &   $\blacktriangle$ S $+$ D   &100 & 0.424 & 0.989 & 0.740 & 0.726  & 0.518 & 0.425& 0.988& 0.740&0731& 0.520~&  1705.3 \\
           4. &    \bf S $+$ CluSD &0.3& 0.425 & 0.987 & 0.744 & 0.724  & 0.516 & 0.426& 0.987& 0.744&0.734 & 0.518 & 44.4 \\
              \hline
            &&& \multicolumn{10}{c}{\bf{OPQ $m=128$. Embedding space  1.1GB}}\\
              \hline
            5. &   $\blacktriangle$  S $+$ D-OPQ &100 & 0.420 & 0.988 & 0.735 &  0.719  & 0.508 & 0.416 & 0.988 & 0.737 & 0.732 & 0.515& 600.1 \\
            6. &  S $+$ D-IVFOPQ &10& 0.414$^\dag$& 0.987 & 0.726 & 0.734  & 0.505 & 0.404$^\dag$& 0.987& 0.713&0.722& 0.513 &  126.4 \\
           7. &   &5& 0.407$^\dag$& 0.987 & 0.717 & 0.733  & 0.499  & 0.394$^\dag$& 0.987& 0.687&0.817&0.507&  80.0 \\
           8. &   &2& 0.392$^\dag$& 0.986$^\dag$& 0.691 & 0.738  & 0.467 & 0.374$^\dag$& 0.986$^\dag$& 0.656&0.815& 0.499 & 52.5 \\
           9. &   \textbf{S $+$ CluSD}  &0.3& 0.423 & 0.987 & 0.739& 0.725 &0.514 & 0.417& 0.986& 0.742&0.735& 0.514  & 42.6  \\
             \hline
           & & & \multicolumn{10}{c}{\bf{OPQ $m=64$. Embedding space 0.6GB}}\\
            \hline
           10. & $\blacktriangle$  S $+$ D-OPQ  &100 & 0.409 & 0.986 & 0.718 &  0.721  &0.501 & 0.402 & 0.986 & 0.717 &  0.719 & 0.508 & 321.6 \\
           11. &   S $+$ D-IVFOPQ &10& 0.405 & 0.986 & 0.716 & 0.734 & 0.502 & 0.393$^\dag$& 0.986& 0.676&0.730& 0.505& 75.6 \\
           12. &   &5& 0.397$^\dag$& 0.986 & 0.704 & 0.733  & 0.497 & 0.384$^\dag$& 0.985& 0.659&0.717& 0.500& 55.0 \\ 
            13. &  &2& 0.383$^\dag$& 0.985 & 0.680 & 0.738 & 0.487 & 0.368$^\dag$& 0.985 & 0.643&0.707& 0.493 & 42.4 \\
            14. &  \textbf{S $+$ CluSD}  &0.3& 0.414 & 0.986 & 0.743& 0.726 & 0.511 & 0.403 & 0.987& 0.729&0.724 & 0.506 & 40.8 \\
              \hline\hline
		\end{tabular}
		}
	\caption{
CluSD vs. IVF cluster search with and without quantization.
%Sparse retrieval argumentation with minimum extra space overhead.
%no  with compressed or uncompressed dense emebddings S=SPLADE-HT1, D=SimLM or RetroMAE. 
%Model relevance and latency under compressed or uncompressed dense emebddings S=SPLADE-HT1, D=SimLM or RetroMAE. 
%Row  ``S $+$ D'' marked with $\blacktriangle$ indicates the oracle setting of sparse model interpolated with full dense retrieval. 
For MSMARCO Dev set, $^\dag$ is tagged when statistically significant drop is observed from the oracle $\blacktriangle$ at 95\% confidence level. 
}
\vspace*{-5mm}
	\label{tab:mainspace}
\end{table*}

\subsection{CluSD vs. IVF  cluster search}
\label{sect:eval0space}


	
Table~\ref{tab:mainspace} compares CluSD with other cluster-based selective retrievals when fusing with sparse retrieval results
in searching the MS MARCO and BEIR datasets with and without compression.  
SPLADE-HT1 is  the sparse model, and two dense models used are SimLM and RetroMAE.
%We compare our models on uncompressed embeddings, as well as two quantization configurations.
%There are the uncompressed setting and  two quantization  configurations. 
%The sparse model used is SPLADE-HT1 while the dense models are SimLM and RetroMAE.
%IVFOPQ is compared against CluSD as it selects only top clusters and does not incur extra space overhead. 
%The top portion of this table reports the performance when compression is not used, which captures a peak possible performance.
We also compare against IVFOPQ, which uses a percentage of top dense clusters sorted by the query-centroid distance.
%IVFOPQ is compared, which use some percentage of top dense clusters sorted by query to centroid clusters.
%against CluSD as it selects only top clusters and does not incur extra space overhead.
We include dense retrieval with OPQ quantization  and  IVFOPQ from FAISS.
OPQ quantization  is configured with  the number of codebooks as $m=$ 128 or 64.
We report performance of IVF clustering using the top 10\%, 5\%, or 2\% clusters respectively
as a standard approach which performs   limited top cluster retrieval.
CluSD execution is also based on the the same OPQ or  IVFOPQ index from  FAISS, but clusters are  selected  by our two step algorithm.

Notation ``S+D'' in Table~\ref{tab:mainspace} (and later Table~\ref{tab:maintime})
reports the fused performance of a sparse model and a dense model with linear interpolation.
The column marked with  ``\%D'' means the percentage of document embeddings  evaluated.
The last column,  ``Latency'' is the average single-query time using SPLADE plus SimLM for MS MARCO Dev set.
We only report SimLM latency because the latency of SimLM and RetroMAE are similar.
%When    prefix `+' is marked for a latency entry, it indicates  the extra milliseconds is spent for full or selective dense retrieval without counting   sparse retrieval time.

CluSD uses setting  $N=8192$ and 
$n=32$ 
% Tables~\ref{tab:mainspace} and~\ref{tab:maintime} use
which results in  selection of 22.3 clusters on average per query
and allows CluSD to meet  the latency requirement.
%The main space cost for CluSD is to maintain the inter-cluster similar graph, which 
%takes about 32MB with quantization for $N=8192$. 
%Switching a quantization different  from OPQ  is might result in an improvement in relevance, but it is orthogonal to our proposal.
%The reported CluSD performance on the flat index uses the exact same IVF index.
% for CluSD uses on average 20-25 (0.25 - 0.3\%) clusters per query.
%For re-ranking, we report the results of re-ranking top 1000 results from the sparse model using the dense model.
%The mean latency and 99 percentile latency of CluSD are 13.2 ms and 18.1 ms for searching uncompressed flat index, respectively;
%11.4 ms and 14.6ms for searching OPQ m=128 index;  9.6 ms and 11.1ms for searching OPQ m=128 index.





\comments{
For MS MARCO Dev set, the result of a method is marked with  tag $^\dag$ when
statistically significant drop is observed compared to  an oracle baseline
tagged with $\blacktriangle$ at 5\% confidence level.  This oracle
is sparse retrieval fused with full dense retrieval marked as ``S+D'', which typically delivers the highest relevance
using all uncompressed or quantized dense embeddings ($m=128$ or $m=64$).


%In realistic settings, a flat dense index is usually not affordable when corpus size is not small. Certain compression technique need to be used. 
The top portion of this table reports the performance of  SimLM dense model marked as ``D'' in Row 2.
In Row 1, ``S'' denotes sparse retrieval using  a variation of SPLADE with hard thresholding called HT1~\cite{2023SIGIR-Qiao}.
Sparse results merged with full  dense retrieval  results  are marked in Row 3, ``S $+$ D''.  
Our pipeline is reported in Row 4,``S $+$ CluSD''. 
The second and third portions of this table reports
the search performance   with  two compression configurations using OPQ implemented in FAISS:
1) ``m128'' that compresses dense embeddings from about 27GB into 1.1GB with 128 quantization codebooks.
2) ``m64'' that  yields 0.6GB compressed embeddings with 64 codebooks. 
%Setting where the storage for dense index is 1.1GB and 0.6GB. 
Under these two configurations, we report the Sparse model interpolated with dense retrieval under
IVFOPQ or OPQ using the default FAISS setting.


%In the first section of the table, we include the full dense retrieval SimLM (denoted as D in the table), 
%and full sparse retrieval SPLADE-HT1 (denoted as S in the table), 
%and 
%We then report dense retrieval with two compression configurations, using OPQ 
%with m=128 and m=64 respectively, resulting in an index 
%with 1.1GB and 0.6GB. These compressed configuration result in a 96\% and 97.8\% reduction in storage compared to flat index.
% and compare them against our pipeline.
}

Table ~\ref{tab:mainspace} Row 6 and 11
 show that selective IVF cluster search using  query-centroid distances 
can be under 130ms  when the percentage of clusters searched  drops from 100\% to 10\%. But the relevance drop is significant.  
Moreover, CluSD is as  fast as IVFOPQ  top 2\% search at m=64 (Row 14 vs. Row 13) and 2x fast at m=128 while
its relevance is much higher (Row 9 vs. Row 8).
%CluSD  performs  closely as the oracle at each compression setting, which
There is no statistically significant difference between CluSD and the oracle at each compression setting, which 
indicates CluSD effectively minimizes visitation of unnecessary  dense clusters. 

 



\comments{
 with full dense retrieval can reach a high relevance in all datasets and thus are marked as an oracle sign with or without compression.   
1. Almost no performance degradation when do S+CluSD.  Sometimes S+CluSD achieves slightly higher performance than S+D. It could be due to the fact that when we limit the search scope a lot of noisy documents are not considered by the dense model.

2. Under m=128 setting the performance degradation is acceptable especially on DL19 and 20. 

3. SimLM performs better under compression. This could be due to the fact that SimLM trained embedding is normalized while RetroMAE is not.

4. If we compare S+D-IVFOPQ with S+CluSD, given the same IVFPQ index, S+D-IVFOPQ represents the case where we use default order, even if we use 50x more clusters, the performance is not as good as CluSD. 
}




\subsection{CluSD vs. graph navigation and re-ranking} 
\label{sect:evaltimebudget}
Table~\ref{tab:maintime} compares  CluSD with  re-ranking and selective dense retrieval based on proximity graph navigation, which includes HNSW and LADR.
Since LADR has a variety of configurations, we use configurations under two time budgets.
We do not consider memory space restrictions in this evaluation as proximity graph takes a substantial amount of extra space.
We also compare  a simple re-ranking method,  denoted as ``D-rerank'' or ``rrk'',
that fetches the dense scores of the top-1000 sparse retrieval results to re-rank with interpolation.
Uncompressed dense embeddings  are used to exclude the relevance impact by quantization.
The last two columns report the total latency time in milliseconds including sparse retrieval when needed,
and data space cost. %Extra memory space on the top of sparse retrieval is marked with prefix `+'. 
``MRR'' means  MRR@10 and ``NDCG'' means  NDCG@10.
%The extra space for quantized inter-cluster distances for CluSD takes about 32MB. 

%As discussed in Section~\ref{sect:design}, the overall latency budget is set as 50ms and 25ms respectively. 
We allow some time for budget relaxation since it is difficult to tune parameters of all baselines to meet the constraints exactly. 
%For IVF, we use 1.5$\%$ and 3$\%$ top clusters for ``S+IVF'' and ``IVF''.
%  but we allow some variation for some baselines because it is difficult to find parameters that exactly control the latency under this budget. 
%In this case, we choose the dense configuration such that the overall latency is within 70 or 30 milliseconds. 
For HNSW under 50ms time budget, we set its expansion factor parameter (ef) as 1024, 
2048 for S$+$D-HNSW and D-HNSW. 
Under 25ms time constraint, the expansion factor (ef) is  512 and  1024 respectively. 
%We include option ``S+Re-rank" which uses the top 1,000 sparse retrieval results and only compute dense scores of these top results, and merge the score with an interpolation.
%For HNSW, we fix the number of neighbors to be 128 and vary the expansion factor(ef) to meet the latency constraint.
For LADR, we use its default setting with seed = 200, number of neighbor = 128 and use the exploration depth as 50 to meet the latency budget.
%Table~\ref{tab:maintime}.
\comments{
Under time budget 50ms, 
model  SPLADE-HT1 is used and it has a latency of 31.2 ms in sparse retrieval.  
Under  time budget 25ms, model SPLADE-effi-HT3 is used and it is more aggressive in  efficiency 
with a 12.4ms latency at the cost of a relevance degradation. 

%using the dense model only, We also include sparse retriever 
%IVFOPQ, IVF, OPQ and HNSW using the dense model only, We also include sparse retriever 
%with reranking top 1000 results using the dense model. We also include the results of document evaluation using LADR algorithm. 
Note that when ``S$+$'' is in the row, it means we use the sparse model and the reported results are interpolated. 

}
%[DISCUSS TABLE 4 RESULTS.]
The takeaways from this table are:

\textbullet\ 
%While IVF does not add extra space cost, the relevance  of IVF top cluster search under the time budget performs  worse than others.
Simple re-ranking ``D-rerank'' achieves good MRR@10 but under-performs on recall.
When the recall of a sparse retriever is relatively low, it cannot boost further as seen in the case of using BM25T5 in Table~\ref{tab:sparse} with R@1k 0.935.

\textbullet\ HNSW and LADR perform comparably, at the cost of extra online memory overhead  and extra complexity to compute offline in advance.
HNSW requires extra 9.2GB and LADR requires extra 4.3GB to store graph data in memory. 
When we  try to reduce their graph size by decreasing  the number of neighbors for HNSW and LADR, their  MRR@10 and/or  recall@1000 numbers drop visibly. For example, 
using the default 32 neighbors for the HNSW graph results in 2.4GB graph space, however  MRR@10 drops from 0.407 to 0.400 under the 25ms time budget. 

\textbullet\ CluSD incurs negligible extra space cost other than hosting embeddings, compared to HNSW and LADR.
For both time budget=50ms and 25ms,  CluSD has a higher MRR@10 while its DL19 and DL20 numbers are comparable to HNSW and LADR.


\textbullet\ 
Even when we relax the latency requirements for the baselines, CluSD still maintains its advantages in different datasets. 
For instance, if we double the time budget to around  110ms
for 	``S+D-HNSW'' after  SPLADE-HT1 retrieval, its MRR@10 for MS MARCO Dev is 0.422, which is still below S$+$CluSD with 0.426 in 46.3ms.




 

\begin{table}[htbp]
	\centering
 \resizebox{0.95\columnwidth}{!}{
		\begin{tabular}{r |llll|rr}
			\hline\hline
			& \multicolumn{2}{|c}{\bf{MSMARCO Dev}}& \bf{DL19}& 
\bf{DL20}& \bf{Latency}& \bf{Space}\\
			 & {MRR}& {R@1k}& \smaller{NDCG} &   \smaller{NDCG} & Total(ms)& GB\\
			\hline
        \multicolumn{7}{c}{\bf{Time Budget = 50 ms, S=SPLADE-HT1}}\\
        \hline
            D=SimLM & 0.411 & 0.985$^\dag$& 0.714 &  0.697 & 1674.1 & 27.2 \\
          S& 0.396$^\dag$& 0.980$^\dag$& 0.732   & 0.721    &   31.2 & 3.9 \\
           S $+$ D-rerank &  0.421 & 0.980$^\dag$& 0.745 & 0.728 & 34.6 & 31.1 \\
             $\blacktriangle$  S $+$ D  & 0.424 & 0.989 & 0.740 & 0.726 & 1705.0 & 31.1 \\
              \hline
              % D-IVF & 0.398$^\dag$& 0.935$^\dag$& 0.690 & 0.693 & 81.4 & $+$0.0\\
%            D-IVF & 0.389$^\dag$& 0.907$^\dag$& 0.671 & 0.676 & 49.5 & $+\sim$0\\
%            S $+$ D-IVF & 0.393$^\dag$& 0.987  & 0.678 & 0.715 & 56.5 & $+\sim$0\\
            %D-OPQ& 0.314$^\dag$& 0.957$^\dag$& 0.619 & 0.608 & 109.1 & 0.3 \\
           % D-IVFOPQ & 0.386$^\dag$& 0.929$^\dag$& 0.680 & 0.697 & 48.8 & 1.2\\
            % D-HNSW & 0.409$^\dag$& 0.978$^\dag$& 0.669 & 0.695 & 54.4 & 40.3 \\
            %S $+$ rerank-D &  0.412 & 0.980    &0.715  & 0.811 & 0.698 & 0.815 & $+$2.3 \\
            S $+$ D-LADR & 0.422 & 0.984$^\dag$& 0.743&0.728& 43.6& 35.4\\
%           7.1 &  S $+$ D-LADR & 0.423 & 0.987$^\dag$& 0.745 &0.728& 53.0 & $+$4.3\\
           % S $+$ D-IVF & 0.398$^\dag$& 0.987  & 0.674 & 0.720 & 64.7 & $+$0.0\\
           %S $+$ D-IVFOPQ & 0.392$^\dag$& 0.987 & 0.656 & 0.700 &  52.5 & 4.0\\
           S $+$ D-HNSW & 0.420 & 0.987 & 0.718 & 0.723 & 59.6 & 40.3 \\
            \bf S $+$ CluSD & 0.426 & 0.987 & 0.744 & 0.724 &46.3& 31.1\\
       \hline       
            \multicolumn{7}{c}{\bf{Time Budget = 25 ms, S=SPLADE-effi-HT3}}\\
            \hline
            S& 0.380$^\dag$& 0.944$^\dag$& 0.721 &  0.726 & 12.4 & 3.0 \\
             S + D-rerank & 0.406 & 0.944$^\dag$& 0.728 & 0.738 & 15.1 & 30.2 \\
            $\blacktriangle$  S + D & 0.413 & 0.984 & 0.721 &0.729 & 1654.2& 30.2  \\
            \hline
            %D-HNSW & 0.406 & 0.971$^\dag$& 0.672 & 0.694 & 28.4 & 39.4\\
             S $+$ D-HNSW & 0.407 & 0.984 & 0.706 & 0.724 & 28.7 & 39.4\\
            S $+$ D-LADR & 0.404$^\dag$& 0.984 & 0.728 &  0.736 & 24.2 & 34.5\\
%           16.1 & S $+$ D-LADR & 0.409 & 0.987 & 0.744 &  0.728  & 41.1 & $+$4.3\\
            \bf S $+$ CluSD & 0.412 & 0.984 & 0.733 & 0.728 & 25.4 & 30.2\\
			\hline\hline
		\end{tabular}  }
	\caption{CluSD vs. graph navigation and re-ranking 
% under time budget but  no memory constraints 
}
% \vspace*{-10mm}
	\label{tab:maintime}
\end{table}
%For pipelines with a time budget, we report the additional overhead in the Storage (GB) column. 






==> kddexpe_beir.tex <==
\subsection{Zero-shot retrieval performance with BEIR}
\label{sect:evalbeir}

\comment{
\begin{table*}[h]
	\centering
		\resizebox{1.9\columnwidth}{!}{
		%\begin{small}
		\begin{tabular}{r r r lr  |lllll|lllll}
			\hline\hline
                 &  & &  & &  \multicolumn{5}{c|}{SPLADE-HT1+SimLM} & \multicolumn{5}{c}{SPLADE-HT1+RetroMAE}\\
                  &  & &  & {SPLADE}  &  & &  \textbf{CluSD} & \textbf{CluSD} & \textbf{CluSD} & & & \textbf{CluSD} & \textbf{CluSD} & \textbf{CluSD}\\
		    Dataset & \smaller{BM25} &{SimLM}  &  {RetroMAE} &{-HT1} & \smaller{$\blacktriangle$ 
 flat} &rrk&\textbf{flat}& \textbf{m=128}& \textbf{m=64}& \smaller{$\blacktriangle$ flat} &rrk &\textbf{flat}& \textbf{m=128}& \textbf{m=64}\\
              \hline
              \multicolumn{15}{c}{\bf{Search Tasks}}\\
               \hline
                {DBPedia}	& 0.313	& 0.351 &  0.390&0.447	& 0.426 &0.442& 0.429 & 0.425 & 0.422 & 0.446 & 0.411 & 0.446 & 0.445&0.436 \\
                                {FiQA} &	0.236	& 0.298 &  0.316&0.355 & 0.355 &0.355 &0.365 & 0.361 &0.359 & 0.365 & 0.333 & 0.366 & 0.359& 0.353\\
                {NQ}	& 0.329   & 0.502  &	 0.518&0.550 & 0.568 &0.549&0.568 & 0.566 & 0.560 & 0.563 & 0.520 & 0.564 & 0.553& 0.538\\
                {HotpotQA} & 0.603 & 0.568 &  0.635& {0.681} & 0.672 &0.668&  0.672 & 0.669 & 0.661 & 0.702 & 0.642 & 0.702 & 0.693&0.672 \\
                {NFCorpus}  & 0.325 & 0.318  &  0.308&0.351 & 0.353 &0.347&  0.360 & 0.358 & 0.359 & 0.345 &0.331 & 0.351 & 0.349& 0.346 \\
                {T-COVID}	& 0.656 & 0.515  &  0.772&0.705 & 0.726 &0.692&  0.745 & 0.741 & 0.725 & 0.780 & 0.699 &0.747 &0.740& 0.726\\
                {Touche}	& {0.367}  & 0.292  &  0.237&0.291 & 0.336 &0.292 &0.333 & 0.336 & 0.332 & 0.292 &0.316 & 0.295 &0.288& 0.283\\
                \hline
                \multicolumn{15}{c}{\bf{Semantic Relatedness Tasks}}\\
                 \hline
                {ArguAna} & 0.315 & 0.376  &  0.433&0.446 & 0.481 &0.427&  0.492 & 0.489 & 0.486 & 0.459 & 0.434 & 0.455 &0.455 & 0.451\\
                {C-Fever}	& 0.213 & 0.171  &  0.232&0.234 & {0.239} &0.236&  0.241 & 0.250 & 0.242 & 0.260 &0.198 &0.260 &0.267& 0.262\\
                {Fever} & 0.753  &0.689  &	 0.774& {0.781} & 0.793 &0.784&  0.794 & 0.783 & 0.789 & 0.820 &0.774 &0.820 &0.814& 0.800\\
                {Quora} & 0.789 & 0.797  &	 0.847&0.817 &	0.847 &0.816&  0.847 & 0.849 &0.848 & 0.856 &0.814 &0.855 &0.854& 0.849\\
                {Scidocs}	& 0.158 &0.137  &	 0.15&0.155 &	{0.165} &0.152&  0.166 & 0.166 & 0.165 & 0.167 &0.142 &0.169&0.166& 0.164\\
                {SciFact}	& 0.665 & 0.559  &  0.653& {0.682} & 0.674 &0.682&  0.694 & 0.689 & 0.693 & 0.706  &0.661 &0.703 &0.699& 0.694\\
                            \hline
                \textbf{Avg.} & 0.440 & 0.429  &  0.482&0.500 & 0.518 &0.496&  0.516 & 0.514 & 0.511 & 0.520 &0.483 &0.518 &0.514& 0.506\\
                %\textbf{BM25 Diff} & -- & -2.6\%  &	13.6\% &17.7\% &  6.1\%&12.7\%&14.8\% &  \textbf{15.7\%} \\
                \textbf{{Splade Diff}} & -12.0 \% &  -14.2\%  &	 -3.6\% &-- & 3.6\% & -0.8\% &3.2\% & 2.8\% & 2.2\% &4.0\%& -3.5\%& 3.5\%&2.8\%&1.2\%\\
            \hline\hline
		\end{tabular}
		%\end{small}
		}
%\vspace*{-5mm}
	\caption{Zero-shot performance in average NDCG@10 on BEIR datasets. 
%Row ``SPLADE Diff.'' is the mean relative performance compared to the SPLADE-HT1 performance.
}
 % \vspace*{-5mm}
%For quantization approaches, we adopt M=16, K=256, i.e. compression rate 32$\times$ compared to ColBERT.
	\label{tab:beir}

\end{table*}
}


\begin{table}[h]
	\centering
		\resizebox{1\columnwidth}{!}{
		%\begin{small}
		\begin{tabular}{r r r r  |lllll}
              \hline
              \hline
	\multicolumn{4}{c|}{\bf Average NDCG@10}
                     &  \multicolumn{5}{c}{SPLADE-HT1+SimLM}\\
                  &  & & {SPLADE}  & Full  & &  \textbf{CluSD} & \textbf{CluSD} & \textbf{CluSD} \\
		    Dataset & \smaller{BM25} &{SimLM}  &{-HT1} & \smaller{$\blacktriangle$ 
 flat} &rrk&\textbf{flat}& \textbf{m=128}& \textbf{m=64}\\
              \hline
              \multicolumn{9}{c}{\bf{Search Tasks}}\\
               \hline
                {DBPedia}	& 0.313	& 0.351 &0.447	& 0.426 &0.442& 0.429 & 0.425 & 0.422 \\
                                {FiQA} &	0.236	& 0.298 &0.355 & 0.355 &0.355 &0.365 & 0.361 &0.359 \\
                {NQ}	& 0.329   & 0.502  &0.550 & 0.568 &0.549&0.568 & 0.566 & 0.560 \\
                {HotpotQA} & 0.603 & 0.568 & {0.681} & 0.672 &0.668&  0.672 & 0.669 & 0.661 \\
                {NFCorpus}  & 0.325 & 0.318  &0.351 & 0.353 &0.347&  0.360 & 0.358 & 0.359 \\
                {T-COVID}	& 0.656 & 0.515  &0.705 & 0.726 &0.692&  0.745 & 0.741 & 0.725 \\
                {Touche}	& {0.367}  & 0.292  &0.291 & 0.336 &0.292 &0.333 & 0.336 & 0.332 \\
                \hline
                \multicolumn{9}{c}{\bf{Semantic Relatedness Tasks}}\\
                 \hline
                {ArguAna} & 0.315 & 0.376  &0.446 & 0.481 &0.427&  0.492 & 0.489 & 0.486 \\
                {C-Fever}	& 0.213 & 0.171  &0.234 & {0.239} &0.236&  0.241 & 0.250 & 0.242 \\
                {Fever} & 0.753  &0.689  & {0.781} & 0.793 &0.784&  0.794 & 0.783 & 0.789 \\
                {Quora} & 0.789 & 0.797  &0.817 &	0.847 &0.816&  0.847 & 0.849 &0.848 \\
                {Scidocs}	& 0.158 &0.137  &0.155 &	{0.165} &0.152&  0.166 & 0.166 & 0.165 \\
                {SciFact}	& 0.665 & 0.559  & {0.682} & 0.674 &0.682&  0.694 & 0.689 & 0.693 \\
                            \hline
                \textbf{Avg.} & 0.440 & 0.429  &0.500 & 0.518 &0.496&  0.516 & 0.514 & 0.511 \\
                %\textbf{BM25 Diff} & -- & -2.6\%  &	13.6\% &17.7\% &  6.1\%&12.7\%&14.8\% &  \textbf{15.7\%} \\
                \textbf{{Splade Diff}} & -12.0 \% &  -14.2\%  &-- & 3.6\% & -0.8\% &3.2\% & 2.8\% & 2.2\% \\
            \hline\hline
		\end{tabular}
		%\end{small}
		}
%\vspace*{-5mm}
	\caption{Zero-shot retrieval performance 
%in average NDCG@10 
on 13 BEIR datasets 
%Row ``SPLADE Diff.'' is the mean relative performance compared to the SPLADE-HT1 performance.
}
  \vspace*{-5mm}
%For quantization approaches, we adopt M=16, K=256, i.e. compression rate 32$\times$ compared to ColBERT.
	\label{tab:beir}

\end{table}




Table~\ref{tab:beir} lists  details on how  CluSD  performs 
with  SimLM and  SPLADE-HT1 in searching 13 BEIR datasets that contain out-of-domain documents.
The LSTM model of CluSD  is trained with the  MS MARCO training set,
and it is directly applied to each of the BEIR  datasets to select clusters without further tuning. 
%Zero-shot out-of-domain performance is important since a large dataset can contain document content from many domains.
% to unseen models and datasets, we evaluate the pipeline on out-domain data. For this experiment, we use the BEIR benchmarks which consists 13 released document 
%sets on various semantic relatedness tasks. 
%We directly apply the CluSD model trained on MSMARCO training set to predict the clusters on the BEIR queries and BEIR specific clusters. 


As a baseline, column ``Full $\blacktriangle$ flat'' is to fuse  the uncompressed full dense retrieval  with SPLADE-HT1 sparse  retrieval.
Column marked ``rrk'' is to rerank   top 1,000  sparse retrieval results interpolated with their dense scores. 
%The final score are the interpolation of the sparse ranked list and dense re-ranked list. 
Columns with ``CluSD-flat'', ``CluSD-m128'' and ``CluSD-m64''  are  CluSD results  using uncompressed or compressed embeddings with
m=128 or m=64. 
%\begin{itemize} [leftmargin=*]
%\item 
%Even SimLM underperforms SPLADE retriever for BEIR,  
The relevance of CluSD that fuses  sparse and dense results is higher than each individual retriever.
CluSD with limited dense retrieval   performs  closely to   oracle ``Full $\blacktriangle$ flat'',
and delivers good NDCG@10under two compression settings.
%While embedding compression affects relevance,  CluSD still performs fairly well for the BEID datasets.  
%This indicates good zero-shot performance of our proposed LSTM based strategy.
%\end{itemize}
  


==> kddexpe_feature.tex <==
\subsection{Design options for CluSD}
\label{sect:evalLSTM}

% In this section, we discuss \textbf{RQ3} and \textbf{RQ4}.
Table~\ref{tab:cluster_feat} investigates the following design options 
for cluster selection in CluSD. 
For Stage I selection, we explore two options:
\begin{enumerate}
%[leftmargin=*]
    \item SortByDist: Choose top clusters sorted by the distance of their  centroids to  the  query embedding.
% as implemented in the faiss IVF index.
    \item SortByOverlap:  Choose top  clusters sorted  by $P(C_i, B_j)$ features discussed in Section~\ref{sec:clusd}.
Namely use the overlap degree of clusters with top result bins of sparse retrieval. 
\end{enumerate}
For Stage II selection, we explore three options:
% select  the centroids based on the number of top10/25/100 sparse retrieval results in the clusters. This is the purning technique we propose in the method section.
 \begin{enumerate}
    \item XGBoost: Use the boosting tree XGBoost model to detect if a cluster should be visited.
The features used are the same ones discussed in Section~\ref{sec:clusd}. This is a pointwise approach as we view query-cluster pairs as independent samples and the decision on one cluster doesn't affect other clusters for the same query.
% excluding inter-cluster distances.
%for each query-centroid pair to predict whether the centroid should be evaluted. This is a pointwise approach.
    \item RNN: Use a vanilla RNN model to predict. The feature and sequence setup is the same as our LSTM model. 
    \item LSTM: the model we used in CluSD.
\end{enumerate}
    We also assess  the impact  of removing a  feature group  used CluSD:
\begin{enumerate}
\item w/o inter-cluster dist: removing  the inter-cluster distance feature group;
\item w/o S-C overlap: removing  the overlap-degree feature of top sparse results with each cluster.
\end{enumerate}


The last row marked ``Default'' is the final version used by CluSD with SortByOverlap and LSTM.
To have a fair comparison, this table assumes on average either 3 or 5 clusters are targeted by CluSD.
%We compare the performance of different strategies to select dense clusters.  
For XGBoost, RNN or LSTM, we set their prediction threshold so that 
the average number of clusters is close to the targeted number.
The last column of this table is the time spent to select clusters. 
%chosen depends  on the model prediction thresholds. 
%where top 3 or 5 clusters are selected. 
%In order to compare under same budget, we set the thresholds where on average around 3 or 5 clusters are used averaged over all queries. 
Table~\ref{tab:cluster_feat} shows that  the RNN or LSTM based prediction achieves  higher MRR@10 and recall compared to 
XGBoost. 
%point-wise tree based model. 
%It is reasonable as the tree model doesn't take  into account of incremental the inter-cluster relationships.
%Row  marked ``LSTM+prune'' of Table~\ref{tab:cluster_feat}, we 
%SortbyOverlap in Stage I in CluSD can significantly  decrease  the decision time by reducing the length of input cluster sequence, and can  actually lead a visible relevance increase.
Feature exploration indicates that the overlap degree is important for  cluster selection
while the inter-cluster distance feature group is also useful. 


 

\comments{
%\textbf{Effect of Model Options}
For k-means and topk heuristics, we report the performance where top 3 or 5 clusters are selected. For XGBoost, RNN or LSTM, the number of clusters chosen is dependent on the model prediction thresholds. In order to compare under the same budget, we set the thresholds where on average around 3 or 5 clusters are used averaged over all queries. 
As we can see in Table~\ref{tab:cluster_feat}, RNN or LSTM based prediction achieves much higher MRR and Recall compared to point-wise tree based model. It is reasonable as the tree based model doesn't take into account the relationships between centroids when making predictions. 
}


%\textbf{Impact of feature groups}.  

%  vs. Dense'' has a visible drop in relevance, indicating that the features we use are useful. Especially the sparse vs. dense feature, model performance has a significant drop without the feature group.

\begin{table}
\resizebox{1.0\columnwidth}{!}{
  \begin{tabular}{ r |r r| r r| r }
			\hline\hline
			 Avg \#clusters targeted  & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{5} & Time \\
			& MRR@10 & R@1k& MRR@10 & R@1k & ms\\
                   \hline
                 %RNN+prune & 0.401 & 0.919 & 0.411 & 0.961 & 2.8 \\
                 \multicolumn{6}{l}{\it{Stage II is removed. Stages I only options}}\\
                 SortByDist & 0.297 & 0.655 & 0.331 & 0.740  & 0 \\
                $\blacktriangle$ SortByOverlap & 0.384 & 0.867 & 0.401 & 0.917 & 0.2 \\
                   \hline
                \multicolumn{6}{l}{\it{Stage I=SortByDist;  Stage II model options}}\\
                 XGBoost& 0.398 & 0.888 & 0.404 & 0.929 & 192 \\
                 RNN & 0.404 & 0.908 & 0.406 & 0.938 & 2.8 \\
                 LSTM & 0.406 & 0.923 & 0.406 &0.943 & 2.8\\
                   \hline
             \multicolumn{5}{l}{\it{ Stage II=SortByOverlap;  Stage II LSTM feature group options}}\\
             w/o inter-cluster  dist& 0.402 & 0.915 & 0.406 & 0.941 & --\\
             %w/o Centroid Distance& 0.389 & 0.898 & 0.410 & 0.959 & --\\
             %w/o Sparse vs. Dense& 0.378 & 0.866 & 0.404 & 0.943 & --\\
             w/o  S-C overlap& 0.289 & 0.638 & 0.325 & 0.730 & --\\
             \hline 
             $\blacktriangle$  Default   &  0.408 & 0.943 & 0.410 & 0.953 & 2.8 \\
             %$-$ Query vs. Centroid & 0.405 & 0.925 & 0.406 & 0.941 & --\\
              \hline\hline
		\end{tabular}
}
	\caption{Design options for  CluSD. $\blacktriangle$ is the default choice.}
	 \vspace*{-5mm}
        \label{tab:cluster_feat}
\end{table}

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.42]{ncluster2.pdf}
    \caption{CluSD performance and latency with respect to a different average  number of selected clusters}
    % \vspace*{-4mm}
    \label{fig:ncluster}
\end{figure}


\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.48]{threshold.pdf}
    \caption{Left: Distribution  of \#visited clusters under different selection threshold $\Theta$.
Right: Mean \#visited clusters on MSMARCO Dev set and BEIR datasets.}
     \vspace*{-5mm}
    \label{fig:thresholds}
\end{figure}

\subsection{Impact of  cluster partitioning size}
\label{sect:clusterno}

%The cluster selection technique is built on top of a group of defined clusters. It is important to understand how the cluster selection works and a good rule of thumb to 
%determine the model prediction threshold given different number of clusters. 
CluSD assumes the embeddings are pre-partitioned into $N$ clusters.  Figure~\ref{fig:ncluster} shows the impact of CluSD when
$N$ is  4096 and  8192.
% we plot three scenarios where the total number of clusters is 1024, 4096 and 8192 respectively. 
For stage I, we use $n=128$ in this figure to depict the impact of selecting different numbers of clusters on average in a wider range.
A  solid line refers to the use of uncompressed dense embeddings while  a dash-dot line refers to the quantization with OPQ m=128, 
and a dotted line refers to the quantization  with OPQ m=64. X-axis is the average number of clusters selected by CluSD.
We vary the selection threshold parameter $\Theta$ in CluSD to achieve the different average number of clusters selected. 

Figure~\ref{fig:ncluster} shows that with both $N$,
%MRR@10 reaches above 0.420 when above    $<$ 10 clusters 
MRR@10 reaches above 0.420 when above 10 clusters 
are selected.
As more clusters are selected,  the recall ratio does  increase. 
%Note that when total number of clusters increases, the percentage of documents search will be different given a fixed number of clusters are selected. 
%Given a fixed number of selected clusters,  the latency impact is different with different $n$ values.
%This result in difference in average latency. 
Looking at  a fixed average number of selected clusters, 
different $N$ values imply different latency numbers.
For example, when 10 clusters are selected on average, 
CluSD  scans through 0.1\% and  0.2\% of embeddings corresponding to N=4096 and 8192, respectively. 
%As we can see in the bottom two sub-figures, 
When $N= 8192$, its latency in milliseconds is smaller  with a  smaller size per cluster
as the CluSD time complexity is proportional  to  the size per cluster and the number of clusters selected.
%With $N$ becomes much bigger,  the overhead of clusters in stage II optimization starts to offset or outweigh latency benefits of small clusters. 
% while the overall CluSD time is still  
\comments{
In this case, given a 20 
%(35 ms for 99\%) 
millisecond mean latency constraint, 
CluSD  with flat index can achieve 0.425 and 0.988 in MRR@10 and recall@10 by visiting  about 50 clusters (0.6\% of documents), 
which is the same performance compared to the full index search. 
This observation is logical, as for each cluster, there are possibly only tens or a few hundred relatively important documents to be evaluated for 
a given query. Majority of the documents in the clusters are not worth exploring. As the size of each clusters decreases, we are able to see more top important documents. 
}

Lastly, as CluSD makes a query-specific decision to dynamically select  clusters, each query has  a  different number of clusters visited
given a fixed threshold value and query latency can vary. 
The bottom right subfigure shows that the 99\textsuperscript{th}
percentile latency is around 2x longer than the mean latency, which is reasonable by
looking at the previous retrieval latency studies (e.g. ~\cite{mallia2019pisa, mackenzie2021anytime}). 




\subsection{Impact of  selection threshold $\Theta$}
\label{sect:threshold}
\comments{
\textbf{RQ6}: does the cluster selection model dynamically select different numbers of clusters for different queries? How the selection differs for different datasets?
For the first question, we plot out the distribution of number of clusters selected for each query as a boxplot in 
}
The left portion of Figure~\ref{fig:thresholds} shows
the average number of SimLM dense clusters selected by CluSD for MS MARCO Dev set under different threshold $\Theta$ values  when
the input sequence length $n$ for Stage II LSTM is 32.
%Model prediction threshold refers to the threshold which we use to determine the selection of a cluster. 
A threshold can be chosen for CluSD to follow a  time budget. 
%As we can see, there is a variety in the number of clusters selected. 
%While the median number of clusters selected is  10 clusters, the 75th percentile is around 18 clusters. 
In our experiments,  the default setting of
CluSD is to use threshold 0.02  for MS MARCO passages and the average number of clusters selected by CluSD using this threshold is 22.3.

The right portion of Figure~\ref{fig:thresholds} 
shows  the mean number of clusters selected for MS MARCO Dev set and averaged over 
the zero-shot BEIR datasets.
This subfigure shows that for a fixed $\Theta$ value, CluSD  adaptively chooses a fewer number of clusters for a
BEIR dataset compared to the MS MARCO Dev set.  
%This aligns with our expectation that  
This is intuitive as
SimLM underperforms SPLADE on the BEIR datasets in general. Thus, it is unnecessary to evaluate a lot of clusters. 
%CluSD adaptively selects fewer clusters for BEIR% to conduct selective dense retrieval. 



==> kddexpe_io.tex <==
\subsection{ Search with on-disk data}
\label{sect:evaldisk}
%{\bf CDFS vs. re-ranking and nearest-neighbor search baselines with in-memory or on-disk data.}

Table~\ref{tab:disktime} examines the performance  of CluSD fused with SPLADE when MS MARCO passage 
embeddings  cannot fit in memory and is stored on an SSD disk.
We use  $N=65,000$ for CluSD to reduce the cluster size and the extra space for quantized inter-cluster distances takes about 40MB. 
We also compare other selective dense retrieval baselines using  reranking or proximity graph navigation.
%The mean response time (MRT) and 99 percentile time (P99) include the I/O cost while their cost breakdown for I/O and CPU time is also listed. 
The mean response time (MRT) and 99\textsuperscript{th} percentile time (P99) only
include the total dense retrieval time, while their cost breakdown for I/O and CPU time is also listed. 
All times reported are in milliseconds. 
Column ``MRR@10'' means  MRR@10 for the Dev set. 
Column ``\#Doc'' is the number of embeddings fetched for performing full or partial dense retrieval.
%A small table on the top specifies the data location of configured retrieval algorithms.
The reranking method simply fetches top-$k$ embeddings  from the disk for fusion. 
LADR is designed for in-memory search~\cite{2023SIGIR-LADR} and we run it by  assuming  memory can sufficiently host the proximity  graph while letting LADR access  embeddings from the disk. 
Excluding the I/O cost portion of LADR in this table, the in-memory search cost of LADR is marked in the CPU time column.
We test two configurations of LADR, its default with 128 neighbors, 200 seed documents, and a search depth of 50,
as well as a faster configuration, selected such that its CPU time is similar to CluSD. 
LADR\textsubscript{fast} uses 128 neigbhors, 50 seed documents, and a depth of 50.
DiskANN~\cite{NEURIPS2019_DiskANN} assumes the graph and original embeddings are on disk  while the memory  hosts
compressed embeddings for quick guidance.  SPANN~\cite{chen2021spann} searches disk data in a cluster-based manner based on query-centroid distances.
Both DiskANN and SPANN  are designed for on-disk search from scratch without fusing with others, and thus we simply fuse their outcome with SPLADE results.
HNSW~\cite{2020TPAMI-HNSW} is not included because its in-memory relevance  is similar as DiskANN while it is not designed to be on disk. 

\comments{
As the size of dense embeddings or the number of documents in a dataset increases, it is likely that dense embeddings are too large to be fully stored in memory. For instance, RepLLaMA requires 135.6GB for the 8.8M documents in MS MARCO; BERT-based dense embeddings for a 1B document dataset would require 2.8 TB. This problem is exacerbated when a large navigation graph is also required to be loaded in memory. We compare CluSD with several baselines when the embeddings are stored on disk and must be loaded to memory before ranking. We memory-map the dense embeddings and load them on-demand during our algorithm. We measure both the disk access time (I/O) and the associated computation required by each method (Overhead). Our results are shown in Table \ref{tab:disktime}. 
% TODO (above): Latency figures given in the table only represent the dense portion of retrieval. 
% TODO (above): We compare each method with RepLLaMA and SimLM embeddings for WHY DO WE DO THIS?
}

Reranking is similar to CluSD in terms of  mean latency while having a much slower 99\textsuperscript{th} percentile latency, lower MRR@10 and  recall@1000.% in this case.
CPU-time of reranking is short but its total time is dominated by 1,000 random I/O operations for fetching top embeddings. 
%and reaches about  715MB/second I/O speed. 
Our setting stores embeddings in clusters grouped by their similarity on disk, thus
random I/O operations in reranking  benefits from spatial locality in clustered data, because top results tend to 
be similar. Meanwhile  its  99\textsuperscript{th} percentile latency is 5.1x slower when  spatial locality cannot be well exploited or  is 
less available. 
The column ``Worst'' lists  the estimated worst-case latency when documents are not clustered on the disk. 
We find that  each  I/O operation has about a 0.3ms queueing and other software overhead on our tested PCIe SSD.
Thus, more fine-grained operations in reranking yields more overhead.
In comparison, CluSD issues  much fewer  I/O operations to fetch 4,423 embeddings per query on average in a block I/O manner.
Its 99\textsuperscript{th} percentile latency is 2x faster than re-ranking.

CluSD outperforms LADR with higher MRR@10 and a lower latency for the two tested configurations.
% taking much less and  99\textsuperscript{th} percentile latency.   
The above I/O spatial locality  explanation for reranking is also applicable to LADR.  
CluSD outperforms  DiskANN in relevance and latency.
% which is designed for more general nearest neighbor search. 
CluSD is comparable to SPANN in relevance  but is 6.98x faster in the mean latency.

% while CDFS, which fetches clusters of consecutive embeddings, utilizes block I/O that incurs less access overhead. 



\comments{
We find that the disk access time required by CluSD is significantly less than the time required by LADR or a simple rerank. We suggest that SSD random seeks have significant overhead compared to consecutively reading. Thus, reading many documents consecutively from a cluster is quick, and the number of random seeks is limited to the number of clusters accessed. During other methods, it is likely that the number of random seeks is equal to the number of documents accessed. A simple least-squares model for our RepLLaMA results suggests that each random seek takes 167 us, whereas the time to read one document is only 11.8 us.
}


\comments{
We find that the disk access time required by CluSD is significantly less than the time required by LADR or a simple rerank. We suggest that SSD random seeks have significant overhead compared to consecutively reading. Thus, reading many documents consecutively from a cluster is quick, and the number of random seeks are limited to the number of clusters accessed. During other methods, it is likely that the number of random seeks is equal to the number of documents accessed. A simple least-squares model for our RepLLaMA results suggests that each random seek takes 167 us, whereas the time to read one document is only 11.8 us.
}

% CluSD is with XXXX configuration and XXXX average clusters per query. Reranking reranks the top-1000 documents from bm25 + docT5query. LADR_S are results from a "small" version of adaptive LADR, with k=128, n=8, c=200. LADR_L are results from a "large" version of proactive LADR, with k=128, n=200 that retrieves approximately ten times more documents than LADR_S






%Added for KDD 2024


\begin{table}[htbp]
        \centering
 \resizebox{1.0\columnwidth}{!}{
                \begin{tabular}{r |lll|lll|rr}
                        \hline\hline
                        & \multicolumn{2}{c}{\bf{Relevance}}& \bf{\#Docs} &  \multicolumn{5}{c}{\bf{Dense Latency \& Breakdown (ms)}}\\
            & MRR@10 & R@1k & fetched&  MRT & P99 & Worst&I/O  & CPU  \\
        \hline
        Rerank& 0.421 & 0.980 & 1000.0 &  18.8& 95.70 & 454.9  &16.9& 1.9\\
        %S+LADR & 0.422 & 0.984 & 82.99 & 28.86 & 8521.6 & 111.85 &  \\
% Above: Default configuration
        LADR\textsubscript{fast} & 0.419 & 0.980 & 2431.0 & 42.3 & 191.5 & 1105.9 &31.3 & 11.0\\ % ladr n=50, c=50, k=128
        LADR\textsubscript{default} & 0.422 & 0.984 & 8521.6 &  119.3 & 349.8 & 3876.5 & 91.4 & 27.9\\
% Above: LADR with time budget of CPU time ~= CluSD CPU time ~= 6-7ms
      %  D-ANN-Wentai & 0.398 & 0.970 & 271.4 & 5.24 & -- & 276.6 & 321.2\\
   %     SPANN-Wentai & 0.405 & 0.965 & -- & -- & -- & 123.6 & 159.6 \\
           DiskANN& 0.417 & 0.984 & -- &  276.5 & 312.2 & -- &272.3& 5.2\\ 
        SPANN& 0.420 & 0.989 & -- &  123.6 & 159.6  & -- &-- & -- \\
%Did Yingrui adds fusion and adds this on Wentai's result?  Yes  S+DiskANN & 0.417 & 0.984 & -- & -- & -- & 276.5 & 312.2\\ov
       % S+SPANN* & 0.424 & 0.985 & 6.54 & 6.20 & 3484.9 & +12.74 & 84.73\\
% Above: Parker selected clusters from top-16 SPLADE results -> thus relevance is too strong
        %CluSD& 0.425 & 0.986  & 6.19 & 6.48 & 4423.51 & 12.67 & 42.77\\
    %CluSD& 0.425 & 0.986  & 4423.5&  17.7& 47.8 & 178.1 &6.2& 11.0\\
    CluSD& 0.425 & 0.986  & 4423.5&  17.7& 47.8 & -- &6.2& 11.0\\
                \hline\hline
                \end{tabular}  }
        \caption{Search when uncompressed embeddings and/or the proximity graph are on disk for SPLADE + SimLM}
% Embedding space = 25.9 GB. Here we only report the latency of the dense retrieval part.
\vspace*{-10mm}
        \label{tab:disktime}
\end{table}
                                     


==> kddexpe_sparse.tex <==
\subsection{CluSD with other sparse models}
\label{sect:evalsparse}

%We explore the model performance when we interpolate different sparse model with SimLM with cluster selection in 
Table~\ref{tab:sparse} examines the CluSD's fusion of SimLM
with  other three sparse models under  different efficiency/relevance tradeoffs.
For each of three models, CluSD boosts overall relevance.
%These sparse models accomplish  different relevance  scores: 
%CluSD fused with  the   fastest BM25T5 model delivers the lowest MRR number while its fusion  with the slowest LexMAX delivers
%the highest MRR@10 number.
%The final relevance outcome of using two SPLADE models is better  than that for BM25 retriever.
%That is partially caused by dependence of LSTM training where  the positive clusters are identified by the overlap of top 10 SPLADE results with these  clusters.
As  CluSD's cluster selection  replies on  the overlap feature  of top sparse results with dense clusters,
the guidance from the fastest BM25 results is less accurate than the other  sparse models. On the other hand, with a guidence from 
the slowest but stronger LexMAE retrieval, CluSD yields the highest MRR@10, comparable to full search. 
%the quality of top sparse results still has an impact on the final outcome.  
%consists of the distribution of sparse top results into clusters. 
%When the sparse model doesn't identify good top candidates, the input features to the LSTM model becomes more noisy which affect performance. 
\comments{
From left to right, the model performance degrades. 
We can observe that when sparse model performance degrades, 
the performance of S + CluSD degrades as well on the flat index. 
For example, on Splade-HT1-fast, the relevance is around the same as S $+$ D on MRR@10, and 0.6\% degradation on recall@1k. 
When we use BM25-T5 model, the degradation is 1.7\% and 1.5\% respectively on MRR@10 and recall@1k. 
This indicates that when the Splade model model does not perform well, CluSD becomes less effective. 
It is expected because the input to the LSTM model consists of the distribution of sparse top results into clusters. 
When the sparse model does not identify good top candidates, the input features to the LSTM model become more noisy which affects performance.
}

\comments{
\begin{table}[htbp]
	\centering
		\resizebox{\columnwidth}{!}{%
		\begin{tabular}{ r l l  |ll |ll |r }
			\hline\hline
                Sparse model& \multicolumn{2}{c|}{\bf{Splade-HT1-fast}} & \multicolumn{2}{c|}{\bf{Splade\_effi-HT3}}   & \multicolumn{2}{c|}{\bf{BM25-T5}} & Extra\\ 
%\cline{1-7}
%                Latency & \multicolumn{2}{c|}{22.4ms} & \multicolumn{2}{c|}{12.4 ms}   & \multicolumn{2}{c|}{9.2 ms} & Latency\\ 
\cline{1-7}
			& {MRR@10} & {R@1k}  & {MRR@10} & {R@1k}   & {MRR@10} & R@1k  & latency \\
   \hline
   \multicolumn{8}{c}{\bf{Uncompressed SimLM embeddings with  27.2 GB space}}\\
			\hline
			S & 0.385$^\dag$& 0.949$^\dag$& 0.380$^\dag$& 0.944$^\dag$& 0.259$^\dag$& 0.935$^\dag$& -\\
                $\blacktriangle$  S $+$ D & 0.416 & 0.986 & 0.413 & 0.984 & 0.415 & 0.985  & +1674.1\\
                {\textbf{S $+$ CluSD}} & 0.415 & 0.981$^\dag$& 0.411 & 0.979$^\dag$& 0.408& 0.970$^\dag$& +12.1 \\
                \hline
                \multicolumn{8}{c}{\bf{OPQ m=128. SimLM embedding space  1.1 GB}}\\
%, Report S+*
\hline
                S $+$ D-IVFOPQ & 0.384$^\dag$& 0.981$^\dag$& 0.381$^\dag$& 0.978$^\dag$& 0.369$^\dag$& 0.975$^\dag$& +21.9 \\
                %S $+$ D=HNSWOPQ & & & & & & &  \\
                \bf{S $+$ CluSD} & 0.413& 0.984& 0.412& 0.984& 0.402$^\dag$& 0.975$^\dag$& +9.8  \\
                %\hline
                %\multicolumn{8}{c}{OPQ M=64. Embedding space  0.6 GB}\\
%, Report S+*
                % S $+$ IVFOPQ-5\% & 0.389 & 0.981 & 0.389 & 0.980 & 0.370 & 0.975 & 23.7 \\
                %S $+$ HNSWOPQ & & & & & & &  \\
                %S $+$ \bf{CS} & 0.402& 0.981& 0.402& 0.981& 0.380& 0.973& 10.2 \\
            \hline\hline
		\end{tabular}
		}
	\caption{CluSD performance  under  other  sparse models}

\vspace*{-5mm}
	\label{tab:sparse}
\end{table}
% For all three sparse models, we use the same dense model configuration so for each row we only report one latency number. 
}

\comment{
\begin{table}[htbp]
	\centering
		\resizebox{\columnwidth}{!}{%
		\begin{tabular}{ r r r r r  r r r}
			\hline\hline
			& \multicolumn{2}{c}{MSMARCO Dev}& \multicolumn{2}{c}{DL19}& 
\multicolumn{2}{c}{DL20} \\
			& \% n& MRR@10 & R@1k & NDCG@10 & R@1k &  NDCG@10 & R@1k\\
   			\hline
 D& -- & 0.416& 0.988& 0.720& 0.744& 0.703&0.755\\
            $\blacktriangle$  S $+$ D & -- & 0.425 & 0.988 &  0.740& 0.816&   0.731& 0.819\\
            \bf S $+$ \bf{CluSD} & 0.5 &  0.426 & 0.987 &  0.744&  0.820& 0.734&  0.818\\
            \hline
            \multicolumn{8}{c}{OPQ M=128 setting, Storage 1.1GB, Report S+*}\\
            \hline
            IVFOPQ &10 & 0.404 & 0.987 & 0.713 & 0.818 & 0.722 & 0.817 \\
            & 5 & 0.394 & 0.987 & 0.687 & 0.817 & 0.706 & 0.817 \\
            & 2 & 0.374 & 0.986 & 0.656 & 0.815 & 0.700 & 0.817 \\
            HNSWOPQ & & & & & & \\
            \bf{CS} & 0.5 & 0.417& 0.986& 0.742 & 0.818 & 0.735  &0.815 \\
            \hline
            \multicolumn{8}{c}{OPQ M=64, Storage 0.6 GB, Report S+*}\\
            \hline
            IVFOPQ & 10 & 0.393 & 0.986 & 0.676 & 0.814 & 0.730 & 0.818 \\
            & 5 & 0.384 & 0.985 & 0.659 & 0.814 & 0.717 & 0.817 \\
            & 2 & 0.368 & 0.985 & 0.643 & 0.814 & 0.707 & 0.816 \\
            HNSWOPQ & & & & & & & \\
            \bf{CS} & 0.5  & 0.403& 0.987& 0.729 & 0.812 &0.724 & 0.814 \\           
			\hline\hline
		\end{tabular}
		}
	\caption{RetroMAE
%For quantization methods on top of ColBERT, we also report \% degradation from ColBERT.
}
	\label{tab:retromae}
\end{table}
}

%Added for KDD 2024

\begin{table}[htbp]
	\centering
		\resizebox{\columnwidth}{!}{%
		\begin{tabular}{ r l l  |ll |ll |r }
			\hline\hline
                Sparse model& \multicolumn{2}{c|}{\bf{LexMAX}} & \multicolumn{2}{c|}{\bf{uniCOIL}}   & \multicolumn{2}{c|}{\bf{BM25T5}} & \bf{Dense}\\ 
%\cline{1-7}
                % & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{}   & \multicolumn{2}{c|}{} & Latency\\ 
\cline{1-7}
			& {MRR@10} & {R@1k}  & {MRR@10} & {R@1k}   & {MRR@10} & R@1k  & \bf{latency}\\
   \hline
   \multicolumn{8}{c}{\bf{Uncompressed SimLM  embeddings  with 27.2 GB space}}\\
			\hline
			S & 0.425& 0.988& 0.347 & 0.957& 0.259&  0.935& -\\
                $\blacktriangle$  S $+$ D &    0.430& 0.990& 0.413 & 0.985& 0.415& 0.985& 1674ms\\
                S $+$ Rerank& 0.432& 0.988& 0.415& 0.957& 0.409& 0.935& 21.9ms\\
                %S $+$ LADR& 0.430& 0.990& 0.414& 0.983& 0.412& 0.983& 21.9ms\\
                {\textbf{S $+$ CluSD}} & 0.431& 0.989& 0.414 &  0.980&  0.410&  0.980& 12.1ms\\
                \hline
                \multicolumn{8}{c}{\bf{OPQ m=128. SimLM embedding space  1.1 GB}}\\
%, Report S+*
\hline
                S $+$ D-IVFOPQ & 0.383& 0.988& 0.354& 0.961& 0.369& 0.975& 21.9ms\\
                %S $+$ D=HNSWOPQ & & & & & & &  \\
                \bf{S $+$ CluSD} & 0.429& 0.989& 0.404 & 0.980&  0.402& 0.975& 9.8ms\\
                %\hline
                %\multicolumn{8}{c}{OPQ M=64. Embedding space  0.6 GB}\\
%, Report S+*
                % S $+$ IVFOPQ-5\% & 0.389 & 0.981 & 0.389 & 0.980 & 0.370 & 0.975 & 23.7 \\
                %S $+$ HNSWOPQ & & & & & & &  \\
                %S $+$ \bf{CS} & 0.402& 0.981& 0.402& 0.981& 0.380& 0.973& 10.2 \\
            \hline\hline
		\end{tabular}
		}
	\caption{ Performance  under  three  sparse models}

\vspace*{-5mm}
	\label{tab:sparse}
\end{table}


==> kddintro-backup.tex <==


\section{Introduction and Related Work}



\comments{
Sparse and dense retrievers are two main categories of retrieval techniques for text  document search.
Traditional sparse retrieval models, such as BM25, use lexical text matching and run
%to retrieve results from the collection 
efficiently by traversing  an inverted index on an inexpensive  CPU platform.
Recently sparse retrieval studies have exploited learned neural representations~\cite{Dai2020deepct,
Mallia2021deepimpact, Lin2021unicoil,2021NAACL-Gao-COIL, Formal2021SPLADE, Formal2021SPLADEV2} for better semantic matching. 
%and SPLADE~\cite{Formal2021SPLADE, Formal2021SPLADEV2} has demonstrated the strong relevance performance among these models. 
The second category of document retrieval 
exploits a pre-trained language model with a dual encoder architecture to produce a dense document representation, 
e.g. ~\cite{gao-2021-condenser,2021SIGIR-Zhan-ADORE-dense,Ren2021RocketQAv2, 
%e.g. ~\cite{Lin2021tctcolbert, 2021CIKM-JPQ-Zhan, xiong2021-ANCE, gao-2021-condenser,2021SIGIR-Zhan-ADORE-dense,Ren2021RocketQAv2}. 
%There are numerious studies recently to enhance  dense retrieval with knowledge distillation
%and  improved  langage model pretraining~\cite
Lin2021tctcolbert, Santhanam2021ColBERTv2,  Wang2022SimLM,  Liu2022RetroMAE}.
}

Recent studies have found that combining  sparse and dense retrieval scores  can further boost
retrieval recall and relevance~\cite{Lin2021unicoil,2022LinearInterpolationJimLin,kuzi2020leveraging},
suggest  that both categories  of retrievers tend to capture  different relevant signals. 
These studies  make an assumption that  a search platform has to run two retrievers separately and a dense retriever.
%delivers   its maximum effectiveness, and the impact of compression and IVF clustering is not considered. 
There is an imbalance of computing platform requirement for running  these two retrievers.
dense retrieval typically requires GPU support unless significant  
%We study the use of dense retrieval results to argument sparse retrieval. 
Sparse retrieval with an inverted index has an advantage that a low-cost CPU server can run the online inference  without GPU.
This paper is targted at a low-cost CPU-friendly retrieval design.
%A judicious tradeoff consideration of retrieval  effectiveness and efficiency is critical on  a low-cost CPU-friendly search platform. 
%The importance of CPU-friendly search is recognized 
%in neural ranking studies~\cite{Yang2021WSDM-BECR,2022WWWforwardIndex,2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
For a large-scale  dataset (e.g. with billions of documents), a practical search system often employs  a multi-stage 
search architecture, which divides the dataset into many partitions so that  a fast first-stage  retrieval 
method  can  search these partitions in parallel.  Such a system  prefers low-cost
CPU-only servers for first-stage retrieval, and both time and memory space complexity of retrieval should be considered 
so that  each server can host as many documents as possible
to reduce the total number of servers to support a large data size and high query traffic. 
%Thus the challenge for retrieval on such an architecture needs to consider both time and space complexity. 
% small search index needs to be as small as possible.
%and the in-memory footprint size of 
%server  needs to host documents in memory as many as possible 
%given a large number  of data partitions involved for parallel search.
%Each server employs multiple CPU cores and is replicated with many copies  for dealing high traffic of  concurrent 
%search requests, and thus 


\comments{
There are recent efficiency studies 
for 
%advancing the inverted index implementation for 
fast sparse retrieval with learned neural 
representations~\cite{Lassance2022SPLADE-efficient,mallia2022faster,qiao2023optimizing,2023SIGIR-Qiao, 2023SIGIR-SPLADE-pruning},
%which run  efficiently  on a single CPU without hardware accelerators  GPU
%which re  retaining strong relevance effectiveness
%%Another development in learned sparse retrieval is that
%sparse retrieval with a learned representation
which accelerates learned sparse retrieval with BM25-guided traversal or index pruning.
% with a single thread on  a 2.25GHz AMD EPYC 7742  CPU server.
%There is a tradeoff  in relevance effectiveness if BM25 guidance or threshold-based pruning  is too aggressive.
%and dense retrieval can boost if it does not add much overhead. 
}

There are recent efficiency studies on
fast  sparse retrieval with learned
representations~\cite{Lassance2022SPLADE-efficient,mallia2022faster,qiao2023optimizing,2023SIGIR-Qiao, 2023SIGIR-SPLADE-pruning}.
For example, Row 3 of Table~\ref{tab:costbudget} shows the latency, memory space cost, and  MRR@10  of
a latest efficient SPLADE retriever for searching 8.8 million
MS MARCO passages~\cite{2023SIGIR-Qiao} on a CPU only server.
Row 2 is performance of a BM25 based retriever after document expansion. 
Dense retrieval can be accelerated  by approximate nearest neighbor  search with 
IVF clustering~\cite{johnson2019billion, 2021Facebook-DrBoost-Lewis}, quantization~\cite{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ},
%and hierachical navigable  small world graphs (HNSW)
and  proximity graph based navigation~\cite{2020TPAMI-HNSW,2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
Limited IVF cluster search and quantization can lead to  a significant  relevance drop while 
For example, last two rows of Table~\ref{tab:costbudget} shows the latency, memory space cost, and  MRR@10  of
RetroMAE~\cite{Liu2022RetroMAE} dense retrieval without compression is slow, use of
IVF clustering and OPQ quantization substantially accelerates but leads to a significant drop  of   MRR@10 score when searching up-to 20\%  
of top dense clusters. 
%There is also a cost-relevance tradeoff  with proximity graph based search  using inter-document similarity distances~\cite{2020TPAMI-HNSW, 
%2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}.  
%Construction of a large document-level  graph   is  expensive
%during offline processing. 
online hosting of a document similarity graph  for graph navigation adds a large space cost.
%For example, the proximity graph  can take extra 4.3GB memory space~\cite{2023SIGIR-LADR} for 8.8M  MS MARCO passages. 
None of above studies has considered to exploit the selective fusion of dense and sparse  retrievers. 

\begin{table}[htbp]
        \centering      
         \resizebox{0.82\columnwidth}{!}{ 
                \begin{tabular}{ r | r  rr}
                        \hline\hline
Sparse or dense methods  & Latency & Memory & MRR@10\\ 
\hline
BM25/DocT5Query & 9.2ms & 1.2GB & 0.261\\  
SPLADE/HT1 & 31.2ms & 3.9GB & 0.396 \\ 
RetroMAE/Uncompressed & 1677ms & 27.2GB & 0.419 \\ 
%SimLM /OPQ             & 225-1579ms & 0.57-2.3GB & $<$ 40.2 \\
RetroMAE /IVFOPQ  & 38-339ms & 1.2-2.3GB  & 0.37-0.401\\ 
                        \hline\hline
\end{tabular}
}
\caption{Latency and space cost of sampled sparse and dense models for MS MARCO passages with Dev query  set}
% \vspace*{-5mm}
\label{tab:costbudget}
\end{table}


\comments{
That is true also with the  navigation of  a  proximity graph based on inter-document similarity distances called HNSW~\cite{2020TPAMI-HNSW}. 
The proximity graph approach to guide dense retrieval is revisited recently in GAR~\cite{2022CIKM-MacAvaneyGraphReRank}, which is furthered improved by
%LADR Kulkarni  et al.~\cite{2023SIGIR-LADR} improves HNSW.
LADR~\cite{2023SIGIR-LADR}.
%~\cite{2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
The weakness of  the  proximity graph approach is that its graph  construction requires a quadratic computing complexity, which is expensive
for a large dataset and the online hosting of such a graph also adds a significant space requirement  on a low-cost
computing platform. For example, LADR takes extra 4.3GB memory space for 8.8M  passages in the MS MARCO dataset to keep top 128 
top neighbors per document. 
%Similarily HNSW also incurs a high space cost for graph connections.  
%In comparison, cluster-based selective dense retrieval can achieve in a comparable time complexity
%while adding  insignificant extra  space  overhead.


  
%with a latency controled within 4 to 8 milliseconds on a single CPU, but with a significant tradeoff in relevance effectiveness.
%For example, MRR@10 for MS MARCO Dev set drops from RetroMAE has dropped from  0.416 to 0.356.
%This paper does not impose 4-8 millisecond latency, but rather looks for a solution that can leverage both dense and sparse retrieval
%and relax the latency constraint in some degree while maximizing its relevance effectiveness as much possible.
%a range below or around  100 milliseconds 

%The response time  for such a system for an interactive service needs to be fast enough a
%and thus search needs to be completed within a few hundred milliseconds. 

%which only requires triggering of dense embedding  computation for a relaively small subset of documents.
%The proposed scheme called cluster-based selective dense  retrieval

}

This paper proposes  a selective fusion of dense and sparse retrieval results 
%Because sparse retrieval is fast on CPU-only servers, this paper 
%augmenting sparse retrieval with 
called CluSD to argument  sparse retrieval with limited cluster-based dense retrieval results.
CluSD includes an LSTM based model with cluster prioritization and pruning to trigger limited dense computation. 
CluSD exploits inter-cluster and query-to-cluster distances and   the overlapping degree between top sparse retrieval results and dense clusters
to optimize cluster selection. 
%and then make a decision to determine which document clusters should be selected  to conduct dense retrieval computation.
The extra memory space overhead required to assist CluSD is negligible, and it  
works well when embedding vectors are highly compressed.
%  and  the extra memory required for hosting dense embeddings can be limited  after compression. 

\comments{
This paper evaluates  the usefulness   of CluSD  under a time and space constraint on a CPU only server when
 searching MS MARCO and BEIR  datasets  and provides a comparison with other baselines.
The evaluation  shows that CluSD can effectively identify a small number of document clusters to augment sparse retrieval results efficiently 
for  a stronger relevance  even though such a  sparse retriever is fast with  a relevance tradeoff. 
} 
%provides a flexibility and reduces  the relevance reqirement of sparse retrieval.
%Namely protentially we can choose a relatively fast sparse retrival with the slightly lower accuracy/recall,
%and  let dense retrivsal make up the loss. Our design needs to  adapt to  sparse retrieval quality and plans

%CSDR in improving the effectiveness of sparse retrieval with limited dense  retrieval
%traversal for low-cost search.  Our emprial findings suggest that SRF  can consistently outperform other baselines on a single CPU server 
%without GPUs 
% and achieve a strong tradeoff of effectiveness and efficiency compared to an exhausitve dense retrieval search.


%from pretrained language models to provide effective semantic text matching between a query and a document.





%0.419 by RocketQAv2~\cite{Ren2021RocketQAv2}, 
%which are the two latest state-of-the-art retrieval-reranker pipelines using cross-encoder based rerankers.
%Re-ranking in  recent dense retrieval work SimLM~\cite{Wang2022SimLM} has  used an expensive cross-encoder to
%achieve impressive MRR score 0.437 
%Re-ranking in RocketQAv2~\cite{Ren2021RocketQAv2} achieves 0.419 with a similar strategy.  



\comments{Modern search engines for text documents
typically employ two-stage ranking design. 
The first retrieval stage extracts top candidate
documents matching a query from a large search index with a fast ranking method. 
The second stage uses a more complex algorithm to 
re-rank top results thoroughly.
Recently neural ranking techniques from transformer-based architectures
have achieved impressive relevance scores 
for both retrieval and top $k$ document re-ranking. 
However, many recent work treats retrieval and reranking stage as two independent tasks and optimize them separately. Only a few works take into consideration the interplay of a retriever and a reranker. RocketQAv2 trains a cross encoder reranker and dual encoder retriever jointly with a strong reranker as teacher and train the retriever by dynamically distilling from reranker. Leonhardt (2022)\footnote{https://arxiv.org/pdf/2110.06051.pdf} uses a linear combination of the semantic similarity scores from the re-ranking phase and lexical matching scores from the retrieval phase with respect to the query for query evaluation.  

These methods either uses the reranker as a teacher to train the re-retriever, or consider the shallow combination of the results from two stages. In these training strategies, both the retriever and reranker are trained towards the same goal. In real application, as the two stages work jointly, either model does not need to perform perfectly by itself. Instead, by taking a more integrated view of the two stages in training and inference, the joint performance of the two stage models will be more efficient and effective. 

Moreover, these approaches typically requires a reranker (such as a cross-encoder in the case of RocketQA). In text retrieval applications, efficient rerankers with low online inference latency are often favored. In recent years, the late interaction reranking model ColBERT, TILDE, BECR provide reasonable performance with low query latency. We demonstrate that pipelines with such efficient models can be improved using our training strategy. 


In our work, we train the efficient reranker and retriever iteratively to improve the integrated performance of the two stage pipeline through a process termed dynamic integrated training.
 To achieve optimal performance under such setting, when training the reranker, we upweight the poorly ranked samples in the joint pipeline through a soft-hard loss. In the meanwhile we gradually update the training set with the top combined ranked results from pipeline during training. With these shifts, the model will automatically be geared towards the weak point of the joint ranking results of the pipeline. In addition, we employ the top documents retrieved by the retriever to provide additional ranking signal in both training and evaluation in the reranking stage. 


During inference, the retriever would return top documents and their corresponding rank order to formulate a pseudo query. The reranker then matches both the original query and the pseudo query with top documents to get two ranking scores for each query-document pair. As the reranker is trained as a booster, the final ranking order from the pipeline naturally becomes the combination of the retrieval and reranking ranked lists. The final top-k ranking scores is determined by the reciprocal ranked fusion~\footnote{https://plg.uwaterloo.ca/~gvcormac/cormacksigir09-rrf.pdf} of ranks given by both the retrieval and reranking models.

We find that the propose integrated strategy enjoys several advantages. First, under same model setting and training condition, the dynamic integrated training strategy improves the relevance of the two stage pipeline under both scenarios where reranker is an efficient one or reranker strongly outperforms retriever on MS MARCO passage dataset and TREC19 and TREC20 datasets. This indicates that the integrated training strategy is generally applicable.  Secondly, as the two models learn slightly different goals, the joint performance of the two is less likely to overfit. Indeed, we observe a good zero-shot performance of the pipeline on the BEIR dataset. Lastly, we find that our training strategy can be applicable to the currently popular sparse and dense retrieval pipeline where two retrieval models jointly determine the final ranking list. 

}


==> kddintro.tex <==


\section{Introduction}

\label{sect:intro}
Dense and sparse retrievers are two main categories of retrieval techniques for text  document search.
%It can be time-consuming to compute query-document similarities for the whole corpus on a CPU-only platform. The cost is often mitigated through approximate nearest neighbor search techniques. However, this reduction in latency comes with a tradeoff in relevance effectiveness. 
Traditional sparse retrieval models, such as BM25, use lexical text matching and run
%to retrieve results from the collection 
efficiently by traversing  an inverted index on an inexpensive  CPU platform.
Recently, sparse retrieval studies have exploited deep learning models~\cite{Dai2020deepct,
Mallia2021deepimpact, Lin2021unicoil,2021NAACL-Gao-COIL, Formal2021SPLADE, shen2023lexmae} to learn lexical representations of documents for better matching.
Dense retrieval 
exploits a dual encoder architecture to produce single document representations, 
e.g. ~\cite{gao-2021-condenser,2021SIGIR-Zhan-ADORE-dense,Ren2021RocketQAv2, 
Lin2021tctcolbert, Santhanam2021ColBERTv2,  Wang2022SimLM,  Liu2022RetroMAE}.
This paper is focused on the efficiency optimization to combine the above  two retrieval approaches on a low-cost CPU-only platform.
This  is important in a large-scale  search system  which employs  a multi-stage search architecture, and 
runs partitioned first-stage retrieval in parallel  on a massive number of inexpensive machines.  

%and SPLADE~\cite{Formal2021SPLADE, Formal2021SPLADEV2} has demonstrated the strong relevance performance among these models. 
\comments{
Recent studies have found that combining  sparse and dense retrieval scores  can further boost
retrieval recall and relevance~\cite{Lin2021unicoil,2022LinearInterpolationJimLin,kuzi2020leveraging},
suggest  that both categories  of retrievers tend to capture  different relevant signals. 
These studies  make an assumption that  a search platform has to run two retrievers separately and a dense retriever.
%delivers   its maximum effectiveness, and the impact of compression and IVF clustering is not considered. 
There is an imbalance of computing platform requirements for running  these two retrievers.

dense retrieval typically requires GPU support unless significant  
%We study the use of dense retrieval results to argument sparse retrieval. 
Sparse retrieval with an inverted index has the advantage that a low-cost CPU server can run the online inference  without GPU.
A judicious tradeoff consideration of retrieval  effectiveness and efficiency is critical on  a low-cost CPU-friendly search platform. 
The importance of CPU-friendly search is recognized 
in neural ranking studies~\cite{Yang2021WSDM-BECR,2022WWWforwardIndex,2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
For a large-scale  dataset (e.g. with billions of documents), a practical search system often employs  a multi-stage 
search architecture, which divides the dataset into many partitions so that  a fast first-stage  retrieval 
method  can  search these partitions in parallel.  Such a system  prefers low-cost
CPU-only servers for first-stage retrieval, and both time and memory space complexity of retrieval should be considered 
so that  each server can host as many documents as possible
to reduce the total number of servers to support a large data size and high query traffic. 
%Thus the challenge for retrieval on such an architecture needs to consider both time and space complexity. 
% small search index needs to be as small as possible.
%and the in-memory footprint size of 
%server  needs to host documents in memory as many as possible 
%given a large number  of data partitions involved for parallel search.
%Each server employs multiple CPU cores and is replicated with many copies  for dealing high traffic of  concurrent 
%search requests, and thus 
}

%which run  efficiently  on a single CPU without hardware accelerators  GPU
%which re  retaining strong relevance effectiveness
%%Another development in learned sparse retrieval is that
%sparse retrieval with a learned representation
\comments{
There are several recent efficiency studies advancing the
inverted index implementation for sparse retrieval with learned neural 
representations~\cite{Lassance2022SPLADE-efficient,mallia2022faster,qiao2023optimizing,2023SIGIR-Qiao, 2023SIGIR-SPLADE-pruning}.
which accelerates learned sparse retrieval with BM25-guided traversal or index pruning.

For example, Row 3 of Table~\ref{tab:costbudget} shows the latency, memory space cost, and  MRR@10  of
the latest efficient SPLADE retriever for searching 8.8 million 
MS MARCO passages~\cite{2023SIGIR-Qiao} on a CPU-only server.
% with a single thread on  a 2.25GHz AMD EPYC 7742  CPU server.
Row 2 is performance of a BM25-based retriever after document expansion. 
%There is a tradeoff  in relevance effectiveness if BM25 guidance or threshold-based pruning  is too aggressive.
%and dense retrieval can boost if it does not add much overhead. 
}

As shown in previous literature~\cite{Lin2021unicoil,2022LinearInterpolationJimLin, kuzi2020leveraging}, combining  sparse and dense retrieval scores with linear interpolation
can boost relevance. 
However, none of above studies has considered to exploit the relationship of sparse and dense retrieval results for selective fusion. 
Dense retrieval is expensive, typically requiring GPUs. 
The cost of dense retrieval can be greatly reduced  by using  approximate nearest neighbor (ANN) search with 
partial IVF cluster search~\cite{johnson2019billion, 2021Facebook-DrBoost-Lewis} and proximity graph based navigation~\cite{2020TPAMI-HNSW}.
%2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
However, there is a  relevance tradeoff for a  reduced search cost in these efforts.
Table~\ref{tab:costbudget} shows that  
while RetroMAE~\cite{Liu2022RetroMAE}, a state-of-the-art  dense retriever,  is slow on CPU without compression, the use of
5\% IVF cluster search reduces CPU time substantially  but there is a  7.5\% MRR@10 drop.
The use  of  OPQ quantization further reduces memory space  to 1.2GB but causes an extra 4.6\% MRR@10 drop.

\begin{table}[htbp]
        \centering      
         \resizebox{0.82\columnwidth}{!}{ 
                \begin{tabular}{ r | r  rr}
                        \hline\hline
Dense methods  & Latency & Memory & MRR@10\\ 
\hline
%BM25/DocT5Query & 9.2ms & 1.2GB & 0.261\\  
%SPLADE/HT1 & 31.2ms & 3.9GB & 0.396 \\ 
RetroMAE/Uncompressed & 1677ms & 27.2GB & 0.416 \\ 
%RetroMAE/IVF SimLM perhaps 3\% & 49.6ms  & 27.2GB & 0.389 \\ 
RetroMAE/IVF 5\% & 107ms  & 27.2GB & 0.387 \\ 
%SimLM /OPQ             & 225-1579ms & 0.57-2.3GB & $<$ 40.2 \\
RetroMAE /IVF 5\% OPQ  & 38ms & 1.2GB  & 0.370 \\ 
%RetroMAE SimLM? /IVF  OPQ  & 38-339ms & 1.2-2.3GB  & 0.37-0.401\\ 
                        \hline\hline
\end{tabular}
}
\caption{Latency, relevance, and space  tradeoff  in a dense model for passage retrieval with MS MARCO Dev set}
 \vspace*{-7mm}
\label{tab:costbudget}
\end{table}


%Quantization~\cite{2021CIKM-JPQ-Zhan,  2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ} is another orthorgonal cost reduction technique.

LADR~\cite{2023SIGIR-LADR}, as a follow-up study of  GAR~\cite{2022CIKM-MacAvaneyGraphReRank},
has studied partial dense retrieval by  
taking  the results of a sparse retriever as a seed to select embeddings
%That takes an approach of augmenting sparse retrieval results using graph-based navigation based on
based on a document-to-document proximity graph. This strategy  follows  the previous graph-based ANN approach~\cite{2020TPAMI-HNSW,2021KDDgraphANN}. 
While such a graph navigation approach has demonstrated its  efficiency  with a time budget, 
use  of a document-wise similarity graph adds a significant online space requirement  on a low-cost computing platform. 
%document-level  proximity graph  construction is  expensive for a large dataset during offline processing. 
For example, the proximity graph  can take an extra 4.3GB memory space~\cite{2023SIGIR-LADR} for an 8.8M  MS MARCO passage dataset.
% to keep top 128 top neighbors per document.  
Another weakness is that like HSNW, it assumes proximity graphs and dense vectors are  available from memory. 
% PARKER's suggestion:
For large datasets or higher-dimension embedding vectors, some or all of the embeddings and proximity graphs will have to be stored on disk,
especially when such  applications desire uncompressed embeddings for  a higher relevance effectiveness. 
%For example, recent RepLLaMA model~\cite{ma2023finetuning}, based on LLaMA-2~\cite{touvron2023llama}, requires 145GB storage space for 
%MARCO passage embeddings of dimension 4096.
% these 
Further, the random access of dense embeddings and/or graph nodes, as necessitated by document-level proximity graph navigation, can incur substantial 
fine-grained I/O overhead.
% to replace: 
%When the dense embeddings or its proximity graph of a large dataset cannot fit into memory, this approach that access can suffer 
%large random fine-grained I/O access overhead. 
%Nevertheless, random access of dense embeddings and/or graph nodes, as necessitated by document-level proximity graph navigation, can incur substantial
%fine-grained I/O overhead.  

%In contrast, cluster-based structuring captures  similar documents from  statically-formed  groups and enables faster  block-level I/O.
%DiskANN  and its variant study on-disk graph navigation for ANN search~\cite{NEURIPS2019_DiskANN,2023Web-Filtered-DiskANN},
%and SPANN is an effort on cluster-based ANN search. They are targeted for a stand-alone and geneal ANN problem while our 
%work takes an advange of sparse retrieval for better relevance  in the context of text document search.

%None of above studies has considered to exploit the relationship  of sparse and dense retrieval results for selective fusion. 

\comments{
That is true also with the  navigation of  a  proximity graph based on inter-document similarity distances called HNSW~\cite{2020TPAMI-HNSW}. 
The proximity graph approach to guide dense retrieval is revisited recently in GAR~\cite{2022CIKM-MacAvaneyGraphReRank}, which is furthered improved by
%LADR Kulkarni  et al.~\cite{2023SIGIR-LADR} improves HNSW.
LADR~\cite{2023SIGIR-LADR}.
%~\cite{2022CIKM-MacAvaneyGraphReRank,2023SIGIR-LADR}. 
The weakness of  the  proximity graph approach is that its graph  construction requires a quadratic computing complexity, which is expensive
for a large dataset and the online hosting of such a graph also adds a significant space requirement  on a low-cost
computing platform. For example, LADR takes an extra 4.3GB memory space for 8.8M  passages in the MS MARCO dataset to keep top 128 
top neighbors per document. 
%Similarily HNSW also incurs a high space cost for graph connections.  
%In comparison, cluster-based selective dense retrieval can achieve in a comparable time complexity
%while adding  insignificant extra  space  overhead.
}



  
%with a latency controled within 4 to 8 milliseconds on a single CPU, but with a significant tradeoff in relevance effectiveness.
%For example, MRR@10 for MS MARCO Dev set drops from RetroMAE has dropped from  0.416 to 0.356.
%This paper does not impose 4-8 millisecond latency, but rather looks for a solution that can leverage both dense and sparse retrieval
%and relax the latency constraint in some degree while maximizing its relevance effectiveness as much possible.
%a range below or around  100 milliseconds 

%The response time  for such a system for an interactive service needs to be fast enough a
%and thus search needs to be completed within a few hundred milliseconds. 

%which only requires triggering of dense embedding  computation for a relaively small subset of documents.
%The proposed scheme called cluster-based selective dense  retrieval


This paper proposes a lightweight approach called CluSD to 
conduct Cluster-based Selective Dense retrieval at a low CPU-time and space cost after sparse retrieval. 
%and  combine its results  with  sparse retrieval. 
%It exploits the relationship  of sparse and dense retrieval results to conduct  selective fusion. 
%To accomplish that, 
CluSD limits query-document similarity computations through a two-stage cluster selection algorithm via an LSTM model, which  
exploits inter-cluster distances and the overlapping degree between top sparse retrieval results and dense clusters.
%CluSD leverages IVF clustering and does not require an extra document similarity graph. 
%and then make a decision to determine which document clusters should be selected  to conduct dense retrieval computation.
%The extra memory space overhead required to assist CluSD is negligible, and it  works well when embedding vectors are highly compressed.
%  and  the extra memory required for hosting dense embeddings can be limited  after compression. 
When dense clusters are not available in memory, CluSD selects and loads a limited number of clusters with efficient disk block I/O.
Thus, it can handle a large dataset with high-dimension embeddings that cannot fit in memory, with less I/O overhead compared to a
graph-based ANN approach.  % TODO: second comma? split into two sentences? come back later Parker



%0.419 by RocketQAv2~\cite{Ren2021RocketQAv2}, 
%which are the two latest state-of-the-art retrieval-reranker pipelines using cross-encoder based rerankers.
%Re-ranking in  recent dense retrieval work SimLM~\cite{Wang2022SimLM} has  used an expensive cross-encoder to
%achieve impressive MRR score 0.437 
%Re-ranking in RocketQAv2~\cite{Ren2021RocketQAv2} achieves 0.419 with a similar strategy.  






%0.419 by RocketQAv2~\cite{Ren2021RocketQAv2}, 
%which are the two latest state-of-the-art retrieval-reranker pipelines using cross-encoder based rerankers.
%Re-ranking in  recent dense retrieval work SimLM~\cite{Wang2022SimLM} has  used an expensive cross-encoder to
%achieve impressive MRR score 0.437 
%Re-ranking in RocketQAv2~\cite{Ren2021RocketQAv2} achieves 0.419 with a similar strategy.  







%0.419 by RocketQAv2~\cite{Ren2021RocketQAv2}, 
%which are the two latest state-of-the-art retrieval-reranker pipelines using cross-encoder based rerankers.
%Re-ranking in  recent dense retrieval work SimLM~\cite{Wang2022SimLM} has  used an expensive cross-encoder to
%achieve impressive MRR score 0.437 
%Re-ranking in RocketQAv2~\cite{Ren2021RocketQAv2} achieves 0.419 with a similar strategy.  





This paper evaluates  the effectiveness of CluSD  under time and space constraints on a CPU-only server, 
using the standard text retrieval benchmarks (MS MARCO and BEIR  datasets).
We compare against other baseline methods, including in a case in which the dataset does not fit into memory.
Our goal is to show that CluSD reaches state-of-the-art relevance levels at a much lower space and/or time cost.
We also compare our method to DiskANN~\cite{NEURIPS2019_DiskANN} and SPANN~\cite{chen2021spann},
two general-purpose on-disk ANN search algorithms that are not designed to leverage sparse retrieval.
%Our evaluation also compares DiskANN~\cite{NEURIPS2019_DiskANN,2023Web-Filtered-DiskANN} and SPANN~\cite{chen2021spann}
%that conduct on-disk  ANN search, and these studies are targeted for general ANN search without considering the leverage of
%sparse retrieval.
%and  shows that CluSD can effectively identify a small number of document clusters to 
%for  a stronger relevance  even though such a sparse retriever is fast with a relevance tradeoff. 
 
%provides a flexibility and reduces  the relevance requirement of sparse retrieval.
%Namely protentially we can choose a relatively fast sparse retrival with the slightly lower accuracy/recall,
%and  let dense retrivsal make up the loss. Our design needs to  adapt to  sparse retrieval quality and plans

%CSDR in improving the effectiveness of sparse retrieval with limited dense  retrieval
%traversal for low-cost search.  Our emprial findings suggest that SRF  can consistently outperform other baselines on a single CPU server 
%without GPUs 
% and achieve a strong tradeoff of effectiveness and efficiency compared to an exhausitve dense retrieval search.


%from pretrained language models to provide effective semantic text matching between a query and a document.



==> kddmethod.tex <==
%\section{SRF with Query-Specific Cluster Skipping }
%\section{CluSD: Selective Dense Retrieval}

  
%\section{Selective Dense Cluster Retrieval}
%%%%%%%%%\label{sec:clusd}

\comments{
It is common practice to interpolate the results from a sparse system and a dense system. We propose two directions to improve the latency of such system by avoiding the unnecessary dense evaluation on query level and per query level. We envision a hybrid system where sparse retrieval runs first and partial query and documents are evaluated by the dense retrieval system. 

The proposed CluSD method contains two components  during runtime inference to 
decide if  dense retrieval augmentation  can be skipped for a query and which  top dense document clusters should be selected  during supplemental retrieval.
}

%Per-query inference latency depends on the number of document evaluated and how per query-document evaluate is approximated. We do not touch per-query-document approximation in this paper and focus on reducing the number of documents evaluated. We cluster document using kmeans as IVF and would like to intelligently select a few most promising clusters to retrieve candidate results. 
\comments{
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.9]{lstm.png}
    \caption{LSTM prediction for each query}
    \label{fig:lstm}
\end{figure}
}
\comments{
As discussed earlier, documents with embedding vectors are clustered based on their similarity to the cluster centroids. 
Our experiments take an advantage of the FAISS library which  provides such a support such as k-mean clustering.
Once a query is determined by CluSD to trigger  partial dense retrieval that selects and visits a subset of dense clusters. 
% online inference  will  visit the dense clusters one by one in
%an incresing order of   their centroid distance to the input query.
%A decision procedure is invoked to decide if a cluster to be visited should be skipped or not. 
Our objective is to examine the features of each cluster and  incrementally decide if this cluster should  be visited or not.
This section will first describe the overall flow of CluSD in online inference for selective fusion of sparse and dense retrieval,
 then present an LSTM-based  cluster selection algorithm. 
}


\subsection{ Online inference}
\label{sect:online}
\begin{figure}[htbp]
    \includegraphics[scale=0.79]{sparse_dense_flow_lout.drawio.pdf}
    \caption{The flow of cluster-based selective dense retrieval}  
 \vspace*{-5mm}
    \label{fig:flow}

\end{figure}





%Step 3. Call the LSTM selection (Section 4.1)  to choose a small number of dense clusters. That is about 25 in our MS MARCO evaluation.





The online inference algorithm of CluSD has the following steps:

\textbf{Step 1}:   Conduct sparse retrieval to obtain top-$k$ results.

%\item Conduct the query filter  to determine if the cluster-based dense retrieval is necessary.If needed, 
%Step 2:  Sort clusters based on the overlap degree of dense clusters and top sparse retrieval results and their  centroid-to-query  distances.

\textbf{Step 2}:  Conduct a two-stage selection process. 
Stage I selects the top-$n$ clusters from  the given $N$ dense embedding clusters, discussed in detail in Section~\ref{sect:stage1}.
%The  key  features collected include the overlap degree of dense clusters and top sparse retrieval results and their centroid-to-query distances.
Stage II  applies an LSTM model to the $n$ top clusters
to choose  a limited number of dense clusters to evaluate, discussed in Section~\ref{sect:lstm}. 

\textbf{Step 3}: Expand the top-$k$ sparse retrieval results to include the documents vectors of these dense clusters and
merge their sparse and dense scores with linear interpolation.  

%During the above linear interpolation, only top $k$ of sparese retrieval contains a lexical score,
%and thus we  impute the lexical scores of other documents expanded by cluster-based selective dense retrieval 
%as the bottom document score in the top $k$ sparse retrieval list scalled by a factor. We use 0.95 in our evaluation.
\comments{
Notice that  the two ranked lists from two retrievers are usually not fully overlapped and  some documents only exist in one list. While
different  treatments on these documents affect fusion performance,
we resort  to imputing the score of such a document using  the top $k+1$ score   in the missed rank list scaled by 
a factor.
%While there are options to We consider a few options
For example,  we  impute the lexical scores of new documents added  by dense retrieval
using  the scaled lexical score of  top $(k+1)$ in the sparse retrieval list. We use scale $0.95$  in our evaluation.
}
%\item Remove the documents when they only exist in one ranked list
%    \item  Take the document and compute the score for only one ranked list

%When we have access to a relatively strong sparse retrieval system and a dense retrieval system, it is feasible to selectively choose queries that requires evaluation of both systems. We hypothesize that the sparse system is economical and we can afford to run it for every query. The problem boils down to dynamically select queries to evaluate by dense retrieval.

{\bf Time  and space  cost for CluSD.} 
%We only consider the cost of  online partial dense retrieval. 
The embedding space is $O(D)$  for a corpus with $D$ vectors.
For MS MARCO, this  cost is around 27GB without compression. Quantization can reduce the total size to about  0.5GB  to 1GB, depending on codebook parameters.
Then this cost becomes a fraction of sparse retrieval index cost.  
Excluding embeddings, the extra space overhead for CluSD is to maintain  the similarity among centroids of $N$ clusters.
We only maintain top $m$ cluster neighbors for each cluster in terms of their centroid similarity. 
For our evaluation, $m=128$ and this reduces the extra space overhead as $O(N)$, which
is negligible compared  to the embedding space with $N << D$. 
For example,  with $N=8192$,  the inter-cluster graph for MS MARCO passages takes about 5MB with quantization.
%In our evaluation, %we use  $N=8192$ or  $4096$.
%the inter-cluster similar graph for MS MARCO passages with $N=8192$ takes about 32MB with quantization.

Excluding sparse retrieval cost, the time  cost of 
CluSD is dominated by the cost of cluster selection and  dense similarity computation of selected dense clusters.
The former is about $O(n)$ while the latter is
proportional to the number of clusters selected, which is capped by $O(\frac{D}{N} n)$. 
In  our evaluation of MS MARCO and BEIR, $n$ is chosen to be 32, and
the actual number of clusters selected and visited is about 22.3.
%Given the short time added by the pruned LSTM model, 
Thus, the overall latency overhead introduced by CluSD is fairly small. 


\subsection{ Stage I: Selection of  top $n$ candidate clusters} 
\label{sect:stage1}
\comments{
As discussed earlier,  we control 
the input length  of the above  LSTM model  to be  $n$  as 
the number of top candidates clusters to be examined, and then the inference 
}

Given  $N$ clusters grouped using dense document embeddings, 
we devise a strategy below to conduct a preliminary selection that
prunes low-scoring clusters that contain  only less relevant documents.
%prunes low-scoring clusters that may not provide a meaningful boosting of relevance quality,
%and  choose  top $n$ candidate clusters for Stage II for further refinement.
The two-stage approach is motivated by the fact that the LSTM model used in the second stage is time consuming to examine all clusters. 
%Thus, we truncate the sequence of clusters to maximum length $n$ and then take a sequence of top $n$ clusters as the input to this LSTM. 
Thus, we choose the top-$n$ candidate clusters first.
\comments{
There are  $n$ nodes corresponding to these clusters in the LSTM model.
We will discuss how to truncate with a prioritization shortly below.
%Because this decision procedure uses the document scoring information  of each cluster visted 
}
\comments{
Table ~\ref{tab:LSTMclustertime} shows that the number of clusters to be examined
varies from 32 to 512, the LSTM inference time increases from  2.8ms to 33.9ms.
As we would like to make a quick decision given the overall  time budget,
we devise another strategy to prune clusters that may not provide a meaningful boosting
of relevance quality. 

% dependent on the length of the sequence input. 

\begin{table}[h]
	\centering
		\resizebox{0.68\columnwidth}{!}{ 
%		\begin{small}
		\begin{tabular}{r | rrrrr}
			\hline\hline
			  \#Clusters examined & 512 & 256 & 128 & 64 & 32 \\
\hline
            Time (ms) & 33.9 & 16.2 & 6.2 & 3.8 & 2.8\\
                \hline\hline
		\end{tabular}
%		\end{small}
	}
	\caption{LSTM inference time with different input lengths.}
	\label{tab:LSTMclustertime}
 \vspace{-4mm} 
\end{table}

\comments{
\begin{figure}[htbp]

    \includegraphics[scale=0.27]{dist.pdf}
    \caption{Distribution of Good Documents }
    \label{fig:dist}
%\vspace{-1em} 
\end{figure}
}
}

To prioritize clusters, one idea is to adopt their query-centroid distance used
in IVF cluster selection.  We find this does not work well for CluSD.
For example, if we rank clusters based on the query-centroid distance for MS MARCO passages, 
around 10\% of top-10 dense results reside in clusters ranked beyond the 175th cluster, which means we would have to select 175 clusters in order to recover 90\% of top-10 documents. 
  
\comments{
Table~\ref{tab:dist} shows the distribution of top 10 documents from the full dense retrieval  
in embedding clusters under the different query percentile when searching an MS MARCO passage dataset using queries from its  Dev set. 
Row 2 of Table~\ref{tab:dist} shows the number of top clusters needed to cover  top 10 
documents from the full dense retrieval  when clusters are sorted by sorted by  the query-centroid distance.
This row shows that to cover top 10 dense results, $n$ needs  to be larger than 175.
%On the other hand, Row 2 is  the number of lusters decided by the LSTM to visit  under the different query percentiles. 
%At most  66 clusters are  selected  by the LSTM model for all queries.
%We further propose to skip unnecessary clusters. 
\begin{table}[h]
 \vspace*{-1mm}
	\centering
		\resizebox{0.78\columnwidth}{!}{ 
%		\begin{small}
		\begin{tabular}{r |r  r r r r}
			\hline\hline
			  Query percentile & 10\% & 50\% & 75\% & 90\% & 95\% \\
            \hline
%            \#clusters selected by  LSTM & 1 & 4 & 14 & 40 & 66\\
            %Relevant doc coverage & 1 & 2 & 7 & 29 & 69\\
             Top 10 dense result coverage & 1 & 6 & 25 & 92 & 175\\
                \hline\hline
		\end{tabular}
%		\end{small}
	}
	\caption{ Distribution of  top 10 dense results in sorted clusters 
% \% of Good Documents Among Clusters Sorted by Query-Centroid Distance
}
 \vspace*{-5mm}
	\label{tab:dist}
\end{table}
}


%provides an explanation.  evidence on the effectivness of the above LSTM model.
%After searching an MS MARCO passage dataset using queries from the MAMARCO dev set, 
%under the different query percentile shown in Row 2 is  the number of clusters decided by the LSTM to visit.
%Row 3 is  the number of clusters needed to 
%For a lot of queries, the top 5 or even top 10 clusters do not contain enough information, for example, around 10\% of queries need more than 92 top clusters to recover the top results from the full dense retrieval. It demonstrates the necessity of doing cluster selection and skipping.  
%On the other hand, there is a reasonable distribution resemblance between  Row 2 and  Row 3, which shows the LSTM model provides a reasonable guidance on where relevance results are.
%%While it does not exactly follow the distribution of top 10 results of sparse retrieval, the feature 
%From  Table~\ref{tab:dist}, we observe that
%the distribution of top 10 results from a sparse are contained is not necessarily concentrated in the top  clusters.
%With the above design consideration,  we propose to use the following strategy to 
%sort the candidate clusters based their feature vectors from Group  (3).


Our method   for the preliminary selection at this stage is to rely on
the degree of overlap between dense clusters and the top sparse retrieval results. 
Specifically, we divide $k$ top sparse retrieval results into $v$ top sparse result bins denoted $B_1, \cdots, B_v$,  
as depicted in Figure~\ref{fig:LSTMfeaturegroup}(b).
We  assign each embedding cluster $C_i$ with a priority vector $(P(C_i, B_1), \cdots, P(C_i, B_v))$ where
\[
P(C_i, B_j)=  |C_i  \cap  B_j|.
\]
Namely, $P(C_i, B_j)$ is the number of documents in top sparse bin $B_j$ included in cluster $C_i$.
A larger $P(C_i, B_j)$ value indicates a higher priority for $C_i$ with respect to sparse result position bin $B_j$.
In our evaluation with  retrieval depth $k = 1000$ for the MS MARCO and BEIR datasets,
we use $v=6$ result bins, divided into the top-10 results, top 11-25, top 26-50, top 51-100, top 101-200, top 201-500, and top 501 to $k$ documents.
%top $k$ sparse results are divided into $v$ result bins where $v=6$, and these bins are top 10, top 11 to 25,  and so on.
%top 26-50, top 51-100, top 101-200, top 201-top 500, and 
%top 501 to k documents.  
    %\item $\{  AvgScore (c_i  \cap  B_j)    \}^{6}_{j=1} $: 
% bin 
%top 10/25/50/100/200/500/1000 documents  in the sparse retrival results.

Then, we sort clusters based on the lexicographic ordering of cluster priority vectors $(P(C_i, B_1), \cdots, P(C_i, B_v))$.
%$(P_1, \cdots, P_v)$. A higher value for each dimension entry represents a higher priority and is prefered.
If there is a tie between two clusters, then we rank them by their centroid distance to the query.
%We first use a simple heuristic to reorder the clusters, refered as Top K heuristic. 
%We order the clusters based the six features then 
%followed by q-c-orders. 
%Then, the  top $n$ ranked candidate cluster list is used as the input sequence to the LSTM model. 
The top-$n$ ranked candidate clusters will be  the  input for the LSTM model described below.
%We will stop the LSTM computation of  this list
%after visiting $\tau$ clusters and when the predicted $f(c_i)$  values of a few consecutive clusters are all below a threshold. 
%For our evaluation in MS MARCO and BEIR datasets, $\tau=20$. 

\comments{
Section~\ref{sect:evalLSTM} studies the effectiveness of features used in Stage II, and explains our choice of features for preliminary cluster selection. 
For the choice of $n$,
our evaluation finds  that a relatively small number of candidate clusters, such as $n=32$, yields competitive results  for our
evaluations when $k=1000$.
%As a result, the LSTM computation for cluster selection can be completed within  1.8 milliseconds. 
%The number of clusters selected varies from a few to 20 on average, which yields a quick argumentation with dense cluster results.
%Features marked with Hexgos 1 and 4 are used for a boosting tree to make a decision if cluster selection should be triggered or not.

}
\subsection{Stage II: Selection with LSTM}
\label{sect:lstm}

%{\bf LSTM design.}

\begin{figure}[htbp]
    \includegraphics[scale=0.9]{dense_separse_feature_lout.drawio.pdf}
    \vspace*{-1mm}
    \caption{Illustration of CluSD and its features.}
    \label{fig:features}
%     \vspace*{-5mm}
\end{figure}


\comments{
The LSTM model outputs 1 for each cluster node if this cluster should be visited to perform the corresponding dense retrieval.
The goal of this procedure  is to visit  dense clusters as few as possible while still delivering a competitive fusion performance.
The number of predicted clusters are different across queries and the overall budget is controlled by the prediction threshold.
}
%  a few clusters as possible to recover the top results from the original dense retrieval. 
%The label of each query-cluster is 1 when the cluster contains the top k results of the query in the exact full search of dense retrieval.  
%The input is the a sequence of cluster nodes in the order of the centroid-query distance. 
%The feature of each input include: statistics on query-centroid distance, centroid-to-centroid distances, distribution of sparse top results across clusters. 
%The model will predict for each query which clusters to choose. 
%The input features of our proposed LSTM model are listed below.
%These clusters are sorted by the the similarity distance of the given query with the  centroid of each cluster.

To select which dense clusters we visit, we adopt a simple LSTM model~\cite{hochreiter1997long}
which takes a sequence of clusters as input along with their features. 
The time complexity of the LSTM model is limited by $O(n)$,
where the $n$ top clusters are  given from  Stage I.
%We denote $n$ as the  input length  to our LSTM  throughout the rest of this paper.

The LSTM sequentially visits each cluster, denoted $C_1$ to $C_{n}$. 
For each cluster $C_i$, the LSTM predicts a score $f(C_i)$ such that $0\leq f(C_i) \leq 1$.
If $f(C_i) \ge \Theta$, where $\Theta$ is a set prediction threshold, then cluster  $C_i$ should be visited. 
$\Theta$ controls the tradeoff between efficiency and relevance; in practice, $\Theta$ can be tuned based on the overall latency requirement.
The evaluation in Section~\ref{sect:threshold} demonstrates the impact of varying this threshold on the number of clusters selected.

%In practice, the strictness on selecting a cluster to evaluate is controlled by $\Theta$ and it can be determined based on the overall latency requirement. 

\comments{
When the dense vectors of all documents are grouped into $N$ clusters, 
we limit our cluster search scope to top $n$ clusters in terms of query and cluster centroid similarities. 
we limit $n=128$ in our evaluation out of 1000 clusters.
%Query-specific information derived from  dense clusters:
}

As depicted in Figure~\ref{fig:features}, the feature input vector for the current cluster  $C_i$ for the above LSTM computation to produce $f(C_i)$
%$f(q, c_i)$  
is composed of the following three groups of features:


\comments{
\[ sim(q,c_i),   
\{ AvgDist(sim(c_i, c_l) \mbox{ for } c_l \in A_j) \}^u_{j=1}, 
\]
\[ 
     \{  |c_i  \cap  B_j|    \}^{v}_{j=1},  
\{  AvgScore (c_i  \cap  B_j)    \}^{v}_{j=1}. 
\] 
}
%\begin{enumerate}[leftmargin=*]
%KDD style does not recognize leftmargin
\begin{itemize}
\item \textbf{Query-cluster similarity:} $sim(q,c_i)$.
The similarity distance of this query $q$ with the centroid $c_i$ of cluster $C_i$.  
%\item $sim(q,c_i)$: The similarity distance of this query $q$ with the centroid $c_i$ of cluster $C_i$.  
%\item  $\{ sim(c_i, c_j) \}^{n-1}_{j=0}$: The distance vector between the centroid $c_i$ of cluster $C_i$ to  all other clusters.
%the top  clusters that have been visited (or skipped).  We limit this number as $K=128$.
%other top k centroids for this query (k=128)??
  

%\item  $\{ AvgDist(sim(c_i, c_l)) \mbox{ for } c_l \in A_j \}^u_{j=1}$: 

\item \textbf{Inter-cluster similarity:} $AvgDist(C_i, Aj)$ for $1 \leq j \le u$.

%\item  $AvgDist(C_i, Aj)$ for $1 \leq j \le u$.
As depicted in   Figure~\ref{fig:LSTMfeaturegroup}(a),
given the $n$ sorted clusters derived from Stage I, we uniformly partition  these $n$ consecutive  clusters into $u$ consecutive cluster bins:
$\{ A_1, A_2, \cdots, A_u\}$. Then we define
\[
AvgDist(C_i, Aj) = \frac{1}{|A_j|} \sum_{ c_l \in A_j}
 sim(c_i, c_l) 
\]
where  $c_l$ is the centroid representing cluster $C_l$ in bin $A_j$.
The above formula computes the mean distance between centroid $c_i$ and the centroid of each cluster within  Bin $A_j$.


%These six bins  are formed by partitioning all clusters into consecutive position bins.
%For example, $A_1$ contains clusters from Postions  1 to 5, Positions 6-10, 
%$A_2$  contains clusters from Postions  6 to 10, and so on.   Bin $A_6$ contains the rest of uncovered clusters.  
%After all the $N$ centroids are ordered based on a criterion discussed shortly, we partition the sequence of sorted clusters into $u$ consecutive 
%cluster bins.

The purpose of this feature group is to capture the distances of a cluster to previously examined clusters and unexamined clusters 
following the LSTM flow. 
When the mean distance  between cluster $c_i$  and clusters in a previously-examined  bin is close, if  
many clusters in that bin have been selected, cluster 
$c_i$ may have a good  chance to  be selected.
In our evaluation with MS MARCO and BEIR datasets, we found that $u=6$ is appropriate.
% these 6 cluster bins respectively contain clusters in Positions  1-5, Positions 6-10, Positions 11-20, Positions 21-50, Positions 51-100, and the rest of N clusters. 
%Since the clusters are processed from a lower position to a higher position one by  one,
%these features represent the distance to the groups 
As discussed earlier in Section~\ref{sect:online}, to reduce the extra space cost, 
we only maintain top-$m$ cluster neighbors of each cluster where $m$ is not large  (128 in our evaluation).
    
%\item $ \{  |c_i  \cap  B_j|    \}^{v}_{j=1} $ and $\{  AvgScore (c_i  \cap  B_j)    \}^{v}_{j=1} $: 

\item \textbf{Cluster overlap:} $P(C_i, B_j)$ and $Q(C_i,   B_j)$     for $1 \leq j \le v$.
%\item $P(C_i, B_j)$ and $Q(C_i,   B_j)$     for $1 \leq j \le v$.

As shown in   Figure~\ref{fig:LSTMfeaturegroup}(b),
this group of features captures the position-weighted and score-weighted overlap degree of this embedding cluster $C_i$ with the top sparse results.
Stage I in Section~\ref{sect:stage1} divided the top-$k$ sparse retrieval results into $v$ position bins
$B_1, \cdots B_v$ and defined   $P (C_i, B_j)$ as  the count-based overlap measure.
Now, we define a score-weighted overlap degree $Q (C_i,   B_j)$     
as the average sparse rank score of documents that  are in both $C_i$ and sparse position bin $B_j$.  
Namely,
\[
Q (C_i,   B_j) = \frac{ \sum_{d \in C_i \cap B_j} SparseRankScore(d)} { |C_i  \cap  B_j|}.    
\]


%With a high score from this feature, a cluster that contains many top sparse results may be selected.
Clusters with high $Q$ scores for the top bins contain many top sparse results and may be selected.

%In our evaluation with  retrieval depth $k = 1000$ for MS MARCO and BEIR datasets,
%top $k$ sparse results are divided into $v$ bins where $v=6$, and 
%these bints are top 10, top 11 to 25, top 26-50, top 51-100, top 101-200, top 201-top 500, and 
%top 501 to k documents.  

    %\item $\{  AvgScore (c_i  \cap  B_j)    \}^{6}_{j=1} $: 

% bin 
%top 10/25/50/100/200/500/1000 documents  in the sparse retrival results.

\end{itemize}

In total, we extract $1+u+2v$ features for each top-$n$ cluster.



\begin{figure}[htbp]
    \includegraphics[scale=0.85]{LSTM\_feature.drawio.pdf}
    \vspace*{-3mm}
    \caption{Cluster distance   and result  overlap features } 
\vspace*{-1mm}
    \label{fig:LSTMfeaturegroup}
\end{figure}

%Section~\ref{sect:evaluation} provides more details on the effectiveness 
 

\comments{
\subsection{Query filtering}
%When computing the embedding of each query token or the whole  original query, we use 
%the denser retriever's encoder. 


We also exploit the possibility to skip dense retrieval completely.
Modifying the above LSTM-based decision mechanism does not yield a satisfactory result.
We sort to add a classifier with  boosted decision trees with supervised learning
to make an earlier  determination before triggering the LSTM computation.
}
\comments{

a query needs an argumentation from dense retrieval 
%A challenge is to identify features and infer based on such features with supervised learning.
Given that sparse retrieval is conducted first,
our idea is to predict the quality of sparse retrieval and its relative strength  compared to unexecuted
dense retrieval based on quality of query token expansion by the sparse model,
the statistical behavior of  sparse retrieval results, and
the relationship between dense document embedding summary and sparse retrieval scoring structure.

}


\comments{
\begin{table}[ht]       
    \centering          
%    \resizebox{1.05\columnwidth}{!}{

\begin{small}                        

    \begin{tabular}{l |l}
        \hline
    Query    & "how long nyquil kicks in"\\
    \hline
 Query Expanded&["in", 36],  ["time", 74], ["years", 71], ["long", 97], \\
 & ["total", 60],\textcolor{red}{["move", 23]}, ["effect", 22], \textcolor{red}{["weapon", 21]}, \\
 & \textcolor{red}{["jump", 24]}, ["kick", 100], ["ny", 111], ["timing", 34], \\
 & ["kicks", 76], ["\#\#quil", 139]\\
    \hline  
Relevance Doc &["\#\#quil", 410.1], ["ny", 301.0], ["long", 216.7], \\
& ["time", 134.7], ["years", 131.5], ["total", 87.4],\\
& ["effect", 34.4], ["timing", 17.4]\\
\hline
Top 5 Doc & ["\#\#quil", 392.6], ["ny", 295.7], ["kick", 236.1], \\
& ["long", 198.3], ["time", 141.2], ["years", 116.9], \\ 
& ["kicks", 101.8], ["total", 86.3],\\
& ["in", 35.3], ["effect", 24.1], ["timing", 23.6],\\
& \textcolor{red}{["jump", 10.0], ["move", 6.0]}\\
        \hline
    \end{tabular}
\end{small}                        
%}     

\caption{An example of weak query expansion in SPLADE} 
\label{tab:queryencoder}
\end{table} 
}

\comments{
\begin{table*}[ht]       
    \centering          
%    \resizebox{1.05\columnwidth}{!}{

\begin{small}                        

    \begin{tabular}{l  l l}
        \hline\hline
    Query   &  \multicolumn{2}{l}{ "why do we push others away"}\\
    \cline{2-3}
&  \multicolumn{2}{l}{('push', 105), ('away', 104), ('because', 97), ('others', 94), ('people', 44), ('why', 44), ('purpose', 43), ('cause', 42), (',', 40), ('we', 38),} \\
&\multicolumn{2}{l}{ ('other', 38), ('effect', 33), ('them', 29), \boldred{('responsibility', 28),} ('help', 20), \boldred{('move', 19), ('severe', 17),}  ('step', 17), ('do', 16),...}\\
%& & ('things', 15)， ('fear', 15), ('method', 10), ('to', 6), ('language', 5), ('anger', 5), ('when', 2), ('feeling', 2), ('\#\#ness', 1), ('dangerous', 1)]\\
    \hline  \hline
   Doc Relevant? & \ rank & Text and Expanded Tokens \\
\hline
\comments{
Yes & 17 & From a psychological standpoint, pushing away the people you love the most is a very basic and common, defense mechanism.\\
&& As the relationship develops, people become inundated with their own fears and insecurities that they will not be accepted\\
&& and therefore hurt by their loved one.\\
\cline{3-3}
& & [('push', 198), ('away', 196), ('fear', 127), ('people', 104), ('effect', 81), ('because', 70), ('severe', 67), (',', 61), ('method', 61),
\\
& &  ('when', 59), ('anger', 58), ('dangerous', 55), ('feeling', 53), ('purpose', 53), ('responsibility', 53), ('move', 44), ('cause', 43),... \\
%& & ('them', 37), ('things', 31), ('\#\#ness', 27), ('step', 23), ('why', 13), ('help', 9), ('to', 3), ('do', 1), ('language', 0)]\\
\specialrule{.1em}{.05em}{.05em} 
}
No & 10 & Different types of push factors can be seen further below. A push factor is a flaw or distress that drives a person away from \\
&&  a certain place. A pull factor is something concerning the country to which a person migrates. It is generally a benefit that  \\
&&attracts people to  a certain place. Push and pull factors are usually considered as north and south poles on a magnet.\\
\cline{3-3}
&& [('push', 283), ('away', 162), \boldred{('move', 80),} \boldred{('severe', 74)}, ('people', 70), ('because', 68), ('effect', 58), ('cause', 44), ('purpose', 43),\\
& & \boldred{('responsibility', 41),} (',', 36), ('method', 35), ('\#\#ness', 33), ('step', 23), ('them', 22), ('to', 18), ('when', 13), ...\\ 
%& &  ('things', 11), ('anger', 9), ('dangerous', 8), ('fear', 3), ('do', 0)]\\
\specialrule{.1em}{.05em}{.05em} 
No & 8& Most of the universe is rushing away from us. It\textbackslash{}'s not that we\textbackslash{}'re particularly repellent; it\textbackslash{}'s just that the universe is\\
&&  expanding, pushing most other galaxies away. Light from distant galaxies travels toward us through this \\
&& expanding space, which stretches their light to longer, or redder, wavelengths.\\
\cline{3-3}
&& [('away', 184), ('push', 158), ('other', 111), \boldred{('move', 103)}, ('we', 101), ('effect', 83), (',', 73), ('because', 66), ('method', 53),\\
&&  ('others', 39), ('cause', 39), ('severe', 39), ('them', 36), ('do', 29), ('things', 29), ('dangerous', 29), ('feeling', 28), ... \\
% & & ('when', 27), ('help', 19), ('purpose', 13), ('to', 4), ('why', 2)]\\
         \hline\hline
    \end{tabular}
\end{small}                        
%}     

\caption{An example of weak SPLADE query expansion that boosts  irrelevant documents  } 
\label{tab:queryencoder}
\end{table*} 

Our consideration 
%is that the necessity of invoking a dense retrieval model after running a sparse model depends on 
%\begin{enumerate}
%the relative strength of results scored by this sparse retriever. If a
    is that  if a chosen
sparse retriever has  well-performed, the benefit of addition of dense scoring  is limited. 
Notice that a learned neural sparse retriever expands the original query with a transformer-based encoder
We found that the quality of query encoding with expansion in SPLADE impacts the quality of sparse retrieval. 
%and we form features using both the original query  and the expanded query.
When  there is a low similarity value  between the original query and the tokens of 
its expanded  query, the confidence for  strong sparse retrieval can be low.
Table~\ref{tab:queryencoder} gives such an example and lists an original query and its expanded query tokens
sorted by token weights.  Expanded query words  in red color
not highly relevant to the original query and they are weighted high in two irrelevant documents, which boosts their ranking.  
Thus    excessive presence of un-similar  query tokens  after expansion  can misrank irrelevant documents. 
Another consideration is that the alignment of sparse retrieval ranking  with the 
query-cluster based similarity can shed light  on the necessity of  dense retrieval.
When top sparse retrieval results are concentrated in a few top  ordered dense clusters, dense retrieval may bear
a resemblance  in  ranking.


With the above consideration  in mind, we use the  following categories of features
to train a boosted decision tree model.

}
% with these featuers an input by using the xgboost package. 
\comments{
To evaluate the performance of the sparse system, we design some features to describe the quality of sparse encoder. 
For example, the length of expanded query, distribution of token impact scores and their corresponding matching scores with top k documents.

To evaluate the discrepancy between the performance of sparse and dense system. We encode the original query with the dense retrieval encode and each expanded token and generate distributional features around the similarity between them. 


%We take a supervised approach to the construction of a query filter that classifies  a query after sparse retrieval 
%needs an argumentation from  dense retrieval or not. We consider the following two categories of the feautres.
}
\comments{
\begin{itemize}[leftmargin=*]
\item Quality of query expansion by the sparse retriever model.
    For example, the query-level matching score, define as the similarity  between the CLS embeddings of the orginal query and the expanded query.
    Another one is the token-based matching histogram vector between the expanded query and the original query. 
For each query token in the expanded query, we evaluate the matching score in terms of similarity
 between its token embedding and  the oringal query embedding. 
We map  these values into five bins with  ranges <0.5, 0.5-0.6, 0.6-0.7, 0.7-0.8, >0.8.
Then derive a matching histgram count  vector for each bin.
}

\comments{
{\bf WILL DELETE THIS LIST.}
\begin{enumerate}
    \item The length of the original query and the expanded query in terms of  the  number of words or tokens, respectively. 
    \item The token-based matching  vector between the expanded query and the original query. 
For each query token in the expanded query, we evaluate the matching score in terms of similarity
 between its token embedding and  the original query embedding. 
We map  these values into five bins with  ranges <0.5, 0.5-0.6, 0.6-0.7, 0.7-0.8, >0.8.
Then derive a matching count vector based on this bin mapping???
    \item The query-level matching score, define as the similarity  between the CLS embeddings of the original query and the expanded query.
    \item The sum of matching scores within each of above token similarity bin, divided by
the  query-level matching score. 
%The token groups are the tokens with similarities in each bin.
    \item The sum of matching scores of tokens not in NLTK English corpus, divided by  the query-level matching score. 
    \item The number of overlapping tokens between expanded and original query / number of all unique queries in both expanded and original query.
    \item number of  tokens only in expanded query / number of all unique queries in both expanded and original query.
    \item overall/mean/max of token weight of overlapping tokens between expanded and original query in the expanded query.
    \item max/min/mean of token weights of expanded query tokens.
\end{enumerate}

}
%\item
\comments{
Ranking characteristics of documents scored by sparse retrieval.
We compute  the mean sparse retrieval score of top 10-20/20-30/30-40/40-50/50-100/100-400/400-700/700-1000 documents.

%Sparse  retrieval score distribution:
\begin{enumerate}
    \item Sparse retrieval scores of top 10 results
    \item The mean sparse retrieval score of top 10-20/20-30/30-40/40-50/50-100/100-400/400-700/700-1000 documents.
\end{enumerate}
%Sparse and Dense relational features:
\item Overlapping degree of sparse retrieval with dense clusters:
\begin{enumerate}
    \item The number of dense clusters containing top 5/10/20/50/100/1000 results from the sparse system
\end{enumerate}
}

%\end{itemize}


%\subsection{Partial Document Evaluation}
{\bf Training of LSTM.} 
We assume that the training data  contains
a set of queries and relevance-labeled documents,  that allows the computation of a ranking metric such as MRR or NDCG.
For example, from MS MARCO training set we randomly sample 5000 training instances, where each training instance contains a query and  one or more  relevant documents. 
%Then we run a sparse retriever this instance, and seperately run a fusion with a dense retriever. If the result of sparse retriever results merged with dense results  exceeds the standalone sparse retrival,  we label consider training instance as an positive example for dense retrieval, otherwise consider this as a negative example. The converted training isntances are used for training In this way, we convert a set of training instances for ranking as a set of training instances for fusion.
To train the LSTM for cluster selection, 
for each training instance, we mark the positive and negative examples for  top cluster selection.
If a cluster contains one of top-10 dense retrieval results, we mark this cluster as positive otherwise negative.
This approximately indicates that such an embedding cluster should be visited for a fusion.

 
\comments{
We convert We define the labels as 
\begin{equation}
       y(q)= 
\begin{cases}
    1,& \text{if } U(s(q), d(q)) > U(s(q))\\
    0,              & \text{otherwise,}
\end{cases}
\end{equation}
where $U(.)$ is a evaluation metric we choose, for example, NDCG@10 or MRR. $s(q)$ is the scoring of a sparse system of query $q$ and $d(q)$ represents the scoring of a dense system.
}

\comments{
\subsection{How to combine two ranked lists}
There are two commonly used methods to combine the sparse and dense ranked lists:
\begin{enumerate}
    \item linear combination
    \item reciprocal rank fusion
\end{enumerate}
For linear combination, the final ranking score of a document is the weighted sum of the ranking score of two systems respectively. The weight on each system can be determined through grid search on a left-out training set or just use 1:1 combination. In this case, rescaling of the two ranked lists is necessary as it largely affects the impact of a ranked list on the merged ranked list. 

On the other hand, reciprocal rank fusion alleviates the scoring distribution difference by only considering the ranking positions when merging. 
  Another consideration is the missing values. The two ranked lists usually do not fully overlap. Some documents only exist in one ranked list. Thus 
the treatment on these documents affects model performance. We consider a few options
\begin{enumerate}
    \item Remove the documents when they only exist in one ranked list
    \item  Take the document and compute the score for only one ranked list
    \item Impute the missing document with rank K+1 or score as 0.95 * min(score) in the ranked list.
\end{enumerate}

}




==> kddproblem.tex <==
\section{Background and Related Work }
%\section{Problem Definition}
\label{sect:background}

\comments{
\begin{table}[h]
	\centering
		%\resizebox{1.02\columnwidth}{!}{ 
		\begin{small}
		\begin{tabular}{l l}
			\hline
			Symbol & Def. \\
                \hline
                %$\mathcal{D}$ & A set of documents in a dataset\\
                %$N$ & Total number of documents in a dataset \\
                $Q$ & A query \\
                $d_i$ & A document \\
                $\mathcal{D}^{+}$, $\mathcal{D}^{-}$ & Positive/negative document subsets corresponding to $Q$  \\
                $|.|$ &  The size of a set\\
		$\Theta$& Parameters of a scoring model\\
		$S(Q,d_i, \Theta)$ & The rank score of a document for a query using a model\\
%			& based on a model with parameters $\Theta$. \\
                $p_i$ & Teacher's top one probability of document $d_i$,\\
			& standing for  $P(d_i|Q, \mathcal{D}^+, \mathcal{D}^-, \Theta$) \\
                $q_i$ & Student's top one probability of document $d_i$\\
                $\pi(.)$ & The rank position of a document for a query\\
                $\beta_i$ & Exponent weight bias for negative  document $d_i$\\
                $\gamma, \alpha$ & CKL hyper-parameters\\
                \hline
		\end{tabular}
		\end{small}
	%}
	\caption{Table of Symbols}

	\label{tab:data}
\end{table}
}

\textbf{Problem definition}
Given query $q$ for searching a collection of $D$ text documents:   $ \{d_i\}^D_{i=1}$, 
retrieval  obtains the top $k$ relevant documents from this collection based on
the similarity between query $q$ and document  $d_i$ using  their
representation vectors.

With a lexical representation, each  representation vector of a document or a query is sparse.
Sparse retrieval uses  the dot product of their lexical representation vectors as the similarity function
and implements its search efficiently using an inverted index. 
\begin{equation}
\label{eq:sparseretrieval}
L(q) \cdot  L(d_i)
\end{equation}
%L(q,d_i ) = 
where $L(.)$ is a lexical representation   which is a vector of weighted term tokens for a document or a query.
For BM25 based lexical representation~\cite{Robertson2009BM25}, 
$L(.)$ treats each document or a query as a bag of terms.
% Q: do we want to keep referring to everything as bag of terms?
%and term weights  are scaled based on   frequency of terms within a bag and  across all bags involved.
Term weights are scaled based on the frequency of terms within a document and across all documents in the collection.
For a learned sparse representation~\cite{Dai2020deepct, Mallia2021deepimpact, Lin2021unicoil,2021NAACL-Gao-COIL}, 
a document or a query is encoded using  a trained neural ranking model, which
%produces a bag which may contain original  and  expanded terms.
produces modified representations of document or query which may contain both original and expanded terms.
The encoding functions for a query and document can be different. Without the loss of generality, we assume they are the same in this paper.

With a single-vector dense  representation, each  representation vector of a document or a query is a dense vector. 
Dense retrieval computes the following rank score
\begin{equation}
\label{eq:denseretrieval}
R(q) \cdot  R(d_i)
\end{equation}
%D(q,d_i) 
where $R(.)$ is a dense representation vector  of a fixed size~\cite{Karpukhin2020DPR}.


  %revises the SparTerm model~\cite{Bai2020SparTerm} to predict the weight 
%The weights of these terms evaluated in this paper use the SPLADE model as discussed below while other options are possible.
%(e.g., a bag of words or a neural encoder). 
%The implementation of such a dot product for a sparse retriever uses the inverted index data structure.
\comments{
%{\bf Learned term weights with SPLADE}.
For each document, the SPLADE term weighting revises the SparTerm model~\cite{Bai2020SparTerm} to predict the weight 
score $w_j$ of $j$-th token term in BERT WordPiece vocabulary.
\begin{equation}
\label{eq:splade}
w_j = \sum_{i \in d}  log (1 + ReLU ( H(h_i)^T E_j + b_j)) 
\end{equation}
where document $d$ consists of a sequence of BERT last layer's embeddings $(h_1, h_2, $
$\cdots, h_n)$.
$E_j$ is the BERT input embedding of the $j$-th token and $b_j$ is a token level bias.
$H(.)$ is a linear layer with activation and layer normalization. 
% (In SPLADE GeLU activation is used). 

{\bf Combining the results of a dense retriever and a sparse retriever.}
}
Following the work of~\cite{kuzi2020leveraging, 2022LinearInterpolationJimLin, Gao2020ComplementingLR}, 
linear interpolation is used  to  ensemble  dense and sparse retrieval scores. 
%Let $S$ be the set of top results obtained by a sparse retriever, and $D$ be
%be the set of results obtained by dense retrieval. 
%For any document $d_i \in S \cup D$, its  
The fused rank score for document $d_i$ in responding  query $q$ is:
\begin{equation}
\label{eq:fusion}
\alpha L(q) \cdot  L(d_i) +
(1-\alpha) R(q) \cdot  R(d_i) 
\end{equation}
where $\alpha$ is a coefficient in a range between 0 and 1.

\comments{
Notice that   the two ranked lists $S$ and $D$ are usually not fully overlapped and  some documents only exist in one list. While 
different  treatments on these documents affect fusion performance,
we take an option to  impute the score of such a document score   using $\beta * score (top \  k+1) $  in the missed  ranklist where $\beta$
is a scaling factor.
%While there are options to We consider a few options
For example,  we  impute the lexical scores of documents expanded by dense retrieval
as the top-$(k+1)$ lexical  score scaled by a factor. We use $\beta=0.95$  in our evaluation.
 
%\item Remove the documents when they only exist in one ranked list
%    \item  Take the document and compute the score for only one ranked list
}


Our goal is to maintain a relevance competitive to full dense retrieval, while minimizing the time and memory overhead of cluster-based dense retrieval.
We propose leveraging sparse retrieval to minimize the scope of dense clusters to visit.
% Parker: below is awkard, and a bit of a run-on sentence. Above I reworked it, but it's still not great
%Our optimization goal is to minimize the scope of cluster-based dense retrieval and extra memory space overhead by leveraging sparse retrieval 
%while maintaining a relevance competitive to full dense retrieval.  
%In this way, limited dense retrieval that augments sparse retrieval is fast with minimum space consumption  on a CPU server. 
\comments{
The ensembling method used in our evaluation is 
%The final ranking of the top $K$ documents is 
the reciprocal rank fusion (RRF) following Cormack et al.~\cite{Cormack2009RRF}, considering ranking positions of each candidate 
generated by a retriever and by a re-ranker. 
We use RRF
% above reciprocal rank fusion 
instead of linear interpolation as it has a similar performance with a simplified combination of two scoring models. 
%We choose RRF because it is easily applicable to multiple ranked lists ignoring the score distribution differences. 
\begin{equation}
     %RRF(Q,d) =  \sum_{r \in {rt, rr,}} \frac{1}{k_r + r(d)},
     RRF(Q,d) =  
\frac{1}{c_1 + \pi_1(d)} + 
\frac{1}{c_{2} + \pi_2(d)},
     \label{eq:score}
\end{equation}
where $c_{1}$ and $c_{2}$ are fixed smoothing constants. $\pi_2(d)$ is the rank position based  a re-ranker formula
while $\pi_1(d)$ is the rank position based on a retriever.
}



==> method.tex <==
%\section{SRF with Query-Specific Cluster Skipping }
%\section{CluSD: Selective Dense Retrieval}

  
\section{Selective Dense Cluster Retrieval}
\label{sec:clusd}
\comments{
It is common practice to interpolate the results from a sparse system and a dense system. We propose two directions to improve the latency of such system by avoiding the unnecessary dense evaluation on query level and per query level. We envision a hybrid system where sparse retrieval runs first and partial query and documents are evaluated by the dense retrieval system. 

The proposed CluSD method contains two components  during runtime inference to 
decide if  dense retrieval augmentation  can be skipped for a query and which  top dense document clusters should be selected  during supplemental retrieval.
}

\subsection{Selection of dense clusters}
%Per-query inference latency depends on the number of document evaluated and how per query-document evaluate is approximated. We do not touch per-query-document approximation in this paper and focus on reducing the number of documents evaluated. We cluster document using kmeans as IVF and would like to intelligently select a few most promising clusters to retrieve candidate results. 
\comments{
\begin{figure}[h!]
    \centering
    \includegraphics[scale=1.0]{lstm.png}
    \caption{LSTM prediction for each query}
    \label{fig:lstm}
\end{figure}
}
As discussed earlier, documents with embedding vectors are clustered based on their similarity to the cluster centroids. 
\comments{
Our experiments take an advantage of the FAISS library which  provides such a support such as k-mean clustering.
Once a query is determined by CluSD to trigger  partial dense retrieval that selects and visits a subset of dense clusters. 
% online inference  will  visit the dense clusters one by one in
%an incresing order of   their centroid distance to the input query.
%A decision procedure is invoked to decide if a cluster to be visited should be skipped or not. 
}
Our objective is to examine the features of each cluster and  incrementally decide if this cluster should  be visited or not.

\begin{figure}[htbp]
    \includegraphics[scale=0.75]{dense_separse_feature_lout.drawio.pdf}
    \vspace*{-1mm}
    \caption{Illustration of CluSD and its features.}
    \label{fig:features}
     \vspace*{-5mm}
\end{figure}

{\bf LSTM design.}
%Because this decision procedure uses the document scoring information  of each cluster visted 
We adopt a simple LSTM model based on  a recurrent neural network~\cite{hochreiter1997long}, 
taking a sequence  of clusters as an input along with their features.
Assume there are $N$ document clusters grouped using dense document embeddings, and 
it is time consuming for the LSTM model to examine all clusters. Thus
 we truncate the sequence of clusters at maximum length $n$ and then take a sequence of top $n$ clusters as the input to this LSTM. 
There are  $n$ nodes corresponding to these clusters in the LSTM model.
We will discuss how to truncate with a prioritization shortly below.



\comments{
The LSTM model outputs 1 for each cluster node if this cluster should be visited to perform the corresponding dense retrieval.
The goal of this procedure  is to visit  dense clusters as few as possible while still delivering a competitive fusion performance.
The number of predicted clusters are different across queries and the overall budget is controlled by the prediction threshold.
}
%  a few clusters as possible to recover the top results from the original dense retrieval. 
%The label of each query-cluster is 1 when the cluster contains the top k results of the query in the exact full search of dense retrieval.  
%The input is the a sequence of cluster nodes in the order of the centroid-query distance. 
%The feature of each input include: statistics on query-centroid distance, centroid-to-centroid distances, distribution of sparse top results across clusters. 
%The model will predict for each query which clusters to choose. 
%The input features of our proposed LSTM model are listed below.
%These clusters are sorted by the the similarity distance of the given query with the  centroid of each cluster.



Given the above  $n$ top clusters,
 the LSTM computation flow goes from the left most cluster called $c_1$ to the right most $c_{n}$.
Assume the current cluster is $c_i$,  
the LSTM computation outputs a predicted value $f(c_i)$ where $0\leq f(c_i) \leq 1$.
If $f(c_i) \ge \Theta$, where $\Theta$ is a predefined prediction threshold, then cluster  $c_i$ should be visited. In practice, the strictness on selecting a cluster to evaluate is controlled by $\Theta$ and it can be determined based on the overall latency requirement. 

\comments{
When the dense vectors of all documents are grouped into $N$ clusters, 
we limit our cluster search scope into top $n$ clusters in terms of query and cluster centroid similarities. 
we limit $n=128$ in our evaluation out of 1000 clusters.
%Query-specific information derived from  dense clusters:
}

As shown in Figure~\ref{fig:features}, the feature input vector for the current cluster  $c_i$ for the above LSTM computation to produce $f(c_i)$
%$f(q, c_i)$  
is composed of:
\[
[ sim(q,c_i),   
\{ AvgDist(sim(c_i, c_l) \text{ for } c_l \in A_j) \}^6_{j=1}, 
\]
\[ 
     \{  |c_i  \cap  B_j|    \}^{6}_{j=1},  
\{  AvgScore (c_i  \cap  B_j)    \}^{6}_{j=1} 
]. 
\] 
\begin{enumerate}[leftmargin=*]
    \item $sim(q,c_i)$: The similarity distance of this query $q$ with the centroid of cluster $c_i$.  
  %\item  $\{ sim(c_i, c_j) \}^{n-1}_{j=0}$: The distance vector between the centroid of $c_i$ to  all other clusters.
%the top  clusters that have been visited (or skipped).  We limit this number as $K=128$.
%other top k centroids for this query (k=128)??
  
\item  \{  $AvgDist(sim(c_i, c_l)) \text{for } c_l \in A_j \}^6_{j=1}$: 
The mean distance between this centroid and the centroids in each of six position bins $A_j$.
%These six bins  are formed by partitioning all clusters into consecutive position bins.
%For example, $A_1$ contains clusters from Postions  1 to 5, Positions 6-10, 
%$A_2$  contains clusters from Postions  6 to 10, and so on.   Bin $A_6$ contains the rest of uncovered clusters.  
These six position bins  are formed by cluster centriods. 
After all the $N$ centroids are ordered based on a criterion discussed shortly, we partition the sequence of sorted clusters into consecutive position bins.
These bins respectively contain clusters in Positions  1-5, Positions 6-10, 
Positions 11-20, Positions 21-50, Positions 51-100, and the rest of N clusters. 
The purpose of this feature group is to capture the distances of a cluster to previously examined clusters and unexamined clusters following the LSTM flow. 
When the mean distance  between cluster $c_i$  and clusters in a previously-examined  bin is close, if  many clusters in that bin have been selected, cluster 
$c_i$ may have a good  chance to  be selected.

%Since the clusters are processed from a lower position to a higher position one by  one,
%these features represent the distance to the groups 
    
    \item $ \{  |c_i  \cap  B_j|    \}^{6}_{j=1} $ and $\{  AvgScore (c_i  \cap  B_j)    \}^{6}_{j=1} $: 
The number of documents and average sparse ranking score from this  cluster contained in each of   the six bins $B_j$  formed by
top $k$ sparse retrival results. In our evaluation, we limit the retrieval depth to be $k$ where $k = 1000$.
Top $k$ sparse results are divided into six bins:
top 10, top 11 to 25, top 26-50, top 51-100, top 101-200, top 201-top 500, and 
top 501 to k documents.  These bins are called $B_j$ where $1\leq j \leq 6$. 
The purpose of this feature group is to capture the overlap degree  of a cluster with the top results of sparse retrieval.
A cluster that contains many top sparse results may be selected.
    %\item $\{  AvgScore (c_i  \cap  B_j)    \}^{6}_{j=1} $: 

% bin 
%top 10/25/50/100/200/500/1000 documents  in the sparse retrival results.
\end{enumerate}



%Section~\ref{sect:evaluation} provides more details on the effectiveness 
 

\textbf{Re-order candidate clusters for prioritization and pruning.} 
The inference time of an LSTM model is proportional to its input length ($n$) in terms of
the number of clusters to be examined. We denote $n$ as the  input length  to our LSTM  throughout the rest of this paper.
Table ~\ref{tab:LSTMclustertime} shows that as the number of clusters to be examined
varies from 32 to 512, the LSTM inference time increases from  2.8ms to 33.9ms.
As we would like to make a quick decision given the overall  time budget,
we devise another strategy to prune clusters that may not provide a meaningful boosting
of relevance quality. 

% dependent on the length of the sequence input. 

\begin{table}[h]
	\centering
		\resizebox{0.68\columnwidth}{!}{ 
%		\begin{small}
		\begin{tabular}{r | rrrrr}
			\hline\hline
			  \#Clusters examined & 512 & 256 & 128 & 64 & 32 \\
\hline
            Time (ms) & 33.9 & 16.2 & 6.2 & 3.8 & 2.8\\
                \hline\hline
		\end{tabular}
%		\end{small}
	}
	\caption{LSTM inference time with different input length.}
	\label{tab:LSTMclustertime}
 \vspace{-7mm} 
\end{table}

\comments{
\begin{figure}[htbp]

    \includegraphics[scale=0.27]{dist.pdf}
    \caption{Distribution of Good Documents
}
    \label{fig:dist}
%\vspace{-1em} 
\end{figure}
}

To prune clusters, one may prioritize a few top clusters sorted by the query-centroid distance.
We find this does not work well in the context of augmenting sparse retrieval results.  
Table~\ref{tab:dist} shows the distribution of top 10 documents from the full dense retrieval  
in embedding clusters under the different query percentile when searching an MS MARCO passage dataset using queries from its  Dev set. 
Row 2 of Table~\ref{tab:dist} shows the number of top clusters needed to cover  top 10 
documents from the full dense retrieval  when clusters are sorted by sorted by  the query-centroid distance.
This row shows that to cover top 10 dense results, $n$ needs  to be larger than 175.
%On the other hand, Row 2 is  the number of lusters decided by the LSTM to visit  under the different query percentiles. 
%At most  66 clusters are  selected  by the LSTM model for all queries.
%We further propose to skip unnecessary clusters. 
\begin{table}[h]
 \vspace*{-1mm}
	\centering
		\resizebox{0.78\columnwidth}{!}{ 
%		\begin{small}
		\begin{tabular}{r |r  r r r r}
			\hline\hline
			  Query percentile & 10\% & 50\% & 75\% & 90\% & 95\% \\
            \hline
%            \#clusters selected by  LSTM & 1 & 4 & 14 & 40 & 66\\
            %Relevant doc coverage & 1 & 2 & 7 & 29 & 69\\
             Top 10 dense result coverage & 1 & 6 & 25 & 92 & 175\\
                \hline\hline
		\end{tabular}
%		\end{small}
	}
	\caption{ Distribution of  top 10 dense results in sorted clusters 
% \% of Good Documents Among Clusters Sorted by Query-Centroid Distance
}
 \vspace*{-5mm}
	\label{tab:dist}
\end{table}

%provides an explanation.  evidence on the effectivness of the above LSTM model.
%After searching an MS MARCO passage dataset using queries from the MAMARCO dev set, 
%under the different query percentile shown in Row 2 is  the number of clusters decided by the LSTM to visit.
%Row 3 is  the number of clusters needed to 
%For a lot of queries, the top 5 or even top 10 clusters do not contain enough information, for example, around 10\% of queries need more than 92 top clusters to recover the top results from the full dense retrieval. It demonstrates the necessity of doing cluster selection and skipping.  
%On the other hand, there is a reasonable distribution resemblance between  Row 2 and  Row 3, which shows the LSTM model provides a reasonable guidance on where relevance results are.
%%While it does not exactly follow the distribution of top 10 results of sparse retrieval, the feature 
%From  Table~\ref{tab:dist}, we observe that
%the distribution of top 10 results from a sparse are contained is not necessarily concentrated in the top  clusters.
Since our ablation  analysis finds that Group  (3) of the above feature list
is important for the accuracy of LSTM to make a sound cluster selection, we resort to this feature group in making 
a preliminary selection of  necessary clusters. 
%With the above design consideration,  we propose to use the following strategy to 
%sort the candidate clusters based their feature vectors from Group  (3).
Specifically we sort the candidate clusters based on the overlap degree of a cluster with the six top sparse retrival result bins. 
If there is a tie between two clusters, then we sort them by their centroid distance to the query.
%We first use a simple heuristic to reorder the clusters, refered as Top K heuristic. 
%We order the clusters based the six features then 
%followed by q-c-orders. 
Then, the sorted  top $n$ candidate cluster list is used as the input sequence to the LSTM model. 
%We will stop the LSTM computation of  this list
%after visiting $\tau$ clusters and when the predicted $f(c_i)$  values of a few consecutive clusters are all below a threshold. 
%For our evaluation in MS MARCO and BEIR datasets, $\tau=20$. 
In our evaluation, we find that a relatively small number such as $n=32$ is a solid choice  to yield competitive results  after the above cluster sorting and prioritization.
%As a result, the LSTM computation for cluster selection can be completed within  1.8 milliseconds. 
%The number of clusters selected varies from a few to 20 on average, which yields a quick argumentation with dense cluster results.


%Features marked with Hexgos 1 and 4 are used for a boosting tree to make a decision if cluster selection should be triggered or not.
\comments{
\subsection{Query filtering}
%When computing the embedding of each query token or the whole  original query, we use 
%the denser retriever's encoder. 


We also exploit the possibility to skip dense retrieval completely.
Modifying the above LSTM-based decision mechanism does not yield a satisfied result.
We sort to add a classifier with  boosted decision trees with supervised learning
to make an earlier  determination before triggering the LSTM computation.
}
\comments{

a query needs an argumentation from dense retrieval 
%A challenge is to identify features and infer based on such features with supervised learning.
Given that sparse retrieval is conducted first,
our idea is to predict the quality of sparse retrieval and its relative strength  compared to unexecuted
dense retrieval based on quality of query token expansion by the sparse model,
the statistical behavior of  sparse retrieval results, and
the relationship between dense document embedding summary and sparse retrieval scoring structure.

}


\comments{
\begin{table}[ht]       
    \centering          
%    \resizebox{1.05\columnwidth}{!}{

\begin{small}                        

    \begin{tabular}{l |l}
        \hline
    Query    & "how long nyquil kicks in"\\
    \hline
 Query Expanded&["in", 36],  ["time", 74], ["years", 71], ["long", 97], \\
 & ["total", 60],\textcolor{red}{["move", 23]}, ["effect", 22], \textcolor{red}{["weapon", 21]}, \\
 & \textcolor{red}{["jump", 24]}, ["kick", 100], ["ny", 111], ["timing", 34], \\
 & ["kicks", 76], ["\#\#quil", 139]\\
    \hline  
Relevance Doc &["\#\#quil", 410.1], ["ny", 301.0], ["long", 216.7], \\
& ["time", 134.7], ["years", 131.5], ["total", 87.4],\\
& ["effect", 34.4], ["timing", 17.4]\\
\hline
Top 5 Doc & ["\#\#quil", 392.6], ["ny", 295.7], ["kick", 236.1], \\
& ["long", 198.3], ["time", 141.2], ["years", 116.9], \\ 
& ["kicks", 101.8], ["total", 86.3],\\
& ["in", 35.3], ["effect", 24.1], ["timing", 23.6],\\
& \textcolor{red}{["jump", 10.0], ["move", 6.0]}\\
        \hline
    \end{tabular}
\end{small}                        
%}     

\caption{An example of weak query expansion in SPLADE} 
\label{tab:queryencoder}
\end{table} 
}

\comments{
\begin{table*}[ht]       
    \centering          
%    \resizebox{1.05\columnwidth}{!}{

\begin{small}                        

    \begin{tabular}{l  l l}
        \hline\hline
    Query   &  \multicolumn{2}{l}{ "why do we push others away"}\\
    \cline{2-3}
&  \multicolumn{2}{l}{('push', 105), ('away', 104), ('because', 97), ('others', 94), ('people', 44), ('why', 44), ('purpose', 43), ('cause', 42), (',', 40), ('we', 38),} \\
&\multicolumn{2}{l}{ ('other', 38), ('effect', 33), ('them', 29), \boldred{('responsibility', 28),} ('help', 20), \boldred{('move', 19), ('severe', 17),}  ('step', 17), ('do', 16),...}\\
%& & ('things', 15)， ('fear', 15), ('method', 10), ('to', 6), ('language', 5), ('anger', 5), ('when', 2), ('feeling', 2), ('\#\#ness', 1), ('dangerous', 1)]\\
    \hline  \hline
   Doc Relevant? & \ rank & Text and Expanded Tokens \\
\hline
\comments{
Yes & 17 & From a psychological standpoint, pushing away the people you love the most is a very basic and common, defense mechanism.\\
&& As the relationship develops, people become inundated with their own fears and insecurities that they will not be accepted\\
&& and therefore hurt by their loved one.\\
\cline{3-3}
& & [('push', 198), ('away', 196), ('fear', 127), ('people', 104), ('effect', 81), ('because', 70), ('severe', 67), (',', 61), ('method', 61),
\\
& &  ('when', 59), ('anger', 58), ('dangerous', 55), ('feeling', 53), ('purpose', 53), ('responsibility', 53), ('move', 44), ('cause', 43),... \\
%& & ('them', 37), ('things', 31), ('\#\#ness', 27), ('step', 23), ('why', 13), ('help', 9), ('to', 3), ('do', 1), ('language', 0)]\\
\specialrule{.1em}{.05em}{.05em} 
}
No & 10 & Different types of push factors can be seen further below. A push factor is a flaw or distress that drives a person away from \\
&&  a certain place. A pull factor is something concerning the country to which a person migrates. It is generally a benefit that  \\
&&attracts people to  a certain place. Push and pull factors are usually considered as north and south poles on a magnet.\\
\cline{3-3}
&& [('push', 283), ('away', 162), \boldred{('move', 80),} \boldred{('severe', 74)}, ('people', 70), ('because', 68), ('effect', 58), ('cause', 44), ('purpose', 43),\\
& & \boldred{('responsibility', 41),} (',', 36), ('method', 35), ('\#\#ness', 33), ('step', 23), ('them', 22), ('to', 18), ('when', 13), ...\\ 
%& &  ('things', 11), ('anger', 9), ('dangerous', 8), ('fear', 3), ('do', 0)]\\
\specialrule{.1em}{.05em}{.05em} 
No & 8& Most of the universe is rushing away from us. It\textbackslash{}'s not that we\textbackslash{}'re particularly repellent; it\textbackslash{}'s just that the universe is\\
&&  expanding, pushing most other galaxies away. Light from distant galaxies travels toward us through this \\
&& expanding space, which stretches their light to longer, or redder, wavelengths.\\
\cline{3-3}
&& [('away', 184), ('push', 158), ('other', 111), \boldred{('move', 103)}, ('we', 101), ('effect', 83), (',', 73), ('because', 66), ('method', 53),\\
&&  ('others', 39), ('cause', 39), ('severe', 39), ('them', 36), ('do', 29), ('things', 29), ('dangerous', 29), ('feeling', 28), ... \\
% & & ('when', 27), ('help', 19), ('purpose', 13), ('to', 4), ('why', 2)]\\
         \hline\hline
    \end{tabular}
\end{small}                        
%}     

\caption{An example of weak SPLADE query expansion that boosts  irrelevant documents  } 
\label{tab:queryencoder}
\end{table*} 

Our consideration 
%is that the necessity of invoking a dense retrieval model after running a sparse model depends on 
%\begin{enumerate}
%the relative strength of results scored by this sparse retriever. If a
    is that  if a chosen
sparse retriever has  well-performed, the benefit of addition of dense scoring  is limited. 
Notice that a learned neural sparse retriever expands the original query with a transformer-based encoder
We found that the quality of query encoding with expansion in SPLADE impacts the quality of sparse retrieval. 
%and we form features using both the original query  and the expanded query.
When  there is a low similarity value  between the original query and the tokens of 
its expanded  query, the confidence for  strong sparse retrieval can be low.
Table~\ref{tab:queryencoder} gives such an example and lists an original query and its expanded query tokens
sorted by token weights.  Expanded query words  in red color
not highly relevant to the original query and they are weighted high in two irrelevant documents, which boosts their ranking.  
Thus    excessive presence of un-similar  query tokens  after expansion  can misrank irrelevant documents. 
Another consideration is that the alignment of sparse retrieval ranking  with the 
query-cluster based similarity can shed light  on the necessity of  dense retrieval.
When top sparse retrieval results are concentrated in a few top  ordered dense clusters, dense retrieval may bear
a resemblance  in  ranking.


With the above consideration  in mind, we use the  following categories of features
to train a boosted decision tree model.

}
% with these featuers an input by using the xgboost package. 
\comments{
To evaluate the performance of the sparse system, we design some features to describe the quality of sparse encoder. 
For example, the length of expanded query, distribution of token impact scores and their corresponding matching scores with top k documents.

To evaluate the discrepancy between the performance of sparse and dense system. We encode the original query with the dense retrieval encode and each expanded token and generate distributional features around the similarity between them. 


%We take a supervised approach to the construction of a query filter that classifies  a query after sparse retrieval 
%needs an argumentation from  dense retrieval or not. We consider the following two categories of the feautres.
}
\comments{
\begin{itemize}[leftmargin=*]
\item Quality of query expansion by the sparse retriever model.
    For example, the query-level matching score, define as the similarity  between the CLS embeddings of the orginal query and the expanded query.
    Another one is the token-based matching histogram vector between the expanded query and the original query. 
For each query token in the expanded query, we evaluate the matching score in terms of similarity
 between its token embedding and  the oringal query embedding. 
We map  these values into five bins with  ranges <0.5, 0.5-0.6, 0.6-0.7, 0.7-0.8, >0.8.
Then derive a matching histgram count  vector for each bin.
}

\comments{
{\bf WILL DELETE THIS LIST.}
\begin{enumerate}
    \item The length of the original query and the expanded query in terms of  the  number of words or tokens, respectively. 
    \item The token-based matching  vector between the expanded query and the original query. 
For each query token in the expanded query, we evaluate the matching score in terms of similarity
 between its token embedding and  the original query embedding. 
We map  these values into five bins with  ranges <0.5, 0.5-0.6, 0.6-0.7, 0.7-0.8, >0.8.
Then derive a matching count vector based on this bin mapping???
    \item The query-level matching score, define as the similarity  between the CLS embeddings of the original query and the expanded query.
    \item The sum of matching scores within each of above token similarity bin, divided by
the  query-level matching score. 
%The token groups are the tokens with similarities in each bin.
    \item The sum of matching scores of tokens not in NLTK English corpus, divided by  the query-level matching score. 
    \item The number of overlapping tokens between expanded and original query / number of all unique queries in both expanded and original query.
    \item number of  tokens only in expanded query / number of all unique queries in both expanded and original query.
    \item overall/mean/max of token weight of overlapping tokens between expanded and original query in the expanded query.
    \item max/min/mean of token weights of expanded query tokens.
\end{enumerate}

}
%\item
\comments{
Ranking characteristics of documents scored by sparse retrieval.
We compute  the mean sparse retrieval score of top 10-20/20-30/30-40/40-50/50-100/100-400/400-700/700-1000 documents.

%Sparse  retrival score distribution:
\begin{enumerate}
    \item Sparse retrieval scores of top 10 results
    \item The mean sparse retrieval score of top 10-20/20-30/30-40/40-50/50-100/100-400/400-700/700-1000 documents.
\end{enumerate}
%Sparse and Dense relational features:
\item Overlapping degree of sparse retrieval with dense clusters:
\begin{enumerate}
    \item The number of dense clusters containing top 5/10/20/50/100/1000 results from sparse system
\end{enumerate}
}

%\end{itemize}


%\subsection{Partial Document Evaluation}
\subsection{ Online inference and model training}

\begin{figure}[htbp]
    \includegraphics[scale=0.75]{sparse_dense_flow_lout.drawio.pdf}
    \caption{The flow of cluster-based selective dense retrieval}  
 \vspace*{-1mm}
    \label{fig:flow}

\end{figure}
As shown in Figure~\ref{fig:flow}, the online inference algorithm is as follows:

1) Conduct sparse retrieval to obtain top $k$ results.

%\item Condcut the query filter  to determine if the cluster-based dense retrieval is necessary.If needed, 
2) Sort clusters based on the overlap degree of dense clusters and top sparse retrieval results and their  centroid-to-query  distances.

3) Call the LSTM to choose   dense clusters. 

4) Expand top $k$ sparse retrieval results to include the document vectors of these dense clusters and
merge their sparse and dense scores with a linear interpolation.  

%During the above linear interpolation, only top $k$ of sparese retrieval contains a lexical score,
%and thus we  impute the lexical scores of other documents expanded by cluster-based selective dense retrieval 
%as the bottom document score in the top $k$ sparse retrieval list scalled by a factor. We use 0.95 in our evaluation.
\comments{
Notice that  the two ranked lists from two retrievers are usually not fully overlapped and  some documents only exist in one list. While
different  treatments on these documents affect fusion performance,
we resort  to  impute the score of such a document using  the top $k+1$ score   in the missed rank list scaled by 
a factor.
%While there are options to We consider a few options
For example,  we  impute the lexical scores of new documents added  by dense retrieval
using  the scaled lexical score of  top $(k+1)$ in the sparse retrieval list. We use scale $0.95$  in our evaluation.
}
%\item Remove the documents when they only exist in one ranked list
%    \item  Take the document and compute the score for only one ranked list

%When we have access to a relatively strong sparse retrieval system and a dense retrieval system, it is feasible to selectively choose queries that requires evaluation of both systems. We hypothesize that the sparse system is economical and we can afford to run it for every query. The problem boils down to dynamically select queries to evaluate by dense retrieval.

{\bf Online computing and space  cost for augmentation.} We only consider cost of  augmenting sparse retrieval results with dense retrieval during online inference. 
The space cost of dense retrieval is $O(D)$  for a corpus with $D$ vectors.
For MS MARCOS, the cost is around 27GB without compression. Quantization can  reduce that  0.5GB  to 1GB or less based on codebook parameters.
Then this cost becomes a fraction of sparse retrieval index cost.  
Excluding dense embeddings, the extra space overhead  for CluSD is to maintain  the similarity among centroids of $N$ clusters, which is  $O(N^2)$.
This cost is  negligible compared  to the embedding space with $N << D$.  In our evaluation, 
%we use  $N=8192$ or  $4096$.
the inter-cluster similar graph for MS MARCO passages with $N=8192$ takes about 32MB with quantization.

The time  cost of CluSD is dominated by the cost of cluster selection and  dense similarity computation of selected dense clusters.
The former is about $O(n)$ while the later is
proportional to the number of clusters selected, which is capped by $O(\frac{D}{N} n)$. 
In  our evaluation of MS MARCO and BEIR, the actual number of clusters selected and visited is relatively small.
%Given the short time added by the pruned LSTM model, 
The overall latency overhead introduced by CluSD is fairly small. 





{\bf Training of cluster selection.} 
We assume that the training data  contains
a set of queries and relevance-labeled documents,  that allows the computation of a ranking metric such as MRR or NDCG.
For example, from MS MARCO training set we randomly sample 5000 training instances, where each training instance contains a query and  one or more  relevant documents. 
%Then we run a sparse retriever this instance, and seperately run a fusion with a dense retriever. If the result of sparse retriever results merged with dense results  exceeds the standalone sparse retrival,  we label consider training instance as an positive example for dense retrieval, otherwise consider this as a negative example. The converted training isntances are used for training In this way, we convert a set of training instances for ranking as a set of training instances for fusion.
To train the LSTM for cluster selection, 
for each training instance, we mark the positive and negative examples for  top clusters.
If a cluster contains one of top 10 sparse retrieval results, we mark this cluster should be visited.
Otherwise this cluster should not be visited.

 
\comments{
We convert We define the labels as 
\begin{equation}
       y(q)= 
\begin{cases}
    1,& \text{if } U(s(q), d(q)) > U(s(q))\\
    0,              & \text{otherwise,}
\end{cases}
\end{equation}
where $U(.)$ is a evaluation metric we choose, for example, NDCG@10 or MRR. $s(q)$ is the scoring of a sparse system of query $q$ and $d(q)$ represents the scoring of a dense system.
}

\comments{
\subsection{How to combine two ranked list}
There are two commonly used method to combine the sparse and dense ranked lists:
\begin{enumerate}
    \item linear combination
    \item reciprocal rank fusion
\end{enumerate}
For linear combination, the final ranking score of a document is the weighted sum of the ranking score of two systems respectively. The weight on each system can be determined through grid search on a left-out training set or just use 1:1 combination. In this case, rescaling of the two ranked lists are necessary as the it largely affects the impact of a ranked list to the merged ranked list. 

On the other hand, reciprocal rank fusion alleviate the scoring distribution difference by only considering the ranking positions when merging. 
  Another consideration is on the missing values. The two ranked lists are usually not fully overlap. Some documents only exists in one ranked lists. Thus 
the treatment on these documents affects model performance. We consider a few options
\begin{enumerate}
    \item Remove the documents when they only exist in one ranked list
    \item  Take the document and compute the score for only one ranked list
    \item Impute the missing document with rank K+1 or score as 0.95 * min(score) in the ranked list.
\end{enumerate}

}




==> problem.tex <==
\section{Background and Related Work }
%\section{Problem Definition}
\label{sect:background}

\comments{
\begin{table}[h]
	\centering
		%\resizebox{1.02\columnwidth}{!}{ 
		\begin{small}
		\begin{tabular}{l l}
			\hline
			Symbol & Def. \\
                \hline
                %$\mathcal{D}$ & A set of documents in a dataset\\
                %$N$ & Total number of documents in a dataset \\
                $Q$ & A query \\
                $d_i$ & A document \\
                $\mathcal{D}^{+}$, $\mathcal{D}^{-}$ & Positive/negative document subsets corresponding to $Q$  \\
                $|.|$ &  The size of a set\\
		$\Theta$& Parameters of a scoring model\\
		$S(Q,d_i, \Theta)$ & The rank score of a document for a query using a model\\
%			& based on a model with parameters $\Theta$. \\
                $p_i$ & Teacher's top one probability of document $d_i$,\\
			& standing for  $P(d_i|Q, \mathcal{D}^+, \mathcal{D}^-, \Theta$) \\
                $q_i$ & Student's top one probability of document $d_i$\\
                $\pi(.)$ & The rank position of a document for a query\\
                $\beta_i$ & Exponent weight bias for negative  document $d_i$\\
                $\gamma, \alpha$ & CKL hyper-parameters\\
                \hline
		\end{tabular}
		\end{small}
	%}
	\caption{Table of Symbols}

	\label{tab:data}
\end{table}
}


{\bf Problem definition.}
Given query $q$ for searching a collection of $D$ text documents:   $ \{d_i\}^D_{i=1}$, 
retrieval  obtains the top $k$ relevant documents from this collection based on
the similarity between query $q$ and a candidate document  $d_i$ using  their
representation vectors.

With a lexical representation, each  representation vector of a document or a query is sparse.
Sparse retrieval uses  the dot product of their lexical representation vectors as the similarity function
and implements its search efficiently using an inverted index. 
\begin{equation}
\label{eq:sparseretrieval}
L(q) \cdot  L(d_i)
\end{equation}
%L(q,d_i ) = 
where $L(.)$ is a lexical representation   which is a a vector of weighted term tokens for a document or a query.

For BM25 based lexical representation~\cite{Robertson2009BM25}, 
$L(.)$ treats each document or a query as a bag of terms
%and term weights  are scaled based on   frequency of terms within a bag and  across all bags involved.
% Do you want to stick to terms/bags, or is the IR version easier to understand?
and term weights are scaled based on the frequency of terms within a document and across all documents in the collection.
For a learned sparse representation~\cite{Dai2020deepct, Mallia2021deepimpact, Lin2021unicoil,2021NAACL-Gao-COIL}, 
a document or a query is encoded using  a learned neural model, which
%produces a bag which may contain original  and  expanded terms.
produces a modified query which may contain the original and expanded terms.
The encoding functions for a query and document can be different. Without the loss of generality, we assume they are the same in this paper.

With a single-vector dense  representation, each  representation vector of a document or a query is a dense vector. 
Dense retrieval computes the following rank score
\begin{equation}
\label{eq:denseretrieval}
R(q) \cdot  R(d_i)
\end{equation}
%D(q,d_i) 
where $R(.)$ is a dense representation vector  of a fixed size~\cite{Karpukhin2020DPR}.


  %revises the SparTerm model~\cite{Bai2020SparTerm} to predict the weight 
%The weights of these terms evaluated in this paper use the SPLADE model as discussed below while other options are possible.
%(e.g., a bag of words or a neural encoder). 
%The implementation of such a dot product for a sparse retriever uses the inverted index data structure.
\comments{
%{\bf Learned term weights with SPLADE}.
For each document, the SPLADE term weighting revises the SparTerm model~\cite{Bai2020SparTerm} to predict the weight 
score $w_j$ of $j$-th token term in BERT WordPiece vocabulary.
\begin{equation}
\label{eq:splade}
w_j = \sum_{i \in d}  log (1 + ReLU ( H(h_i)^T E_j + b_j)) 
\end{equation}
where document $d$ consists of a sequence of BERT last layer's embeddings $(h_1, h_2, $
$\cdots, h_n)$.
$E_j$ is the BERT input embedding of the $j$-th token and $b_j$ is a token level bias.
$H(.)$ is a linear layer with activation and layer normalization. 
% (In SPLADE GeLU activation is used). 

{\bf Combining the results of a dense retriever and a sparse retriever.}
}
Following the work of~\cite{kuzi2020leveraging, 2022LinearInterpolationJimLin, Gao2020ComplementingLR}, 
linear interpolation is used  to  ensemble  dense and sparse retrieval scores. 
%Let $S$ be the set of top results obtained by a sparse retriever, and $D$ be
%be the set of results obtained by dense retrieval. 
%For any document $d_i \in S \cup D$, its  
The fused rank score for document $d_i$ in responding  query $q$ is:
\begin{equation}
\label{eq:fusion}
\alpha L(q) \cdot  L(d_i) +
(1-\alpha) R(q) \cdot  R(d_i) 
\end{equation}
where $\alpha$ is a coefficient in a range between 0 and 1.

\comments{
Notice that   the two ranked lists $S$ and $D$ are usually not fully overlapped and  some documents only exist in one list. While 
different  treatments on these documents affect fusion performance,
we take an option to  impute the score of such a document score   using $\beta * score (top \  k+1) $  in the missed  ranklist where $\beta$
is a scaling factor.
%While there are options to We consider a few options
For example,  we  impute the lexical scores of documents expanded by dense retrieval
as the top-$(k+1)$ lexical  score scaled by a factor. We use $\beta=0.95$  in our evaluation.
 
%\item Remove the documents when they only exist in one ranked list
%    \item  Take the document and compute the score for only one ranked list
}

% Parker: below is awkward, and a run on sentence.
Our optimization goal is to minimize the scope of dense retrieval and extra memory space overhead  
while maintaining a relevance competitive to
the full dense retrieval  which searches  the entire document set. 
In this way, limited dense retrieval that augments sparse retrieval is fast with minimum space consumption  on a CPU server. 
\comments{
The ensembling method used in our evaluation is 
%The final ranking of the top $K$ documents is 
the reciprocal rank fusion (RRF) following Cormack et al.~\cite{Cormack2009RRF}, considering ranking positions of each candidate 
generated by a retriever and by a re-ranker. 
We use RRF
% above reciprocal rank fusion 
instead of linear interpolation as it has a similar performance with a simplified combination of two scoring models. 
%We choose RRF because it is easily applicable to multiple ranked lists ignoring the score distribution differences. 
\begin{equation}
     %RRF(Q,d) =  \sum_{r \in {rt, rr,}} \frac{1}{k_r + r(d)},
     RRF(Q,d) =  
\frac{1}{c_1 + \pi_1(d)} + 
\frac{1}{c_{2} + \pi_2(d)},
     \label{eq:score}
\end{equation}
where $c_{1}$ and $c_{2}$ are fixed smoothing constants. $\pi_2(d)$ is the rank position based  a re-ranker formula
while $\pi_1(d)$ is the rank position based on a retriever.
}


